Introduction to Machine Learning

This book introduces the mathematical foundations and techniques that lead to the development and analysis of many of the algorithms that are used in machine learning. It starts with an introductory chapter that describes notation used throughout the book and serve at a reminder of basic concepts in calculus, linear algebra and probability and also introduces some measure theoretic terminology, which can be used as a reading guide for the sections that use these tools. The introductory chapters also provide background material on matrix analysis and optimization. The latter chapter provides theoretical support to many algorithms that are used in the book, including stochastic gradient descent, proximal methods, etc. After discussing basic concepts for statistical prediction, the book includes an introduction to reproducing kernel theory and Hilbert space techniques, which are used in many places, before addressing the description of various algorithms for supervised statistical learning, including linear methods, support vector machines, decision trees, boosting, or neural networks. The subject then switches to generative methods, starting with a chapter that presents sampling methods and an introduction to the theory of Markov chains. The following chapter describe the theory of graphical models, an introduction to variational methods for models with latent variables, and to deep-learning based generative models. The next chapters focus on unsupervised learning methods, for clustering, factor analysis and manifold learning. The final chapter of the book is theory-oriented and discusses concentration inequalities and generalization bounds.

==> Headers/newcom.tex <==
\RequirePackage{ifthen}
\RequirePackage{kpfonts}

\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}
%\def\qed{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
%\penalty50\hskip1em\null\nobreak\hfil\squareforqed
%\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}



\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bquo}{\begin{quote}}
\newcommand{\equo}{\end{quote}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}

\newcommand{\bac}{\backslash}
\newcommand{\nat}{\natural}
\newcommand{\equ}{\equiv}
\newcommand{\lab}{\label}
\newcommand{\emp}{\emptyset}
\newcommand{\prt}{\partial}
\newcommand{\nab}{\nabla}
\newcommand{\grad}{\nabla}
\newcommand{\sub}{\subset}
\newcommand{\setm}{\setminus}
\newcommand{\cir}{\circ}
\newcommand{\ria}{\rightarrow}
\newcommand{\Lfria}{\Leftrightarrow}
\newcommand{\Ria}{\Rightarrow}
\newcommand{\lria}{\longrightarrow}
\newcommand{\lan}{\langle}
\newcommand{\ran}{\rangle}
\newcommand{\demi}{{1\over 2}}
\newcommand{\beg}{\begin}
\newcommand{\bigo}{\bigotimes}
\newcommand{\ti}{\times}
\newcommand{\oti}{\otimes}
%\newcommand{\lsc}{\lan\ }
\newcommand{\rsc}{\ \ran}
\newcommand{\ccdot}{\,\cdot\,}

\renewcommand{\phi}{\varphi}
\newcommand{\al}{\alpha}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}
\newcommand{\La}{\Lambda}
\newcommand{\la}{\lambda}
\newcommand{\De}{\Delta}
\newcommand{\de}{\delta}
\newcommand{\ep}{\epsilon}
\newcommand{\eps}{\epsilon}
\newcommand{\ze}{\zeta}
\providecommand{\th}{\theta}
\renewcommand{\th}{\theta}
\newcommand{\Th}{\Theta}
\newcommand{\be}{\beta}
\newcommand{\ga}{\gamma}
\newcommand{\ka}{\kappa}
\newcommand{\Ga}{\Gamma}
\newcommand{\sig}{\sigma}
\newcommand{\Sig}{\Sigma}




\newcommand{\cf}{{\mathcal F}}
\newcommand{\CF}{{\mathcal F}}
\newcommand{\CZ}{{\mathcal Z}}
\newcommand{\CE}{{\mathcal E}}
\newcommand{\CY}{{\mathcal Y}}
\newcommand{\CW}{{\mathcal W}}
\newcommand{\CX}{{\mathcal X}}
\newcommand{\CK}{{\mathcal K}}
\newcommand{\CH}{{\mathcal H}}
\newcommand{\CC}{{\mathcal C}}
\newcommand{\CS}{{\mathcal S}}
\newcommand{\CT}{{\mathcal T}}
\newcommand{\CU}{{\mathcal U}}
\newcommand{\CR}{{\mathcal R}}
\newcommand{\CO}{{\mathcal O}}
\newcommand{\CP}{{\mathcal P}}
\newcommand{\CM}{{\mathcal M}}
\newcommand{\CN}{{\mathcal N}}
\newcommand{\CD}{{\mathcal D}}
\newcommand{\CB}{{\mathcal B}}
\newcommand{\CA}{{\mathcal A}}
\newcommand{\CQ}{{\mathcal Q}}
\newcommand{\CL}{{\mathcal L}}
\newcommand{\CG}{{\mathcal G}}
\newcommand{\CV}{{\mathcal V}}
\newcommand{\CI}{{\mathcal I}}
\newcommand{\CJ}{{\mathcal J}}

\newcommand{\hpi}{{\hat{\pi}}}
\newcommand{\hth}{{\hat{\th}}}
\newcommand{\hnu}{\hat{\nu}}
\newcommand{\hga}{\hat{\ga}}
\newcommand{\hal}{\hat{\al}}
\newcommand{\hbe}{\hat{\be}}
\newcommand{\hphi}{\hat{\phi}}
\newcommand{\heta}{\hat{\eta}}
\newcommand{\htau}{\hat{\tau}}
\newcommand{\hrho}{\hat{\rho}}
\newcommand{\hhrho}{\hat{\hat{\rho}}}
\newcommand{\hep}{\hat{\ep}}
\newcommand{\hb}{\hat{b}}
\newcommand{\hf}{{\hat{f}}}
\newcommand{\hx}{\hat{x}}
\newcommand{\hy}{\hat{y}}
\newcommand{\hX}{\hat{X}}
\newcommand{\hl}{\hat{l}}
\newcommand{\hu}{\hat{u}}
\newcommand{\hv}{\hat{v}}
\newcommand{\hz}{\hat{z}}
\newcommand{\hw}{\hat{w}}
\newcommand{\hW}{{\hat{W}}}
\newcommand{\hE}{\hat{E}}
\newcommand{\hL}{\hat{L}}
\newcommand{\hN}{{\hat{N}}}
\newcommand{\hQ}{\hat{Q}}
\newcommand{\hH}{\hat{H}}
\newcommand{\hK}{\hat{K}}
\newcommand{\hP}{\hat{P}}
\newcommand{\hV}{\hat{V}}
\newcommand{\hR}{\hat{R}}


\newcommand{\bth}{\overline{\th}}
\newcommand{\bga}{{\overline{\ga}}}
\newcommand{\bL}{\overline{L}}
\newcommand{\bc}{\overline{c}}
\newcommand{\br}{\overline{r}}
\newcommand{\ba}{\overline{a}}
\newcommand{\bx}{\overline{x}}
\newcommand{\by}{\overline{y}}
\newcommand{\bb}{\overline{b}}
\newcommand{\bh}{\overline{h}}
\newcommand{\bt}{\overline{t}}
\newcommand{\bv}{\overline{v}}
\newcommand{\bw}{\overline{w}}
\newcommand{\bW}{\overline{W}}
\newcommand{\bla}{\overline{\la}}
\newcommand{\bal}{\overline{\al}}
\newcommand{\brho}{\overline{\rho}}
\newcommand{\bz}{{\overline{z}}}
\newcommand{\bze}{{\overline{\zeta}}}
\newcommand{\bT}{{\overline{T}}}
\newcommand{\bB}{{\overline{B}}}
\newcommand{\bre}{{\overline{e}}}
\newcommand{\bmu}{\overline{\mu}}
\newcommand{\bpi}{{\overline{\pi}}}
\newcommand{\bS}{{\overline{S}}}
\newcommand{\bZ}{{\overline{Z}}}
\newcommand{\bY}{{\overline{Y}}}
\newcommand{\bH}{{\overline{H}}}
\newcommand{\bX}{{\overline{X}}}
\newcommand{\bs}{{\overline{s}}}
\newcommand{\bl}{{\overline{l}}}
\newcommand{\ovm}{{\overline{m}}}
\newcommand{\Bla}{\overline{\La}}
\newcommand{\bOm}{\overline{\Om}}
\newcommand{\bE}{\overline{E}}
\newcommand{\bC}{\overline{C}}
\newcommand{\bD}{\overline{D}}
\newcommand{\bF}{\overline{F}}
\newcommand{\Bf}{\overline{F}}
\newcommand{\bu}{{\overline{u}}}
\newcommand{\bg}{{\overline{g}}}
\newcommand{\bDe}{{\overline{\De}}}
\newcommand{\bphi}{{\overline{\phi}}}
\newcommand{\bpsi}{{\overline{\psi}}}
\newcommand{\bCS}{\overline{\CS}}

\newcommand{\tla}{{\tilde{\la}}}
\newcommand{\tnu}{{\tilde{\nu}}}
\newcommand{\ttau}{{\tilde{\tau}}}
\newcommand{\tze}{{\tilde{\ze}}}
\newcommand{\tCC}{{\widetilde{\CC}}}
\newcommand{\tCE}{{\widetilde{\CE}}}
\newcommand{\tCG}{{\widetilde{\CG}}}
\newcommand{\tCD}{{\widetilde{\CD}}}
\newcommand{\tbfu}{{\tilde{\bfu}}}
\newcommand{\tI}{{\tilde{I}}}
\newcommand{\tS}{{\tilde{S}}}
\newcommand{\tY}{{\tilde{Y}}}
\newcommand{\tq}{{\tilde{q}}}
\newcommand{\tv}{{\tilde{v}}}
\newcommand{\tL}{{\tilde{L}}}
\newcommand{\tE}{{\tilde{E}}}
\newcommand{\tG}{{\tilde{G}}}
\newcommand{\tH}{{\tilde{H}}}
\newcommand{\tZ}{{\tilde{Z}}}
\newcommand{\td}{{\tilde{d}}}
\newcommand{\tb}{{\tilde{b}}}
\newcommand{\tal}{{\tilde{\al}}}
\newcommand{\tka}{{\tilde{\ka}}}
\newcommand{\tth}{{\tilde{\th}}}
\newcommand{\tep}{{\tilde{\ep}}}
\newcommand{\tLa}{{\widetilde{\La}}}
\newcommand{\tSig}{{\widetilde{\Sig}}}
\newcommand{\tilh}{{\tilde{h}}}
\newcommand{\tX}{{\tilde{X}}}
\newcommand{\tO}{{\tilde{O}}}
\newcommand{\tA}{{\tilde{A}}}
\newcommand{\tJ}{{\tilde{J}}}
\newcommand{\tC}{{\tilde{C}}}
\newcommand{\tM}{{\tilde{M}}}
\newcommand{\tT}{{\tilde{T}}}
\newcommand{\tR}{{\tilde{R}}}
\newcommand{\tB}{{\tilde{B}}}
\newcommand{\tP}{{\tilde{P}}}
\newcommand{\tU}{{\tilde{U}}}
\newcommand{\ta}{{\tilde{a}}}
\newcommand{\tm}{{\tilde{m}}}
\providecommand{\tt}{tt}
\renewcommand{\tt}{{\tilde{t}}}
\newcommand{\tf}{{\tilde{f}}}
\newcommand{\tg}{{\tilde{g}}}
\newcommand{\tl}{{\tilde{l}}}
\newcommand{\tu}{{\tilde{u}}}
\newcommand{\tr}{{\tilde{r}}}
\newcommand{\tp}{{\tilde{p}}}
\newcommand{\tx}{{\tilde{x}}}
\newcommand{\ty}{{\tilde{y}}}
\newcommand{\tz}{{\tilde{z}}}
\providecommand{\ts}{ts}
\renewcommand{\ts}{{\tilde{s}}}
\newcommand{\tbu}{{\tilde{\vec{u}}}}
%\newcommand{\tbu}{{\tilde{\mbox{\bf u}}}}
\newcommand{\tK}{{\tilde{K}}}
\newcommand{\tV}{{\tilde{V}}}
\newcommand{\txi}{{\tilde{\xi}}}
\newcommand{\tphi}{{\tilde{\phi}}}
\newcommand{\tpsi}{{\tilde{\psi}}}
\newcommand{\trho}{{\tilde{\rho}}}
\newcommand{\tmu}{{\tilde{\mu}}}
\newcommand{\tga}{{\tilde{\ga}}}
\newcommand{\tOm}{{\widetilde{\Om}}}
\newcommand{\tGa}{{\widetilde{\Ga}}}
\newcommand{\tDe}{{\widetilde{\De}}}


\newcommand{\da}{{\dot{a}}}
\newcommand{\dD}{{\dot{D}}}
\newcommand{\dg}{{\dot{g}}}
\newcommand{\df}{{\dot{f}}}
\providecommand{\dh}{dh}
\renewcommand{\dh}{{\dot{h}}}
\newcommand{\doth}{{\dot{h}}}
\newcommand{\dx}{{\dot{x}}}
\newcommand{\dla}{{\dot{\lambda}}}
\newcommand{\dze}{{\dot{\zeta}}}
\newcommand{\dy}{{\dot{y}}}
\newcommand{\dz}{{\dot{z}}}
\newcommand{\du}{{\dot{u}}}
\newcommand{\dv}{{\dot{v}}}
\newcommand{\dV}{{\dot{V}}}
\newcommand{\dal}{{\dot{\al}}}
\newcommand{\dotp}{{\dot{p}}}
\newcommand{\dq}{{\dot{q}}}
\newcommand{\dr}{{\dot{r}}}
\newcommand{\dm}{{\dot{m}}}
\newcommand{\dtm}{{\dot{\tm}}}
\newcommand{\dR}{{\dot{R}}}
\newcommand{\dX}{{\dot{X}}}
\newcommand{\dY}{{\dot{Y}}}
\newcommand{\dphi}{{\dot{\phi}}}
\newcommand{\dchi}{{\dot{\chi}}}
\newcommand{\dPhi}{{\dot{\Phi}}}
\newcommand{\dpsi}{{\dot{\psi}}}
\newcommand{\dDe}{{\dot{\De}}}
\newcommand{\dxi}{{\dot{\xi}}}
\newcommand{\dtilh}{{\dot{\tilh}}}

\newcommand{\ddx}{{\ddot{x}}}
\newcommand{\ddy}{{\ddot{y}}}
\newcommand{\ddf}{{\ddot{f}}}
\newcommand{\ddg}{{\ddot{g}}}
\newcommand{\ddh}{{\ddot{h}}}
\newcommand{\ddphi}{{\ddot{\phi}}}
\newcommand{\ddchi}{{\ddot{\chi}}}
\newcommand{\ddpsi}{{\ddot{\psi}}}
\newcommand{\ddDe}{{\ddot{\De}}}

\newcommand{\bvar}{\overline{\var}}
\newcommand{\bcov}{\overline{\cov}}


%\def\vecbf#1{\mathchoice{\mbox{\boldmath$\displaystyle\bf#1$}}
%{\mbox{\boldmath$\textstyle\bf#1$}}
%{\mbox{\boldmath$\scriptstyle\bf#1$}}
%{\mbox{\boldmath$\scriptscriptstyle\bf#1$}}}

\def\vecbf#1{\mathchoice{\mbox{\boldmath$\displaystyle#1$}}
{\mbox{\boldmath$\textstyle#1$}}
{\mbox{\boldmath$\scriptstyle#1$}}
{\mbox{\boldmath$\scriptscriptstyle#1$}}}


%\newcommand{\bfu}{{\mbox{\bf u}}}
%\newcommand{\bfacd }{{\mbox{\bf a}}}
\usepackage{bm}
\renewcommand{\boldsymbol}{\bm}
\newcommand{\bfx}{{\boldsymbol{x}}}
\newcommand{\bfy}{{\boldsymbol{y}}}
\newcommand{\bfz}{{\boldsymbol{z}}}
\newcommand{\bfu}{{\boldsymbol{u}}}
\newcommand{\bfv}{{\boldsymbol{v}}}
\newcommand{\bfw}{{\boldsymbol{w}}}
\newcommand{\bfc}{{\boldsymbol{c}}}
\newcommand{\bfa}{{\boldsymbol{a}}}
\newcommand{\bfh}{{\boldsymbol{h}}}
\newcommand{\bfj}{{\boldsymbol{j}}}
\newcommand{\bfk}{{\boldsymbol{k}}}
\newcommand{\bfr}{{\boldsymbol{r}}}
\newcommand{\bfg}{{\boldsymbol{g}}}
\newcommand{\bfo}{{\boldsymbol{o}}}
\newcommand{\bfm}{{\boldsymbol{m}}}
\newcommand{\bfF}{{\boldsymbol{F}}}
\newcommand{\bfP}{{\boldsymbol{P}}}
\newcommand{\bfL}{{\boldsymbol{L}}}
\newcommand{\bfT}{{\boldsymbol{T}}}
\newcommand{\bfS}{{\boldsymbol{S}}}
\newcommand{\bfD}{{\boldsymbol{D}}}
\newcommand{\ZZ}{{\mbox{\bf Z}^2}}
\newcommand{\Zd}{{\bf Z}^d}
\newcommand{\bfA}{{\boldsymbol{A}}}
\newcommand{\bfN}{{\boldsymbol{N}}}
\newcommand{\RR}{\mbox{\bf R}}
\newcommand{\bfM}{{\boldsymbol{M}}}
\newcommand{\bfV}{{\boldsymbol{V}}}
\newcommand{\NO}{{\boldsymbol{N}}}
%\newcommand{\bfP}{{\boldsymbol{P}}}
\newcommand{\bfE}{{\boldsymbol{E}}}
\newcommand{\bfI}{{\boldsymbol{I}}}
\newcommand{\bfW}{{\boldsymbol{W}}}
\newcommand{\bfJ}{{\boldsymbol{J}}}
\newcommand{\bfH}{{\boldsymbol{H}}}
\newcommand{\bfK}{{\boldsymbol{K}}}
\newcommand{\bfb}{{\boldsymbol{b}}}
\newcommand{\bfs}{{\boldsymbol{s}}}
\newcommand{\bfq}{{\boldsymbol{q}}}
\newcommand{\bfp}{{\boldsymbol{p}}}
\newcommand{\bfZ}{{\boldsymbol{Z}}}
%\newcommand{\bfE}{{\boldsymbol{E}}}
\newcommand{\bfR}{{\boldsymbol{R}}}
\newcommand{\bfQ}{{\boldsymbol{Q}}}
\newcommand{\bfC}{{\boldsymbol{C}}}
\newcommand{\bfX}{{\boldsymbol{X}}}
\newcommand{\bfY}{{\boldsymbol{Y}}}
\newcommand{\bfO}{{\boldsymbol{O}}}
\newcommand{\bfal}{{\boldsymbol{\otheralpha}}}
\newcommand{\bfrho}{{\boldsymbol{\otherrho}}}
\newcommand{\bfla}{{\boldsymbol{\la}}}
\newcommand{\bfphi}{{\boldsymbol{\phi}}}
\newcommand{\bfeta}{{\boldsymbol{\eta}}}
\newcommand{\bfzeta}{{\boldsymbol{\zeta}}}
\newcommand{\bfxi}{{\boldsymbol{\xi}}}
\newcommand{\bfTh}{{\boldsymbol{\Th}}}

\newcommand{\dbfX}{{\dot{\bfX}}}
\newcommand{\dbfY}{{\dot{\bfY}}}
\newcommand{\dbfa}{{\dot{\bfa}}}

\newcommand{\usc}{{\underline{c}}}
\newcommand{\usal}{{\underline{\alpha}}}
\newcommand{\usth}{{\underline{\theta}}}
\newcommand{\useta}{{\underline{\eta}}}
\newcommand{\usz}{{\underline{z}}}
\newcommand{\usx}{{\underline{x}}}
\newcommand{\usZ}{{\underline{Z}}}
\newcommand{\usX}{{\underline{X}}}

\newcommand{\mR}{{\mathbb{R}}}
\newcommand{\mN}{{\mathbb{N}}}
\newcommand{\mC}{{\mathbb{C}}}
\newcommand{\mQ}{{\mathbb{Q}}}
\newcommand{\mZ}{{\mathbb{Z}}}
\newcommand{\mZd}{{\mZ}^d}


\newcommand{\diam}{{\mbox{\rm diam}}}
\newcommand{\Id}[1][]{\ifthenelse{\equal{#1}{}} 
				{\ensuremath{\mathrm{Id}}}
				{\ensuremath{\mathrm{Id}_{\mR^{#1}}}}
				}
\newcommand{\id}[1][]{\ifthenelse{\equal{#1}{}} 
				{\ensuremath{\mathrm{id}}}
				{\ensuremath{\mathrm{id}_{\mR^{#1}}}}
				}
\newcommand{\bfone}{{\mathbb 1}}
\newcommand{\inte}{{\mathrm{int}}}
\newcommand{\cte}{{\mathrm cst}\ }
\newcommand{\var}{\mathrm{var}}
\newcommand{\Var}{\mathrm{\bf Var}}
\newcommand{\cov}{{\mathrm cov}}
\newcommand{\Cov}{{\mathrm Cov}}
\newcommand{\acos}{{\mathrm{acos}}}
\newcommand{\card}{{\mathrm card}}
\newcommand{\Log}{{\mathrm{ln}}}
\newcommand{\real}{{\mathrm real}}
\providecommand{\imag}{{\mathrm imag}}
\renewcommand{\imag}{{\mathrm imag}}
\newcommand{\signe}{{\mathrm{signe}}}
\newcommand{\trace}{{\mathrm{trace}}}
\newcommand{\Hom}{{\mathrm{Hom}}}
\newcommand{\ev}{{\mathrm{ev}}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator{\dd}{d}
\DeclareMathOperator{\Exp}{Exp}
\DeclareMathOperator{\mdiv}{div}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\prox}{prox}
\DeclareMathOperator{\sign}{sign}
%\newcommand{\argmin}{{\operatorname{\mathrm{argmin}}}}

%\newcommand{\ppi}{{ \pi_a}}
%\newcommand{\ppsi}{{\psi_a}}
%\newcommand{\pixy}{\pi(xy)}
\newcommand{\dift}{{\frac{\rm d}{{\rm d}t}}}
\newcommand{\difs}{{{\rm d}\over {\rm d}s}}
\newcommand{\ddth}{{\mbox{d}\over \mbox{d}\th}}
\newcommand{\pdth}{{\partial\over \partial\th}}
\newcommand{\pdal}{{\partial\over \partial\al}}
\newcommand{\ddtt}{{{\rm d^2}\over {\rm d}\th^2}}
\newcommand{\dt}{{{\rm d}\over {\rm d}t}}
\newcommand{\ch}{{\mbox{\bf 1}}}
\newcommand{\zz}{{\mbox{\bf Z}}}
%\newcommand{\inte}{\rm int }
\newcommand{\trp}[1]{{\,{\vphantom{#1}}^t\!#1}}




\newcommand{\vv}{\vskip .3cm}
\newcommand{\hh}{\hskip .5cm}
\newcommand{\vw}{\vskip .6cm}
\newcommand{\intp}[1]{{\left[ \, {#1} \, \right]}}
\newcommand{\scp}[2]{{\langle {#1}\mathbin{,} {#2}\rangle}}
\newcommand{\Scp}[2]{{\big\langle {#1}\mathbin{,} {#2}\big\rangle}}
\newcommand{\SCP}[2]{{\Big\langle {#1}\mathbin{,} {#2}\Big\rangle}}
\newcommand{\lform}[2]{{\left( {#1} |\, {#2}\right)}}
\newcommand{\ang}[2]{{\left\lan\!\left\lan {#1}\, , \, {#2}\right\ran\!\right\ran}}
\newcommand{\der}[2]{\frac{d {#1}}{d{#2}}}
\newcommand{\pder}[2]{\frac{\partial {#1}}{\partial {#2}}}
\newcommand{\dco}[2]{{\nabla_{#2}\left({#1}\right)}}
\newcommand{\mder}[3]{\frac{d^{#1} {#2}}{ d{#3}^{#1}}}
\newcommand{\dder}[2]{\frac{d^2 {#1}}{d{#2}^2}}
\newcommand{\pdr}[2]{\frac{\prt {#1}}{\prt{#2}}}
\newcommand{\ppdr}[2]{\frac{\prt^2 {#1}}{\prt{#2}^2}}
\newcommand{\pddr}[3]{\frac{\prt^2 {#1}}{\prt{#2}\prt{#3}}}
\newcommand{\mdr}[2]{\frac{D {#1}}{D{#2}}}
\newcommand{\dps}{\displaystyle}
\newcommand{\bul}{$\bullet$ }
\newcommand{\cond}[1]{{[\bf {#1}]}}
\newcommand{\defset}[1]{\left\{ #1 \right\}}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\bin}[2]{\left(\begin{array}{c}  #1\\#2\end{array}
\right)}
\newcommand{\rotmat}[1]{\left(\begin{array}{cc}  \cos #1& - \sin
#1\ \\sin #1 & \cos#1\end{array}
\right)}
\newcommand{\avg}[1]{\left\langle#1\right\rangle}
\newcommand{\lfrac}[2]{ #1\, / \, #2}
\newcommand{\Lfrac}[2]{ #1\, \big/ \, #2}

\newcommand{\pe}[2]{#1^{(#2)}}
\newcommand{\bke}[2]{#1^{[#2]}}


\newcommand{\map}[5]{\begin{array}{lrcl}#1:& #2&\ria&#3\\&#4&\mapsto&#5\end{array}}
\newcommand{\encadre}[1]{\par\noindent\framebox{\parbox{\textwidth}{#1}}

\medskip}
\newcommand{\todo}[1]{{\textcolor{red}{#1}}}
\newcommand{\dpm}{\displaymath}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% TeX-master: t
%%% End: 


==> boosting.tex <==
% !TEX root = machine_learning.tex
\chapter{Boosting methods}

Boosting methods refer to algorithms in which classifiers are enhanced by
recursively training them on harder data. We first address the issue
of classification, and describe the original  algorithm (Adaboost). We then
interpret it as greedy gradient descent to optimize a combination of
classifiers.

\section{Classification}
Boosting for classification is essentially restricted to two-class
problems. In this context, we want to design a function $x \mapsto f(x) \in \{-1, 1\}$ on the
basis of a training set $(y_1, x_1), \ldots, (y_N, x_N)$. With the 0-1
loss, minimizing the  empirical error is equivalent to maximizing
$$
\CE_T(f) = \frac{1}{N} \sum_{i=1}^N y_i f(x_i)
$$

Boosting algorithms build a function $f$ as a weighted combination of
simple classifiers, $f_1, \ldots, f_M$, taking
$$
f(x) = \text{sign}\left(\sum_{k=1}^M \al_k f_k(x)\right)\,.
$$

Each $f_j$ is learned on the basis of weighted
data. We therefore assume that the  learning algorithm for simple classifiers takes as input the training set $X_1,\ldots,X_N$ as well as positive weights $w_1, \ldots, w_N$,   minimizing, for example, a loss function of the form
$$
\sum_{k=1}^N w_k R(y_k, f(x_k)).
$$
Boosting algorithms  estimate new $f_j$ and $\al_j$ at step $j$, while updating the current data weights. The basic algorithm works as follows.
\begin{enumerate}[label=(\arabic*),wide]
\item Start with uniform weights, letting  $w_k = 1/N$, $k=1, \ldots, N$.
\item Step $j$: fit a classifier $f_j$ using the current weights and
estimate the weighted error
$$\CE_{w} = \sum_{k=1}^N w_k \chi_{[y_k\neq f_j(x_k)]}/\sum_{k=1}^N
w_k.$$
Define $\al_j = (1/2)\log((1-\CE_w)/\CE_w)$ and update the weights by
$$ w_k \mapsto w_k \exp(-\al_j \chi_{[y_k\neq f_j(x_k)]}).$$
\item Iterate the previous step while $j\leq M$.
\end{enumerate}

Notice that for the algorithm to run, $\al_j$ should be positive (i.e., the $j$th classifier must do
better than pure chance on the training set).
The boosting effect comes from the fact that misclassified data at step $j$
are provided with a higher weight for the next step. This implies that
the algorithm focuses on the hardest cases. 


We now provide an interpretation of this algorithm. Even if the $f_q$ are binary, their linear combination is not
anymore. The classification rule only uses the sign of the product $Yf(X)$, but the value also has an
important interpretation, since, when it is positive, it can be interpreted as a margin with which
$X$ is correctly classified (provided, of course that $f$ is properly
normalized, since one can always improve the margin by multiplying $f$
by a constant). 

Assume that the function $f$ is evaluated, not only on the basis of
its classification error, but also based on this margin,
using a loss function of the kind
$$
\sum_{k=1}^N g(y_kf(x_k))
$$
where $g$ is decreasing. The boosting algorithm can then be interpreted as an classifier which
incrementally improves this cost function.
Denote by
$f^{(j)}$ the  classifier at step $j$:
$$
f^{(j)} = \sum_{q=1}^j \al_q f_q\,.
$$
The new classifier $f^{(j+1)}$ takes the form $f^{(j)} + \al_{j+1}
f_{j+1}$, where  
$f_{j+1}$ and $\al_{j+1}$ minimize, with respect
to $\tilde f$ and $\al \geq 0$, the function
$$
U(\al, \tilde f) = \sum_{k=1}^N g\left(y_kf^{(j)}(x_k) + \al y_k \tilde
f(x_k)\right)
$$

Using the fact that $\tilde f$ is a binary classifier, this can be written
\begin{eqnarray*}
U(\al, \tilde f) &=& \sum_{k=1}^N g(y_kf^{(j)}(x_k) + \al) \chi_{[y_k
= \tilde f(x_k)]} + \sum_{k=1}^N g(y_kf^{(j)}(x_k) - \al) \chi_{[y_k
\neq \tilde f(x_k)]}\\
&=& \sum_{k=1}^N (g(y_kf^{(j)}(x_k) - \al) - g(y_kf^{(j)}(x_k) + \al)) \chi_{[y_k
\neq \tilde f(x_k)]} \\
&&+ \sum_{k=1}^N g(y_kf^{(j)}(x_k) + \al)
\end{eqnarray*}
This shows that, for a given $\al$, the classifier $\tilde f$ must
minimize a weighted empirical error with weights
$$ w_k  = g(y_kf^{(j)}(x_k) - \al) - g(y_kf^{(j)}(x_k) + \al) \geq 0,$$
since $g$ is decreasing. 
However, the combined derivation of $\al_{j+1}$ and $f_{j+1}$ is, in general, computationally intensive, typically requiring to  loop over an estimation of
$f_{j+1}$ with fixed $\al_{j+1}$, and optimization of $\al_{j+1}$
by gradient descent, for example, with fixed $f_{j+1}$. There is anyway one situation in which the
computation can be made analytically: it is when the function $g$ is
exponential, $g(t) = e^{- t}$. In this case, the weights are
$$w_k = (e^{\al} - e^{-\al})   e^{- y_k f^{(j)}(x_k)}$$
and the constant factor $(e^{\al} - e^{-\al})$ does not affect
the solution of the minimization in $\tilde f$, which can therefore be
computed with
$w_k = \exp(- y_k f^{(j)}(x_k))$, a problem which is independent of $\al$. The value of $\al$, afterward,
can be computed by  minimizing:
$$
(e^{\al} - e^{-\al}) \left(\sum_k w_k \chi_{[y_k
\neq \tilde f(x_k)]}\right) + e^{-\al} \sum_k w_k
$$
This yields $ \al = \frac{1}{2} \log((1-E)/E)$ with
$$
E = \sum_k w_k \chi_{[y_k
\neq \tilde f(x_k)]}/ \sum_k w_k.
$$
This provides the previously described algorithm.

\bigskip
One critic that can be addressed to this algorithm is that it does
not properly handles the maximization of the margin, since the
$f^{(j)}$'s  are not normalized. One possibility is to require that
the $\al_q$ are positive and sum to 1.
The new classifier $f^{(j+1)}$ will then have the form $(1-\al_{j+1})f^{(j)} + \al_{j+1}
f_{j+1}$, and the function to minimize would be
$$
U(\al, \tilde f) = \sum_{k=1}^N g((1-\al) y_kf^{(j)}(x_k) + \al y_k \tilde
f(x_k)).
$$

Taking as before an exponential $g$: $g(t) = e^{-\la t}$, the final
problem becomes less simple because $\al$ and $\tilde f$ do not
separate: the weights are    
$$w_k = (e^{\la \al} - e^{-\la \al})   e^{-\la(1-\al) y_k f^{(j)}(x_k)}$$
and $\al$ cannot be factorized out. The solution has to be computed
numerically, which can be costly in some cases. The general algorithm
for creating a new component $f_{j+1}$ is to loop over the following
two steps, starting with an initial guess $f_{j+1}$ (computed, for
example, with the weights provided by the standard boosting algorithm).
\begin{enumerate}[label=(\arabic*),wide]
\item Minimize $U$ with respect to $\al$.
\item Update $f_{j+1}$ using the new weights 
$$
w_k = g((1-\al) y_kf^{(j)}(x_k) - \al) - g((1-\al) y_kf^{(j)}(x_k) + \al)
$$
\end{enumerate}
One can compute the derivatives of $U$ with respect to $\al$; we have
\begin{eqnarray*}
\prt_\al{U} & = & \sum_{k=1}^N y_k (f(x_k)-f^{(j)}(x_k)) g'((1-\al) y_kf^{(j)}(x_k) + \al y_k \tilde
f(x_k))\\
{\prt^2_\al U} & = & \sum_{k=1}^N (f(x_k)-f^{(j)}(x_k))^2 g''((1-\al) y_kf^{(j)}(x_k) + \al y_k \tilde
f(x_k))
\end{eqnarray*}
One sees in particular that $U$ is convex as a function of $\al$ as
soon as $g$ is convex (as is the exponential). A typical Newton-Raphson algorithm to solve
step 1 is
$$
\alpha(t+1) = \alpha(t) - \frac{1}{2} \prt_\al {U}/
{\prt^2_\al U}.
$$


\subsection{Choice of $f_j$}
The ``simple classifiers'' $f_j$ can be anything that accepts
weights. Notice that, for the algorithm to work, the
classifier does not have to minimize the weighted  classification error, but
simply to reduce it: the cost in the Adaboost algorithm is 
\begin{eqnarray*}
\CE{(j+1)}  &=& (e^{\al_{j+1}} - e^{-\al_{j+1}}) \sum_{k=1}^N w_k^{(j+1)} \chi_{[y_k
\neq \tilde f_{j+1}(x_k)]} + e^{-\al_{j+1}} \CE^{(j)}\\
&=&  \left((e^{\al_{j+1}} - e^{-\al_{j+1}}) \ep_{j+1} +
e^{-\al_{j+1}}\right)\CE^{(j)}
\end{eqnarray*}
where $\ep_{j+1}$ is the error corresponding to the $(j+1)$th
classifier alone and $\CE^{(j+1)}$ the combined cost. So, to have a
reduction of the cost, it suffices that 
$$(e^{\al_{j+1}} - e^{-\al_{j+1}}) \ep_{j+1} +
e^{-\al_{j+1}} < 1\,.$$
This is exactly the expression minimized by the boosting algorithm, and
at the optimal, $\al_{j+1} = \frac{1}{2}
\log((1-\ep_{j+1})/\ep_{j+1})$, this factor is $2
\sqrt{\ep_{j+1}(1-\ep_{j+1})}$, which is always smaller than 1, and
strictly smaller as soon as the error is strictly smaller than
$1/2$. So, exact minimization of the error is not needed at each step.

This implies that estimators such as LDA, linear separating hyperplanes,
etc. can be used as soon as they do better than chance. They do not
directly minimize the error, but weights on the training set always
have a natural way to be incorporated in their learning algorithms. For
example, assuming that weights sum to 1, a weighted LDA would use the class
centroids
$$
\mu_g = \sum_{k, y_k=g} w_k x_k
$$
and within-class covariance matrix
$$
\sum_{k=1}^N w_k (x_k - \mu_{y_k})(x_k - \mu_{y_k})^T.
$$ 

Similarly, a weighted SVM would minimize
$$
\norm{\be}^2 + \lambda N \sum_{k=1}^N w_k \xi_k
$$
under the constraints $\xi_k \geq 0$, $y_k(\be_0 + \scp{\be}{x_k})
\geq 1 - \xi_k$. In the dual variables, the problem becomes: maximize
$$
\sum_{k=1}^N \al_k - \frac{1}{2} \sum_{k,l=1}^N \al_k\al_l y_ky_l
K(x_k, x_l)
$$
under the constraints $0\leq \al_k\leq N\ga w_k$, $\sum_{k=1}^N \al_k y_k =
0$. One retrieves the usual SVM formulation with the change of
variables $\al_k \to \al_k/w_k$ and $y_k \to w_ky_k$.

\subsection{Boosting and regression}
The same idea can be applied, up to some extent, to non-linear regression problems. Here,
the coefficients  $\al_j$ are not needed because, most of the time,
if a function $f$ belongs to a regression class, the function $\al f$
will also belong to it. So, in this case, the issue is to find 
$$
f = f_1 + \cdots + f_K$$
by a greedy (online) procedure, to minimize, say, the mean square
error. Then, the procedure at step $j+1$ is to minimize
$$
\sum_{k=1}^N (y_k - f^{(j)}(x_k) - f(x_k))^2,
$$
which corresponds to the regression of the residuals $y_k -
f^{(j)}(x_k)$ on $x_k$. This has been applied with tree models, which are described in the next chapter.



==> generative_.tex <==
\chapter{Deep Generative Methods}
\label{chap:generative}


\section{Normalizing flows}
\label{sec:norm.flows}
\subsection{General concepts}
We develop, in this chapter, methods that model stochastic processes using  a feed-forward approach that generates complex random variables using non-linear transformations of simpler ones. Many of these methods can be seen as instances of structural equation models (SEMs), described in \cref{sec:sem}, with, for deep-learning implementations, high-dimensional parametrizations of \cref{eq:sem}. 

With start with the formally simple case where the modeled variable takes values in $\mathbb R^d$ and is modeled as
\[
X = g(Z)
\]
where $Z$ also takes values in $\mR^d$, with a known distribution, and $g$ is $C^1$, invertible, with a $C^1$ inverse on $\mathbb R^d$, i.e., is a {\em diffeomorphism} of $\mR^d$. Let us denote by $h$ the inverse of $g$.

If $Z$ has a p.d.f. $f_Z$ with respect to Lebesgue's measure, then, using the change of variable formula, the p.d.f. of $X$ is 
\[
f_X(x) = f_Z(h(x))\ |\det{\partial_x h(x)}|.
\]

Now, given a training set $T = (x_1, \ldots, x_N)$, the log-likelihood, considered as a function of $h$, is given by
\begin{equation}
\label{eq:norm.flow.lik}
\ell(h) = \sum_{k=1}^N \log f_Z(h(x_k)) + \sum_{k=1}^N \log |\det{\partial_x h(x_k)}|\,.
\end{equation}
This expression should then be maximized with respect to $h$, subject to some restrictions or constraints to avoid overfitting.

%which can be implemented using standard optimization techniques if $h$ (and its differential) is known explicitly. Note that both $g$ and $h$ are needed in this framework: $g$ to sample from the distribution of $X$ and $h$ to estimate the parameter $\theta$.

\subsection{A greedy computation}
One can define a rich class of diffeomorphisms through iterative compositions of simple transformations. This framework was introduced in \citep{tabak2010density}, where a greedy approach was suggested to build such compositions. The method was termed ``normalizing flows,'' since it create a discrete flow of diffeomorphisms that transform the data into a sample of a normal distribution.

We quickly describe the basic principles of the algorithm. One starts with a 
parametrized family, say $(\psi_\alpha, \alpha \in A)$ of diffeomorphisms of $\mR$. Such families are relatively easy to design, one example proposed in \citep{tabak2010density} being a smoothed version of the piecewise linear function
\[
u \mapsto v_0 + (1-\sigma) u + \gamma |(1-\sigma) u - u_0|
\]
which is increasing as soon as $0\leq \max(\sigma, \gamma) < 1$. The smoothed version has an additional parameter, $\epsilon$, and takes the form
\[
u \mapsto v_0 + (1-\sigma) u + \gamma \sqrt{\epsilon^2 + ((1-\sigma) u - u_0)^2}.
\]
This transformation is parametrized by $\alpha = (v_0, \sigma, \gamma, u_0, \epsilon)$. 
Other families of parametrized transformations can be designed. 


A multivariate transformation $\phi_{\boldsymbol\alpha, U}: \mR^d\to\mR^d$ can then be associated to families $\boldsymbol\alpha = (\alpha_1, \ldots, \alpha_d)$ and orthogonal matrices $U$  by taking
\[
\phi_{\boldsymbol\alpha, U}(x) = \begin{pmatrix}
\psi_{\alpha_1}(\pe y1)\\ \vdots \\ \psi_{\alpha_d}( \pe yd)
\end{pmatrix}
\]
with $y = Ux$. 


The algorithm in \citep{tabak2010density} is initialized with $h_0 = \id[d]$ and updates the transformation at step $n$ according to 
\[
h_{n} = \phi_{\boldsymbol\alpha_n, U_n}\circ h_{n-1}.
\] 

In this update, $U_n$ is generated as a random rotation matrix, and $\boldsymbol\alpha_n$ is determined as a gradient ascent update (starting from $\boldsymbol\alpha = 0$) for the maximization of 
\[
\boldsymbol\alpha \mapsto \ell(\phi_{\boldsymbol\alpha, U_n}\circ h_{n-1}).
\]
(Here, the current value $h_{n-1}$ is not revisited, therefore providing a ``greedy'' optimization method.)

Letting $z_{n,k} = h_n(x_k)$, the chain rule implies that   
\begin{multline*}
\ell(\phi_{\boldsymbol\alpha, U_n}\circ h_{n-1})) = \sum_{k=1}^N \log f_Z(\phi_{\boldsymbol\alpha, U_n}(z_{n-1,k})) + \sum_{k=1}^N \log |\det{\phi_{\boldsymbol\alpha, U_n}(z_{n-1,k})}| \\+ \sum_{k=1}^N \log |\det{\partial_x h_{n-1}(x_k)}|\,.
\end{multline*}
Since the last term does not depend on $\boldsymbol\alpha$, we see that it suffices to keep track of the ``particle'' locations,  $z_{n-1, k}$ to be able to compute $\boldsymbol\alpha_n$. Note also that these locations are easily updated with
$z_{n, k} = \phi_{\boldsymbol\alpha_n, U_n}(z_{n-1, k})$.

\subsection{Neural implementation}
This iterated composition of diffeomorphisms obviously provides a neural architecture  similar to those discussed in \cref{chap:neural.nets}. Fixing the number of iterations to be, say, $m$, one can consider families of diffeomorphisms $(\phi_\theta)$ indexed by a parameter $w$ (we had $w = (\boldsymbol\alpha, U)$ in the previous discussion), and optimize 
\cref{eq:norm.flow.lik} over all functions $h$ taking the form $h = \phi_{w_m} \circ \cdots \circ \phi_{w_1}$. Letting $z_{j,k} =  \phi_{w_j} \circ \cdots \circ \phi_{w_1}(x_k)$ for $j\leq m$ (with $z_{0,k} = x_k$), we can write
\[
\ell(h) = \sum_{k=1}^N \log f_Z(z_{m,k}) + \sum_{k=1}^N \sum_{j=1}^m \log |\det{\partial_x \phi_{w_j}(z_{j-1,k})}|.
\]

Normalizing flows in this form are described in \citep{rezende2015variational,kobyzev2020normalizing,
papamakarios2021normalizing}. The gradient of $\ell$ with respect to the parameters $w_1, \ldots, w_m$ can be computed by backpropagation. We note however that, unlike typical neural implementations, the parameters may come with specific constraints, such as $U\in \CO_d(\mR)$ when $w = (\boldsymbol\alpha, U)$, so that the gradient and associated displacement may have to be adapted compared to standard gradient ascent implementations (see \cref{sec:grad.orthogonal} for a discussion of first-order implementations of gradient methods for functions of orthogonal matrices, and \citep{absil2008optimization} for more general methods on optimization over matrix groups).

\subsection{Time-continuous version}
In \cref{sec:continuous.nn}, we described how diffeomorphisms could be generated as flows of differential equations, and this remark can be used to provide a time-continuous version of normalizing flows. Using \cref{eq:neural.ode}, one generates trajectories $z(\cdot)$ by solving over, say, $[0, T]$
\[
\partial_t z(t) = \psi_{w(t)}(z(t))
\]
with $z(0) = x$ for some function $w: t\mapsto w(t)$. Letting $z(t) = h_{w}(t, x)$ (which defines $h_w$), we know that, under suitable assumptions on $\psi$, the mapping $x \mapsto h_w(t, x)$ is a diffeomorphism of $\mR^d$. 
%Denoting by $h_{w}(T, \cdot)$ the inverse of $g_w(T,\cdot)$, 
One can then maximize  
\[
\ell(h_w(T, \cdot)) = \sum_{k=1}^N \log f_Z(h_w(T, x_k)) + \sum_{k=1}^N \log |\det{\partial_x h_w(T, x_k)}|
\]
with respect to the function $w$. Let $z_k(t) = h_w(t, x_k)$ and $J_k(t) = \log |\det{\partial_x h_w(t, x_k)}|$. We have, by definition 
\[
\partial_t z_k(t) = \psi_{w(t)}(z_k(t))
\]
with $z_k(0) = x_k$. One can also show that
\[
\partial_t J_k(t) = \nabla\cdot \psi_{w(t)}(z_k(t))
\]
with $J_k(0) = 0$,
where the r.h.s. is the divergence of $\psi_{w(t)}$ evaluated at $z_k(t)$. We provide a quick (and formal) justification of this fact. First note that differentiating $\partial_t h_w(t,x) = \psi_{w(t)}(h_w(t,x))$ with respect to $x$ yields
\[
\partial_t \partial_x h_w(t,x) = \partial_x \psi_{w(t)}(h_w(t,x)) \partial_x h_w(t,x).
\] 
The mapping $\mathcal J: A \mapsto \log |\det(A)|$ is differentiable on the set of invertible matrices and is such that $d\mathcal J(A) H = \trace(A^{-1}H)$. Applying the chain rule, we find
\begin{align*}
\partial_t \log|\det{\partial_x h_w(t,x)}| &= \trace(\partial_x h_w(t,x)^{-1} \partial_x \psi_{w(t)}(h_w(t,x)) \partial_x h_w(t,x))\\
& = 
\trace(\partial_x \psi_{w(t)}(h_w(t,x))) = \nabla\cdot \psi_{w(t)}(h_w(t,x)).
\end{align*}

From this, it follows that the time-continuous normalizing flow problem can be reformulated as maximizing
\[
\sum_{k=1}^N \log f_Z(z_k(T)) + \sum_{k=1}^N J_k(T)
\]
subject to $\partial_t z_k(t) = \psi_{w(t)}(z_k(t))$, 
$\partial_t J_k(t) = \nabla\cdot \psi_{w(t)}(z_k(t))$, $z_k(0)=x_k$, $J_k(0) = 0$. This is an optimal control problem, whose analysis can be done similarly to that made in \cref{sec:neural.ode}, provided that $\nabla\cdot \psi_{w(t)}$ can be expressed in closed form.

Note that the inverse of $h_w(T, \cdot)$, which provides the generative model going from $Z$ to $X$ can also be obtained as the solution of an ODE. Namely, if one solves the differential equation
\[
\partial_t x(t) = - \psi_{w(T-t)}(x(t))
\]
with initial condition $x(0) = z$, then $x(T)$ solves the equation $h_w(T, \cdot) = z$.

\section{Non-diffeomorphic models and variational autoencoders}
\label{sec:gen.nondiff}
\subsection{General framework}
The previous discussion addressed the situation  $X = g(Z)$ when $g$ is a diffeomorphism, which required, in particular, that $X$ and $Z$ are real vectors with identical dimensions. This may not always be desirable, as one may prefer a small-dimensional variable $Z$ (in the spirit of the factor analysis methods discussed in \cref{chap:dim.red}), or a high-dimensional $Z$ to increase, for example the modeling power. In addition, the observation variables may be discrete, which precludes the use of the change of variables formula. In such cases, $Z$ has to be treated as a hidden variable using one of the methods discussed in \cref{chap:var.bayes}.  

It will convenient  to model the generative process in the form of a conditional distribution of $X$ given $Z$ rather than a deterministic function. We place ourselves in the framework of \cref{chap:var.bayes} (with slightly modified notation) and let $\CR_X$ and $\CR_Z$ denote the measured spaces over where $X$ and $Z$ take their values, with measures $\mu_X$ and $\mu_Z$, and assume that the conditional distribution of $X$ given $Z=z$ has density $f_X(x\mid z, \theta)$ with respect to $\mu_X$, for some parameter $\theta$. We also assume that $Z$ has a distribution with density $f_Z$ with respect to $\mu_Z$, that we assume given and unparametrized. One can then directly apply the algorithms provided in \cref{chap:var.bayes}, and in particular the variational methods described in \cref{sec:var.approx} with an appropriate definition of the approximation of the conditional density of $Z$ given $X$. An important example in this context is provided by variational autoencoders (VAEs) that we now present.


\subsection{Generative model for VAEs}
\label{sec:vae}
VAEs \citep{kingma2014auto-encoding,kingma2019introduction} model $X\in \mR^d$ as $X = g(Z, \theta) + \ep$ where $\ep$ is a centered Gaussian noise with covariance matrix $Q$. The function $g$ is typically nonlinear, and VAEs have been introduced with this function modeled as a deep neural network (see \cref{chap:neural.nets}). Letting $\phi_\CN(\ccdot;\,0, Q)$ denote the p.d.f. of the Gaussian distribution $\CN(0, Q)$, the conditional distribution of $X$ given $Z=z$ has density
\[
f_X(x\mid z, \theta) = \phi_\CN(x - g(z, \theta))\,;\, 0, Q)
\]
with respect to Lebesgue's measure on $\mR^d$.

Following the procedure in \cref{sec:var.approx}, we define an approximation of the conditional distribution of $Z$ given $X$. Assuming that $Z\in \mR^p$, we let this distribution be $\CN(\mu(x, w), \Sigma(x, w))$ for some functions $\mu$ and $\Sigma$, $w$ being a parameter. To ensure that $\Sigma \succeq 0$, we will represent it in the form $\Sigma(x, w) = S(x, w)^2$ where $S$ is a symmetric matrix. In \citep{kingma2014auto-encoding}, both functions $\mu$ and $S$ are represented as neural networks parametrized by $w$. The joint density of $X$ and $Z$ is such that
\begin{align*}
\log f_{X,Z}(x,z\,;\,\theta, Q) &= \log \phi_\CN(x - g(z, \theta))\,;\, 0, Q) + \log f_Z(z)\\
&= -\frac12 (x - g(z, \theta))^T Q^{-1} (x - g(z, \theta)) - \frac12 \log \det Q - \frac d2 \log 2\pi + \log f_Z(z)
\end{align*}
We also have
\[
\log \phi_\CN(z\,;\, \mu(x, w), S(x, w)^2) = -\frac12 (z - \mu(x,w))^T S(x, w)^{-2} (z - \mu(x,w)) - \log\det S(x, w) - \frac p2 \log 2\pi.
\]

We can then rewrite the algorithm in \cref{eq:sga.var.2} as
\begin{equation}
\label{eq:sga.vae}
\left\{
\begin{aligned}
\theta_{n+1} &= \theta_n +\gamma_{n+1} \partial_\theta \log f_{X,Z}(X_{n+1},Z_{n+1};\theta_n, Q_n)
\\
Q_{n+1} &= Q_n +\gamma_{n+1} \partial_Q \log f_{X,Z}(X_{n+1},Z_{n+1};\theta_n, Q_n)
\\
w_{n+1} &= w_n + \gamma_{n+1} \log \left( \frac{f_{X,Z}(X_{n+1},Z_{n+1};\theta_n, Q_n)}{\phi_\CN(X_{n+1}\,;\, \mu(X_{n+1}, w_n), S(X_{n+1}, w_n)^2)}\right) \\
& \qquad\qquad \times \partial_w \log \phi_\CN(X_{n+1}\,;\, \mu(X_{n+1}, w_n), S(X_{n+1}, w_n)^2)
\end{aligned}
\right.
\end{equation}
where $X_{n+1}$ is drawn uniformly from the training data and 
\[
Z_{n+1} \sim \CN(\mu(X_{n+1}, w_n), S(X_{n+1}, w_n)^2).
\]
The derivatives in this system can be computed from those of $g, \mu$ and $S$ (typically involving back-propagation) and the  expression of the derivatives of the  determinant and inverse of a matrix provided in \cref{eq:det.der,eq:inv.der}. 
%Of course, one can modify the algorithm by sampling a minibatch of more than one training samples and their associated $Z$ variable.

The computations can be simplified if one  assumes that $f_Z$ is the p.d.f. of a standard Gaussian, i.e., $f_Z = \phi_\CN(\cdot;0, \Id[p])$. Indeed, in that case, the integral in \cref{eq:em.var}, which is, using the current notation,
\begin{equation}
\label{eq:var.vae}
\int_{\mR^p}\log \frac{\phi_\CN(x-g(z,\theta)\,;\, 0, Q)
\phi_\CN(z\,;\,0, \Id[p])}{\phi_\CN(z\,;\, \mu(x, w), S(x,w)^2)}
 \phi_\CN(z\,;\, \mu(x, w), S(x,w)^2) dz,
 \end{equation}
can be partially computed. For any two $p$-dimensional Gaussian p.d.f.'s, one has
\begin{multline}
\label{eq:gauss.kl}
\int_{\mR^p} \log \phi_\CN(z\,;\,\mu_1, \Sigma_1)\ \phi_\CN(z\,;\,\mu_2, \Sigma_2)\, dz = -\frac12\trace(\Sigma_1^{-1} \Sigma_2) - \frac{1}{2} (\mu_2-\mu_1)^T \Sigma_1^{-1} (\mu_2-\mu_1)\\ - \frac12 \log \det(\Sigma_1) - \frac{p}{2} \log(2\pi).  
\end{multline}
As a consequence, \cref{eq:var.vae} becomes
\begin{multline}
\label{eq:var.vae.2}
-\frac{1}{2} \myE_w\left((X-g(Z, \theta))^T Q^{-1}(X-g(Z, \theta))\right) - \frac12 \log \det Q - \frac{d}2 \log 2\pi \\ - \myE_w\left(\frac12 \trace(S(X,w)^2) + \frac{1}{2} |\mu(X,w)|^2 - \log \det(S(X,w))\right) + \frac p2,
\end{multline}
where $\myE_w$ denotes the expectation for the random variable $(X,Z)$ where $X$ follows a uniform distribution over training data and the  conditional distribution of $Z$ given $X=x$ is $\CN(\mu(x,w)\,,\,S(x,w)^2)$.

The algorithm proposed in \citet{kingma2014auto-encoding} introduces a change of variable $Z = \mu(X, w) + S(X,w) U$ where $U\sim\CN(0, \Id[p])$, rewriting \cref{eq:var.vae.2} as
\begin{multline}
\label{eq:var.vae.3}
-\frac{1}{2} \myE\left((X-g(\mu(X,w) + S(X,w)U, \theta))^T Q^{-1}(X-g(\mu(X,w) + S(X,w)U, \theta))\right) \\  - \myE_w\left(\frac12 \trace(S(X,w)^2) + \frac{1}{2} |\mu(X,w)|^2   - \log \det(S(X,w))\right)\\
- \frac12 \log \det Q - \frac{d}2 \log 2\pi + \frac p2,
\end{multline}
with a modified version of \cref{eq:sga.vae}. Letting
\begin{multline*}
F(\theta, Q, w, x, u) = -\frac{1}{2} (x-g(\mu(x,w) - S(x,w)U, \theta))^T Q^{-1}(x-g(\mu(x,w) - S(x,w)U, \theta))\\ - \frac12 \log \det Q  - \frac12 \trace(S(x,w)^2) - \frac{1}{2} |\mu(x,w)|^2   +  \log \det(S(x,w))
\end{multline*}
the resulting algorithm is
\begin{equation}
\label{eq:sga.vae.4}
\left\{
\begin{aligned}
\theta_{n+1} &= \theta_n +\gamma_{n+1} \partial_\theta F(\theta_n, Q_n, w_n, X_{n+1},U_{n+1})\\
Q_{n+1} &= Q_n +\gamma_{n+1} \partial_Q F(\theta_n, Q_n, w_n, X_{n+1},U_{n+1})
\\
w_{n+1} &= w_n - \gamma_{n+1} \partial_w F(\theta_n, Q_n, w_n, X_{n+1},U_{n+1})
\end{aligned}
\right.
\end{equation}
where $X_{n+1}$ is drawn uniformly from the training data and 
$U_{n+1} \sim \CN(0, \Id[p])$.

\subsection{Discrete data}
This framework can be  adapted to situations in which the observations are discrete. Assume, as an example, that $X$ takes values in $\{0,1\}^V$, where $V$ is a set of vertexes, i.e., $X$ is a binary Markov random field on $V$. Assume, as a generative model, that  conditionally to the latent variable $Z\in \mR^p$, the variables $\pe Xs, s\in V$ are independent and $\pe Xs$ follows a Bernoulli distribution with parameter $\pe gs(z, \theta)$, where $g: \mR^p \to [0,1]^V$. Assume also that $Z \sim \CN(0, \Id[p])$, and define, as above, an approximation of the conditional distribution of $Z$ given $X=x$ as a Gaussian with mean $\mu(x,w)$ and covariance matrix $S(x, w)^2$. Then, the joint density of $X$ and $Z$ (with respect to the product of the counting measure on $\{0,1\}^V$ and Lebesgue's measure on $\mR^p$) is
\[
\log f_{X,Z}(x,z\,;\,\theta) = \sum_{s\in V} (\pe xs \log \pe gs(z, \theta)+ (1-\pe xs)\log(1-\pe gs(z,\theta))) + \log \phi_\CN(z\,;\, 0, \Id[p])
\]
and \cref{eq:sga.vae} becomes
\begin{equation}
\label{eq:sga.vae.disc}
\left\{
\begin{aligned}
\theta_{n+1} &= \theta_n +\gamma_{n+1} \partial_\theta \log f_{X,Z}(X_{n+1},Z_{n+1};\theta_n, Q_n)
\\
\\
w_{n+1} &= w_n + \gamma_{n+1} \log \left( \frac{f_{X,Z}(X_{n+1},Z_{n+1};\theta_n)}{\phi_\CN(X_{n+1}\,;\, \mu(X_{n+1}, w_n), S(X_{n+1}, w_n)^2)}\right) \\
& \qquad\qquad \times \partial_w \log \phi_\CN(X_{n+1}\,;\, \mu(X_{n+1}, w_n), S(X_{n+1}, w_n)^2)
\end{aligned}
\right.
\end{equation}



\section{Generative Adversarial Networks (GAN)}
\label{sec:gan}

\subsection{Basic principles}
Similarly to the methods discussed so far, GAN's \citep{goodfellow2014generative}, use a one-step nonlinear generator
$X = g(Z, \theta)$, with $\theta\in \mR^K$, to model observed data (we here switch back to a deterministic relation), where $Z$ has a known distribution, with p.d.f. $f_Z$, for example $Z\sim \CN(0, \Id[p])$. However, unlike the exact or approximate likelihood maximization that were discussed in \cref{sec:norm.flows,sec:gen.nondiff}, GANs us a different criterion for estimating the parameter $\theta$ by minimizing metrics that can be approximated by optimizing a classifier.
 The classifier is a function $x \mapsto f(x, w)$, parametrized by $w\in \mR^M$, whose goal is to separate simulated samples from real ones: it takes values in $[0,1]$ and estimates the (posterior) probability that its input $x$ is real.  The adversarial paradigm in GAN's consists in estimating $\theta$ and $w$ together so that generated data, using $\theta$, are indistinguishable from real ones using the optimal $w$.
Their basic structure is summarized in Figure \ref{fig:gan.1}.

\begin{figure}[h]

	\begin{center}
		\begin{tikzpicture}[roundnode/.style={rectangle, draw=green!60, fill=green!5, thin, minimum size=20mm}, squarednode/.style={rectangle, draw=black!60, fill=gray!5, very thick},]
		\node[squarednode, minimum height=1cm] (C) {Classifier} ;
		\node[squarednode, minimum height= 1cm, minimum width = 1cm] (P) [above=.5cm of C] {Prediction} ;
		\node[squarednode, minimum height= 1cm, minimum width = 1cm] (W) [below=.5cm of C] {$W$} ;
		\node[squarednode, minimum height= 1cm, minimum width = 2cm] (T) [above right=-.4cm and .75cm of C] {Data} ;
		\node[squarednode, minimum height= 1cm, minimum width = 2cm] (S) [below right=-.4cm and .75cm of C] {Simulation} ;
		\node[squarednode, minimum height= 1cm, minimum width = 1cm] (G) [above right=-.4cm and .75cm of S] {Generator} ;
		\node[squarednode, minimum height= 1cm, minimum width = 1cm] (TH) [below=.5cm of G] {$\theta$} ;
		\node[squarednode, minimum height= 1cm, minimum width = 1cm] (N) [right=.75cm of G] {Noise} ;
		\draw[blue, thick,->>] (C.north) -- (P.south) node[midway, above] {};
		\draw[blue, thick,->>] (W.north) -- (C.south) node[midway, above] {};
		\draw[blue, thick,->>] (T.west) -- (C.east) node[midway, above] {};
		\draw[blue, thick,->>] (S.west) -- (C.east) node[midway, above] {};
		\draw[blue, thick,->>] (G.west) -- (S.east) node[midway, above] {};
		\draw[blue, thick,->>] (N.west) -- (G.east) node[midway, above] {};
		\draw[blue, thick,->>] (TH.north) -- (G.south) node[midway, above] {};
		\end{tikzpicture}
\caption{\label{fig:gan.1}
Basic structure of		
GAN's: $W$ is optimized to improve the prediction problem: ``real data'' vs. ``simulation''. Given $W$, $\th$ is optimized to worsen the prediction.}
		\end{center}
\end{figure}


\subsection{Objective function}
 Let $P_\th$ denote the distribution of $g(Z, \th)$, and $P_{\mathrm{true}}$ the target distribution of real data, represented by the variable $X$. 
One can formalize the ``real data'' vs. ``simulation'' problem with a  pair of random variables $(X_\theta, Y)$ where $Y$ follows a Bernoulli distribution with parameter $1/2$, and $P(X_\theta \in A \mid Y=y)$ is $P_{\mathrm{true}}(A)$ when $y=1$ and $P_\th(A)$ when $y=0$. 
 Given a loss function $r: \{0,1\} \times [0,1] \to [0, +\infty)$, one can define 
\[
U(\th, w) = \myE(r(Y, f(X_\theta, w)))
\]
and 
\[
U^*(\th) = \min_{w\in \mR^M} U(\th, w).
\]
 We want to maximize $U^*$ or, equivalently,  solve the optimization problem
\[
\th^* = \argmax_{\th \in \mR^K} \min_{w\in \mR^M} U(\th, w).
\]

Note that
\[
2 U(\th, w) = \myE(r(1, f(X, w))) + \myE(r(0, f(X_\theta, w)))
\]
so that choosing the cost requires to specify the two functions $t\mapsto r(1, t)$ and $t\mapsto r(0, t)$. 
 In \citet{goodfellow2014generative}, they are:
\begin{equation}
\label{eq:gan.original.cost}
\begin{aligned}
r(1,t) &=  -\log t\\
r(0,t) & = -\log (1-t).
\end{aligned}
\end{equation}

\subsection{Algorithm}
Using costs in \cref{eq:gan.original.cost}, one must compute
\[
\begin{aligned}
\th^* &= \argmin_{\th \in \mR^K} \max_{w\in \mR^M} \Big(\myE(\log f(X, w)) + \myE(\log(1-f(X_\theta, w)))\Big)\\
 &= \argmin_{\th \in \mR^K} \max_{w\in \mR^M} \Big(\myE(\log f(X, w)) + \myE(\log(1-f(g(Z, \th), w)))\Big).
 \end{aligned}
\]

Such min-max, or saddle-point problem are numerically challenging. The following algorithm was proposed in \citet{goodfellow2014generative}, and also includes a stochastic approximation component. Indeed,  in practice, $E_{\mathrm{true}}$ is only known through the observation of training data, say $x_1, \ldots, x_N$. Moreover, 
 $E_\th$ is only accessible through Monte-Carlo simulation, so that both  expectations can only be approximated through finite-sample averaging. 


\begin{algorithm}[GAN training algorithm]
\label{alg:gan}
\begin{enumerate}[label = \arabic*., wide=0.5cm]
\item Extract a batch of $m$ examples from training data, simulate $m$ samples according to $P_\th$ and run a few (stochastic) gradient ascent steps with fixed $\th$ to update $w$, replacing expectations by averages.
\item Generate $m$ new samples of $Z$ and update $\th$ with fixed $w$ by iterating a few steps of (stochastic) gradient descent.
\end{enumerate}
\end{algorithm}
\bigskip

\subsection{Associated probability metric and Wasserstein GANs}
Let $\CF$ be the family of all measurable functions: $f: \mR^d\to [0,1]$.
Given two  random variables $X_1, X_2:\Omega\to \mR^d$, with respective distributions $P_1, P_2$ (so that $\myP(X_i\in A) = P_i(A)$, consider the function
\[
D(P_1, P_2) = 2\log 2 + \max_{f\in\CF} \Big(\myE(\log f(X_1)) + \myE(\log(1-f(X_2)))\Big)
\]
 Assume that $X_1$ (resp. $X_2$) has a p.d.f. $g_1$ (resp. $g_2$) with respect to some measure $\mu$.
 Then
\[
\myE(\log f(X_1)) + \myE(\log(1-f(X_2))) = \int_{\mR^d} (g_1\log f + g_2\log(1-f)) d\mu
\]
which is maximal at $f^* = g_1/(g_1+g_2)$.
 For this $f^*$, 
\[
\begin{aligned}
2\log 2 + \myE(\log f^*(X_1)) + \myE(\log(1-f^*(X_2))) 
&= \int_{\mR^d} g_1 \log \frac{2g_1}{g_1+g_2} dx + \int_{\mR^d} g_2 \log \frac{2g_2}{g_1+g_2} d\mu\\
&= \KL\left(g_1\ \big\|\ \frac{g_1+g_2}2\right) + \KL\left(g_2\ \big\|\ \frac{g_1+g_2}2\right).
\end{aligned}
\]

 This last expression is the {\em Jensen-Shannon divergence} between $g_1$ and $g_2$ (cf. \cref{sec:divergence}).   One can then define
\[
\what D(P_1, P_2) = 
\max_{w\in \mR^M} \Big(\myE(\log f(X_1, w)) + \myE(\log(1-f(X_2, w)))\Big)
\]
as an approximation of $D$ in which the set of all possible functions with values in $[0,1]$ is replaced by those arising from the GAN classification network, parametrized by $w$.
 This approximation is useful when $g_1, g_2$ are only observable through random sampling or simulation.
 With this interpretation, GANs minimize $\what D(P_{\mathrm{true}}, P_\th)$.


 This discussion suggests that new types of GAN's may be designed using other discrepancy functions between probability distributions, provided that they can be expressed in terms of the maximization of some quantity over some space of functions.
  Consider, for example, the norm in total variation, defined by (for discrete distributions)
\[
D_{\mathrm{var}}(P_1,P_2) = \frac 12 \sum_{x} |P_1(x) - P_2(x)|.
\]
or, in the general case $D_{\mathrm{var}}(P_1,P_2)  = \max_A(P_1(A) - P_2(A))$.

 If $\CF$ is the space of continuous functions $f: \mR^d \to [0,1]$, then we also have (cf. \cref{prop:var.dist})
\[
D_{\mathrm{var}}(P_1,P_2)  = \max_{f\in\CF} (\myE(f(X_1)) - \myE(f(X_2))).
\]
 Since neural nets typically generate continuous functions with values in $[0,1]$, one could train GANs by maximizing 
\[
\what D_{\mathrm{var}}(P_1, P_2) = 
\max_{w\in \mR^M} \Big(\myE(f(X_1, w)) - \myE(f(X_2, w))\Big).
\]
However, the total variation distance can be too crude as a way to compare probability distributions, especially when these distributions have atoms (points $x$ such that $P_i(\{x\})>0$. For example, the total variation distance between two Dirac distributions at, say,  $x_1$ and $x_2$ in $\mR^d$ is always 1, unless $x_1=x_2$. As a consequence, if $x_n$ converges to $x$, with $x_n\neq x$, then $D_{\mathrm{var}}(\delta_{x_n}, \delta_x)\not\to 0$.

 
 The  Monge-Kantorovich distance (introduced in \cref{sec:monge}) is better adapted. Using \cref{eq:monge} with $\rho(x,y) = |x-y|$ and \cref{th:kant.rub}, we have
\begin{equation}
\label{eq:gan.MK}
D_{\mathrm{MK}}(P_1,P_2)  = \max_{f\in\CF} (\myE(f(X_1)) - \myE(f(X_2)))
\end{equation}
where $\CF$ is now the space of contractive (or 1-Lipschitz) functions. 
 Using the fact that a neural network with all weights bounded by a constant $K$ generates a function whose Lipschitz constant is controlled solely by $K$, one can then approximate (up to a  multiplicative constant) the Wasserstein distance by
\[
\what D_{\mathrm{MK}}(P_1,P_2)  = \max_{w\in \mathbb W} \Big(\myE(f(X_1, w)) - \myE(f(X_2, w))\Big)
\]
where $\mathbb W$ is the set of all weights bounded by a fixed constant. Wasserstein GANs (WGANs \citep{arjovsky2017wasserstein}) must then solve the saddle-point problem 
\[
U(\th, w) = \max_{w\in \mathbb W} \Big(\myE(f(X, w)) - \myE(f(X_\theta, w))\Big)
\]
and 
\[
U^*(\th) = \min_{w\in \mR^M} U(\th, w), 
\]
with an algorithm similar to that described earlier.

\begin{remark}
\label{rem:improved.gan}
As a final reference, we note the ``improved WGAN'' algorithm introduced in \citet{gulrajani2017improved} in which the boundedness constraint in the weights is replaced by an explicit control of the derivative in $x$ of the function $f$. Given independent $X_1$ and $X_2$ with respective distributions $P_1$, $P_2$, define a random variable $Z = (1-U) X_1 + U X_2$ where $U$ is uniformly distributed over $[0, 1]$ and $(U, X_1, X_2)$ are independent. Then, \citet{gulrajani2017improved} use the following approximation of the Wasserstein distance between $P_1$ and $P_\th$:
\[
\what D_{\mathit{MK}}(P_{\mathrm{true}},P_\th)  = \max_{w\in \mathbb W} \Big(E_{\mathrm{true}}(f(X, w)) - E_{\th}(f(X, w)) - \tilde E_\th((|\prt_z f(Z, w)| - 1)^2) 
\Big).
\]
This approximation is justified by the fact that optimal solutions of \cref{eq:gan.MK} satisfy (almost surely for the optimal coupling)
\[
f(y) - f(x) = |x-y|
\]
(see \citet{villani2009optimal}, theorem 5.10 and \citet{gulrajani2017improved}).
\end{remark}

\section{Reversed Markov chain models}

\subsection{General principles}
The discussions in \cref{sec:gen.nondiff,sec:gan} can be applied to sequences of structural equations (describing finite Markov chains) in the form
\[
\left\{
\begin{aligned}
Z_0 &= \bfxi_0\\
Z_{k+1} &= g(Z_k, \bfxi_k; \theta_k), \ k=0, \ldots, m-1\\
X &= Z_m
\end{aligned}
\right.
\]
where $\bfxi_0, \ldots, \bfxi_{m-1}$ are random variables with fixed distribution. Indeed, letting $\tilde Z = (\bfxi_0, \ldots, \bfxi_{n-1})$ and $\tilde \theta = (\theta_0, \ldots, \theta_{m-1})$ the whole system can be considered as a function $X = G(\tilde Z, \tilde{\theta})$ as considered in these sections. This representation, however, includes a large number of hidden variables, and it is unclear whether much improvement can be added to the case $m=1$ to justify the additional computational load. 

While direct Markov chain modeling may have a limited appeal, reversed Markov chains use a different generative approach in that they first model a forward Markov chain $Z_n, n\geq 0$ which is ergodic with known (and easy to sample from) limit distribution $Q_\infty$, and initial distribution $Q_{\mathrm{true}}$, the true distribution of the data. If one fixes  a large enough number of steps, say, $\tau$, then it is reasonable to assume that $Z_\tau$ approximately follows the limit distribution, $Q_\infty$. One can then (approximately) sample from $Q_{\mathrm{true}}$ by sampling $\tilde Z_0$ according to $Q_\infty$ and then applying $\tau$ steps of the time-reversed Markov chain.  

Reversed chains were discussed in \cref{sec:mcmc.reversible}. Assuming that $Q_{\mathrm{true}}$ and $P(z, \, \cdot\, )$ have a density with respect to a fixed measure $\mu$ on $\CR_Z$,  we found that $\tilde Z_k = Z_{\tau-k}$ is a non-homogeneous Markov chain whose transition probability $\tilde P_k(x, A) = P(\tilde Z_{k+1} \in A\mid \tilde Z_k = x)$ has density
\[
\tilde p_k(x,y) =  \frac{p(y,x)q_{\tau-k-1}(y)}{q_{\tau-k}(x)}
\]
with respect to $\mu$, where $q_n$ is the p.d.f. of $Q_n = Q_{\mathrm{true}} P^n$, the distribution of $Z_n$.

The distributions $Q_n, n\geq 0$ are unknown, since they depend on the data distribution $P_{\mathrm{true}}$, and the transition probabilities above must be estimated from data to provide a sampling algorithm from the reversed Markov chain. While, at first glance, this does not seem like a simplification of the problem, because one now has to sample from a potentially large number ($\tau$) of distributions instead of one, this leads, with proper modeling and some intensive learning, to powerful generative models.

To make this approach more efficient, the forward chain should be making small changes to the current configuration at each step (e.g., adding a small amount of noise). This ensures that the reversed transition probabilities $\tilde p_k(x, \cdot)$ are close to Dirac distributions and are therefore likely to be well approximated by simple unimodal distributions such as Gaussians. Importantly, the estimation problem does not have hidden data: given an observed sample, one can simulate $\tau$ steps of the forward chain to obtain, after reversing the order, a full observation of the reversed chain. Moreover, in some cases, analytical considerations can lead to partial computations that facilitate the modeling of the reversed transitions.

\subsection{Binary model}
We now take some examples, starting with a discrete case. Let $Q_{\mathrm{true}}$ be the distribution of a binary random field with state space $\{0, 1\}$ over a set of vertexes $V$, i.e., with the notation of \cref{sec:random.fields}, $\CR_X = \CF(V)$ with $F = \{0,1\}$. Fix a small $\ep>0$ and define the transition probability $p(x,y)$ for $x,y \in \CF(V)$ by
\[
p(x,y) = \prod_{s\in V} \left((1-\epsilon) \bfone_{\pe y s = \pe x s} + \epsilon\bfone_{\pe y s = 1 - \pe x s}\right).
\]
Since $p(x,y) >0$ for all $x$ and $y$, the chain converges (uniformly geometrically) to its invariant probability $Q_\infty$ and one easily checks that this probability is such that all variables are independent Bernoulli random variables with success probability $1/2$. Assuming that $\tau$ is large enough so that $Q_\tau \simeq Q_\infty$, the sampling algorithm initializes the reversed chain as independent Bernoulli$(1/2)$ variables and runs $\tau$ steps using the transitions $\tilde p_k$, which must be learned from data. 

For this model, we have 
\[
q_k(x) = \sum_{y\in \CF(V)} q_{k-1}(y) p(y,x).
\]
For this transition, the probabililty of flipping two or more values of $y$ is 
\[
1 - (1-\epsilon)^N - N\epsilon (1-\epsilon)^{N-1}  = \frac{N(N-1)}2 \epsilon^2 + o(\epsilon^2)
\]
with $N = |V|$. We will write $x\sim_s y$ if $\pe ys = 1 - \pe x s$ and $\pe yt = \pe xt$ for $s\neq t$, and we will write $x\sim y$ if $x\sim_s y$ for some $s$.
With this notation, we have 
\[
q_k(x) = (1-N\epsilon) q_{k-1}(x) + \epsilon \sum_{y: y\sim x} q_{k-1}(y) + O(\epsilon^2)
\]

Since it implies that $q_k(x) = q_{k-1}(x) + o(\epsilon)$, this expression can be reversed as
\[
q_{k-1}(y) = (1+N\epsilon) q_{k}(y) - \epsilon \sum_{x: x\sim y} q_{k}(x) + O(\epsilon^2)
\]
Similarly, we have
\[
p(y,x) = (1-N\epsilon) \bfone_{x=y} + \epsilon \bfone_{x \sim y } + O(\epsilon^2).
\]
This gives
\[
p(y,x)q_{k-1}(y) =  q_{k}(x) \bfone_{x=y} - \epsilon \bfone_{x=y}  \sum_{x': x'\sim y} q_{k}(x' ) + \epsilon
q_k(y) \bfone_{x\sim y } + O(\epsilon^2),
\]
and we finally get
\[
\tilde p_k(x,y) = \left(1 - \epsilon   \sum_{x': x'\sim y} \frac{ q_{\tau-k}(x' )}{q_{\tau-k}(x)}\right) \bfone_{x=y} + \epsilon
\frac{q_{\tau-k}(y)}{q_{\tau-k}(x)} \bfone_{x\sim y } + O(\epsilon^2)
\]

If one lets $\pe{\sigma_k}s(x) = \frac{q_{\tau-k}(y)}{q_{\tau-k}(x)}$ with $y\sim_s x$, and defines
\[
\hat p_k(x,y) = \prod_{s\in V} \left((1-\epsilon \pe{\sigma_k}s(x)) \bfone_{\pe y s = \pe x s} + \epsilon \pe{\sigma_k}s(x)\bfone_{\pe y s = 1 - \pe x s}\right),
\]
one checks easily that $\hat p_k(x,y) = \tilde p_k(x,y) + O(\epsilon^2)$. This suggests modeling the reversed chain using transitions $\hat p_k$, for which the mapping $x\mapsto (\pe{\sigma_k}s(x), s\in V)$ needs to be learned from data (for example using a deep neural network).  Note that $1 - \sigma_k(x)$ is precisely the score function introduced for discrete distributions in \cref{rem:score.discrete}. 

\subsection{Model with continuous variables}
We now switch to an example with vector-valued variables, $\CR_X = \mR^d$, and assume that the forward Markov chain is such that, conditionally to $X_n=x$,  
\[
X_{n+1} \sim \CN(x + h f(x), \sqrt h\Id[d]),
\]
 where $f$ is $C^1$. We saw in \cref{sec:mcmc.rd} that, when $f = -\nabla H/2$ for a $C^2$ function $H$ such that $\exp(-H)$ is integrable, this chain converges (approximately for small $h$) to a limit distribution with p.d.f. (with respect to Lebesgue's measure) proportional to $\exp(-H)$.  In the linear case, in which $f(x) = -Ax/2$ for some positive definite symmetric matrix $A$, so that $H(x) = \frac12 x^TAx$, the limit distribution can be identified exactly as $\CN(0, \Sigma_h)$ where $\Sigma_h$ satisfies the equation
\[
A\Sigma_h + \Sigma_h A - \frac{h}{2} A^2 - 2\Id[d] = 0
\]  
whose solution is $\Sigma_h = (A - hA^2/4)^{-1}$
(details being left to the reader). This implies that this limit distribution can be easily sampled from for any choice of $A$. 

We now return to general $f$'s and make, like in the discrete case, a first-order identification of the reversed chain. We note that, for any smooth function $\gamma$, 
\[
\myE(\gamma(X_{n+1})\mid X_n = x) = \myE(\gamma(x + h f(x) + \sqrt hU))
\]
where $U \sim \CN(0, \Id[d])$. Making the second order expansion
\[
\gamma(x + h f(x) + \sqrt hU) = \gamma(x)  + \sqrt h \nabla \gamma(x)^T U + h \nabla \gamma(x)^Tf(x) + \frac{h}{2} U^T \nabla^2\gamma(x) U + o(h)
\]
and taking the expectation gives
\begin{equation}
\label{eq:forward.markov}
\myE(\gamma(X_{n+1})\mid X_n = x) = \gamma(x) + h \nabla \gamma(x)^Tf(x) +\frac{h}{2} \Delta \gamma(x) + o(h).
\end{equation}

Considering the reversed chain, and letting $q_k$ denote the p.d.f. of $X_k$ for the forward chain, we have
\begin{align*}
\myE(\gamma(X_{k-1}) \mid X_{k} = x) & = \int_{\mR^d} \gamma(y) \tilde p_{k}(x,y) dy\\
& = \int_{\mR^d} \gamma(y)  p(y,x)  \frac{q_{k-1}(y)}{q_k(x)}dy\\
& = \frac{1}{(2\pi h)^{d/2}}\int_{\mR^d} \gamma(y)    \frac{q_{k-1}(y)}{q_k(x)} e^{-\frac1{2h} |x - y - h f(y)|^2} dy\\
& = \frac{1}{(2\pi)^{d/2}}\int_{\mR^d} \gamma(x - \sqrt h u)    \frac{q_{k-1}(x - \sqrt h u)}{q_k(x)} e^{-\frac1{2} |u - \sqrt h f(x - \sqrt h u)|^2} dy,
\end{align*}
with the change of variable $u = (x - y)/\sqrt h$. We make a first-order expansion of the terms in this integral, with
\[
\gamma(x - \sqrt h u)  q_{k-1}(x - \sqrt h u) = \gamma(x)  q_{k-1}(x) - \sqrt h \nabla (\gamma q_{k-1})(x)^T u + \frac h2 u^T \nabla^2(\gamma q_{k-1})(x) u + o(h)
\]
and
\begin{align*}
e^{-\frac1{2} |u - \sqrt h f(x - \sqrt h u)|^2} &=  e^{-\frac1{2}|u|^2} e^{ \sqrt h u^T f(x) - h u^Td f(x) u - \frac12 |f(x)|^2 + o(h)}\\
&=  e^{-\frac1{2}|u|^2} \left(1 + \sqrt h u^T f(x) - h u^Td f(x) u - \frac h2 |f(x)|^2 + \frac h2  |u^T f(x)|^2 + o(h)\right).
\end{align*}
Taking products
\begin{align*}
&\gamma(x - \sqrt h u)  q_{k-1}(x - \sqrt h u) e^{-\frac1{2} |u - \sqrt h f(x - \sqrt h u)|^2} \\
&=  e^{-\frac1{2}|u|^2} \gamma(x)  q_{k-1}(x) \left(1 + \sqrt h u^T f(x) - h u^Td f(x) u - \frac h2 |f(x)|^2 + \frac h2  |u^T f(x)|^2\right)\\
& + e^{-\frac1{2}|u|^2}\left(-\sqrt h \nabla (\gamma q_{k-1})(x)^T u - h (\nabla (\gamma q_{k-1})(x)^T u)(f(x)^Tu) + \frac h2 u^T \nabla^2(\gamma q_{k-1})(x) u \right) + o(h)
\end{align*}
We now take the integral with respect to $u$ (recall that $\myE(U^T A U) = \trace(A)$ if $A$ is any square matrix and $U$ is standard Gaussian), so that
\begin{align*}
&\frac{1}{(2\pi)^{d/2}}\int_{\mR^d}\gamma(x - \sqrt h u)  q_{k-1}(x - \sqrt h u) e^{-\frac1{2} |u - \sqrt h f(x - \sqrt h u)|^2} du\\
&=  \gamma(x)  q_{k-1}(x) + h \left( -\gamma(x)  q_{k-1}(x) \nabla \cdot f(x) 
- \nabla (\gamma q_{k-1})(x)^T f(x) + \frac 12 \Delta(\gamma q_{k-1})(x)\right) + o(h)\\
&=  q_{k-1}(x) \left(\gamma(x)  + h \left( -\gamma(x)  \nabla \cdot f(x) 
- \left(\frac{\nabla (\gamma q_{k-1})(x)}{q_{k-1}(x)}\right)^T f(x) + \frac 12 \frac{\Delta(\gamma q_{k-1})(x)}{q_{k-1}(x)}\right)\right) + o(h),
\end{align*}
where $\nabla\cdot f$ is the divergence of $f$.

To compute an expansion of  $q_k(x)$, it suffices to take $\gamma = 1$ above, so that
\[
q_k(x) =   q_{k-1}(x) \left(1  + h \left( - \nabla \cdot f(x) 
- \left(\frac{\nabla q_{k-1}(x)}{q_{k-1}(x)}\right)^T f(x) + \frac 12 \frac{\Delta q_{k-1}(x)}{q_{k-1}(x)}\right)\right) + o(h).
\]
We now take the first-order expansion of the ratio, removing terms that cancel, and get 
\[
\myE(\gamma(X_{k-1}) \mid X_{k} = x) = \gamma(x) - h \nabla \gamma(x)^T f(x) + h\nabla \gamma(x)^T\left(\frac{\nabla q_{k-1}(x)}{q_{k-1}(x)} \right) + \frac{h}{2} \Delta \gamma(x) + o(h).
\]

Comparing with \cref{eq:forward.markov}, we find that  $\tilde X_k = X_{\tau-k}$ behaves, for small $h$, like the non-homogeneous Markov chain
such that the conditional distribution of $\tilde X_{k+1}$ given $\tilde X_{k} = x$ is $\CN(x - h f(x) - h s_{\tau-k-1}(x), \sqrt h \Id[d])$, with $s_{\tau-k-1}(x) = - \nabla \log q_{\tau-k-1}$, the score function introduced in \cref{sec:score.matching}. One can therefore use score-matching methods from that section to estimate this distribution from observations of the forward chain initialized with training data. 

\subsection{Continuous-time limit}
\label{sec:reversed.diffusion}

The forward schemes described in the previous examples can be interpreted as continuous time processes over discrete or continuous variables. In the latter case, the example $X_{k+1} \sim \CN(x + h f(x), \sqrt h \Id[d])$ conditionally to $X_k = x$ is a discretization of the stochastic differential equation 
\[
dx_t = f(x_t) dt + dw_t
\]
(see \cref{rem:langevin}), where $w_t$ is a Brownian motion and the diffusion is initialized with $Q_{\mathrm{true}}$. We found that going backward meant (at first order and conditionally to $X_k=x$)
\[
X_{k-1} \sim \CN(x - h f(x) - h s_{k-1}(x), \sqrt h \Id)
\]
that we can rewrite as
\[
x_\tau - X_{k-1} \sim \CN(x_\tau - x + h f(x) + h s_{k-1}(x), \sqrt h \Id).
\]
Following the definition in \citet{anderson1982reverse}, this corresponds to a first-order discretization of the {\em reverse diffusion}
\[
dx_t = (f(x_t) + s_t(x_t)) dt + d\tilde w_t,\ t\leq \tau
\]
where $\tilde w_t$ is also a Brownian motion. This reverse diffusion with $X_\tau \sim Q_\infty$ will therefore approximately sample from $Q_{\mathrm{true}}$. (With this terminology, forward and reverse diffusions have similar differential notation, but mean different things.) Note that, in the continuous-time limit, the reverse Markov process follows the distribution of the reversed diffusion exactly.


\subsection{Differential of neural functions}

As we have seen in the previous two examples, estimating the reversed Markov chain requires computing the score functions of the forward probabilities. In the case of continuous variables, this score function is typically parametrized as  a neural network, so that the function $s_k(x) = -\nabla \log q_k(x)$ is computed as $s_k(x) = F(x;\CW_k)$, with the usual definition $F(x, \CW_k) = z_{m+1}$ with $z_{j+1} = \phi_j(z_j, w_{jk})$, $z_0 = x$ and $\CW_k =  (w_{0k}, \ldots, w_{mk})$. 

Assume that a training set $T$ is observed. Running the forward Markov chain initialized with elements of $T$ generates a new training set at each time step, that we will denote $T_k$ at step $k$. We have seen in \cref{sec:score.matching} that the score function $s_k$ could be estimated by minimizing, with respect to $\CW$
\[
 \sum_{x\in T_k} \left(|F(x,\CW) |^2  - 2\nabla \cdot  F(x,\CW)\right).
\]
This term involves the differential of $F$, which is defined recursively by (simply taking the derivative at each step)
\[
dF(x, \CW) = \zeta_{m+1}, \ \zeta_{j+1} = d\phi_j(z_j, w_{j})\zeta_j,
\]
 with $\zeta_0 = \Id[d]$. From this recursive definition, back-propagation can be applied, in principle, to compute the derivative of $dF(x, \CW)$ with respect to $\CW$.  The feasibility of this computation, however, is limited when $d$ is large ($d$ could be tens of thousands if one models images), since computing the $d\times d$ matrix $dF(x, \CW)$ is then intractable. 
 
One can note that, for any $h\in \mR^d$, the vector $dF(x, \CW) h$ also satisfies the recursion
\[
dF(x, \CW)h = \zeta_{m+1}h, \ \zeta_{j+1}h = d\phi_j(z_j, w_{j})\zeta_jh,
\]
with $\zeta_0h = h$ and 
\[
\nabla \cdot  F(x,\CW) = \sum_{i=1}^d \mathfrak e_i^T dF(x,\CW) \mathfrak e_i
\]
where $\mathfrak e_1, \ldots, \mathfrak e_d$ is the canonical basis of $\mR^d$. Putting the divergence of $F$ in this form does not reduce the computation cost (which is, roughly $d^2 m$, assuming that all $z_j$'s have the same dimension), but expresses the divergence term in a form that is amenable to stochastic gradient descent (which is typically already used to approximate the sum over $x$). Indeed, if $\xi$ follows any distribution with zero mean and covariance matrix equal to the identity (such as a standard Gaussian, or the uniform distribution on the unit sphere), then
\[
\nabla \cdot  F(x,\CW) = \myE(\xi^T dF(x,\CW) \xi)
\]
so that $\xi$ can be generated in minibatches in SGD implementations (see \citep{song2020sliced}, where this approach is called ``sliced score matching'').


==> higher_.tex <==
% !TEX root =  machine_learning.tex
\chapter{Inner Products and Reproducing Kernels}
\label{chap:higher}

\section{Introduction}
We will discuss later in this book various methods that specify the prediction is  as a linear function of the input. These methods are often applied after taking transformations of the original variables, in the form $x\mapsto h(x)$ (i.e., the prediction algorithm is applied to $h(x)$ instead of $x$). We will refer to $h$ as a ``feature function,'' which typically maps the initial data $x\in \CR$ to a vector space, sometimes of infinite dimensions, that we will denote $H$ (the ``feature space''). 

The present chapter provides a formal description of this framework, focusing, in particular, on situations in which $H$ has an inner product, as this inner product is often instrumental in the design of linear methods on $H$. Many machine learning methods can indeed be expressed either as functions of the coordinates of the input data in some space, or as functions of the inner products between the input samples. Such methods can bypass the difficulty of using high-dimensional features with the help of the theory of ``reproducing kernels,'' \citep{aronszajn1950theory,wahba1990spline} which ensures that the inner product between special classes of feature functions $h(x)$ and $h(x')$ can be explicitly computed as a function of $x$ and $x'$. 


\section{Basic Definitions}

\subsection{Inner-product spaces}
We recall that a real vector space\,\footnote{All vector spaces in these notes will be real, and will therefore only be referred as vector spaces.} is a set, $H$, on which an addition and a scalar product are defined, namely $(h,h') \in H\times H \mapsto h+h'\in H$ and $(\lambda, h) \in \mR \times H \mapsto \la h\in H$, and we assume that the reader is familiar with the theory of finite-dimensional spaces. 

An inner product on a vector space $H$ is a bilinear function, typically denoted $(\xi,\eta) \mapsto \scp{\xi}{\eta}$ such that $\scp{\xi}{\xi} \geq 0$ with $\scp{\xi}{\xi} = 0$ if and only if $\xi=0$. A vector space equipped with an inner product is called an inner-product space. We will often denote the inner product with a subscript referring to the space (e.g., $\scp{\cdot}{\cdot}_H$). Given such a product, the function
\[
\xi \mapsto \|\xi\|_H = \sqrt{\scp{\xi}{\xi}_H}
\]
is a norm, so that $H$ is also a normed space (but not all normed spaces are inner-product spaces)\,\footnote{Note that we are using double bars for the norm in $H$, which, in most applications, is infinite dimensional}.  

When a normed space is {\em complete} with respect to the topology induced by its norm, it is called a Banach space, or a Hilbert space when the norm is associated with an inner product. Completeness means that Cauchy sequences in this space always have a limit, i.e., if the sequence $(\xi_n)$ is such that, for any $\ep>0$, there exists $n_0>0$ such that $\|\xi_n-\xi_m\|_H < \ep$ for all $n,m\geq n_0$, then there exists $\xi$ such that $\|\xi_n - \xi\|_H \to 0$. Completeness is a very natural property. It allows, for example, for the definition of integrals such as $\int h(t) dt$ as limits of Riemann sums for suitable functions $h: \mR \to H$, leading (with more general notions of integrals) to proper definitions of expectations of $H$-valued random variables. Using a standard (abstract) construction, one can prove that any normed space (resp. inner-product) can be extended to a Banach (resp. Hilbert) space within which it is dense. 

Note that finite-dimensional normed spaces are always complete.


\subsection{Feature spaces and kernels}

Now, consider an input set, say $\CR$, and a mapping $h$ from $\CR$ to $H$, where $H$ is an inner product space. For us, $\CR$ is the set over which the original input data is observed, typically $\mR^d$, and $H$ is the feature space.  One can define the function
$K_h: \CR\times\CR \to \mR$ by 
\[
K_h(x,y) = \scp{h(x)}{h(y)}_H.
\]
The function $K_h$ satisfies the following two properties.
\begin{enumerate}[label={[K\arabic*]}, wide=0pt]
\item $K_h$ is symmetric, namely $K_h(x,y) = K_h(y,x)$ for all $x$ and $y$ in $\CR$. 
\item For any $n>0$, for any choice of scalars $\la_1, \dots, \la_n\in \mR$ and any $x_1, \ldots, x_n \in \CR$, one has
\begin{equation}
\label{eq:pos.kernel}
\sum_{i,j=1}^n \lambda_i \lambda_j K_h(x_i, x_j) \geq 0.
\end{equation}
\end{enumerate}
The first property is obvious, and the second one results from the fact that one can write
\begin{equation}
\label{eq:kh.pos.def}
\sum_{i,j=1}^n \lambda_i \lambda_j K_h(x_i, x_j) = \sum_{i,j=1}^n \lambda_i \lambda_j \scp{h(x_i)}{h(x_j)}_H = \Big\|\sum_{i=1}^n \lambda_i h(x_i)\Big\|_H^2 \geq 0.
\end{equation}

This leads us to the following definition.
\begin{definition}
\label{def:pos.kernel}
A function $K: \CR \ti\CR \mapsto \mR$ satisfying  properties [K1] and [K2]
%\begin{enumerate}[label={[K\arabic*]}]
%\item $K$ is symmetric, namely $K(x,y) = K(y,x)$ for all $x$ and $y$ in $\CR$. 
%\item For any $n>0$, for any choice of scalars $\la_1, \dots, \la_n\in \mR$ and any $x_1, \ldots, x_n \in \CR$, one has
%\begin{equation}
%\label{eq:pos.kernel}
%\sum_{i,j=1}^n \lambda_i \lambda_j K(x_i, x_j) \geq 0.
%\end{equation}
%\end{enumerate}
is called a positive kernel.

One says that
the kernel is positive definite if the sum in \cref{eq:pos.kernel} cannot vanish unless (i) $\la_1 = \cdots = \la_n=0$ or (ii) $x_i=x_j$ for some $i\neq j$.
\end{definition}

An equivalent definition of positive kernels can be given using kernel matrices, for which we introduce a notation.
\begin{definition}
\label{def:kernel.mat}
If $K: \CR \ti\CR \mapsto \mR$ is given, we define, for every $x_1, \ldots, x_n\in \CR$, the kernel matrix 
$\CK_K(x_1, \ldots, x_n)$ with entries $K(x_i, x_j)$, for $i,j = 1, \ldots, n$. (If $K$ is understood from the context, we will simply write $\CK(x_1, \ldots, x_n)$ instead of $\CK_K(x_1, \ldots, x_n)$.)
\end{definition}
Given this notation, it is clear that $K$ is a positive kernel if and only if  for all $x_1, \ldots, x_n\in \CR$, the matrix $\CK_K(x_1, \ldots, x_n)$ is symmetric, positive semidefinite. It is a positive definite kernel if $\CK_K(x_1, \ldots, x_n)$ is positive definite as soon as all $x_j$'s are distinct. This latter condition is obviously needed since, if $x_i=x_j$, the $i$th and $j$th columns of $\CK$ coincide and this matrix cannot be full-rank.

\begin{remark}
\label{rem:positive.kernel}
It is important to point out that $K$ being a positive kernel {\em does not require} that $K(x,y) \geq 0$ for all $x,y\in\CR$ (see examples in the next section). However, it does imply that $K(x,x) \geq 0$ for all $x\in \CR$, since diagonal elements of positive semi-definite matrices are non-negative.
\end{remark}

\bigskip

The function $K_h$ defined above is therefore always a positive kernel, but not always positive definite, as seen below. We will also see later that the converse statement is true: any positive kernel $K: \CR \ti\CR \mapsto \mR$ can be expressed as $K_{h}$ for some feature function $h$ between $\CR$ and some feature space $H$.


Given a feature function $h: \CR \to H$, we will denote by $V_h = \vspan(h(x), x\in\CR)$ the vector space generated by the features, which, by definition, is the space of all linear combinations
\[
\xi = \sum_{i=1}^n \la_i h(x_i)
\]
with $\la_1, \ldots, \la_m\in\mR$, $x_1, \ldots, x_n\in \CR$ and $n\geq 0$ (by convention, $\xi=0$ if $n=0$). Then $K_h$ is positive definite if and only if any family $(h(x_1), \ldots, h(x_n))$ with distinct $x_i$'s is linearly independent. This is a direct consequence of  \cref{eq:kh.pos.def}.
\[
\sum_{i,j=1}^n \lambda_i \lambda_j K_h(x_i, x_j) =  \left\|\sum_{i=1}^n \lambda_i h(x_i)\right\|_H^2.
\]
This implies in particular that positive-definite kernels over infinite input spaces $\CR$ can only be associated to infinite-dimensional spaces $H$, since $V_h\subset H$. 



%Looking ahead to regression methods, a model that is linear in feature space will try to predict a  dependent variable $y\in \mR$ from an input $x$ in the form
%\[
%f(x) = \beta_0 + \scp{b}{h(x)}_H
%\]
%with $\be_0\in\mR$ and $b\in H$. 
%Furthermore, we will see that, for most methods, the optimal ``coefficient'' $b$ will have to  belong to $V_h$, so that, letting $b = \sum_{i=1}^n \la_i h(x_i)$, we have
%\[
%f(x) = \beta_0 + \sum_{i=1}^n \la_i K_h(x, x_i)\,.
%\]
%
%
%We now review a few examples.
\section{First examples}

\subsection{Inner product}
Clearly, if $\CR$ is an inner product space, it has an associated reproducing kernel, defined by
\[
K(x,y) = \scp{x}{y}_{\CR}\,.
\]
This kernel is equal to $K_h$ with $H = \CR$ and $h=\id$ (the identity mapping). In particular $K(x,y) = x^Ty$ is a positive kernel if $\CR = \mR^d$. This kernel can obviously take positive and negative values.

Notice that this kernel is not positive definite, because the rank of $\CK(x_1, \ldots, x_n)$ is equal to the dimension of $\mathrm{span}(x_1, \dots, x_n)$, which can be less than $n$ even when the $x_i$'s are distinct. 

\subsection{Polynomial Kernels}

Consider $\CR = \mR^d$ and define 
\[
h(x) = (\pe x {i_1} \dots \pe x {i_k}, 1\leq i_1, \ldots, i_k \leq d),
\]
 which contains all products of degree $k$ formed from variables $\pe x 1, \ldots,\pe x d$, i.e., all monomials of degree $k$ in $x$. This function takes its values in the space $H = \mR^{N_k}$, where $N_k = d^k$. Using, in $H$, the inner product $\scp{\xi}{\eta}_H = \xi^T\eta$, we have
\begin{eqnarray*}
K_h(x,y)& =& \sum_{1\leq i_1, \ldots, i_k\leq d} (\pe x {i_1}\pe y {i_1})
\cdots (\pe x {i_k} \pe y {i_k})\\
&=& (x^Ty)^k.
\end{eqnarray*}
This provides  the homogeneous polynomial kernel of order $k$.

If one now takes all monomials of order less than or equal to $k$, i.e.,  
\[
h(x) = (\pe x {i_1} \dots \pe x {i_l}, 1\leq i_1, \ldots, i_l \leq d, 0\leq l\leq k),
\]
 which now takes values in a space of dimension $1 + d + \cdots + d^k$, the corresponding kernel is 
$$
K_h(x,y) = 1 + (x^Ty) + \cdots + (x^Ty)^k =
\frac{(x^Ty)^{k+1} - 1}{x^Ty - 1}\,.
$$
This provides a polynomial kernel of order $k$. It is important to notice here that, even though the dimension of the feature space increases exponentially in $k$, so that the computation of the feature function rapidly becomes intractable, the computation of the kernel itself remains a relatively mild operation. 

One can make variations on this construction. For example, choosing any family $c_0, c_1, \ldots, c_k$ of positive numbers, one can take 
\[
h(x) = (c_l \pe x {i_1} \dots \pe x {i_l}, 1\leq i_1, \ldots, i_l \leq d, 0\leq l\leq k)
\]
yielding
\[
K_h(x,y) = c_0^2 + c_1^2 (x^Ty) + \cdots + c_k^2 (x^Ty)^k.
\]
Taking $c_l = \bin{k}{l}^{1/2} \al^{l}$ for some $\al>0$, we get another form of polynomial kernel, namely,
\[
K_h(x,y) = (1 + \al^2 x^T y)^k.
\]

\subsection{Functional Features}
\label{sec:functional.feat}
We now consider an example in which $H$ is infinite dimensional.
Let $\CR = \mR^d$. We assume that a  function $s: \mR^d \to \mR$ is chosen, such that $s$ is both (absolutely) integrable and square integrable. We also fix a scaling parameter $\rho>0$. Associate to $x\in \mR^d$ the function 
\[
\xi_x: y \mapsto s((y-x)/\rho),
\] 
which is also square integrable (as a function of $y$). We define the feature function $h: x\mapsto \xi_x$ from $\mR^d$ to $H = L^2(\mR^d)$, the space of square integrable functions on $\mR^d$ with inner product 
\[
\scp{\xi}{\eta}_H = \int_{\mR^d} \xi(z)\eta(z) dz.
\]

The resulting kernel is
\Eq{
K_h(x,y) = \int_{\mR^{d}} s(z/\rho - x) s(z/\rho - y)\,dz = \rho^d \int_{\mR^{d}} s(z)s(z - (y-x)/\rho) \, dz.
}
Note that $K_h(x,y)$ is ``translation-invariant,'' which means that it only depends on $x-y$. It takes the form $K_h(x,y) = \rho^d \Gamma((y-x)/\rho)$ where
\Eq{
\Gamma(u) = \int_{\mR^{d}} s(z)s(z-u) \,dz.
}
is  the convolution\footnote{The convolution between two absolutely integrable functions $f$ and $g$ is defined by $f*g(u) = \int_{\mR^d} f(z) g(u-z)\,dz$} of $s$ with $\tilde s: z\mapsto s(-z)$.


Let $\sigma$ be the Fourier transform of $s$, i.e., 
\Eq{
\sigma(\om) = \int_{\mR^d} e^{-2i\pi \om^Tu} s(u) du.
}
Because $s$ is real-valued, we have $\sigma(-\omega) = \bar \sigma(\omega) $, the complex conjugate of $\sigma$. Moreover,
$\bar \sigma$ is also the Fourier transform of $\tilde s$. Using the fact that the Fourier transform of the convolution of two functions is the product of their Fourier transforms, we see that the Fourier transform of $\Gamma = s * \tilde s$ is equal to $|\sig|^2$. 
Applying the inverse transform, we find
\Eq{
\Gamma(u) = \int_{\mR^{d}} e^{2i\pi\om^{T}u } |\sigma(\om)|^{2}  \,d\om = \int_{\mR^{d}} e^{-2i\pi\om^{T}u } |\sigma(-\om)|^{2}  \,d\om\,.
}
This form is (almost) characteristic of translation-invariant kernels.
\bigskip

Let us consider a few examples of kernels that can be obtained in this way.
\begin{enumerate}[label=(\arabic*), wide=0pt]
\item
Take $d=1$ and let $s$ be the indicator  function of the interval $[-\frac12, \frac12]$.  
Then, one finds
\Eq{
\Gamma(t) = \max(1-|t|, 0)\,.
}
In this case, the space $V_h$ is the space of all functions expressed as finite sums
\Eq{
z\mapsto \sum_{j=1}^n \la_j \bfone_{[x_j - \rho/2, x_j+\rho/2]}(z)\,,
}
and therefore is a space of compactly-supported piecewise constant functions. 
Such a function computed with distinct $x_j$'s cannot vanish everywhere unless all $\la_j$'s vanish, so that $K_h$ is positive definite. 
Indeed, let
\[
f(z) = \sum_{j=1}^n \la_j \bfone_{[x_j - \rho/2, x_j+\rho/2]}(z)
\]
and assume without loss of generality that $x_1 < x_2 < \cdots < x_n$ and let $x_{n+1} = \infty$. Let $i_0$ be the smallest index $j$ such that $\la_j \neq 0$, assuming that such an index exists. Then $f(z) = \la_{i_0}>0$ for all $z\in [x_{i_0}-\rho/2, x_{i_0+1} - \rho/2)$ which is a non-empty interval.  So, if $f$ vanishes almost everywhere, we must have $\la_j=0$ for all $j=1, \ldots, n$.
\item Still with $d=1$, let $s(z) = e^{-|z|}$. Then, for $t>0$, 
\begin{align*}
\Ga(t) &= \int_{-\infty}^\infty e^{-|z|} e^{-|z-t|}\, dz\\
&= \int_{-\infty}^0 e^{z} e^{z-t}\, dz + \int_0^t e^{-z} e^{z-t}\, dz + \int_{t}^\infty e^{-z} e^{-z+t}\, dz\\
&= \frac{e^{-t}}2 + t e^{-t} + \frac{e^{-t}}{2}\\
&= (1 + t) e^{-t}
\end{align*}
Using the fact that $\Ga(-t) = \Ga(t)$ (make the change of variable $z\to -z$ in the integral), we get 
\[
\Ga(t) = (1 + |t|) e^{-|t|}.
\]
for all $t$. This shows that 
\[
K(x,y) = (1+|x-y|) e^{-|x-y|}
\] 
is a positive kernel on $\mR^d$.
\item Take $s(z) = e^{-|z|^2/2}$,  $z\in \mR^d$. Then 
\begin{align*}
\Ga(u) &= \int_{\mR^d} e^{-\frac{|z|^2 + |u-z|^2}2}\, dz
= e^{-\frac{|u|^2}4} \int_{\mR^d} e^{- |z-u/2|^2}\, dz\\
&= (4\pi)^{d/2} e^{-\frac{|u|^2}4}.
\end{align*} 
\end{enumerate}
This provides a special case of Gaussian kernel.

%One way to interpret this construction is to think of $\xi_x$ as a kind of fuzzy representation of $x$, reflecting some uncertainty that can be associated with its exact value. The difference between two values $x$ and $y$ is then evaluated using the $L^2$ norm $\|\xi_x - \xi_y\|_H$. This leads to the expression of the kernel
%\[
%K_h(x,y) = \int_{\mR} s(z/\rho - x) s(z/\rho - y)\,dz = \rho^d \int_{\mR} s(z)s(z - (y-x)/\rho) \, dz.
%\]
%Notice that $K_h$ takes the form $K_h(x,y) = \rho^d \gamma((y-x)/\rho)$ where
%\[
%\gamma(t) = \int_{\mR} s(z)s(z-t) \,dz
%\]
%is  the convolution of $s$ with $\tilde s: z\mapsto s(-z)$. 
%
%This construction is useful when $\gamma$ can be computed analytically. Take, as a first example, $d=1$ and let $s$ be the indicator  function of the interval $[-0.5, 0.5]$.  Then
%\[
%\gamma(t) = \max(1-|t|, 0)\,.
%\]
%In this case, the space $V_h$ is the space of all functions expressed as finite sums
%\[
%z\mapsto \sum_{j=1}^n \la_j \chi_{[x_j - \rho/2, x_j+\rho/2]}(z)\,,
%\] 
%and therefore is a space of compactly supported piecewise constant functions. We also notice that such a function computed with distinct $x_j$'s cannot vanish everywhere unless all $\la_j$'s vanish, so that $K_h$ is positive definite. 
%
%
%
%Here are a few more examples, still with $d=1$, leaving details to the reader. If $s(z) = e^{-|z|}$, then $\ga(t) = (1 + |t|) e^{-|t|}$. If $s(z) = e^{-z^2/2}/\sqrt{2\pi}$, then $\ga(t) = e^{-z^2/2\sqrt 2}/\sqrt{4\pi}$.   

\subsection{General construction theorems}

\subsubsection{Translation invariance}
As introduced above, a kernel $K$ is translation invariant if it takes the form $K(x,y)  = \Ga(x-y)$ for some continuous function
$\Ga$ defined on $\mR^d$. 
Bochner's theorem \citep{bochner1933vorlesungen} states that such a $K$ is a positive kernel if and only if $\Ga$
is the Fourier transform of a positive measure, namely,
\Eq{
\Ga(x) = \int_{\mR^d} e^{-2i\pi\scp{x}{\om}} d\mu(\om)
}
where $\mu$ is a positive and symmetric (invariant by sign change) measure on $\mR^d$. For
example one can take $d\mu(\om)  = \nu(\om) d\om$, where $\nu$ is a integrable, positive and even function.

This theorem provides an at least numerical,
and sometimes  analytical, method for constructing kernels. The previous section exhibited a special case of translation-invariant kernel for which $\nu = |\sigma|^2$. 

\subsubsection{Radial kernels}
 A radial kernel takes the form 
 $K(x,y)
= \ga(|x-y|^2)$, for some continuous function $\ga$ defined on $[0,
+\infty)$. 
Shoenberg's theorem \citep{schoenberg1938metric} states that, if this function $\ga$ is
universally valid, i.e., $K$ is a kernel for all dimensions $d$, then, it must take the form
\Eq{
\ga(t) = \int_0^{\infty} e^{-\la t} d\mu(\la) 
}
for some positive finite measure $\mu$ on $[0, +\infty)$. 

 For example, when
$\mu$ is a Dirac measure, i.e., $\mu = \de_{(2a)^{-1}}$ for some $a>0$, then
$K(x,y) = \exp(-|x-y|^2/2a)$, which is the Gaussian kernel.
Taking $d\mu = e^{-a\la} d\la$ yields $\ga(t) = 1/(t+a)$, and $d\mu =
\la e^{-a\la}d\lambda$ yields $\ga(t) = 1/(a+t)^2$.

There is also, in \citet{schoenberg1938metric}, a characterization of radial
kernels for a fixed dimension $d$. Such kernels must take the form
$$
\ga(t) = \int_0^{+\infty} \Om_d(t\la) d\mu(\la)
$$
with $\Om_d(t) = \Ga(d/2) (2/t)^{(d-2)/2} J_{(d-2)/2}(t)$ where $J_{(d-2)/2}$ is Bessel's function of the first kind.


\subsection{Operations on kernels}

Kernels can be combined in several ways as described in the next proposition. 
\begin{proposition}
\label{prop:combine.K}
Let  $K_1: \CR\times\CR \to \mR$ and $K_2: \CR\times\CR \to \mR$ be positive kernels. Then the following assertions hold.
\begin{enumerate}[label=(\roman*),leftmargin=1cm]
\item  If  $\la_1, \la_2 >0$, $\la_1K_1+\la_2 K_2$ is a positive kernel. It is positive definite as soon as either $K_1$ or $K_2$ is positive definite.
\item For any function $f: \CR' \to \CR$, $K'_1(x',y') \defeq K_1(f(x'), f(y'))$ is a positive kernel. It is positive definite as soon as $K_1$ is positive definite and $f$ is one-to-one.
\item $K(x,y) = K_1(x,y)K_2(x,y)$ is a positive kernel. It is positive definite as soon as $K_1$ and $K_2$ are positive definite.
\item Let $K_1$ and $K_2$ be translation-invariant with $\CR = \mR^d$, taking the form $K_i(x,y) = \Ga_i(x-y)$, where $\Ga_i$ is continuous  ( $i=1,2$). Assume that one of the two functions $\Ga_1, \Ga_2$ is integrable on $\mR^d$. Then
\[
K(x,y) = \int_{\mR^d} K_1(x, z) K_2(z,y) dz 
\]
is also a positive kernel.
\end{enumerate}
\end{proposition}
\begin{proof}
Point (i) is obvious. Point (ii) is almost as simple, because, for any $\la_1, \ldots, \la_n\in \mR$ and $x'_1, \ldots, x'_n\in \CR'$,
\[
\sum_{i,j=1}^n \la_i\la_j K'_1(x'_i, x'_j) = \sum_{i,j=1}^n \la_i\la_j K_1(f(x'_i), f(x'_j))\geq 0.
\]
If $K_1$ is positive definite, then the latter sum can only vanish if all $\la_i$ are zero, or some of the points in $(f(x'_1), \ldots, f(x'_n))$ coincide. If, in addition, $f$ is one-to-one, then this is equivalent to all $\la_i$ are zero, or some of the points in $(x'_1, \ldots, x'_n)$ coincide, so that $K'_1$ is positive definite.



To prove point  (iii), take $x_1, \ldots, x_N\in \mR^d$ and form the matrices $\CK_i = \CK_i(x_1, \ldots, x_N)$, $i=1,2$, which are, by assumption positive semi-definite. The matrix $\CK = \CK(x_1, \ldots, x_N)$ is the element-wise (or Hadamard) product of $\CK_1$ and $\CK_2$, and the conclusion follows from the linear algebra result stating that the Hadamard product of two positive semi-definite (resp. positive definite) matrices $A = (a(i,j), 1\leq i,j\leq N)$ and $B= (b(i,j), 1\leq i,j\leq N)$ is positive semi-definite (resp. positive definite). This is proved by diagonalizing, say, $A$ in an orthonormal basis $u_1, \ldots, u_N$, with eigenvalues $\la_1, \ldots, \la_N$ and writing
\begin{align*}
\sum_{i,j=1}^N \pe \al i a(i,j)b(i,j)\pe \al j & = \sum_{i,j, k=1}^N \pe \al i \pe {u_i} k \pe {u_j} k \la_k b(i,j)\pe \al j\\
& = \sum_{k=1}^N \la_k \sum_{i,j=1}^N (\pe \al i \pe {u_i} k) (\pe \al j \pe {u_j}k)) b(i,j) \geq 0
\end{align*}
If $B$ is positive definite, then the sum above can be zero only if, for each $k$, either $\la_k=0$ or $\pe \al i \pe {u_i} k = 0$ for all $i$. If $A$ is also positive definite, then the only possibility is $\pe \al i \pe {u_i} k = 0$ for all $i$ and $k$, which implies $\pe \al i=0$ for all $i$ since $u_i\neq 0$. 

To prove point (iv)\,\footnote{This part of the proof uses some measure theory.}, we first note that a translation invariant kernel $K'(x,y) = \Ga'(x-y)$ is always bounded. Indeed, the matrix $\CK'(x,0)$ is positive semi-definite, with determinant $\Ga'(0)^2 - \Ga'(x)^2 >0$, showing that $|\Ga'(x)| < \Ga'(0)$. 
This shows that the integral defining $K(x,y)$ converges as soon as one of the two functions $\Ga_1$ or $\Ga_2$ is integrable. Moreover, we have 
$K(x,y) = \Ga(x-y)$ with
\[
\Ga(x) = \int_{\mR^d} \Ga_1(x-z) \Ga_2(z)\,dz = \int_{\mR^d} \Ga_1(x-u) \Ga_2(u-y)\,du
\]
Using the fact that both $\Ga_1$ and $\Ga_2$ are even, and making the change of variable $z\mapsto -z$, one easily shows that $\Ga(x) = \Ga(-x)$, which implies that $K$ is symmetric. 

We proceed with the assumption that $\Ga_2$ is integrable and use Bochner's theorem to write 
\[
 \Ga_1(y) = \int_{\mR^d} e^{-i\xi^Ty} d\mu_1(\xi)
 \]
 for some positive finite measure $\mu_1$. Then
\begin{align*}
\Ga(x) &= \int_{\mR^d} \left(\int_{\mR^d} e^{-2i\pi\xi^T(x-z)} d\mu_1(\xi)\right) \Ga_2(z)\,dz\\
&= \int_{\mR^d} e^{-2i\pi\xi^Tx} \left(\int_{\mR^d} e^{2i\pi\xi^Tz}  \Ga_2(z)\,dz\right) d\mu_1(\xi)\\
\end{align*}
The shift in the order of the variables $\xi$ and $z$ uses Fubini's theorem. The function
\[
\psi(\xi) = \int_{\mR^d} e^{2i\pi\xi^Tz}  \Ga_2(z)\,dz
\]
is the inverse Fourier transform of $\Ga_2$. Because $\Ga_2$ is bounded and integrable, it is also square integrable, which implies that its inverse Fourier transform is also a square integrable function. Since Bochner's theorem implies that $\Ga_2$ is the Fourier transform of a positive measure $\mu_2$, we find, using the injectivity of the Fourier transform, that $\psi$ is non-negative. So $\Ga$ is the Fourier transform of the finite positive measure $\psi d\mu_1$, which implies that $K$ is a positive kernel.
\end{proof}

Point (iv)  can be related to the following discrete statement on symmetric matrices: assume that $A$ and $B$ are positive semi-definite and that they commute, so that $AB = BA$: then $AB$ is positive semi-definite. 
%(see \cref{prob:9}). 
In the case of kernels, one may consider the symmetric linear operators $\mathbb K_i : f \mapsto \int_{\mR^d} K_i(\cdot,y) f(y) dy$ which maps the space of square integrable functions into itself. Then $\mathbb K_1$ and $\mathbb K_2$ commute and $\mathbb K = \mathbb K_1 \mathbb K_2$. 

% provided that $K_i(\cdot, x)\in L^2(\mR^d)$ for all $x\in \mR^d$ and $i=1,2$.

\subsection{Canonical Feature Spaces}

Let $K$ be a positive kernel on a set $\CR$. The following construction, which is fundamental, shows that $K$ can always be associated with a feature function $h$ taking values in a suitably chosen inner-product space $H$. 

Associate to each $x\in \CR$ the function $\xi_x: y \mapsto K(y,x)$ (we will also write $\xi_x = K(\cdot, x)$), and let $H_K = \vspan(\xi_x, x\in \CR)$, a subspace of the vector space of all functions from $\CR$ to $\mR$. Define the feature function $h: x\mapsto \xi_x$ from $\CR$ to $H_K$. There is a unique inner product on $H_K$ such that $K = K_h$. Indeed, by definition, this requires
\begin{equation}
\label{eq:reprod}
\scp{K(\cdot, x)}{K(\cdot, y)}_{H_K} = K(x,y)\,.
\end{equation}
Moreover, by linearity, for any $\xi = \sum_{i=1}^n \la_i K(\cdot, x_i)$ and $\eta = \sum_{i=1}^m \mu_i K(\cdot, y_i)$, one needs
\[
\scp{\xi}{\eta}_{H_K} = \sum_{i=1}^n\sum_{j=1}^m \la_i\mu_j K(x_i, y_j)\,,
\]
so that the inner product is uniquely specified on $H_K$.
To make sure that this inner-product is well defined, we must check that there is no ambiguity, in the sense that, if $\xi$ has an alternative decomposition $\xi = \sum_{i=1}^{n'} \la'_i K(\cdot, x'_i)$, then, the value of $\scp{\xi}{\eta}_{H_K}$ remains unchanged. But this is clear, because one can also write
\[
\scp{\xi}{\eta}_{H_K} = \sum_{j=1}^m \mu_j \xi(y_j)\,,
\]
which only depends on $\xi$ and not on its decomposition. The linearity of the product with respect to $\xi$ is also clear from this expression, and the bilinearity by symmetry. 

The Schwartz inequality implies that 
\[
|\scp{\xi}{\eta}_{H_K}| \leq \|\xi\|_{H_K}\,\|\eta\|_{H_K}
\]
From which we deduce that $\|\xi\|_{H_K} = 0$ implies that $\scp{\xi}{\eta}_{H_K}=0$ for $\eta\in H_K$. Since 
$\scp{\xi}{K(\cdot, y)}_{H_K} = \xi(y)$ for all $y$, this also implies that $\xi=0$, completing the proof that $H_K$ is an inner-product space.
\bigskip

Equation \eqref{eq:reprod} is the ``reproducing property'' of the kernel for the inner-product on $H_K$. In functional analysis, the completion, $\hat H_K$, of $H_K$ for the topology associated to its norm is then a Hilbert space, and is referred to as a ``reproducing kernel Hilbert space,'' or RKHS. 

More generally, an inner-product space $H$ of functions $h: \CR \to \mR$ is a reproducing kernel Hilbert space if $H$ is a complete space (which makes it Hilbert) and there exists a positive kernel $K$ such that, 
\begin{enumerate}[label={[RKHS\arabic*]}, wide=0pt]
\item For all $x\in \CR$, $K(\cdot, x)$ belongs to $H$,
\item For all $h\in H$ and $x\in \CR$, 
\[
\scp{h}{K(\cdot, x)}_H = h(x)\,.
\] 
\end{enumerate}



%These concepts are however more advanced than what we need in the present notes, and we will not have to invoke use them. 

Returning to the example of functional features in \cref{sec:functional.feat}, we have two different representations of the kernel in feature space, namely in $H = L^2(\mR^d)$, or in $H_K$, with a different inner product. There is not a contradiction, and simply shows that the representation of a positive kernel in terms of a feature function is not unique. 

\begin{remark}
\label{rem:rkhs}
RKHS's are defined as function spaces. While feature space representations, provided by functions
$h: \CR \to H$  from $\CR$ to a Hilbert space $H$ are apparently more general, a simple transformation allows for an identification of (a subspace of) $H$ with an RKHS. We will assume that the subset $h(\CR)$ (containing all $h(x)$, $x\in \CR$) is a dense subset of $H$. If not, one can simply replace $H$ by the closure of $h(\CR)$ which is a Hilbert subspace of $H$.

One can always interpret elements $u\in H$ as functions by letting $\phi_u(x) = \scp{u}{h(x)}_H$. The representation $u\mapsto \phi_u$ is not one-to-one under our assumption that $h(\CR)$ is a dense subset of $H$: if $\phi_u = \phi_v$, then $\scp{u-v}{h(x)}_H = 0$ for all $x\in \CR$, and since $h(\CR)$ is dense in $H$, this implies $u=v$. Letting $\wtilde H = \{\phi_u, u\in H\}$ and defining the inner product $\scp{\phi_u}{\phi_{u'}}_{\wtilde H} = \scp{u}{u'}_H$, one obtains a Hilbert space $\wtilde H$ isometric to $H$ with a new feature function $\tilde h(x) = \phi_{h(x)}$. By definition, $\tilde h(x)(y) = \scp{h(x)}{h(y)}_H = K_h(x,y)$ so that $K_h(x, \cdot)$ belongs to $\wtilde H$ and 
$\scp{\tilde h(x)}{\tilde h(y)}_{\wtilde H} = \scp{h(x)}{h(y)}_H = K_h(x,y)$. This shows that $\wtilde H$ is an RKHS with kernel $K_h$.
\end{remark}


\section{Projection on a finite-dimensional subspace}
\label{sec:orth.proj}
 If $H$ is an inner-product space and $V$ is a subspace of $H$, one defines the orthogonal projection of an element $\xi\in H$ on $V$ as its closest point in $V$, that is, the element $\eta^*$ of $V$ minimizing  the function $F: \eta \mapsto \| \eta - \xi\|^2_H$ over all $\eta\in V$. This closest point does not always exist, but it does in the special case in which $V$ is finite dimensional (or, more generally, when $V$ is a closed subspace of $H$; see \citet{yos70}). We state, without proof, some of the properties of this operation.
 
Assuming that $V$ is closed,  this minimizer is unique and will be denoted $\eta^* = \pi_V(\xi)$. Moreover, $\pi_V$ is a linear transformation from $H$ to $V$, and $\eta^*$ is characterized by the properties
 \[
 \left\{ \begin{aligned} &\eta^*\in V \\ &\xi-\eta^* \perp V,\end{aligned}
 \right.
 \]
 the last condition meaning that $\scp{\xi-\eta^*}{\eta}_H = 0$ for all $\eta\in V$.
 
 Because $\|\xi\|_H^2 = \|\pi_V(\xi)\|_H^2 + \|\xi- \pi_V(\xi)\|_H^2$, one always has $\|\pi_V(\xi)\|_H \leq \|\xi\|_H$, with inequality if and only if $\pi_V(\xi) = \xi$, i.e., if and only if $\xi\in V$.

 
 If $V$ is finite-dimensional and $\eta_1, \ldots, \eta_n$ is a basis of $V$, then $\pi_V(\xi)$ is given by
 \[
 \pi_V(\xi) = \sum_{i=1}^n \pe \alpha i \eta_i
 \]
 with $\alpha$ (considered as a column vector in $\mR^n$) given by
 \[
 \alpha = \mathrm{Gram}(\eta_1, \ldots, \eta_n)^{-1} \la\,,
 \]
 where $\la\in\mR^n$ is the vector with coordinates $\pe \la i = \scp{\xi}{\eta_i}_H$, $i=1, \ldots, n$. The Gram matrix of $\eta_1, \ldots, \eta_n$, denoted $\mathrm{Gram}(\eta_1, \ldots, \eta_n)$, is the $n$ by $n$ matrix with entries $\scp{\eta_i}{\eta_j}_H$ for $i,j = 1, \ldots, n$. 
 

If $A$ is a subset of $H$, the set $A^\perp$ consists of all vectors perpendicular to $A$, namely
\[
A^\perp = \defset{h\in H: \scp{h}{\tilde h}_H = 0 \text{ for all } \tilde h \in A}\,.
\]
If $V$ is a finite-dimensional  (or, more generally, closed) subspace of $H$, then any point in $h$ is decomposed as $h = \pi_V(h) + h- \pi_V(h)$ with $h-\pi_V(h) \in V^\perp$. This shows that $\pi_{V^\perp}$ is well defined and equal to $\mathrm{id}_H - \pi_V$.

\bigskip

Orthogonal projections can be applied to function interpolation in an RKHS. Indeed, assuming that $H$ is an RKHS, as described at the end of the previous section, with a positive-definite kernel.   Given distinct points $x_1, \ldots, x_N\in \CR$ and values $\alpha_1, \ldots, \alpha_N\in \mR$, the interpolation problem consists in finding $h\in H$ with minimal norm satisfying $h(x_k) = \alpha_k$, $k=1, \ldots, N$. Consider the finite dimensional space
\[
V = \vspan\defset{K(\cdot, x_k), k= 1, \ldots N}.
\]
Then there exists an element $h_0\in V$ that satisfies the constraints. Indeed, looking for $h_0$ in the form
\[
h_0(x) = \sum_{l=1}^N K(x, x_l) \lambda_l 
\]
one has
\[
h_0(x_k) = \sum_{l=1}^N K(x_k, x_l) \lambda_l
\]
so that 
\[
\begin{pmatrix}
\lambda_1 \\ \vdots \\ \lambda_N 
\end{pmatrix}
 =
 \CK(x_1, \ldots, x_N)^{-1} \begin{pmatrix}
\alpha_1 \\ \vdots \\ \alpha_N 
\end{pmatrix}
 \]
 
Any other function $h$ satisfying the constraints satisfies $h(x_k) - h_0(x_k) = 0$, which, using RKHS2, is equivalent to $\scp{h-h_0}{K(\cdot, x_k)}_H = 0$, i.e., to $h-h_0\in V^\perp$. This shows that $h_0 = \pi_V(h)$, so that 
$\|h\|_H \geq \|h_0\|_H$ and $h_0$ provides the optimal interpolation. We summarize this in the proposition:
\begin{proposition}
\label{prop:rkhs.interpolation}
Let $H$ is an RKHS with a positive-definite kernel.   Let $x_1, \ldots, x_N\in \CR$ be distinct points  and $\alpha_1, \ldots, \alpha_N\in \mR$. Then the function $h\in H$ with minimal norm satisfying $h(x_k) = \alpha_k$, $k=1, \ldots, N$ takes the form
\begin{subequations}

\begin{equation}
\label{eq:rkhs.interpolation.1}
h(x_k) = \sum_{l=1}^N K(x_k, x_l) \lambda_l
\end{equation}
with 
\begin{equation}
\label{eq:rkhs.interpolation.2}
\begin{pmatrix}
\lambda_1 \\ \vdots \\ \lambda_N 
\end{pmatrix}
 =
 \CK(x_1, \ldots, x_N)^{-1} \begin{pmatrix}
\alpha_1 \\ \vdots \\ \alpha_N 
\end{pmatrix}.
 \end{equation}
\end{subequations}
\end{proposition}

A variation of this problem replaces the constraint by a penalty that complete the minimization associated with the orthogonal projection, namely, minimizing (in $h\in H$)
\[
\|h\|_H^2 + \sigma^2 \sum_{k=1}^N |h(x_k) - \alpha_k|^2.
\]
Letting $h_0 = \pi_V(h)$, so that $h_0(x_k) = h(x_k)$ for all $k$, this expression can be rewritten as
\[
\|h_0\|_H^2 + \|h-h_0\|^2_H + \sigma^2 \sum_{k=1}^N |h_0(x_k) - \alpha_k|^2.
\]
This shows that the optimal $h$ must coincide with its projection on $V$, and therefore belong to that subspace. Looking for $h$ in the form
\[
h(\cdot) = \sum_{l=1}^N K(\cdot, x_l) \lambda_l,
\]
the objective function is rewritten as
\[
\sum_{k,l=1}^N K(x_k, x_l) \lambda_k\lambda_l + \sigma^2 \sum_{k=1}^N \left|\sum_{l=1}^N K(x_k, x_l) \lambda_l - \alpha_k\right|^2, 
\]
which, in vector notation gives, writing $\boldsymbol{\lambda} = \begin{pmatrix}
\lambda_1 \\ \vdots \\ \lambda_N 
\end{pmatrix}$ and $\boldsymbol\alpha = \begin{pmatrix}
\alpha_1 \\ \vdots \\ \alpha_N 
\end{pmatrix}$, 
\[
\boldsymbol\lambda^T
\CK(x_1, \ldots, x_N)\boldsymbol\lambda +
 \sigma^2 \left(\CK(x_1, \ldots, x_N)\boldsymbol\lambda
 - \boldsymbol \alpha\right)^T \left(\CK(x_1, \ldots, x_N)\boldsymbol\lambda
 - \boldsymbol \alpha\right).
\]

The differential of this expression in $\boldsymbol\lambda$ is 
\[
\CK(x_1, \ldots, x_N)\boldsymbol\lambda + 2\sigma^2 \CK(x_1, \ldots, x_N)(\CK(x_1, \ldots, x_N)\boldsymbol\lambda  - \boldsymbol\alpha).
\]
Assuming that $x_1, \ldots, x_N$ are distinct, this vanishes if and only if
\[
\boldsymbol\lambda = (\CK(x_1, \ldots, x_N) + (1/\sigma^2) \Id[N])^{-1}\boldsymbol\alpha.
\] 

We have just proved the proposition:
\begin{proposition}
\label{prop:rkhs.interpolation.soft}
Let $H$ is an RKHS with a positive-definite kernel.   Let $x_1, \ldots, x_N\in \CR$ be distinct points  and $\alpha_1, \ldots, \alpha_N\in \mR$. Then the unique minimizer of 
\[
h \mapsto
\|h\|_H^2 + \sigma^2 \sum_{k=1}^N |h(x_k) - \alpha_k|^2
\]
on $H$ is given by
\begin{subequations}

\begin{equation}
\label{eq:rkhs.interpolation.soft.1}
h(x_k) = \sum_{l=1}^N K(x_k, x_l) \lambda_l
\end{equation}
with 
\begin{equation}
\label{eq:rkhs.interpolation.soft.2}
\begin{pmatrix}
\lambda_1 \\ \vdots \\ \lambda_N 
\end{pmatrix}
 =
( \CK(x_1, \ldots, x_N)+ (1/\sigma^2) \Id[N])^{-1} \begin{pmatrix}
\alpha_1 \\ \vdots \\ \alpha_N 
\end{pmatrix}.
 \end{equation}
\end{subequations}
\end{proposition}


==> linear0.tex <==
% !TEX root = machine_learning.tex





\chapter{Linear Models for Regression}
We study, in this chapter and in the following one, linear models for regression and
classification. The  term ``linear models'' roughly refers to ``models in which the quantity of
interest can be, after an explicit transformation, put into a form
which depends linearly on the parameters of the model.'' Notice that
this does not imply that the solution of the problem (the method) is
also linear (ie. expressed as a solution of a linear system), and we
will review in fact several nonlinear methods in this chapter. 



\section{Mean square estimators}
\subsection{Linear regression}
As usual, $Y$ and $X$ are random variables, with $Y\in \mR$ and
$X\in\mR^d$, and  we first consider  the case when the cost function is
the mean square error, so that the optimal Bayes estimator is the
conditional expectation. We assume here that, for $x\in\mR^d$
$$
f(x) := E(Y|X=x) = \be_0 + \sum_{j=1}^d b_j x(j) = \tilde x^T \beta\,.
$$
with the notation $\tilde   x = (1, x(1), \ldots, x(d))^T$ and $\beta =
(\beta_0, b_1\ldots, b_d)^T$.

Based on a training set $(y_1, x_1), \ldots, (y_N, x_N)$, the mean
square estimator for $\tilde\be$ minimizes
$$
RSS(\tilde\be) = \sum_{k=1}^N (y_k - f(x_k))^2  = \sum_{k=1}^N (y_k - \tilde
x_k^T \be)^2 
$$
Introduce the $N\ti (d+1)$ matrix $\mathcal X$ the rows of which
being $\tilde x_1^T, \ldots, \tilde x_N^T$, and the column vector
$\mathcal Y$ with coefficients $y_1, \ldots, y_N$, we have
$$
RSS(\be) = |\mathcal Y - \mathcal X \tilde\be|^2.
$$
The solution of this problem, provided by the following theorem, is
standard.
\begin{theorem}
\label{th:ls.reg}
Assume that the matrix $\mathcal X$ has rank $d+1$. Then the RSS is
minimized for 
$$
\hat \beta = (\CX^T\CX)^{-1} \CX^T Y
$$
\end{theorem}
This can be proved with an elementary optimization argument, or by simply
checking that
$$
RSS(\be) = RSS(\hat\be) + |\mathcal X(\hat\be - \be)|^2.
$$


The estimator $\hat\be$ depends on the random observation and
therefore is a random variable. Its expectation can be computed {\em
under the assumption that the linear model is valid} as follows:  
\begin{eqnarray*}
E(\hat \beta) &=& E\left[E((\CX^T\CX)^{-1} \CX^T Y|\CX)\right]\\
&=& E\left[(\CX^T\CX)^{-1} \CX^T E(Y|\CX)\right]\\
&=& E\left[(\CX^T\CX)^{-1} \CX^T \CX\tilde\be \right]\\
&=& \tilde\be.
\end{eqnarray*}
This implies that $\hat\be$ is unbiased. Assume that the conditional distribution of $Y$ given $X=x$ has
constant variance, $\sigma^2$. Then
\begin{eqnarray*}
E(\hat \beta \hat\beta^T) &=& E\left[E((\CX^T\CX)^{-1} \CX^T YY^T\CX(\CX^T\CX)^{-1} |\CX)\right]\\
&=& \sig^2 E\left[(\CX^T\CX)^{-1} \CX^T \CX(\CX^T\CX)^{-1} \right]\\
&=& \sig^2 E\left[(\CX^T\CX)^{-1} \right]\\
\end{eqnarray*}

Here is another classical result on the least square regression
estimator. Recall that a symmetric matrix $A$ is said to be larger than another
symmetric matrix, $B$, if $A-B$ is nonnegative.
\begin{theorem}[Gauss-Markov]
%Assume that $\CX$ is deterministic. 
Assume that an estimator $\be^* $ takes the form $\be^* = A(\CX)Y$ (it is
linear) and is unbiased conditionally to $\CX$: $E_{\tilde \be}(\be^*|\CX) =
\tilde \be$ (for all $\tilde \be$).
Then the variance of $\be^*$ cannot be smaller than the variance
of the least square estimate, $\hat\be$.
\end{theorem}
\begin{proof}
The constraint
that $E(A\CY|\CX) = \tilde\be$ for all $\tilde\be$ yields $A\CX \tilde\be = \tilde\be$
or $A\CX = \Id_{\mR^{d+1}}$ ($A$ is a $(d+1) \times N$ matrix). The variance is $\sig^2 E(A^TA)$. What
must be shown is that, for any $u\in\mR^{d+1}$, 
$$ u^T E(AA^T)  u \geq u^TE[(\CX^T\CX)^{-1}] u$$
when $A\CX = \Id$. We in fact have the stronger result: 
$$
A\CX = \Id \Ria u^T AA^T  u \geq u^T(\CX^T\CX)^{-1} u \text{ for all }
u.
$$

To see this, consider the problem of minimizing  $A \mapsto u^T AA^T
u$ subject to the constraint $A\CX = \Id$. The Lagrange multipliers for
this constraint can be organized in a matrix $C$ and the
Lagrangian is
$$ u^T AA^T u - \trace(C^T A\CX)$$
Consider a variation $A\to A+ \ep H$ to obtain the Euler-Lagrange equation
$$ 2 u^T AH^T u - \trace(C^T H\CX) = 0$$
which yields $\trace(H^T (2 uu^TA - C \CX^T)) = 0$ for all $H$ at the
minimum, so that $2 uu^TA - C \CX^T = 0$. In
particular, this implies that 
$2 uu^TA\CX =   C \CX^T\CX$, which yields, using the constraint,
$$
C  = 2 uu^T (\CX^T\CX)^{-1}
$$
so that
$uu^TA = uu^T (\CX^T\CX)^{-1} \CX^T$.
This implies that $A = (\CX^T\CX)^{-1} \CX^T$ is a minimizer for all
$u$ (and the only one in this case).
\end{proof}

One can avoid introducing the intercept $\beta_0$ by centering all variables.
Denote 
$$\bar y = \frac{1}{N} \sum_{k=1}^N y_k \text{ and } \bar x =
\frac{1}{N} \sum_{k=1}^N x_k.
$$
It is easy to prove that the solution of the regression problem with  
observations $y_k-\bar y$, $k=1, \ldots, N$ and predictive variables
$x_k-\bar x$, $k=1, \ldots, N$ has least square solution $\hat\be^c$
such that  $\hat\be^c_0 =
0$, and that the solution of the original problem satisfies $\hat b
= \hat b^c$ and $\hat \be_0 = \bar y - \bar x^T b$. Given this fact,
we can, when convenient, assume that all variables are centered and
use a model without intercept.


\subsection{Ridge regression}

Ridge regression adds a penalty to the RSS in order to limit the size of the regression coefficients. The resulting estimator minimizes
\begin{equation}
\label{eq:rr.1}
\sum_{k=1}^N (y_k - \tilde x_k^T \be)^2 + \la \sum_{i=1}^d \be_i^2
\end{equation}

More generally, we can consider the problem of minimizing 
$$
|CY - \CX\tilde\be|^2 + \la \be^T\De\be
$$
for some matrix $\De$, so that \eqref{eq:rr.1} corresponds to
$\De = \text{diag}(0, 1, \ldots, 1)$.  Another popular choice is 
$\De = \text{diag}(0, \hat\sig^2_1, \ldots, \hat\sig^2_N)$, where $\hat\sig_i^2$ is the empirical variance of the $i$th coordinate of $X$ in the training set.

Using the same argument as with
linear regression, one finds the optimal solution to be given by
$$
\hat\be^\la = (\CX^T\CX + \la \De)^{-1}\CX^T \CY\,.
$$


We obviously retrieve the original formula for regression when
$\la=0$. We now analyze the prediction error for this estimator. In the
following computation, we assume that the training set is fixed, or,
more precisely, that probabilities and expectations are made
conditional to it.
Also, to simplify notation, we
denote
$$
S_\la = \CX^T\CX + \la \De = \sum_{k=1}^N \tx_k^T\tx_k + \la\De
$$
and 
$\Sig = E(\tX^T\tX)$ for a single realization of $X$. 
%Also, with little
%loss of generality, let us assume that all variables are centered and
%that the training set is centered too, so that we can use $X$ instead of $\tX$.

The mean square prediction error is 
\begin{eqnarray*}
R(\la) &=& E((Y - \tX^T \hat\be_\la)^2)\\
& =& E((\tX^T(\be - \hat\be_\la) + \ep)^2\\
&=& (\hat\be_\la- \be)^T \Sig (\hat\be_\la - \be) + \sig^2.
\end{eqnarray*}
Now, we have
\begin{eqnarray*}
\hat\be_\la &=& S_\la^{-1}\CX^T\CY \\
&=& S_\la^{-1}S_0 \be + S_\la^{-1}\CX^T\eta\\
&=& \be - \la S_\la^{-1}\De \be + S_\la^{-1}\CX^T\eta
\end{eqnarray*}
in which we have denoted $\eta_k$ the noise residual $\eta_k = y_k -
\tx_k \be$ over the training set.
So we can rewrite
$$
R(\la) = \la^2 \be^T \De S_\la^{-1} \Sig S_\la^{-1} \De \be -2\la \eta^T\CX
S_\la^{-1} \Sig S_\la^{-1}\De \be + \eta^T\CX S_\la^{-1} \Sig
S_\la^{-1} \CX^T\eta + \sig^2.
$$
Let us analyze the quantities that depend on the training set in this
expression. The first one is $S_\la = S_0 + \la \De$. From the law of
large numbers, $S_0/N \to \Sig$ when $N$ tends to infinity, so that
$S_\la^{-1} = O(1/N)$ (provided the order of $\la$ is no more than
$N$). The second one is 
$$
\eta^T\CX = \sum_{k=1}^N \eta_k \tx_k
$$
which, according to the central limit theorem, is such that
$N^{-1/2}\eta^T\CX \sim \CN(0, \sig^2 \text{Cov}(\tX))$ when
$N\to\infty$. So, we can expect the coefficient of $\la^2$  in
$R(\la)$ to have order $N^{-2}$, the coefficient of $\la$ to have
order $N^{-3/2}$ and the constant coefficient of have order
$N^{-1}$. This suggests taking $\la = \mu \sqrt{N}$ so that all
coefficients have roughly the same order when expanding in powers of
$\mu$. So $S_\la = N(S_0/N + \mu\De/\sqrt N) \sim N\Sig$ and we will
make the approximation, letting $\xi = N^{-1/2} \sig^{-1/2}\eta \CX^T$
and $\ga = \Sig^{-1/2} \De\be$,
$$
N(R(\la) - \sig^2) \simeq \mu^2  |\ga|^2 - 2 \mu \xi^T
\ga  + \xi^T \xi.
$$
So the optimal $\mu$ should be 
$$
\mu = \frac{\xi^T\ga}{|\ga|^2}.
$$
Of course, this one cannot be computed from  data, but we can see
that, since $\xi$ converges to a centered Gaussian random variable,
its value cannot be too large. It is therefore natural to choose it to
be constant and use ridge regression in the form
$$
\sum_{k=1}^N (y_k - \tilde x_k^T \be)^2 + \sqrt N\mu \be^T \De \be
$$ 

\section{The Lasso and other sparsity estimators}

\subsection{Equivalence of constrained and penalized formulations}
 
Let us consider an alternate formulation
of the ridge regression estimator. Let $\mathit{ridge}(\la)$ denote
the ridge regression problem for some parameter $\la$. Consider the
following problem, which will be called $\mathit{ridge}'(C)$:
minimize $\sum_{k=1}^N (y_k - \tx_k^T\be)^2$ subject to the constraint
$\sum_{i=1}^d \be_i^2 \leq C$. We claim that this problem is
equivalent to the ridge regression problem, in the following sense:
for any $C$, there exists a $\la$ such that the solution of
$\mathit{ridge}'(C)$ coincides with the solution of
$\mathit{ridge}(\la)$ and vice-versa. 

Indeed, fix a $C>0$. To solve $\mathit{ridge}'(C)$, we first look for
a solution such that $\sum_i \be_i^2 < C$. If such a solution exists,
it provides a local minimum of the unconstrained least-square problem; but the
only local minimum is the least square solution itself, which corresponds to 
$\mathit{ridge}(\la)$ for $\la=0$. Now consider the other case, when the solution
satisfies $\sum_i \be_i^2 = C$. This solution can be computed with
Lagrange multipliers, via the stationary
points of the Lagrangian
$$
\sum_{k=1}^N (y_k - \tx_k^T\be)^2 - \mu \sum_{i=1}^d \be_i^2.
$$
The resulting computation is similar to ridge regression, and the stationary points must take the
form
$$
\hat\be_\mu  = (\CX^T\CX -\mu \De)^{-1} \CX^T Y.
$$
By hypothesis, the mean square estimator, $\hat\be_0$ is such that
$\hat\be_0^T\De\hat\be_0 \geq C$. On the other hand, when $\mu \to
-\infty$, then $\be_\mu \to 0$ so that there must exist a $\mu = \mu_C
\leq 0$ such that $\hat \be_\mu^T\De\hat \be_\mu = C$. This provides the
solution of $\mathit{ridge}'(C)$ and also of $\text{ridge}(\la)$ for
$\la = -\mu_C$.

The converse statement is obvious: a solution $\hat\be$ of
$\mathit{ridge}(\la)$ is solution of $\mathit{ridge}'(C)$ for $C =
\hat\be^T \De\hat\be$. 

\bigskip

This fact is more general than just ridge regression. Consider a
general penalized optimization problem, denoted $\mathit{var}(\la)$
which consists in minimizing in $\be$ some objective function of the form $E(\be)
+ \la \phi(\be), \la \geq 0$. 

We assume that $E$ and $\phi$ are continuous and $\phi(\be) \to
\infty$ when $\be\to\infty$. We also assume that the problem is
all but convex, namely that, for any $\la$, there is a unique solution
of $\mathit{var}(\la)$, that will be denoted  $\be_\la$, and that $\be_0$ is the unique local minimum of $E$.

Consider the family of problems $\mathit{var}'(C)$, $C>\min(\phi)$ which minimize
$E(\be)$ subject to $\phi(\be) \leq C$ and let $\be'_C$ be the
minimizer, also assumed to be uniquely defined. As done with ridge
regression, we want to show that these
two families of problems are equivalent.

We first discuss the penalized problems and prove the following
proposition, which has its own interest.
\begin{proposition}
\label{prop:pen.prop}
The function $\la \mapsto E(\be_\la)$ is nondecreasing, and
$\la\mapsto \phi(\be_\la)$ is non-increasing.

Moreover, $\be_\la$ varies continuously as a function of $\la$.
\end{proposition} 
\begin{proof}
Consider two parameters $\la$ and $\la'$. By definition, we have
\begin{eqnarray*}
E(\be_\la) + \la \phi(\be_\la) &\leq& E(\be_{\la'}) + \la
\phi(\be_{\la'})\\
\text{and } E(\be_{\la'}) + \la'
\phi(\be_{\la'}) &\leq& E(\be_\la) + \la' \phi(\be_\la) 
\end{eqnarray*}
since both left sides are minimizers. This implies
\begin{equation}
\label{eq:pen.gen}
\la (\phi(\be_\la) - \phi(\be_{\la'})) \leq E(\be_{\la'}) - E(\be_{\la})
\leq \la' (\phi(\be_\la) - \phi(\be_{\la'})).
\end{equation}

In particular: $(\la'-\la) (\phi(\be_\la) - \phi(\be_{\la'})) \geq
0$. Assume that $\la < \la'$. Then this last inequality implies
$\phi(\be_\la) \geq \phi(\be_{\la'})$ and \eqref{eq:pen.gen} then
implies that $E(\be_\la) \leq E(\be_{\la'})$, which proves the first
part of the proposition.

We now prove that $\la \mapsto \be_\la$ is continuous.
Define $G(\be,
\la)  = E(\be) + \la\phi(\be)$. 
Since we assume that $\phi(\be)\to\infty$ when $\be\to \infty$, and we
have just proved that $\phi(\be_\la) \leq \phi(\be_0)$ for any $\la$,
we obtain the fact that the set $(|\be_\la|, \la\geq 0)$ is bounded, say by a
constant $B\geq 0$. 

Consider a sequence $\la_n$ that converges to $\la$. We want to prove
that $\be_{\la_n} \to \be_\la$, for which (because $\be_\la$ is bounded)
it suffices to show that if $\be_{\la_n}$ converges to some
$\tilde \be$, then $\tilde \be = \be_\la$.

So assume that  $\be_{\la_n}$ converges to $\tilde \be$. Since 
$G$ is continuous, this implies that $G(\be_{\la_n}, \la_n) \to G(\tilde\be , \la)$ when $n$ tends
to infinity. Let us prove that $G(\be_\la, \la)$ is continuous {\em in $\la$}.
For any pair $\la, \la'$ and any $\be$, we have
$$
G(\be_{\la'}, \la')\leq G(\be, \la') = G(\be, \la) + (\la'-\la) \phi(\be) \leq G(\be, \la) + 
|\la'-\la| \phi(\be)
$$
which implies (taking the minimum of the upper bound over $\be$ such
that $\phi(\be) \leq \phi(\be_0)$) that $G(\be_{\la'}, \la') \leq
G(\be_\la, \la) + B|\la'-\la|$. This yields, by symmetry,
$|G(\be_{\la'}, \la') - G(\be_\la, \la)| \leq B|\la-\la'|$, proving
the continuity in $\la$.

So we must have $G(\tilde\be, \la) = G(\be_\la, \la)$. This implies
that both $\tilde\be$ and $\be_\la$ are solutions of
$\mathit{var}(\la)$, so that $\be_\la = \tilde \be$ because we assume
that the solution is unique. 
\end{proof}

We now prove
that the classes of problems
$\mathit{var}(\la)$ and $\mathit{var}'(C)$ are  equivalent. First,
$\be_\la$ is obviously a minimizer of $E(\be)$ subject to the
constraint $\phi(\be) \leq C$, with $C =
\phi(\be_\la)$. Indeed, if $E(\be) <E(\be_\la)$ for some $\be$ with $\phi(\be)
\leq C = \phi(\be_\la)$, then
$E(\be) + \la \phi(\be) < E(\be_\la) + \la \phi(\be_\la)$ which is a
contradiction. So $\be_\la = \be'_C$ for $C = \phi(\be_\la)$. This
proves the equivalence of the problems when $C$ is in the range $(a,
\phi(\be_0))$ where $a = \lim_{\la\to\infty} \phi(\be_\la)$, which is
easily shown to equal $\min(\phi)$. 

So, the only remaining case is with $C>
\phi(\be_0)$, but for such a $C$,  the solution of $\mathit{var}'(C)$
must be $\be_0$ since it is a solution of the unconstrained
problem, and satisfies the constraint.

\subsection{The Lasso}
The lasso's formulation is a simple variation of constrained
ridge regression. Let $\hat \sig_i^2$ be the empirical variance of the
$i$th variable $X(i)$. Then, the lasso estimator is defined as
a minimizer of
$\sum_{k=1}^N (y_k - \tx_k^T\be)^2$ subject to the constraint
$\sum_{i=1}^d \hat \sig_i|\be(i)| \leq C$. So, compared to ridge regression, the sum of squares for $\be$ is
simply replaced by a weighted sum of absolute values. Such a simple change,
however, can drastically modify the nature of the solutions.

To simplify the exposition, and without loss of generality, we will
assume that the variables have been normalized so that $\sig(i) = 1$
and the constraint simply is the sum of absolute values.
The minimization for the lasso can be written as a quadratic programing problem by introducing
slack variables, $\xi_i$, $i=1, \ldots, d$ and noting that the
constrained 
formulation above is equivalent to minimizing 
$\sum_{k=1}^N (y_k - \tx_k^T\be)^2$ subject to the constraints
$\sum_{i=1}^d\xi_i \leq C$, $\xi_i+\be_i \geq 0$, $\xi_i-\be_i\geq 0$
and $\xi_i \geq 0$. This can be solved using widely available optimization
routines. 

Although convex programming algorithms can be very efficient, there is
a more direct way to compute a solution to the lasso problem. For
this, it is interesting to first analyze how the solution changes when
$C$ varies, or how the solution of the equivalent penalization problem
varies with $\la$.

Interesting situations
are , of course, when $C$ is small enough to ensure that the solution
differs from ordinary least squares. In this case, the solution is on
the set $\sum_{i=1}^d |\be_i| = C$, and it coincides, as we have just shown, with one of the
solutions of the penalized problem that minimizes 
$$
G(\be) = \sum_{k=1}^N (y_k - \tx_k^T\be)^2 + \la \sum_{k=1}^d |\be(i)|.
$$

Let us study the penalized problem. For a vector $h$, we can compute the limit of $(G(\be+th) -
G(\be))/t$ when $t$ tends to 0, $t>0$; $\be$ is a minimizer if and
only if this limit is non-negative for all $h$. The expression of this
limit, however, depends on whether $\be_i=0$ or not, so let's denote
$J = J(\be)$ the set of $i$ in $\defset{1, \ldots, d}$ such that
$\be_i \neq 0$. Then, letting $\prt^+ G(\be, h)$ denote the limit, we
have
$$
\prt^+ G(\be, h) = -2\sum_{k=1}^N \sum_{i=0}^d (y_k - \tx_k^T\be)
\tx_k(i)h(i) + \la \sum_{i\in J} \mathrm{sign}(\be(i)) h(i) + \la
\sum_{i\not\in J, i\neq 0} |h(i)|.
$$
The conditions for optimality therefore are
$$
\sum_{k=1}^N (y_k - \tx_k^T\be) = 0,
$$

$$
2\sum_{k=1}^N (y_k - \tx_k^T\be)
\tx_k(i) = \la \mathrm{sign}(\be(i)) \text{ if } i\in J
$$
and
$$
- 2\sum_{k=1}^N (y_k - \tx_k^T\be)
\tx_k(i)h(i) + \la |h(i)| \geq 0 \text{ for all $h(i)$ if } i\not\in J
$$
which is equivalent to
$$
2\Big|\sum_{k=1}^N (y_k - \tx_k^T\be)
\tx_k(i)\Big| \leq  \la  \text{ if } i\not\in J.
$$
We see that the condition for optimality is just an inequality when
$\be_i=0$, which is easier to satisfy. This is why typical solutions
to the lasso problem are {\em sparse}, which means that they contain
many zero coordinates.

 We can rewrite the consistency conditions for the
equations in a more convenient form. We introduce some notation.
Denote $\be(J) = (\be_0, b(i), i\in J)$. Let $\de = \de^J$ be the vector
starting with 0 and followed by the signs of $b(i)$ for $i\in J$. Let
$\tx_k(J)$ be the vector $(1, x_k(i), i\in J)^T$. Let
$$
S_{XX}^J = \frac{1}{N} \sum_{k=1}^N \tx_k(J)\tx_k(J)^T
$$
and 
$$
S_{XY}^J = \frac{1}{N} \sum_{k=1}^N \tx_k(J)y_k.
$$
Then, the equality constraints give
\begin{equation}
\label{eq:cons.lasso.0}
\be_\la(J) = \hat \be^J + \frac\la2 u^\de
\end{equation}
where
$\hat\be^J = (S_{XX}^J)^{-1}S_{XY}^J$ is the least square estimator
for the model restricted to the set $J$, and $u^\de =
(S_{XX}^J)_{-1}\de$. This solution is consistent with the signs in
$\de$ if and only if
\begin{equation}
\label{eq:cons.lasso.1}
\de(i)(\hat \be^J(i) + \frac\la2 u^\de(i)) > 0, i\in J.
\end{equation}

To write the inequality constraints, define
$$
r^J(i) = \frac1N \sum_{k=1}^N (y_k - \tx_k(J)^T\hat\be^J) x_k(i)
$$
to be the empirical correlation between the residual for the least
square estimator on $J$ and the variable $X(i)$ for $i\not\in
J$. Define also
$$
d^J(i) = \frac{1}{N} \sum_{k=1}^N \tx_k(J)^Tu^\de x_k(i).
$$
Then, the second set of conditions is
\begin{equation}
\label{eq:cons.lasso.2}
|2r^J(i) + \la d^J(i)| \leq \la, i\not\in J.
\end{equation}

If conditions \eqref{eq:cons.lasso.1} and \eqref{eq:cons.lasso.2} are
satisfied, then the parameter provided by \eqref{eq:cons.lasso.0} is
the solution of the penalized lasso problem for the given value of
$\la$. It is important to notice that \eqref{eq:cons.lasso.1} and
\eqref{eq:cons.lasso.2} only involve $\la$, $J$, $\de$. 

If $J$ and $\de$ are consistent for a given value of $\la$, it will
remain so, by continuity, for small variations of $\la$, provided that no
equality occurs in \eqref{eq:cons.lasso.2}. So, when $\la$
varies, changes in $J$ and $\de$ occur as discrete
events, corresponding to equalities in the consistency conditions.


The simplest situation is with $J = \emp$ which corresponds
to large $\la$'s. Indeed, the consistency conditions are satisfied
with $J=\emp$ as soon as
$$
\la \geq 2\max_{i=1, \ldots, d} |r^\emp(i)|
$$
since $d^\emp = 0$. If we now let $\la$ decrease from these large
values, the set $J$ and the signs, $\de$ will change when one of the
following events occurs:
\begin{itemize}
\item[1.] For some $i\in J$, $\hat \be^J(i) + \frac\la2 u^\de(i) = 0$,
in which case $i$ must be removed from $J$.
\item[2.] For some $i\not\in J$, $|2r^J(i) + \la d^J(i)| = \la$, in which
case we must add $i$ to $J$ and 
$\de(i) = \mathrm{sign}(2r^J(i) + \la d^J(i))$.
\end{itemize}

This directly leads to an algorithm that computes a solution of the
penalized problem by progressively adding and removing elements to $J$
until the correct set is found for the desired value of $\la$. For
this, start with $J_0 = \emp$ $\de_0 = 0$ and $\la_0 = 2\max_{i=1, \ldots, d} |r^\emp(i)|$. Let $J_n$ be the current
set in the algorithm, with signs provided by $\de_n$, and let
$\la_{n}$ be the last transition value. Denote $\hat \be_n = \hat\be^{J_n}$, the least square
estimator for $J_n$, $u_n = u^{\de_n}$, $r_n = r^{J_n}$ and $d_n =
d^{J_n}$ using the formulae above.
We want to compute $J_{n+1}$,
$\de_{n+1}$  and $\la_{n+1}$. 

The latter will be the first value
smaller than $\la_n$ at which one of the events in items 1. and
2. above occurs. Consider the first case. We have, for each $i\in J$:
$$
\de_n(i) \hat\be_n + \frac{\la_n}{2} u_{n}(i)\de_n(i) > 0
$$
this will remnain true for $\la <\la_n$ if $u_n(i)\de_n(i) \leq
0$ so that only indices with $u_n(i)\de_n(i) > 0$ are relevant
and a null value occurs with $\la = -\hat \be_n(i) /
u_n(i)$. 

For 2., we have 
$$
-\la_n < 2r_n(i) + \la_n d_n(i) < \la_n
$$
for all $i\not\in J$ and we must find the largest $\la <\la_n$ for
which the upper of the lower bound becomes an equality. Like in the
previous discussion, we see that an equality is possible in the lower
bound only if $(1+d_n(i))>0$ and in the upper-bound only if
$(1-d_n(i))>0$, the corresponding value being $\la = -2r_n(i)
/(1+d_n(i))$ in the frst case and $\la = 2r_n(i)
/(1-d_n(i))$ in the second case. So the update algorithm proceeds as follows:
 Compute 
$$\la'_n = \max\defset{- \frac{\hat\be_n(i)}{u_n(i)}: i\in J_n, \de_n(i)
  u_n(i) \geq 0};$$
Then compute
\begin{eqnarray*}
\la''_n &=& \max\defset{-\frac{2r_n(i)}{1+d_n(i)}, (1+d_n(i))>0,
  i\not\in J_n} \text{ and } \\
\la^{(3)}_n &=& \max\defset{\frac{2r_n(i)}{1-d_n(i)}, (1-d_n(i))>0,
  i\not\in J_n} \text{ and }
\end{eqnarray*}
We have the following cases (in which we assume, to simplify, that no
tie occurs in the determination of the maxima):
\begin{itemize}
\item[1.] $\max(\la'_n, \la''_n, \la^{(3)}_n) \leq \la$: stop the procedure; the solution
  is given by \eqref{eq:cons.lasso.0} with $J=J_n$.
\item[2.] $\la_n' >\max(\la, \la''_n, \la^{(3)}_n)$. Let $i^*$ be the index achieving
  the maximum in the definition of $\la'_n$: define $\la_{n+1} = \la'_n$
  and $J_{n+1} = J_n \setm \{i^*\}$.
\item[3.] $\la_n''  >\max(\la, \la^{(3)}_n, \la'_n)$ (resp. $\la_n^{(3)}  >\max(\la, \la^{''}_n, \la'_n)$). Let $i^*$ be the index achieving
  the maximum in the definition of $\la''_n$ (resp.  $\la^{(3)}_n$):
  define $\la_{n+1} = \la''_n$ (resp. $\la_{n+1}  =  \la^{(3)}_n$)
  and $J_{n+1} = J_n \cup \{i^*\}$, with $\de_{n+1}(i^*) =
  \mathrm{sign}(2r_n(i^*) + \la_n'' d_n(i^*))$. 
\end{itemize}

To solve the constrained problem, with constant $C$, it suffices to
compute, at each step $n$, the value $C_n = \sum_{i=1}^d |\be(i)|$. As
soon as $C_{n+1} \geq C$, we know that the correct set $J$ is $J_n$
with correct signs given by $\de_n$. It remains to find $\la$ such that
$$
C = \sum_{i\in J_n} \de_n(i)(\hat \be_n(i) + \la u_n(i)) = \sum_{i\in
  J_n} |\hat \be_n(i) + \la u_n(i)|
$$
and use \eqref{eq:cons.lasso.0} to obtain the solution.


\subsection{LARS estimator}
LARS, which holds for {\em Least Angle Regression}, is a variant of the
lasso in which only the incremental part of the set of active
variables is implemented. We now provide the interpretation that led
to the acronym. If $\mu$ denote the residual after regression, i.e.,
$$
\mu_k = y_k - \tx_k\be_\la,
$$
so that $r_\la(i)$ is the empirical correlation between $mu$ and $X(i)$.
The consistency equations imply that $|r(i)|$ is constant over all
variables $i\in J$, and larger than any $r(j)$ for $j\not\in J$. Since
we have normalized the variables, $r(i)$ is proportional to the cosine
of the angle between the residual and the selected variables. The
algorithm then chooses the next variable as the one which maximizes
this cosine, i.e., as the one which provides the least angle with the
current residual.

\subsection{The Dantzig selector}

The Dantzig selector is a regression method adapted to
underconstrained situations in which the number of predictive
variables, $d$, is large compared to the observations. Before
describing it, let us consider the noise-free case and the ill-posed problem of
solving the equation
$\CX \be = \CY$ when the dimension of $\CY$ ($N$) is small compared to
number of columns in $\CX$ ($d$). To simplify the discussion, we
assume that all variables are centered and do not consider the
intercept.

To select a solution that is well defined, additional constraints
are needed. A particularly appealing one is that the solution should
be sparse, i.e., have a small number of non-zero coefficients. This
naturally leads to the issue of finding a solution of $\CX \be
= \CY$ which  has the largest number of vanishing coefficients, but this problem,
is numerically intractable. Given that, as we have seen with
the lasso, minimizing the sum of absolute values often provides sparse
solutions, the problem can be replaced with the more tractable one
consisting in minimizing 
$$
\sum_{i=1}^d |b_i|
$$
subject to the constraint $\CX \be = \CY$ (as done with the lasso, we
assume that the empirical variance of each variable is normalized, so
that, denoting $\CX(i)$ the $ith$ column of $\CX$, we have $|\CX(i)| = 1$.)

This results in  a linear
programming problem. Introducing slack variables, it is 
equivalent to minimizing $\sum_{i=1}^d \xi_i$ subject to constraints
$\xi_i \geq b_i$, $\xi_i\geq -b_i$ and $\CX \be = \CY$.


Besides the numerical advantages of this method, there are interesting
theoretical properties that are satisfied, too. The natural issue is 
whether using the sum of absolute values permits to recover a sparse
solution when it exists. More precisely, let $\hat\be$ be the solution
of the linear programming problem and assume that there is a set $J\sub\{1,
\ldots, d\}$ such that $\CX\be = \CY$ for some $\be \in \mathbb R^d$
with $\be(i) = 0$ if $i\not\in J$;  under which conditions will
$\hat\be$ be equal to
$\be$? 

Sufficient conditions for this are provided in \cite{ct05} and involve
the correlation between the columns of $\CX$ and the size of $J$.
That the size of $J$ must be considered is
clear, since, for the statement to make sense, there cannot exist two
$\beta$'s satisfying $\CX\be = \CY$ and $\be(i) = 0$ for $i\not\in
J$. Uniqueness is obviously not true if $|J|>N$, because the condition
would become under-constrained for $\be$. Furthermore, the set
$J$ is not known, and we want to avoid any other solution associated
to a set of same size. So, there
cannot exist $\be$ and $\tilde\be$ respectively vanishing outside of $J$ and
$\tilde J$, where $J$ and $\tilde J$ have same cardinality, such that $\CX\be = \CY = \CX\tilde \be$. Having
$\CX(\be-\tilde\be) = 0$ is possible as soon as the number of non-zero
coefficients of $\be-\tilde\be$ is larger than $N$, and since this
number can be as large as $|J|+|\tilde J|$, we see that we should
impose at least $|J| \leq N/2$ in the statement. 


Another obvious remark is that, if the set $J$ on which $\be$ does not
vanish is known, with $|J|$ small enough, then $\CX\be = \CY$ is
underconstrained and the solution is (typically) unique. So the issue really is
whether one can identify $J$. 

The linear program we consider has an
equivalent dual form, which is also a linear program, and
its solution can be deduced from the one of the dual and
vice-versa. This dual problem admits a very simple form. Introducing
new variables $\al_1, \ldots, \al_N$, it requires
to maximize
$\al^T\CY$
subject to the constraints $|\al^T\CX(i)|\leq 1$ for $i=1, \ldots,
d$. Given a solution to this problem, one can find the Dantzig
selector by solving $\CX\hat\be = \CY$ with $\be(i) = 0$ for $i\not\in
J_\al$, where $J_\al = \defset{i:|\al^T\CX(i)| = 1}$. So the Dantzig
selector provides the correct answer as soon as $J_\al = J$.

Now, since $\al^T\CY = \al^T\CX\be = \sum_{i=1}^d \be(i) \al^T\CX(i)$,
it can be no larger than $\sum_{i\in J} |\be(j)|$, and such a value is
possible only if $\al^T\CX(i) = \mathit{sign}(\be(i))$ for $i\in
J$. If such an $\al$ can be found with, in addition $|\al^T\CX(j)|<1$
for $j\not \in J$, then it is a solution of the dual problem with
$J_\al = J$ and therefore provides the correct $\be$. For $T,T'\sub
\{1, \ldots, d\}$, define 
$\Sig_{TT'}$ to be the $|T|$ by $|T'|$ matrix formed by the dot
products $X(j)^TX(j')$, $j\in T$, $j'\in T'$.

Letting $s_J =
(s_j, j\in J)$ be defined by  $s_j = \mathit{sign} \be(j)$, a little
algebra proves that $\al$ should take the form
$$
\al = \sum_{j\in J} \rho(j) \CX(j) + w
$$
for some $w\perp \mathrm{span}(\CX(j), j\in J)$, with $\rho = \Sig_{JJ}^{-1}
s$. Letting $\al_J$ be the solution with $w=0$, the question is
therefore whether one can fond $w$ such that
$$
\left\{\begin{array}{ll}
w^\CX(j) = 0, & j\in J\\
|\al_J\cdot X(k) + w\cdot X(k)| < 1, & k\not \in J
\end{array}
\right.
$$
One can show that such a solution exists when the matrices
$\Sig_{TT}$ are close to the identity for $|T|$ smaller than a
constant \cite{ct05}. More precisely, denote, for $q\leq d$
$$
\de(q) =\max_{|T| \leq q} \max(\|\Sig_{TT}\|, \|\Sig_{TT}\|^{-1}) - 1
$$
and
$\th(q,q') = \max_{|z| = |z'| = 1} z^T \Sig_{TT'} z'$. Then, the
following proposition is true
\begin{proposition}[Candes-Tao]
Let $q = |J|$ and $s = (s_i, j\in J)\in \mR^q$. Assume that $\de(2q)
+ \th(q,2q) <1$. Then there exists $\al\in \mR^N$ such that
$\al^T\CX(j) = s(j)$ for $j\in J$ and
$$
|\al^T\CX(j)| \leq \frac{\th(q,q)}{1-\de(2q) - \th(q,2q)} \text{ if }
j\not\in J.
$$
\end{proposition}
So $\al$ has the desired property as soon as $\de(2q) + \th(q,q) +
\th(q,2q) \leq 1$. The interesting conclusion is that one only needs
to control subsets of variables of size less than $3q$ to obtain the
conclusion, which is important, of course, when $q$ is small compared to
$d$.


\bigskip

Consider now the noisy case, which is the situation for which the
Dantzig selector is defined. We here again introduce quantities that
were pivotal for the lasso and LARS estimator, namely, the correlation
between the variables and the residual error. So, we define, for a
given $\be$
$$
r_\be(i) = \CX(i)^T(\CY - \CX\be)
$$
which depends linearly on $\be$. Then, the {\em Dantzig selector} is defined
by the linear program: Minimize
$$
\sum_{j=1}^d |\be(j)|
$$
subject to the constraint 
$$
\max\limits_{j=1, \ldots, d} |r_\be(j)| \leq C.
$$
The explicit expression of this problem as a linear program is as
before by introducing slack variables $\xi(j), j=1, \ldots, d$ and
minimizing 
$$
\sum_{j=1}^d \xi(j)
$$
with constraints $\xi \geq \be$, $\xi\geq -\be$, $
\max\limits_{j=1, \ldots, d} |r_\be(j)| \leq C.
$

Similar to the noise-free case, the Dantzig selector can identify sparse
solutions (up to a small error) if the columns of $\CX$ are nearly orthogonal, with the same
type of conditions \cite{ct07}. Interestingly enough, the accuracy of
this algorithm can be proved to be comparable to the lasso in the
presence of sparse solution \cite{brt08}.

\section{Support Vector Machines for regression}

We will discuss support vector machines (SVM) in several steps, starting in
this section with the case of regression, without kernel (linear
SVM). Instead of least square, SVM uses the  loss function:
\begin{equation}
\label{eq:svm.v}
V(t) = \left\{
\begin{aligned}
 0 & \text{ if } |t| < \ep\\ 
 |t-\ep| &
\text{ otherwise}\end{aligned}\right.
\end{equation}


Such a loss function is an example of what is often called a robust
loss function. The quadratic error used in linear regression had the
advantage to provide closed form expressions for the solution, but is
very sensitive to outliers. It is often preferable to use loss
functions that increase linearly at infinity. One generally choose
them as smooth convex functions, for example $V(t) = (1-\cos\ga
t)/(1-\cos\ga\ep)$ for $|t|<\ep$ and $f(t) = |t|$ for $t \geq \ep$,
where $\ga$ is chosen so that $\ga\ep\sin\ga\ep /(1-\cos\ga\ep) =
1$. In such a case, minimizing
$$
F(\be) = \sum_{k=1}^N V(y_k - \be_0 - x_k^T b)
$$
can be done using smooth convex programming methods. 

Because $V$ in \eqref{eq:svm.v} is piecewise linear, an interesting
additional reduction of the problem may be obtained in that case. The SVM regression problem is formulated as the minimization of
$$ 
F(\be) = \sum_{k=1}^N V(y_k - \be_0 - x_k^T b) + \la |b|^2
$$
where $b = (\be_1, \ldots, \be_d)^T$. This function exhibits the
following features:
\begin{itemize}
\item A penalty on the coefficients of $\be$ (other than the
intercept), similar to ridge regression.
\item A linear penalty (instead of quadratic) for large errors in the
prediction.
\item An $\ep$-tolerance for small errors, often referred to as {\em the margin} of the SVM.
\end{itemize}

We now  describe the various steps in the analysis and reduction of
the problem. They will lead to simple minimization algorithms, and
possible extensions to nonlinear problems.

\subsection{Step 1: Reduction to a quadratic programming problem} 
Introduce the slack
variables $\xi_k, \xi_k^*, k=1, \ldots, N$. One
show that the original problem
is equivalent to the minimization, with respect to $\be, \xi, \xi^*$, of
$$
\sum_{k=1}^N (\xi_k+ \xi_k^*) + \la |b|^2
$$
under the constraints:
$$
\left\{\begin{array}{l} \xi_k, \xi_k^* \geq 0\\ \xi_k - y_k + \tilde
x_k^T\be +\ep \geq 0\\
\xi_k + y_k - \tilde
x_k^T\be +\ep \geq 0
       \end{array}
\right.
$$
The simple proof of the equivalence between the new and the original problems
is left to the reader. What we have obtained is a reduction to a
quadratic programming problem (minimize a quadratic 
function under linear constraints). We will refer to it as the primal
problem. Interesting insight, and possible nonlinear generalization, comes from reformulating this problem in
terms of what are called the dual variables. 

\subsection{Dual formulation}
There are 4N constraints, and we introduce 4N Lagrange multipliers for
them, $\eta_k, \eta_k^*$ for the positivity constraints, and $\al_k,
\al_k^*$ for the last two. The resulting Lagrangian is
\begin{multline*}
\mathcal L (b , \xi, \xi^*, \alpha, \alpha^*, \eta, \eta^*) = \sum_{k=1}^N (\xi_k+ \xi_k^*) + \la |b|^2 - \sum_{k=1}^N
(\eta_k\xi_k + \eta_k^*\xi_k^*) \\
- \sum_{k=1}^N \al_k (\xi_k - y_k +
\tilde x_k^T\be - \ep)  - \sum_{k=1}^N \al_k^* (\xi_k + y_k -
\tilde x_k^T\be - \ep) .
\end{multline*}
$(b, \xi, \xi^*)$ are the primal variables, and $\alpha, \alpha^*,
\eta, \eta^*$ the dual variables.


The solutions of the problem are characterized by the fact that, for
some set of dual variables, the
partial derivatives of $\mathcal L$ with respect to the primal
variables vanish, and the KKT conditions are satisfied, namely
$\al_k, \al_k^*, \eta_k, \eta_k^* \geq
0$ and 
$$
\left\{\begin{array}{l}
\al_k (\ep + \xi_k - y_k + \tilde x_k^T\beta) = 0  \\
\al_k^* (\ep + \xi_k^* + y_k - \tilde x_k^T\beta) = 0  \\
\eta_k\xi_k = \eta_k^*\xi_k^* = 0
       \end{array}
\right.
$$
(i.e., if a
constraint is satisfied with a strict inequality, then the
corresponding Lagrange coefficient must vanish). 

The same characterization applies to the solution of the dual problem,
which  is associated to the maximization of the function 
$$
L^*(\al, \al^*, \eta, \eta^*) = \inf_{\be, \xi, \xi^*} \mathcal L.
$$
 under the previous
positivity constraints. 

We now compute $L^*$. Since the Lagrangian is linear in $\be_0$,
$\xi_k$ and $\xi_k^*$, its minimum is $-\infty$ unless the
coefficients vanish. We therefore have $L^* = -\infty$ unless the first three conditions in the system below must be satisfied. The fourth one expresses the fact that the derivative in $b$ of $\mathcal L$ must vanish. We have:
$$
\left\{\begin{array}{l}
1 - \eta_k - \al_k = 0 \\
1 - \eta_k^* - \al_k^* = 0 \\
\sum_{k=1}^N (\al_k-\al_k^*) = 0 \\
2 \la b - \sum_{k=1}^N (\al_k-\al_k^*) x_k^T = 0
       \end{array}
\right.
$$ 
Using $\eta_k  = 1- \al_k$ and $\eta_k^* = 1- \al_k^*$ and the
expression of $b$,, we can 
express $L^*$ uniquely as a function of $\al, \al^*$, yielding
$$
L^*(\al, \al^*) = -\frac{1}{4\la} \sum_{k,l=1}^N
(\al_k-\al_k^*)(\al_l-\al_l^*)\scp{x_k}{x_l} - \ep \sum_{k=1}^N
(\al_k+\al_k^*) + \sum_{k=1}^N (\al_k-\al_k^*)y_k
$$
with $\scp{x_k}{x_l} = x_k^Tx_k$.
This must be maximized with the constraints that $0\leq \al_k,
\al_k^*\leq 1$ and $\sum_{k=1}^N (\al_k-\al_k^*) = 0$ 
from the previous system. This still is
a quadratic programming problem, but now has additional nice features
and interpretations.

\subsection{Analysis of the dual problem}
The first fact is that the dual problem only depends on the $x_k$'s
through the matrix of their inner products. This is irrelevant in 
small dimension, but in large dimension, this may become an important
advantage (if the $2N$ unknowns of the dual problem are less that the $d$ original dimensions). Many applications of support vector machines work in fact
with a linear space of infinite dimension, with the help of a 
``kernel trick'' which will be discussed later, in which case the reduction is unavoidable.. The obtained predictor can
also be expressed as a function of the inner products, since
$$
y = \beta_0 + x^T b = \be_0 + \frac{1}{\la} \sum_{k=1}^N (\al_k-\al_k^*)
\scp{x_k}{x}\,.
$$

The parameter $\be_0$ can be determined  using the KKT conditions when the optimal $\al, \al^*$ are computed. We now analyze these conditions, which reduce to
$$
\left\{\begin{array}{l}
\al_k (\ep + \xi_k - y_k + \be_0 + x_k^T b) = 0  \\
\al_k^* (\ep + \xi_k^* + y_k - \be_0 - x_k^T b) = 0  \\
(1-\al_k)\xi_k = (1-\al_k^*)\xi_k^* = 0
       \end{array}
\right.
$$

Let's see how and when these equations are satisfied. First consider indices $k$
such that the error is strictly within the $\ep$-tolerance
margin: $|y_k - \be_0 - x_k^Tb| < \ep$. Then the first two equations and $\xi_k, \xi_k^* \geq 0$ imply that $\al_k  \al_k^* = 0$ and the last two imply $\xi_k  = \xi_k^* = 0$. This provides no information on $\be_0$, but
has the following consequence: {\em the variables $\al$ and $\al^*$
vanish for the samples with prediction error less than $\ep$}. 

Consider now the case when the prediction is strictly less accurate
than the margin. Assume that $y_k - \be_0 - x_k^Tb > \ep$, the other case
being symmetrical. This implies that $\al_k^* = \xi_k^* = 0$. This also implies that 
\[
\xi_k = y_k - \be_0 - x_k^Tb -\ep >0
\]
and $\al_k = 1$. No information is obtained on $\be_0$ in this case also.

The remaining cases are samples for which the prediction error is exactly
at the margin. Assume again that it is positive: this implies that $\xi_k =
0$ (otherwise $\xi_k - y_k + \be_0 + x_k^Tb +\ep > 0$, which implies that $\al_k=0$ and $(1-\al_k)\xi_k=0$ is a contradiction. We therefore have $y_k - \be_0 - x_k^T b = \ep$ which provides the
value of $\be_0$. The points for which the error is exactly at the margin are called {\em support vectors}. These are the points that  can be used to compute 
$\be_0$ and there are, in
general, several such points in practice.

Note also that $\al_k$ and $\al_k^*$ cannot be nonzero together
(because they correspond to incompatible constraints), and that when
they are both zero, the corresponding points do not contribute to the
estimation. Finally, for all points except support vectors, their value is either 0 or 1. 

\subsection{Extension to other cost functions}
This $\ep$-tolerant function is the most commonly used cost function
in the SVM literature. However, the previous analysis would not be much
affected if $V(t)$ were replaced by some other function $C(t) =
c_0(t-\ep)$ if $t\geq \ep$ and 0 otherwise, with a convex
$c_0$. Then, the primal problem is: minimize
$$
\frac{\la}{2} |b|^2 + \sum_{i=1}^N (c_0(\xi_k) + c_0(\xi_k^*))
$$
with the constraints 
$$
-\ep - \xi_k^* \leq y_k - \be_0 - x_k\be \leq \ep+\xi_k
$$
and $\xi_k, \xi_k^* \geq 0$. This is a convex programming problem. Its
equivalent dual formulation is: maximize
$$
- \frac{\la}{2} \sum_{k,l=1}^N (\al_k-\al_k^*)\scp{x_k}{x_l}
(\al_l-\al_l^*) + \sum_{k=1}^N (\al_k-\al_k^*)y_k - \ep \sum_{i=1}^N
(\al_k+\al_k^*) +  \sum_{k=1}^N (T(\xi_k) + T(\xi_k^*))
$$
with the constraints $\al_k, \al_k^*\xi_k, \xi_k^* \geq 0$, $\sum_k (\al_k-\al_k^*)
= 0$, $\xi_k = \inf\defset{t, c'_0(t) > \al}$, and the notation
$$
T(u) = c_0(u) - u c'_0(u).
$$
The dual formulation still has the property to depend only on the
inner products $\scp{x_k}{x_l}$.


\chapter{Models for linear classification}

In this section, $Y$ takes values in a finite set $\CG = \defset{g_1,
\ldots, g_q}$, and the goal is to predict this class variable from the
observation of $X$, which is assumed, as before, to belong to
$\mR^d$. We review in this section some linear models which are used
in this context.

\section{Linear regression and Optimal Scoring}

In this approach, the set $\CG$ is mapped to a collection of $r$
dimensional row vectors $\th_{g_1}, \ldots, \th_{g_q}$. One can for example take $r=q$ and $\th_{g_1} = (1,0,\ldots,0)$,
$u_{g_2} = (0,1,0,\ldots,0)$, until $\th_{g_q} = (0,\ldots,0,1)$. A linear
model is then estimated from this data, by minimizing
$$
\sum_{k=1}^N |\th_{y_k} - \tilde x_k^T\beta|^2
$$ 
as before, with the only difference that $\beta$ now is a $(d+1) \ti
q$ matrix instead of a vector. This yields a least square estimator
$\hat \beta = (\CX^T\CX)^{-1}\CX^T\CY$ where $\CY$ is the
matrix of stacked $\th_{y_k}$ row vectors. 

Given an input vector $x$, the row vector $\tilde x^T\beta$ has
real coefficients which are not $0$ and 1's. Assignment to a class is typically  
made by minimizing $|\tilde x^T \be - \th_{g}|$ over all
$g$ in $\CG$.

This approach is questionable, however, because the choice of
assigning $\th_g$ to $g$ may seem artificial. It can be modified by optimizing also over these choices, leading to {\em optimal scoring}.
In this case, the score  $g\mapsto \th_g$ is an additional parameter of the model. To simplify the discussion, we will first assume that $r=1$, i.e., the scores are scalar.

The problem is
then formulated as a least square minimization of
$$
\sum_{k=1}^N (\th_{y_k} - \be_0 - x_k^T b)^2
$$
with respect to $\th = (\th_1, \ldots, \th_q)$ and $\be = (\be_0, b)$. Since the problem is
invariant by the multiplication of a constant, and to avoid the
trivial solution $\th=\be=0$, $\th$ is normalized by the constraint
$\sum_g N_g \th_g^2 = 1$. Also, to avoid ambiguities in the choice of
$\be_0$, it is also assumed that $\sum_g N_g \th_g=0$. This last
constraint implies that $\sum_k \th_{y_k} = 0$, and this implies in
turn that the optimal $\be_0$ is 
$$
\be_0 = \frac{1}{N} \sum_{k=1}^N (\th_{y_k} - x_k^Tb) = -\bar\mu^Tb
$$
with $\bar \mu = \sum_{k=1}^N x_k /N$.
The problem therefore reduces to minimizing
$$
\sum_{k=1}^N (\th_{y_k} - (x_k-\bar\mu)^T b)^2
$$
with the previous constraints. To lighten the notation, we will assume
in the following that $\bar\mu = 0$. This is no loss of generality, since
this corresponds to assuming that the $x_k$ have been centered before processing.


Introduce the binary column vectors $u_{i} = (0, \ldots,
0,1,0, \ldots, 0)^T$ with a 1 a the $i$th position.  The minimized function can now be written as
$$
\sum_{k=1}^N (u_{y_k}^T\th - (x_k-\bar\mu)^T b)^2
$$
where $\th$ is now the column vector with coordinates $\th_1, \ldots,
\th_n$. We will use the following notation. For $g\in\CG$, denote by $N_g$ the
number of $k$'s for which $y_k = g$. We let
$$
\mu_g = \frac{1}{N_g} \sum_{k=1}^N x_k \chi_{[y_k = g]}
$$
denote the class averages. so that $\bar\mu = \sum_{g\in \CG} c_g \mu_g$ with $c_g = N_g/N$. 
We let
$$
\Sig_g = \frac{1}{N_g} \sum_{k=1}^N (x_k - \mu_{g})(x_k - \mu_{g})^T\chi_{[y_k=g]}\,.
$$
denote the class covariance matrix, and their weighted average
\[
\Sig_w = \sum_{g\in\CG} c_g\Sig_g,
\]
called the {\em within class} covariance matrix. The between class covariance matrix is
\[
\Sig_b = \sum_{g\in\CG} c_g (\mu_g- \bar\mu)(\mu_g- \bar\mu)^T.
\]
The total covariance matrix
\[
\Sig_{XX} = \frac{1}{N}\sum_{k=1}^N (x_k-\bar\mu) (x_k - \bar\mu)^T
\]
then satisfies $\Sig_{XX} = \Sig_w + \Sig_b$.
We will furthermore let $M = [\mu_{g_1}-\bar\mu, \ldots, \mu_{g_q}-\bar\mu]$ (a $d\times q$ matrix) and $C = \mathrm{diag}(c_1, \ldots, c_q)$ so that, for example
\[
\Sig_b  = MCM^T.
\]

With this notation, the optimal scoring problem can be expressed as the minimization of 
\[
L(\th, b) = \th^TC \th - 2 b^TMC \th + b^T\Sig_{XX} b
\]
with respect to $b$ and $\th$, subject to the constraints $\sum_g c_g \th_g = 0$ and $\th^TC\th = 1$. The optimal $b$ is given by
\[
b = \Sig_{XX}^{-1} MC\th
\]
so that $\th$ must maximize
\[
\th^T C^TM^T \Sig_{XX}^{-1} MC\th
\]
subject to the constraints. If we let $\tilde C = C^{1/2}$, $\tilde\th = C^{1/2} \th$, and $z = (\sqrt{c_1}, \ldots, \sqrt{c_q})^T$, then the problem is equivalent to minimizing
\[
\tilde \th^T \tilde C^TM^T \Sig_{XX}^{-1} M\tilde C \tilde \th
\]
subject to $\tilde\th^T\tilde \th = 1$ and $z^T\tilde\th = 0$. The solution is given by letting $\tilde \th$ be the unit eigenvector associated with the largest eigenvalue of $\tilde C^TM^T \Sig_{XX}^{-1} M\tilde C$. This eigenvector automatically satisfies $z^T\tilde\th = 0$ because $z$ is also an eigenvector of this matrix, with eigenvalue 0 (we have $M\tilde C z  = 0$). Returning to the original variable, the optimal $\th$ is therefore given by the eigenvector with largest eigenvalue of $C^TM^T \Sig_{XX}^{-1} M$ normalized so that $\th^TC\th = 1$.


The following computation will link optimal scoring with linear discriminant analysis, which will be discussed in the next section. 
 Let $\eta$ be an eigenvector of $C^TM^T \Sig_{XX}^{-1} M$ with eigenvalue $\la$. Then 
\begin{align*}
&CM^T\Sig_{XX}^{-1} M\eta  = \la\eta\\
\text{thus, }& MCM^T\Sig_{XX}^{-1} M\eta = \la M\eta\\
\text{thus, }& (MCM^T + \Sig_w)\Sig_{XX}^{-1} M\eta - \Sig_w \Sig_{XX}^{-1} M\eta = \la M\eta\\
\text{or, }&  \Sig_w \Sig_{XX}^{-1} M\eta = (1-\la) M\eta
\end{align*}
This implies that 
$$(1-\la)^{-1} M\eta = \Sig_{XX}\Sig_w^{-1} M\eta = (\Id +
\Sig_b\Sig_w^{-1})M\eta$$
so that
$$
\Sig_b\Sig_w^{-1}M\eta = \frac{\la}{1-\la} M\eta
$$
or
$$
\Sig_w^{-1}\Sig_b (\Sig_w^{-1}M\eta) = \frac{\la}{1-\la} (\Sig_w^{-1} M\eta)
$$

This implies that the eigenvectors and eigenvalues of
$CM^T\Sig_{XX}^{-1} M$ are related to those of $\Sig_w^{-1}\Sig_b$ by 
$\th \mapsto \Sig_w^{-1}M\th$ and $\la \mapsto \la/(1-\la)$. Since the
relations between the eigenvalues is increasing, the order of the
eigenvectors is the same.

% the optimal scores directly provide the
%first discriminant direction. More precisely, if $e_1$ is, as above,
%the first eigenvector of $C^{1/2}M^T \Sig_w^{-1} M C^{1/2}$, then , up
%to a renormalization, $\Sig_w^{-1} M\th = \Sig_w^{-1} M C^{1/2}e_1$
%which implies that $\th = C^{1/2} e_1$ (we can ``simplify'' by $M$
%because both $\th$ and $C^{1/2} e_1$ are orthogonal to the null space
%of $M$).



\bigskip

This analysis can be generalized to
vector-valued scores, where $\th_g=(\th_g(1), \ldots, \th_g(r))$ now is
a row vector, $b$ a $d\ti r$ matrix and the minimized function
is
$$
\sum_{k=1}^N |u_k^T\th - \be_0 - x_k^T b|^2
$$
with the constraints $\th^T C\th = \mathrm{Id}$. The result is that the
optimal $\th$ is provided are the first $r$ eigenvectors of
$CM^T\Sig_{XX}^{-1} M$. As just remarked, they can be deduced from the first $r$ eigenvectors of $\Sig_w^{-1}\Sig_b$ by the transformation $\th \mapsto \Sig_w^{-1}M\th$.

Optimal scoring is that it can be modified as
in ridge regression by adding a penalty of the
form $\sum_{i=1}^q \be_i\Om\be$ where $\Om$ is a weight matrix. This
only modifies the previous computation by replacing $\Sig_{XX}$ by
$\Sig_{XX}+\Om$.



\section{Linear Discriminant analysis}
\label{sec:lda}

Linear discriminant analysis (LDA) has two ``flavors''. One is generative, and described in the lines below. The other is discriminative, and will be described next. We will use the notation introduced in the previous section.


Given conditional densities of $X$ given $Y=g$ (denoted
$f_g$) are known and prior probabilities $\pi_g =
P(Y=g)$, the Bayes estimator maximizes the posterior probability
$$
P(Y=g|X=x) = \frac{\pi_g f_g(x)}{\sum_{g'\in \CG} \pi_{g'} f_{g'}(x)}
$$
Consider the region for class $g$ better than class $h$:
$$
R_{gh} = \defset{x\in\mR^d\,/\, \pi_g f_g(x) \geq \pi_{h} f_h(x)}
$$
Linear classification corresponds to the situation in which these regions
are half spaces (delimited by a hyperplane). This occurs in particular
the distributions $f_g$ are all Gaussian densities with
mean $m_g$ and common variance $S$,
$$
f_g(x) = \frac{1}{\sqrt{(2\pi)^d\det \Sig}} e^{-(x-m_g)^T S^{-1}
(x-m_g)},
$$
which are the assumptions made in the generative version of LDA.
In this case, the decision boundaries are such that, for some $g$ and $h$
$$
\log \pi_g + \log f_g = \log\pi_h + \log f_h
$$
which yields, 
$$
\log \pi_g -(x-m_g)^T S^{-1}
(x-m_g) = \log\pi_h - (x-m_h)^T S^{-1}
(x-m_h)
$$
or
$$
2 x^TS^{-1}(m_g-m_h) = \log \frac{\pi_g}{\pi_h} +
m_g^TS^{-1}m_g - m_h^TS^{-1}m_h
$$
which is the equation of a hyperplane. 

\medskip
The means and variance are not known beforehand, and must
be estimated from data, taking $\hat m_g = \mu_g$, $\hat S = \Sig_w$ (see previous section). If one relaxes the assumption of common class variances, and use $\Sig_g$ in place of $\Sig_w$ for class $g$. The decision boundaries are not linear in this case, but provided by quadratic equations (and the resulting method if often called quadratic discriminant analysis, or QDA). QDA requires the estimation of $qd(d+3)/2$, which may be overly ambitious when the sample size of not large compared to the dimension, and QDA is often prone to overfitting. Evan LDA, which  involves  $qd + d(d+1)/2$ parameters, may be unrealistic in such cases (but it is certainly more resilient).
A variant of QDA uses 
a shrinkage operation on $\Sig_g$, working with class covariance
matrices given by
$$
\tilde \Sig_g = \al \Sig_w + (1-\al)\Sig_g.
$$

\subsection{Dimension reduction}

Even in the linear case, the number of required parameters may still
be too high to provide reliable results. One of the interests of LDA
is that it can be combined with a rank reduction procedure, in a way
which resembles principal component analysis\footnote{Principal
component analysis will be discussed in detail in chapter \ref{chap:unsupervised}.}. 
 

We first remark that LDA operates over a $(q-1)-dimensional affine space $V$, in the sense that there one can replace each sample by a skewed projection on that space without changing the result.  To simplify the discussion, we  assume that the data has been ``spherized'', to ensure that  $0 = \bar \mu$ and $\Sig_w = \Id$. This operation consists in replacing $x_k$ by $\tilde x_k = \Sig_w^{-1/2}(x_k-\bar\mu)$, where $\Sig^{1/2}_w$ is positive symmetric square root of $\Sig_w$.
We will denote by $\tilde\mu_g$.

With this notation, the decision rule for $g$ better than $h$ for a new sample $x$ is 
$$
\tilde x^T (\tilde \mu_h- \tilde \mu_g) \geq \frac{1}{2}
\Big(|\tilde \mu_g|^2  - |\tilde \mu_h|^2 + \log \frac{\pi_g}{\pi_h}\Big)
$$
with $\tilde x = \Sig_w^{-1/2}(x-\bar\mu)$.

Now, let $V$ be the affine space space generated by  $\tilde \mu_g, g\in
\CG$, which (because it contains 0) is actually a linear space. Let $P_V$ denote the orthogonal projection on $V$. From elementary
properties of the projection, we have
$\tilde x^T z = (P_V\tilde x)^T z$ for any $z\in V$ and $\tilde x\in \mathbb R^d$, so that, since the $\mu_g$'s
belong to $V$, the decision rules can be replaced by 
$$
(P_V \tilde x)^T (\tilde \mu_h- \tilde \mu_g) \geq \frac{1}{2}
\Big(|\tilde \mu_g|^2  - |\tilde \mu_h|^2 + \log \frac{\pi_g}{\pi_h}\Big)
$$
still with $\tilde x = \Sig_w^{-1/2}(x-\bar\mu)$.\\

So this proves that, for a given $x$, the decision is based only on
$P_V\tilde x$, which can be described by $r \leq (q-1)$ numbers (where
$r = \mathit{dim}(V)$ and $q = |\CG|$). They can be computed
easily as soon as one computes an orthonormal basis $(\tilde e_1,
\ldots, \tilde e_{r})$ of $V$, since, in
this case
$$
P_V \tilde x = \sum_{j=1}^{r} \tilde x^T\tilde e_j \tilde e_j.
$$
Since $\tilde e_j \in V$, they can be written as linear combinations
of the $\tilde\mu_g$'s, so there there must exist a $q$ by $r$
matrix $\tilde A$ such that
$$
\tilde E: = [\tilde e_1, \ldots, \tilde e_{r}] = [\tilde \mu_{g_1}, \ldots, \tilde
\mu_{g_q}] \tilde A
$$
(for some order $\CG = \{g_1, \ldots, g_q\}$). To have an orthonormal
family, we need $\tilde E^T\tilde E = \Id_{r}$ yielding
$$
\Id_{r} = A^T  \tilde M^T \tilde M A
$$
with $\tilde M = [\tilde \mu_{g_1}, \ldots, \tilde
\mu_{g_q}]$ and $\tilde M^T\tilde M$ is the $q$ by $q$ matrix formed
with the dot products of the $\mu_g$'s. Its rank is the dimension of
$V$. Let $\tilde a_1, \ldots, \tilde a_q$ be its eigenvectors,
associated to decreasing eigenvalues $\la_1, \ldots, \la_q$ (the first
$r$ being non-vanishing). Then, it is an easy computation to check
that 
$\tilde A = [\tilde a_1/\sqrt{\la_1},
\ldots, \tilde a_{r}/\sqrt{\la_r}]$ satisfies the required
identity. This is not the only solution that we can get this way,
however. In fact, if $S$ is any invertible $q$ by $q$
matrix, we can apply the same computation replacing $\tilde A$ by
$S\tilde A$,
yielding
$$
\Id_{r} = \tilde A^T S^T  \tilde M^T \tilde M S \tilde A,
$$
and let $\tilde a_1, \ldots, \tilde a_q$ be the eigenvectors of
$S^T \tilde M^T \tilde M S$, still taking 
$\tilde A = [\tilde a_1/\sqrt{\la_1},
\ldots, \tilde a_{r}/\sqrt{\la_r}]$ for the corresponding eigenvalues. We will assume that such an $S$ is
chosen in the rest of the computation.

To classifiy $x$, one must compute the ``scores'' $\ga_j(x) =
\tilde x^T \tilde e_j$, the decision ``$g$ better than $h$'' being 
$$
\sum_{j=1}^r\ga_j(x)(\ga_j(\mu_g) - \ga_j(\mu_h)) \geq \frac{1}{2}
\Big(\sum_{j=1}^r (\ga_j(\mu_g)^2 - \ga_j(\mu_h)^2) + \log \frac{\pi_g}{\pi_h}\Big)
$$


These scores have a nice expression in terms of the original
variables. Define $M = [\mu_{g_1} - \bar\mu, \ldots, \mu_{g_q}-
\bar\mu]$ so that $\tilde M = \Sig_w^{-1/2} M$ and $\tilde M^T \tilde
M = M^T \Sig_w^{-1} M$. By construction
$S^T\tilde M^T\tilde M S\tilde A = \tilde A \La$, where $\La =
\mathit{diag}(\la_1, \ldots, \la_r)$,  yielding
\begin{equation}
\label{eq:lda.1} 
S^TM^T \Sig_w^{-1} MS \tilde A= \tilde A \La. 
\end{equation}
We also have $\tilde A$ $\tilde MS\tilde A = \tilde E$, yielding
$\Sig_w^{-1/2} MS\tilde A = \tilde E$; multiplying both sides in
\eqref{eq:lda.1} by $\Sig_w^{-1/2}MS$ we get
$$
\Sig_w^{-1/2} MSS^TM^T \Sig_w^{-1/2} \tilde E = \tilde E \La.
$$ 
Multiplying the result by $\Sig_w^{-1/2}$ and letting $ E =
\Sig_w^{-1/2} \tilde E$, we finally get
$$
\Sig_w^{-1} MSS^TM^T E = E \La
$$
so that $E$ is a matrix formed with the eigenvectors of $\Sig_w^{-1}
MSS^TM^T $ (but normalized so that $E^T\Sig_w^{-1} E = \Id_r$).
These properties permit to compute $E$, from which all scores can be
computed since
$$
\ga_j(x) = x^T \Sig_w^{-1/2} \tilde e_j = x^T e_j.
$$
Letting $Q = SS^T$ (any positive definite matrix can take this form)
and 
$$
\Sig_b^Q = MQM^T = \sum_{g\in\CG} q_{gh} (\mu_g-\mu) (\mu_h-\mu)^T, 
$$
we see that $e_1, \ldots, e_r$ are eigenvectors of of $\Sig_w^{-1}
\Sig_b^Q$, so that, for some $\la_j$:
$$
\Sig_b^Q e_j = \Sig_w e_j.
$$
This is the generalized eigenvalue problem associated to $\Sig_b^Q$
and $\Sig_w$. The first eigenvector is the maximizer of the ratio
$$
u\mapsto \frac{u^T\Sig_b^Q u}{u^T\Sig_w u}
$$
and the following ones maximize this ratio subject to the constraint of
being perpendicular to those that precede. With $Q =
\mathit{diag}(c_{g_1}, \ldots, c_{g_q})$, we have
$$
\Sig_b^Q = \Sig_b := MCM^T  = \sum_{g\in \CG} c_g (\mu_g-\mu)
(\mu_g-\mu)^T
$$
which is called the between class (or interclass) covariance
matrix. The method or progressively maximizing the ratio 
${u^T\Sig_b^Q u}/{u^T\Sig_w u}$ is called {\em Fisher's linear
  discriminant analysis}. 

\section{Optimal scoring}

\section{Logistic regression} 

Logistic regression uses the fact that, in order to apply the Bayes
rule, only the conditional distribution of the class variables $Y$
given $X$ is needed. Denote $p(g|x)$ for the conditional distribution
of $Y=g$ given $X=x$. Logistic regression corresponds to the model
$$
\log p_\be(g|x) = \tilde x^T \beta(g) - \log(C(\beta, x))
$$
where
$C(\beta, x) = \sum_{g\in \CG} \exp(\tilde x^T \beta(g)).$

From this definition, it is clear that the model is unchanged  if a constant vector is added
to $\be$, so that the model is overparametrized. This can be addressed
by adding a constraint like: $\sum_g
\beta(g) = 0$, or $\beta(g_0) = 0$ for some $g_0\in \CG$.

The classification rule can be applied as soon as a family of vectors $(\be(g),
g\in\CG)$ has been estimated, and this estimation can be done by maximum
likelihood. Let, as usual, $(y_1, x_1), \ldots, (y_N, x_N)$ form the
training data. We need to maximize:
$$
l(\be) = \sum_{k=1}^N \log p_\be(y_k|x_k)\,.
$$
This is a non linear problem, which has however the advantage of being
concave, since 
$$
\pdr{}{\beta(g)} \log p_\be(y|x) = \tilde x^T \chi_{[y=g]} - 
\tilde x^T p_\be(g|x)
$$
and the second derivatives are
$$
\pddr{}{\beta(g)}{\beta(g')} \log p_\be(y|x) = -\tilde x \tilde x^T
\chi_{[g=g']} p_\be(g|x) + 
\tilde x \tilde x^T p_\be(g|x) p_\be(g'|x).
$$
Let us check that the matrix of second derivative is non-positive. If
$a(g), g\in\CG$ is a family of $(d+1)$-dimensional vectors,  we have
\begin{eqnarray*}
\sum_{g,g'\in\CG} a(g)^T\left(\pddr{}{\beta(g)}{\beta(g')} \log
p_\be(y|x)\right)a(g') &=& -\sum_{g\in\CG} a(g)^T \tilde x \tilde x^T a(g)
p_\be(g|x)  \\
&& + \sum_{g,g'\in\CG} a(g)^T \tilde x \tilde x^T a(g') p_\be(g|x)
p_\be(g'|x)\\
&=& -E((\tilde x^T a)^2|x) + E((\tilde x^T a)|x)^2 \leq 0.
\end{eqnarray*}
This proves the concavity. From the computed gradient and second
derivative, an efficient Newton algorithm can be implemented to
estimate $\beta$.
\\

The result of the logistic regression algorithm is, like for the LDA,
decision regions which are separated by pieces of  hyperplanes. For a
2 class problem, in particular, the two regions are linearly
separated.

This raises an issue we have encountered before, on why estimating a
model if we know that in the end, we will find a
separating hyperplane; why not trying to directly estimate it from the
data, by minimizing the empirical risk. This is the subject of the
next section.

\section{SVM for linear classification}

\subsection{Linear perceptrons}
We here restrict to the two-class problem, and let $\CG =
\defset{-1,1}$. A separating hyperplane predicts the class according
to the sign of the linear expression $\be_0 + x^T b$. With this
notation, a pair $(y,x)$ is correctly classified if and only if
$y(\be_0 + x^T b) > 0$.

Assume that a training set is available, denoted as usual by $(y_1,
x_1), \ldots, (y_N, x_N)$. 
The perceptron algorithm estimates $\be_0$ and $b$ by minimizing 
$$
L(\be) = \sum_{k=1}^N [y_k(\be_0 + x_k^T b)]^-
$$
with $u^- = \max(0, -u)$. If $\CM$ is the set of misclassified
examples (those for which $y(\be_0 + x^T b) < 0$), we can write
$$
L(\be) =- \sum_{k\in\CM} y_k(\be_0 + x_k^T b).
$$
Assuming that no points lie on the boundary $\be_0 + x_k^T b = 0$, we
can compute the gradient $L$ with respect to $\be_0$ and $b$, yielding
$$
\pdr{L}{\be_0} = - \sum_{k\in\CM} y_k, \hfill \pdr{L}{b} = -
\sum_{k\in\CM} y_kx_k^T.
$$\\

Rosenblatt's algorithm visits examples belonging to $\CM$
iteratively. When, say, example $k$ is visited, $\be_0$ is replaced by
$\be_0 + \rho y_k$ and $b$ by $b + \rho y_k x$ with a ``learning
parameter $\rho>0$. When the problem has a solution, this algorithms selects a
separating hyperplane in a finite number of steps. 
However, when no solution
exists, the algorithm is very hard to analyze, and runs
indefinitely. \\

A more robust (and efficient) algorithm can be used, relying on the
fact that the perceptron is a linear program. Indeed, it is equivalent
to minimize
$$
\sum_{k=1}^N \xi_k
$$
subject to the constraints $x_k\geq 0, \xi_k-y_k(\be_0 + x_k^Tb) \geq
0$ for $k=1, \ldots, N$. The following algorithm proposes a solution
of the problem in at most $N$ steps if and only if a solution
exists. It starts with $\be = 0$ and a matrix $H = \mathit{Identity}$. At step $n$, the algorithm
selects a misclassified example, $k$, and updates $\be$ and $H$ as
follows:
\begin{eqnarray*}
\be &\to& \be + \frac{1}{n+1} \frac{y_kHx_k}{\sqrt{x_k^THx_k}}\\
H &\to& \frac{n^2}{n^2-1}\big(H - \frac{2}{n+1} \frac{x_k^TH^2x_k}{x_k^THx_k}\big)
\end{eqnarray*}
The algorithm stops if no misclassified example remains. If the method
has not converged at step $N$, there is no solution.

\subsection{Linear SVM}
Note that, when a separating hyperplane exists, it is not unique, and
the perceptron algorithm just finds one of them. Intuitively, one
prefers a solution that would classify the examples with some large
margin, rather than one for which training points are close to the
separating hyperplane. This leads to the maximum margin separating
hyperplane introduced by
Vapnik and Chervonenkis.

We now describe this algorithm, which is commonly called linear support vector machine. It is
easier to understand how it works if we start with the case when a
separating hyperplane exists for the given dataset. Then, the quality
of the split can be measured by the margin with which the
discrimination is performed, ie. the minimal distance over all the
$x_k$'s to the hyperplane $\be_0 + x^Tb = 0$. 

The distance of a point $x\in\mR^d$ to this hyperplane is  $|\be_0 + x^Tb|/\|b\|$, and when $(y,x)$ is a pair of correctly
classified data, this is equal to $y(\be_0 + x^Tb)/\|b\|$. Thus, the
classification margin, over the training set, is given by (for a given
separating hyperplane)
$$
m(\be_0, b) = \min_{k=1, \ldots, N} y_k(\be_0 + x_k^T b)/\|b\|.
$$
Finding the best hyperplane requires maximizing this with respect to all $(\be_0, b)$
which separating the data. This is equivalent to the
problem:\\
maximize $C$ under the constraint $C\|b\| \leq y_k(\be_0 + x_k^T b)$ for
all $k=1, \ldots, N$. Since the solution $(\be_0, b)$ is defined up to
a positive multiplicative, constant, there is no loss of generality in
assuming that $\|b\| = 1/C$ and the problem becomes equivalent to
minimizing $\|b\|^2/2$ under the constraints that $y_k(\be_0 + x_k^T b)
\geq 1$ for $k=1, \ldots, N$, which is a quadratic programming problem.


Before passing to the dual formulation, we modify this framework
to also handle the situation in which the data cannot be separated by
a hyperplane. This is done by introducing slack variables $\xi_k \geq
0, k=1, \ldots, N$ and replacing the $k$th constraint by $y_k(\be_0 +
x_k^T b)
\geq 1 -\xi_k$. Of course, the slack variables must be controlled in
order to avoid trivial solutions, and this is done by either adding a
constraint of the form $\sum_k\xi_k \leq M$, for some parameter $M$,
or by adding a penalty term $\ga \sum_k \xi_k$ in the function to
minimize. We consider the latter case here, and therefore solve the
quadratic optimization problem: minimize
$$
\frac{1}{2} \|b\|^2 + \ga \sum_{k=1}^N \xi_k\,,
$$
under the constraints $\xi_k \geq 0$, $y_k(\be_0 + x_k^T b) + \xi_k
\geq 1$, for $k=1, \ldots, N$. Introduce Lagrange multipliers
$\eta_k\geq 0$
for the positivity constraints and $\al_k\geq 0$ for the other constraints to
write the Lagrangian:
$$
\mathcal L = \frac{1}{2} \|b\|^2 + \ga \sum_{k=1}^N \xi_k - \sum_{k=1}^N
\eta_k\xi_k -  \sum_{k=1}^N \al_k (y_k(\be_0 + x_k^T b +\xi_k - 1).
$$
Minimizing this with respect to $\be$ and $\xi_1, \ldots, \xi_N$
yields $b = \sum_{k=1}^N \al_k y_k x_k$, $\sum_{k=1}^N \al_ky_k  = 0$
and $\al_k = \ga - \mu_k$. The resulting dual formulation is :
maximize
$$
\sum_{k=1}^N \al_k - \frac{1}{2} \sum_{k,l=1}^N \al_k\al_l y_ky_l
\scp{x_k}{x_l}
$$
under the constraints $0\leq \al_k\leq \ga$, $\sum_{k=1}^N \al_k y_k =
0$. 

The KKT conditions in this case are $\xi_k(\ga-\al_k) = 0$ and 
$\al_k (y_k(\be_0 + x_k^Tb +\xi_k - 1) = 0$. If one of the $\al_k$ does
not vanish, the last condition provides $\be_0$.  If all
$\al_k$ vanish, this implies first that $\xi_k = 0$ for all $k$ and
that $b = 0$.  But this yields $y_k \be_0 \geq 1$ for all $k$ which is
impossible excepted in the very uninteresting case when there is only
one class present in the training set.

For data (strictly) beyond the margin ($y_k(\be_0 + x_k^T b ) > 1$),
one has $\xi_k=0$ therefore $\al_k=0$. This implies that the $k$th
example $(y_k, x_k)$ does not contribute to the estimation. Those for
which  $y_k(\be_0 + x_k^Tb ) < 1$  force $\xi_k
> 0$ and therefore $\al_k = \ga$. So, $\al_k$ takes values in the open
interval $(0, \ga)$ only for the examples with  $\be_0 + x_k^T b = y_k$
which are two hyperplanes on both sides of the separating hyperplane,
at distance $C  = 1/\|b\|^2$. These vectors therefore are those which
define the margin, and are called the support vectors.








==> ml_preamble_.tex <==
\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\qed{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\squareforqed
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}
\newcommand{\qedtoo}{\qed}

\newcommand{\mA}{{\mathbb A}}
\newcommand{\mB}{{\mathbb B}}
\newcommand{\mS}{{\mathbb S}}
\newcommand{\mT}{{\mathbb T}} 
\newcommand{\mV}{{\mathbb V}}
\newcommand{\mW}{{\mathbb W}}
\newcommand{\defeq}{\stackrel{{\scriptscriptstyle \Delta}}{=}}
\renewcommand{\bfone}{\boldsymbol 1}
\newcommand{\op}{\mathit{op}}
\newcommand{\dom}{\mathit{dom}}
\newcommand{\relint}{\mathit{relint}}
\newcommand{\epi}{\mathit{epi}}
\newcommand{\prox}{\mathit{prox}}
\newcommand{\sign}{\mathit{sign}}
\newcommand{\KL}{\mathit{KL}}
\newcommand{\VC}{\textit{VC-dim}}
\newcommand{\Sdim}{\textit{S-dim}}
\newcommand{\Pdim}[1][]{P_{#1}\textit{-dim}}
\newcommand{\Rad}{\textit{Rad}}
\newcommand{\vol}{\text{vol}}

\newcommand{\vspan}{\mathrm{span}}
\newcommand{\rank}{\mathrm{rank}}



==> newcom_.tex <==
\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\qed{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\squareforqed
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}



\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bquo}{\begin{quote}}
\newcommand{\equo}{\end{quote}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}

\newcommand{\bac}{\backslash}
\newcommand{\nat}{\natural}
\newcommand{\equ}{\equiv}
\newcommand{\lab}{\label}
\newcommand{\emp}{\emptyset}
\newcommand{\prt}{\partial}
\newcommand{\nab}{\nabla}
\newcommand{\grad}{\nabla}
\newcommand{\sub}{\subset}
\newcommand{\setm}{\setminus}
\newcommand{\cir}{\circ}
\newcommand{\ria}{\rightarrow}
\newcommand{\Lfria}{\Leftrightarrow}
\newcommand{\Ria}{\Rightarrow}
\newcommand{\lria}{\longrightarrow}
\newcommand{\lan}{\langle}
\newcommand{\ran}{\rangle}
\newcommand{\demi}{{1\over 2}}
\newcommand{\beg}{\begin}
\newcommand{\bigo}{\bigotimes}
\newcommand{\ti}{\times}
\newcommand{\oti}{\otimes}
%\newcommand{\lsc}{\lan\ }
\newcommand{\rsc}{\ \ran}
\newcommand{\cqfd}{\qed}

\renewcommand{\phi}{\varphi}
\newcommand{\al}{\alpha}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}
\newcommand{\La}{\Lambda}
\newcommand{\la}{\lambda}
\newcommand{\De}{\Delta}
\newcommand{\de}{\delta}
\newcommand{\ep}{\varepsilon}
\newcommand{\eps}{\epsilon}
\newcommand{\ze}{\zeta}
\providecommand{\th}{\theta}
\renewcommand{\th}{\theta}
\newcommand{\Th}{\Theta}
\newcommand{\be}{\beta}
\newcommand{\ga}{\gamma}
\newcommand{\ka}{\kappa}
\newcommand{\Ga}{\Gamma}
\newcommand{\sig}{\sigma}
\newcommand{\Sig}{\Sigma}




\newcommand{\cf}{{\mathcal F}}
\newcommand{\CF}{{\mathcal F}}
\newcommand{\CZ}{{\mathcal Z}}
\newcommand{\CE}{{\mathcal E}}
\newcommand{\CY}{{\mathcal Y}}
\newcommand{\CW}{{\mathcal W}}
\newcommand{\CX}{{\mathcal X}}
\newcommand{\CK}{{\mathcal K}}
\newcommand{\CH}{{\mathcal H}}
\newcommand{\CC}{{\mathcal C}}
\newcommand{\CS}{{\mathcal S}}
\newcommand{\CT}{{\mathcal T}}
\newcommand{\CU}{{\mathcal U}}
\newcommand{\CR}{{\mathcal R}}
\newcommand{\CO}{{\mathcal O}}
\newcommand{\CP}{{\mathcal P}}
\newcommand{\CM}{{\mathcal M}}
\newcommand{\CN}{{\mathcal N}}
\newcommand{\CD}{{\mathcal D}}
\newcommand{\CB}{{\mathcal B}}
\newcommand{\CA}{{\mathcal A}}
\newcommand{\CQ}{{\mathcal Q}}
\newcommand{\CL}{{\mathcal L}}
\newcommand{\CG}{{\mathcal G}}
\newcommand{\CV}{{\mathcal V}}
\newcommand{\CI}{{\mathcal I}}
\newcommand{\CJ}{{\mathcal J}}

\newcommand{\hpi}{{\hat{\pi}}}
\newcommand{\hth}{{\hat{\th}}}
\newcommand{\hnu}{\hat{\nu}}
\newcommand{\hga}{\hat{\ga}}
\newcommand{\hal}{\hat{\al}}
\newcommand{\hbe}{\hat{\be}}
\newcommand{\hphi}{\hat{\phi}}
\newcommand{\heta}{\hat{\eta}}
\newcommand{\htau}{\hat{\tau}}
\newcommand{\hrho}{\hat{\rho}}
\newcommand{\hhrho}{\hat{\hat{\rho}}}
\newcommand{\hep}{\hat{\ep}}
\newcommand{\hb}{\hat{b}}
\newcommand{\hf}{{\hat{f}}}
\newcommand{\hx}{\hat{x}}
\newcommand{\hy}{\hat{y}}
\newcommand{\hX}{\hat{X}}
\newcommand{\hl}{\hat{l}}
\newcommand{\hu}{\hat{u}}
\newcommand{\hv}{\hat{v}}
\newcommand{\hz}{\hat{z}}
\newcommand{\hw}{\hat{w}}
\newcommand{\hW}{{\hat{W}}}
\newcommand{\hE}{\hat{E}}
\newcommand{\hL}{\hat{L}}
\newcommand{\hN}{{\hat{N}}}
\newcommand{\hQ}{\hat{Q}}
\newcommand{\hH}{\hat{H}}
\newcommand{\hK}{\hat{K}}
\newcommand{\hP}{\hat{P}}
\newcommand{\hV}{\hat{V}}


\newcommand{\bth}{\overline{\th}}
\newcommand{\bga}{{\overline{\ga}}}
\newcommand{\bL}{\overline{L}}
\newcommand{\bc}{\overline{c}}
\newcommand{\br}{\overline{r}}
\newcommand{\ba}{\overline{a}}
\newcommand{\bx}{\overline{x}}
\newcommand{\by}{\overline{y}}
\newcommand{\bb}{\overline{b}}
\newcommand{\bh}{\overline{h}}
\newcommand{\bt}{\overline{t}}
\newcommand{\bv}{\overline{v}}
\newcommand{\bw}{\overline{w}}
\newcommand{\bW}{\overline{W}}
\newcommand{\bla}{\overline{\la}}
\newcommand{\bal}{\overline{\al}}
\newcommand{\brho}{\overline{\rho}}
\newcommand{\bz}{{\overline{z}}}
\newcommand{\bze}{{\overline{\zeta}}}
\newcommand{\bT}{{\overline{T}}}
\newcommand{\bB}{{\overline{B}}}
\newcommand{\bre}{{\overline{e}}}
\newcommand{\bmu}{\overline{\mu}}
\newcommand{\bpi}{{\overline{\pi}}}
\newcommand{\bS}{{\overline{S}}}
\newcommand{\bZ}{{\overline{Z}}}
\newcommand{\bY}{{\overline{Y}}}
\newcommand{\bH}{{\overline{H}}}
\newcommand{\bX}{{\overline{X}}}
\newcommand{\bs}{{\overline{s}}}
\newcommand{\bl}{{\overline{l}}}
\newcommand{\bm}{{\overline{m}}}
\newcommand{\Bla}{\overline{\La}}
\newcommand{\bOm}{\overline{\Om}}
\newcommand{\bE}{\overline{E}}
\newcommand{\bC}{\overline{C}}
\newcommand{\bD}{\overline{D}}
\newcommand{\bF}{\overline{F}}
\newcommand{\Bf}{\overline{F}}
\newcommand{\bu}{{\overline{u}}}
\newcommand{\bg}{{\overline{g}}}
\newcommand{\bDe}{{\overline{\De}}}
\newcommand{\bphi}{{\overline{\phi}}}
\newcommand{\bpsi}{{\overline{\psi}}}
\newcommand{\bCS}{\overline{\CS}}

\newcommand{\tla}{{\tilde{\la}}}
\newcommand{\tnu}{{\tilde{\nu}}}
\newcommand{\ttau}{{\tilde{\tau}}}
\newcommand{\tze}{{\tilde{\ze}}}
\newcommand{\tCC}{{\tilde{\CC}}}
\newcommand{\tCE}{{\tilde{\CE}}}
\newcommand{\tCG}{{\tilde{\CG}}}
\newcommand{\tCD}{{\tilde{\CD}}}
\newcommand{\tbfu}{{\tilde{\bfu}}}
\newcommand{\tI}{{\tilde{I}}}
\newcommand{\tS}{{\tilde{S}}}
\newcommand{\tY}{{\tilde{Y}}}
\newcommand{\tq}{{\tilde{q}}}
\newcommand{\tv}{{\tilde{v}}}
\newcommand{\tL}{{\tilde{L}}}
\newcommand{\tE}{{\tilde{E}}}
\newcommand{\tG}{{\tilde{G}}}
\newcommand{\tH}{{\tilde{H}}}
\newcommand{\tZ}{{\tilde{Z}}}
\newcommand{\td}{{\tilde{d}}}
\newcommand{\tb}{{\tilde{b}}}
\newcommand{\tal}{{\tilde{\al}}}
\newcommand{\tka}{{\tilde{\ka}}}
\newcommand{\tth}{{\tilde{\th}}}
\newcommand{\tep}{{\tilde{\ep}}}
\newcommand{\tLa}{{\tilde{\La}}}
\newcommand{\tSig}{{\tilde{\Sig}}}
\newcommand{\tilh}{{\tilde{h}}}
\newcommand{\tX}{{\tilde{X}}}
\newcommand{\tO}{{\tilde{O}}}
\newcommand{\tA}{{\tilde{A}}}
\newcommand{\tJ}{{\tilde{J}}}
\newcommand{\tC}{{\tilde{C}}}
\newcommand{\tM}{{\tilde{M}}}
\newcommand{\tT}{{\tilde{T}}}
\newcommand{\tR}{{\tilde{R}}}
\newcommand{\tB}{{\tilde{B}}}
\newcommand{\tP}{{\tilde{P}}}
\newcommand{\tU}{{\tilde{U}}}
\newcommand{\ta}{{\tilde{a}}}
\newcommand{\tm}{{\tilde{m}}}
\providecommand{\tt}{tt}
\renewcommand{\tt}{{\tilde{t}}}
\newcommand{\tf}{{\tilde{f}}}
\newcommand{\tg}{{\tilde{g}}}
\newcommand{\tl}{{\tilde{l}}}
\newcommand{\tu}{{\tilde{u}}}
\newcommand{\tr}{{\tilde{r}}}
\newcommand{\tp}{{\tilde{p}}}
\newcommand{\tx}{{\tilde{x}}}
\newcommand{\ty}{{\tilde{y}}}
\newcommand{\tz}{{\tilde{z}}}
\providecommand{\ts}{ts}
\renewcommand{\ts}{{\tilde{s}}}
\newcommand{\tbu}{{\tilde{\vec{u}}}}
%\newcommand{\tbu}{{\tilde{\mbox{\bf u}}}}
\newcommand{\tK}{{\tilde{K}}}
\newcommand{\tV}{{\tilde{V}}}
\newcommand{\txi}{{\tilde{\xi}}}
\newcommand{\tphi}{{\tilde{\phi}}}
\newcommand{\tpsi}{{\tilde{\psi}}}
\newcommand{\trho}{{\tilde{\rho}}}
\newcommand{\tmu}{{\tilde{\mu}}}
\newcommand{\tga}{{\tilde{\ga}}}
\newcommand{\tGa}{{\tilde{\Ga}}}
\newcommand{\tDe}{{\tilde{\De}}}


\newcommand{\da}{{\dot{a}}}
\newcommand{\dD}{{\dot{D}}}
\newcommand{\dg}{{\dot{g}}}
\newcommand{\df}{{\dot{f}}}
\providecommand{\dh}{dh}
\renewcommand{\dh}{{\dot{h}}}
\newcommand{\doth}{{\dot{h}}}
\newcommand{\dx}{{\dot{x}}}
\newcommand{\dla}{{\dot{\lambda}}}
\newcommand{\dze}{{\dot{\zeta}}}
\newcommand{\dy}{{\dot{y}}}
\newcommand{\dz}{{\dot{z}}}
\newcommand{\du}{{\dot{u}}}
\newcommand{\dv}{{\dot{v}}}
\newcommand{\dV}{{\dot{V}}}
\newcommand{\dal}{{\dot{\al}}}
\newcommand{\dotp}{{\dot{p}}}
\newcommand{\dq}{{\dot{q}}}
\newcommand{\dr}{{\dot{r}}}
\newcommand{\dm}{{\dot{m}}}
\newcommand{\dtm}{{\dot{\tm}}}
\newcommand{\dR}{{\dot{R}}}
\newcommand{\dX}{{\dot{X}}}
\newcommand{\dY}{{\dot{Y}}}
\newcommand{\dphi}{{\dot{\phi}}}
\newcommand{\dchi}{{\dot{\chi}}}
\newcommand{\dPhi}{{\dot{\Phi}}}
\newcommand{\dpsi}{{\dot{\psi}}}
\newcommand{\dDe}{{\dot{\De}}}
\newcommand{\dxi}{{\dot{\xi}}}
\newcommand{\dtilh}{{\dot{\tilh}}}

\newcommand{\ddx}{{\ddot{x}}}
\newcommand{\ddy}{{\ddot{y}}}
\newcommand{\ddf}{{\ddot{f}}}
\newcommand{\ddg}{{\ddot{g}}}
\newcommand{\ddh}{{\ddot{h}}}
\newcommand{\ddphi}{{\ddot{\phi}}}
\newcommand{\ddchi}{{\ddot{\chi}}}
\newcommand{\ddpsi}{{\ddot{\psi}}}
\newcommand{\ddDe}{{\ddot{\De}}}

\newcommand{\bvar}{\overline{\var}}
\newcommand{\bcov}{\overline{\cov}}


%\def\vecbf#1{\mathchoice{\mbox{\boldmath$\displaystyle\bf#1$}}
%{\mbox{\boldmath$\textstyle\bf#1$}}
%{\mbox{\boldmath$\scriptstyle\bf#1$}}
%{\mbox{\boldmath$\scriptscriptstyle\bf#1$}}}

\def\vecbf#1{\mathchoice{\mbox{\boldmath$\displaystyle#1$}}
{\mbox{\boldmath$\textstyle#1$}}
{\mbox{\boldmath$\scriptstyle#1$}}
{\mbox{\boldmath$\scriptscriptstyle#1$}}}


%\newcommand{\bfu}{{\mbox{\bf u}}}
%\newcommand{\bfacd }{{\mbox{\bf a}}}
\newcommand{\bfx}{{\mathbf{x}}}
\newcommand{\bfz}{{\mathbf{z}}}
\newcommand{\bfu}{{\mathbf{u}}}
\newcommand{\bfv}{{\mathbf{v}}}
\newcommand{\bfw}{{\mathbf{w}}}
\newcommand{\bfc}{{\mathbf{c}}}
\newcommand{\bfa}{{\mathbf{a}}}
\newcommand{\bfh}{{\mathbf{h}}}
\newcommand{\bfj}{{\mathbf{j}}}
\newcommand{\bfk}{{\mathbf{k}}}
\newcommand{\bfr}{{\mathbf{r}}}
\newcommand{\bfg}{{\mathbf{g}}}
\newcommand{\bfo}{{\mathbf{o}}}
\newcommand{\bfm}{{\mathbf{m}}}
\newcommand{\bfF}{{\mathbf{F}}}
\newcommand{\bfP}{{\mathbf{P}}}
\newcommand{\bfL}{{\mathbf{L}}}
\newcommand{\bfT}{{\mathbf{T}}}
\newcommand{\bfD}{{\mathbf{D}}}
\newcommand{\ZZ}{{\mbox{\bf Z}^2}}
\newcommand{\Zd}{{\bf Z}^d}
\newcommand{\bfA}{{\mathbf{A}}}
\newcommand{\bfN}{{\mathbf{N}}}
\newcommand{\RR}{\mbox{\bf R}}
\newcommand{\bfM}{{\mathbf{M}}}
\newcommand{\bfV}{{\mathbf{V}}}
\newcommand{\NO}{{\mathbf{N}}}
%\newcommand{\bfP}{{\mathbf{P}}}
\newcommand{\bfE}{{\mathbf{E}}}
\newcommand{\bfI}{{\mathbf{I}}}
\newcommand{\bfW}{{\mathbf{W}}}
\newcommand{\bfJ}{{\mathbf{J}}}
\newcommand{\bfH}{{\mathbf{H}}}
\newcommand{\bfK}{{\mathbf{K}}}
\newcommand{\bfb}{{\mathbf{b}}}
\newcommand{\bfs}{{\mathbf{s}}}
\newcommand{\bfq}{{\mathbf{q}}}
\newcommand{\bfp}{{\mathbf{p}}}
\newcommand{\bfZ}{{\mathbf{Z}}}
%\newcommand{\bfE}{{\mathbf{E}}}
\newcommand{\bfR}{{\mathbf{R}}}
\newcommand{\bfQ}{{\mathbf{Q}}}
\newcommand{\bfC}{{\mathbf{C}}}
\newcommand{\bfX}{{\mathbf{X}}}
\newcommand{\bfY}{{\mathbf{Y}}}
\newcommand{\bfO}{{\mathbf{O}}}
\newcommand{\bfla}{{\mathbf{\la}}}
\newcommand{\bfphi}{{\mathbf{\phi}}}
\newcommand{\bfeta}{{\mathbf{\eta}}}
\newcommand{\bfTh}{{\mathbf{\Th}}}

\newcommand{\dbfX}{{\dot{\bfX}}}
\newcommand{\dbfY}{{\dot{\bfY}}}
\newcommand{\dbfa}{{\dot{\bfa}}}

\newcommand{\mR}{{\mathds{R}}}
\newcommand{\mN}{{\mathbb{N}}}
\newcommand{\mC}{{\mathbb{C}}}
\newcommand{\mQ}{{\mathbb{Q}}}
\newcommand{\mZ}{{\mathbb{Z}}}
\newcommand{\mZd}{{\mZ}^d}


\newcommand{\diam}{{\mbox{\rm diam}}}
\newcommand{\Id}{{\mathrm{Id}}}
\newcommand{\bfone}{{\mathbb 1}}
\newcommand{\inte}{{\mathrm{int}}}
\newcommand{\cte}{{\mathrm cst}\ }
\newcommand{\id}{{\mathrm{id}}\,}
\newcommand{\var}{\mathrm{var}}
\newcommand{\Var}{\mathrm{\bf Var}}
\newcommand{\cov}{{\mathrm cov}}
\newcommand{\Cov}{{\mathrm Cov}}
\newcommand{\acos}{{\mathrm{acos}}}
\newcommand{\card}{{\mathrm card}}
\newcommand{\Log}{{\mathrm{ln}}}
\newcommand{\real}{{\mathrm real}}
\providecommand{\imag}{{\mathrm imag}}
\renewcommand{\imag}{{\mathrm imag}}
\newcommand{\signe}{{\mathrm{signe}}}
\newcommand{\trace}{{\mathrm{trace}}}
\newcommand{\Hom}{{\mathrm{Hom}}}
\newcommand{\ev}{{\mathrm{ev}}}
\newcommand{\argmin}{{\mathop{\mathrm{argmin}}}}
\newcommand{\argmax}{{\mathop{\mathrm{argmax}}}}
\newcommand{\mdiv}{{\mathrm{div}}}
\newcommand{\mJ}{{\det d}}
\newcommand{\ppi}{{ \pi_a}}
\newcommand{\ppsi}{{\psi_a}}
\newcommand{\pixy}{\pi(xy)}
\newcommand{\dift}{{\frac{\rm d}{{\rm d}t}}}
\newcommand{\difs}{{{\rm d}\over {\rm d}s}}
\newcommand{\ddth}{{\mbox{d}\over \mbox{d}\th}}
\newcommand{\pdth}{{\partial\over \partial\th}}
\newcommand{\pdal}{{\partial\over \partial\al}}
\newcommand{\ddtt}{{{\rm d^2}\over {\rm d}\th^2}}
\newcommand{\dt}{{{\rm d}\over {\rm d}t}}
\newcommand{\ch}{{\mbox{\bf 1}}}
\newcommand{\zz}{{\mbox{\bf Z}}}
%\newcommand{\inte}{\rm int }
\newcommand{\dd}{\rm d}
\newcommand{\trp}[1]{{\,{\vphantom{#1}}^t\!#1}}
\newcommand{\Exp}{{\mathrm{Exp}}}




\newcommand{\vv}{\vskip .3cm}
\newcommand{\hh}{\hskip .5cm}
\newcommand{\vw}{\vskip .6cm}
\newcommand{\intp}[1]{{\left[ \, {#1} \, \right]}}
\newcommand{\scp}[2]{{\left\langle {#1}\, , \, {#2}\right\rangle}}
\newcommand{\lform}[2]{{\left( {#1} |\, {#2}\right)}}
\newcommand{\ang}[2]{{\left\lan\!\left\lan {#1}\, , \, {#2}\right\ran\!\right\ran}}
\newcommand{\der}[2]{\frac{d {#1}}{d{#2}}}
\newcommand{\pder}[2]{\frac{\partial {#1}}{\partial {#2}}}
\newcommand{\dco}[2]{{\nabla_{#2}\left({#1}\right)}}
\newcommand{\mder}[3]{\frac{d^{#1} {#2}}{ d{#3}^{#1}}}
\newcommand{\dder}[2]{\frac{d^2 {#1}}{d{#2}^2}}
\newcommand{\pdr}[2]{\frac{\prt {#1}}{\prt{#2}}}
\newcommand{\ppdr}[2]{\frac{\prt^2 {#1}}{\prt{#2}^2}}
\newcommand{\pddr}[3]{\frac{\prt^2 {#1}}{\prt{#2}\prt{#3}}}
\newcommand{\mdr}[2]{\frac{D {#1}}{D{#2}}}
\newcommand{\dps}{\displaystyle}
\newcommand{\bul}{$\bullet$ }
\newcommand{\cond}[1]{{[\bf {#1}]}}
\newcommand{\defset}[1]{\left\{ #1 \right\}}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\bin}[2]{\left(\begin{array}{c}  #1\\#2\end{array}
\right)}
\newcommand{\rotmat}[1]{\left(\begin{array}{cc}  \cos #1& - \sin
#1\ \\sin #1 & \cos#1\end{array}
\right)}


\newcommand{\map}[5]{\begin{array}{lrcl}#1:& #2&\ria&#3\\&#4&\mapsto&#5\end{array}}
\newcommand{\encadre}[1]{\par\noindent\framebox{\parbox{\textwidth}{#1}}

\medskip}
\newcommand{\todo}[1]{{\textcolor{red}{#1}}}
\newcommand{\dpm}{\displaymath}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% TeX-master: t
%%% End: 


==> reconnaissance.tex <==
\chapter{Groups of diffeomorphismes}
\label{grp.diff}
\section{Introduction}

Shapes, alone or within images, are typically subject to rigid or
non-rigid deformations. In order to compare two of them, or to extract common
features, one typically needs to develop a matching procedure, which
consists in finding a generally one-to-one correspondence between the shapes.

From a formal point of view, we will consider ``objects'' as functions
defined on some set $\Om$ with values in some set $F$.  For example,
parameterized curves will be defined on an interval, with values in
$\mR^2$. An image is defined on a subset of $mR^2$ (or $\mR^3$), with
values in $\mR$. Similar objects will have similar features (corners,
patterns), at similar, but not identical, locations. The matching
problem consists in aligning the objects, which is a one-to-one map
from $\Om$ onto $\Om$ that register the features between the two objects.

To simplify, we will assume that $\Om$ is a bounded subset of $\mR^n$
(although the theory can be extended to unbounded sets). Its boundary
will be denoted  $\prt\Om$, and its closure $\bOm$. Deformable objects
are functions $m: \bOm \mapsto F$, with $F\sub \mR^d$. Matching two
objects $m$ and $\tm$ consists in defining a bijection $g: \bOm\mapsto
\bOm$ wihich is not too far from the identity, and such that
$m\circ g$ is close to $\tm$.

The issue, of course, is to rigorously define these measures of
proximity, between bijections and objects. In this part, are goals are
as follows.

\begin{itemize}
\item Build a group $G$ that contains diffeomorphisms of $\Om$
\item Equip  $G$ with a differential structure that allows for the
composition of infinitesimal elements, like for Lie groups.
\item Equip $G$ with a metric associated to a Riemannian structure
(\ref{geo.diff}) to evaluate the size of deformations.
\end{itemize}
\index{diffeomorphism}

We will not build here a Lie group of diffeomorphism (Lie groups in
infinite dimensions generally are intricate objects; for
diffeomorphisms, they generally require using $C^\infty$
functions). One of the simple way to define a group of diffeomorphisms
is by
$$
G_k = \defset{g: C^k \text{-diffeomorphisme sur } \overline{\Om}, g^{-1} \text{
    de classe } C^k}.
$$
Although this group can be equipped with a structure of complete
metric space
\cite{mic72, df01}, it is not suitable for differential calculs. One
practical way do induce infinitesimal perturbations in $G_k$ is via
the action of flows of differentla equations  (\cite{df01}). But these
flows can be used directly to build new groups of diffeomorphisms,
typically different from  $G_k$ \cite{tro98}. We will follow this
construction here.


As a motivation for the inroduction of flows, let us study the idea of
building diffeomorphisms by composing small deformations. Let a
diffeomorphism near the identity be written as $h(x) = x + \de v(x)$,
$\de$ being an arbitrarily small number. It is not hard to show that
this is a diffeomorphism for $\de \leq \de_0$, $\de_0$ depending on
$\norm{v}_\infty$ and $\norm{Dv}_\infty$. Consider now $n$ such
deformations,  $h_i = \id +\de v_i$,
$i=1, \ldots, n$, and denote $g_n = h_n\circ\cdots\circ h_1$. We have
the formula
$$
g_{n+1} = (\id + \de v_n) \circ g_n = g_n + \de v_n\circ g_n.
$$
Write this under the form
$$
\frac{1}{\de} (g_{n+1} - g_n) = g_n\circ v_n;
$$
for small $\de$, this equation can be interpreted as a time
discretization of an ordinary differential equation of the form
\begin{equation}
\label{flot.1}
\der{\bfg}{t} = \bfv(t, \bfg).
\end{equation}
Here, $\bfv$ is a time dependent vector field on $\Om$. It is the main
ingredient in the construction of groups of diffeomorphism proposed in
 \cite{tro98} (see also
\cite{dgm98}).

\section{Flows of diffeomorphismes}
\index{flows of diffeomorphisms}
\subsection{Construction}

The general principle is to fix a suitable functional space to which
the time-dependent vector field $\bfv$ belongs, and to define the
elements of $H$ to be solutions of  (\ref{flot.1}). It has to be
ensured that, for the considered  $\bfv$, (\ref{flot.1}) has solutions
over all times, and that they form a group. This is the goal of the
following definitions.

Let $L^\infty(\bOm, \mR^n)$ be the set of bounded measurable functions
from $\bOm\sub \mR^n$ to $\mR^n$. Let $C_0^1(\Om,
\mR^n)$ be the set of all $C^1$ vector fields $v$ on  $\bOm$ such that
$v$ and $Dv$ vanish on  $\prt\Om$. We will use the norm, for which
$C_0^1(\Om, \mR^n)$ is a Banach space:
$$\|v\|_{1, \infty} = \|v\|_\infty + \|dv\|_\infty\,.$$

We define the set $\CW$ of trajectories $\bfv: [0, 1] \ria
C_0^{1}(\Om,\mR^n)$ for which
$$
\|\bfv\| := \int_0^1 \|\bfv(t)\|^2_{1, \infty} dt
$$
is finite.
For all $t$, $\bfv(t)$ is a vector field on $\Om$, that we shall also
denote $\bfv(t, .)$. We also let $\CW^\infty$ be the subset of  $\CW$
that contains time-dependent vector fields  $\bfv$ such that $\bfv(t, .)\in
C^\infty(\Om, \mR^n)$ at all times.


For $\bfv\in\CW$, and for $x\in \bOm$, denote $\bfg_{\bfv}(.,
x)$ the solution (if it exists) of the ODE (\ref{flot.1}) with initial
condition $\bfv(0, x) = x$.

\encadre{
\begin{theorem}
\label{flot.exist}
If $\bfv\in\CW$, then, for all $x\in \bOm$, $\bfg_{\bfv}(t, x)$ exists
for all 
$t\in[0,1]$ and is uniquely defined. At all time $t$, the function $x\mapsto
\bfg_\bfv(t, x)$ is a diffeomorphism of $\Om$. Its differential is the
solution of the linear differential equation
\begin{equation}
\label{flot.diff}
\pdr{}{t}d_x\bfg_\bfv(t, .) = d_{\bfg_\bfv(t, x)} \bfv(t,
.).d_x\bfg_\bfv(t, .)
\end{equation}
with initial condition $d_x\bfg_\bfv(0, .) = \Id$. 
\end{theorem}}
\begin{proof}
We first show existence and uniqueness. Fix $t\in [0, 1]$ and $\de
>0$. Let $I = I(t, \de)$ denote the interval
$[0,1]\,\cap\, ]t-\de, t+\de[$. Fix also $x\in\bOm$.

If $\phi$ is a continuous function from $I$ to $\mR^3$ such that 
$\phi(t)=x$, define, for $s\in I$
$$
\Ga(\phi)(s) = x + \int_t^s \bfv(u, \phi(u)) du
$$
The function $\Ga(\phi)$ is also continuous on $I$ and is such that 
$\Ga(\phi)(t) = x$. The set of all such function being a Banach space
for the supremum norm, it suffices to show that $\Ga$ is contractant
for small enough $\de$ to prove the existence of a unique fixed point.

From Schwartz inequality, we have
%\begin{multline}
\begin{equation}
\label{eq:***} \|\Ga(\phi) - \Ga(\psi)\|_\infty \leq
\|\phi-\psi\|_\infty \int_{s\wedge t}^{s\vee t} \|\bfv(u, .)\|_{1,
\infty} du
%\\ 
\leq
\sqrt{|t-s|}\,\|\bfv\|\,\|\phi-\psi\|_\infty.
\end{equation}
%\end{multline}
So its suffices to take  $\de < \|\bfv\|^{-2}$ to ensure that $\Ga$ is
contractant. This shows that a unique solution (given its value at
$t$) of  (\ref{flot.1})
exists on intervals of radius $\de$ around $t$. But we have found that
$\de$ can be chosen uniformly in $t$, which implies that the solution
exists and is unique over all $[0,1]$ (and in fact any time interval),
since one can extend any solution by intervals of radii smaller than
$\de$.

The continuity of  $\bfg_\bfv$ in its initial conditions is a standard
consequence of Gronwall's lemma that we give without proof:
\begin{theorem}[Gronwall's lemma]
\label{th:gronwall}
Assume that $\phi, \psi$ and $w$ and bounded, positive functions on an
interval $[0, c]$, and that
$$
w(t) \leq \phi(t) + \int_0^t \psi(s) w(s) ds.
$$
Then
$$
w(t) \leq \phi(t) + \int_0^t \phi(s)\psi(s) e^{\int_s^t \psi(u)du}ds.
$$
\end{theorem}

 

If $x,
y\in\bOm$, we have
\begin{eqnarray*}
|\bfg_\bfv(t, x) - \bfg_\bfv(t, y)| &=& \left| x-y + \int_0^t
\left(\bfv(s, \bfg_\bfv(s, x)) - \bfv(s, \bfg_\bfv(s,
y))\right)ds\right|\\
&\leq & |x-y| + \int_0^t \|\bfv(s, .)\|_{1, \infty} |\bfg_\bfv(s, x) -
\bfg_\bfv(s, y)| ds\\
&\leq& |x-y| + \sqrt{\int_0^t \|\bfv(s, .)\|^2_{1, \infty}ds \int_0^t |\bfg_\bfv(s, x) -
\bfg_\bfv(s, y)|^2 ds}
\end{eqnarray*}
Letting $M_t = |\bfg_\bfv(s, x) - \bfg_\bfv(s, y)|^2$,
we get
$$
M_t \leq 2|x-y|^2 + 2\|\bfv\|^2 \int_0^t M_s ds
$$
which implies
\begin{equation}
\label{asc.1}
M_t \leq 2|x-y| \exp(2\|\bfv\|^2),
\end{equation}
which proves the continuity of  $\bfg_\bfv$ with respect to $x$.

To show that $\bfg_\bfv(t, .)$ is a homeomorphism (i.e., invertible
with a continuous inverse), it suffices to notice that, for all $t>0$,
the function $\bfw(s, .) = -\bfv(t-s,
.)$ for  $s\in [0, t]$ and $\bfw(s, .) = 0$ pour $s > t$ belongs to
$\CW$, and is such that $\bfg_\bfw(t,.) =
[\bfg_\bfv(t, .) ]^{-1}$. Indeed, define $\bfh : (s, x)\mapsto
\bfg_\bfv(t-s, x)$. We have $bfh(s,x) = bfg_\bfw(s, \bfg_\bfv(t, x))$,
because these two functions are solutions of 
$$
\pdr{\psi}{s}(s,x) = - \bfv(t-s, \psi(s, x))
$$
with initial conditions $\psi(0, x) = \bfg(t, x)$. Therefore, 
$$
\bfg_\bfw(t, \bfg_\bfv(t, x)) = \bfh(1, x) = \bfg_\bfv(0, x) = x$$
which shows that $\bfg_\bfv(t, .)$ is invertible, with a continuous inverse
(since it also comes from an element of $\CW$), hence is a
homeomorphism of $\bOm$.

Let's show now that  $\bfg_\bfv(t, .)$ is a diffeomorphism. Assuming
that this is the case, we can formally compute the differential of the
equation
$$
\pdr{\bfg_\bfv}{t}(t, x+\ep\de) = \bfv(t, \bfg_\bfv(t, x+\ep\de))
$$ at $\ep=0$ and get
$$
\pdr{}{t}d_x\bfg_\bfv(t,.).\de = d_{\bfg_\bfv(t,x)}\bfv(t, .)d_x\bfg_\bfv(t,.).\de.
$$
In view of this,, let's introduce the linear differential equation
$$
\pdr{W}{t} = d_{\bfg_\bfv(t,x)}\bfv(t, .) W
$$
with initial condition $W(0) = \de$. This equation has a unique
solution on any interval (by the same kind of argument used to prove
that \eqref{flot.1} has a unique solution). The previous formal
computation shows that this solution should coincide with
$d_x\bfg_\bfv(t, .).\de$, but this remains to prove.

For this, introduce
$$
a_\ep(t) = \left(\bfg_\bfv(t, x+\ep\de) - \bfg_\bfv(t, x)\right)/\ep -
W_t.
$$
We need to prove that $a_\ep(t)$ tends to 0 when $\ep$ tends to
0. Introduce a modulus of continuity for $d_x\bfv(t, .)$ on
$\Om$, letting
$$
\mu_t(\al) = \max\defset{\abs{d_x\bfv(t, .) - d_y\bfv(t, .)}: x,
  y\in\Om, \abs{x-y} \leq \al}.
$$
Since $d_x\bfv(t, .)$ is uniformly continuous on the compact set 
$\overline{\Om}$, we know that $\mu_t(\al)\to 0$ if $\al\to 0$. We can
have, using the intehral version of the differential equations that
define  $\bfg_\bfv$
and $W$: 
\begin{align*}
a_\ep(t) &= \frac{1}{\ep}\int_0^t \left(\bfv(s, \bfg_\bfv(s, x+\ep\de)) - \bfv(s,
\bfg_\bfv(s, x))\right) ds - \int_0^t   d_{\bfg_\bfv(s,x)}\bfv(s,.) W(s) ds \\
&= \int_0^t d_{\bfg_\bfv(s,x)}\bfv(s,.) a_\ep(s) ds \\
&+
\frac{1}{\ep}\int_0^t \left(\bfv(s, \bfg_\bfv(s, x+\ep\de)) - \bfv(s,
\bfg_\bfv(s, x))\right. \\
&\ \ \ \ \ \ -\left. \ep d_{\bfg_\bfv(s,x)}\bfv(s,.) \left(\bfg_\bfv(s,
x+\ep\de) - \bfg_\bfv(s, x)\right) \right) ds
\end{align*}
Using the fact that, for all $x, y\in\Om$:
$$
\abs{\bfv(t, y) - \bfv(t, x) - d_x\bfv(t, .)(y-x)} \leq \mu_s(\abs{x-y})
\abs{x-y}
$$
and combining this to \eqref{asc.1}, we can write 
$$
\abs{a_\ep(t)} \leq  \int_0^t \norm{\bfv(s, .)}_{1, \infty}
\abs{a_\ep(s)} ds + C(\bfv) \abs{\de} \int_0^1 \mu_s(\ep
C(\bfv)\abs{\de}) ds
$$
for some constant $C(\bfv)$ which only depends on $\bfv$. The
convergence of $a_\ep$ to 0 will be obtained as a consequence of
Gromwall's lemma as soon as we will have proved that 
$$
\lim_{\al \to 0}  \int_0^1 \mu_s(\al)ds = 0.
$$
But this fact is a consequence of the pointwise convergence of $\mu_s$
to 0, of the upper bound $\mu_s(\al) \leq 2 \norm{\bfv}_{1, \infty}$
and of the dominated convergence theorem.
\end{proof}

The inequality (\ref{asc.1}) shows that, if $\CV$ is a bounded subset
of  $\CW$, the family of functions $\bfg_\bfv(t, .)$ for $\bfv\in \CV$
is equicontinuous (i.e., has a common modulus of continuity). The same
tachnique can be used to prove the analogous result for  $\bfg_\bfv(.,
x)$, and therefore for the family $\bfg_\bfv$ of time dependent vector
fileds. Ascoli's theorem therefore implies that the map $\bfv \mapsto
\bfg_\bfv$ is compact from 
$\CW$ to $C^0([0,1]\ti\bOm, \bOm)$ (i.e., carries bounded sets onto
compact sets).

The other fundamental result that can be deduced from the previous
proof is that the image of  $\CW$ by the map $\bfv
\mapsto \bfg_\bfv$ is a subgroup of the group of diffeomorphisms of
$\bOm$. Indeed, the stability by composition is obtained by
concatenating two flows, and the existence of the inverse has been
shown in the proof of theorem
\ref{flot.exist}. We can therefore provide the following definition.
\begin{definition}
\label{g.infty}
We let $G = G(\CW)$ be the group of diffeomorphisms of $\bOm$ defined by
$$
G = \{\bfg_\bfv(1, .), \bfv\in\CW\}
$$
\end{definition}
(There is no loss of generality in restriction to diffeomorphisms at
time 1since $\bfg_{t\bfv}(1, .) = \bfg_\bfv(t,, .)$.)

The group which is defined in this way is consistent with the
intuition of constructing diffeomorphisms by iterating infinitesimal
deformations. This approach also provides a distance on $G$, letting,
for  $g, g'\in G$
$$
d_\CW(g, g')^2 = \inf\defset{\int_0^1 \|\bfv(t, .)\|_{1, \infty}^2
dt: \bfg_\bfv(1, g(x)) \equiv g'(x)\|}
$$

The fact that $d$ is a distance will be proved later in a more general
case. Another important  property of the space  $\CW$ is the behavior
of the solutions of  (\ref{flot.1}) when $\bfv$ weakly converges in
the following sense.

\begin{definition}
\label{weak*}
A sequence $\bfv_n$ in $\CW$ weakly converges to $\bfv\in \CW$ if and
only ifm for all $C^\infty$ function, $\phi:[0,1]\ti\overline{\Om} \ria
\mR$, 
we have 
$$
\int_0^1\int_\Om \phi(t, x) \bfv_n(t, x)dt dx \ria \int_0^1\int_\Om
\phi(t, x) \bfv(t, x)dt dx
$$
\end{definition}

We then have the following theorem
\medskip
\encadre{
\begin{theorem}
\label{weak.closed}
If $\bfv_n$ is a bounded sequence in $\CW$ that weakly converges to
$\bfv^*\in \CW$, then $\bfg_{\bfv_n}$ converges uniformly on $[0,
1]\ti\bOm$ to $\bfg_{\bfv^*}$.
\end{theorem}}

\begin{proof}
The proof here is adapted from \cite{dgm98}. Since we know that $\bfv \mapsto
\bfg_\bfv$ is compact, it suffices to show that any subsequence of
$\bfg_{\bfv_n}$ that converges uniformly also converges to 
$\bfg_{\bfv^*}$. Fix such a subsequence, that will still be denoted
$\bfv_n$, and let  $\bfg$ be its
limit. To show that $\bfg = \bfg_{\bfv^*}$, it suffices to prove that,
for all $t$ and all $x$
$$
\bfg(t, x) = x + \int_0^t \bfv^*(s, \bfg(s, x)) ds.
$$
Since this identity is true for  $\bfg_{\bfv_n}$ (with $\bfv_n$ in
place of  $\bfv^*$), and since $\bfg_{\bfv_n}$ converges uniformly to
$\bfg$, all we have to show is that, for all $t$ and $x$,
$$
\int_0^t [\bfv^*(s, \bfg(s, x)) - \bfv_n(s, \bfg_{\bfv_n}(s, x))] ds
\ria 0.
$$
We have
\begin{multline*}
\left|\int_0^t [\bfv^*(s, \bfg(s, x)) - \bfv_n(s, \bfg_{\bfv_n}(s,
x))] ds\right|
\leq \\
\int_0^t
\left|\bfv_n(s, \bfg(s, x)) - \bfv_n(s, \bfg_{\bfv_n}(s,
x))\right| ds
+ \left|\int_0^t \bfv^*(s, \bfg(s, x)) - \bfv_n(s,
\bfg(s,x)) ds \right|
\end{multline*}
For the first integral, write
\begin{eqnarray*}
\int_0^t
\left|\bfv_n(s, \bfg(s, x)) - \bfv_n(s, \bfg_{\bfv_n}(s,
x))\right| ds &\leq& \int_0^1 \|\bfv_n(t, .)\|_{1, \infty} |\bfg(s, x)
- \bfg_{\bfv_n}(s, x)| ds\\
&\leq& \|\bfg-\bfg_{\bfv_n}\|_\infty \|\bfv_n\|.
\end{eqnarray*}
Since $\|\bfv_n\|$ is bounded and 
$\bfg_{\bfv_n}$ uniformly converges to $\bfg$, this integral converges
to 0. For the second integral, we can use the following lemma:
\begin{lemma}
\label{lemme.weak}
If $\bfv_n$ is bounded in $\CW$ and weakly converges to $\bfv^*$,
then, for all continuous function $\phi: [0, 1]\to \bOm$, we have, for
all
$t\in [0,1]$,
\begin{equation}
\label{eq.weak}
\lim_{n\ria\infty} \int_0^t (\bfv_n(s, \phi(s)) - \bfv^*(s, \phi(s)))
ds  = 0.
\end{equation}
\end{lemma}
Since any continuous function can be uniformly approached by a piecewise
constant function, it suffices to prove this for a piecewise constant
function (we skip the limiting argument here, which can be done like
we have estimated the first integral, using the fact that $\bfv_n$ is
bounded in $\CW$). Moreover,  as piecewise constant
functions, we obviously only need to consider  $\phi$ of the form $\phi(s) =
x.\bfone_A(s)$ where $A= [t_1, t_2]$ is a subinterval of  $[0,
1]$. Writing the associated integral as a difference between an
integral on $[0,
t_1]$ and an integral on $[0, t_2]$, we see that the lemma only needs
to be proved for all $t$ and constant $\phi$. So let's assume that
$\phi(s) = x$ and denote 
$$
Q_n(t, x) = \int_0^t (\bfv_n(s, x) - \bfv^*(s, x)) ds.
$$
Proceding like for equation (\ref{eq:***}), we show that 
$Q_n$ is an equicontinuous family of functions $[0,
1]\ti\bOm$; since $Q_n(0, x) = 0$ for all $x$, Azrela-Ascoli's theorem
implies that this sequence is relatively compact. It therefore
suffices to show that any converging subsequence of  $Q_n$ converges to 0.
Fix such a subsequence, still denoting it  $Q_n$ to save on notation,
and let $Q$ be its limit. Let $f(t, x)$ be a $C^\infty$ function on
$[0, 1]\ti \bOm$. We have 
$$
\int_0^1\int_\Om Q^n(t, x) f(t, x) dt dx = \int_0^1 \int_\Om
(\bfv_n(s, x) - \bfv^*(s, x)) \left(\int_s^1 f(t, x) dt\right)ds dx.
$$
From the weak convergence of  $\bfv_n$, the right-hand term tends to
0. Since  $Q_n$ converges uniformly to $Q$, we have
$$
\int_0^1\int_\Om Q(t, x) f(t, x) dt dx = 0
$$ 
for all $C^\infty$ $f$, which implies the desired result.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Extension}
\label{ext.diff}

The group $G$ in the previous section has been built using vector
fields in the space $\CW = C^{1}_0(\Om, \mR^n)$. Clearly, all the properties
that have been shown above remain valid in this space is replaced by a
smaller Banach spaces (i.e., that can be continuously embedded in
it). Following  \cite{tro98}, we introduce the definition
\encadre{
\begin{definition}
\label{adm}
A Banach space $\CB\subset L^2(\Om, \mR^n)$, with norm $\|.\|_\CB$,
is admissible if and only if $C^\infty_0(\Om, \mR^n)$ is dense in
$\CB$ and there exists a constant $K > 0$ such that, for all
$v\in C^\infty_0(\Om, \mR^n)$, we have
$$
\|v\|_{1, \infty} \leq K\|v\|_\CB
$$
\end{definition}}

All the results that precede remain true if the norm $\|\,.\,\|_{1,
\infty}$ is replaced by $\|\,.\,\|_\CB$. One can therefore build a
group $G(\CB) \sub G(\CW)$ and a new distance  $d_\CB$ on $G(\CB)$
defined by
$$
d_\CB(g, g')^2 = \inf\defset{ \int_0^1 \|\bfv(t, .)\|_\CB^2 dt:
\bfv(1, g(x)) \equiv g'(x)\|}
$$

Using Sobolev inclusions \cite{ada75,bre83}, $\CB$ can be chosen to be
some $W^{m, p}_0(\Om)$, which contains functions for which all partial
derivatives of order lower or equal to  $m$ belong to $L^p$ (the
subscript 0 means null boundary conditions). Whithin these spaces, the
easier to use (both in theory and practice) are the Hilbert spaces
$W_0^{m,2}$, that can be equipped with the norm
$$
\|v\|_m^2 = \sum_{|\al| = m} \int_\Om
\left(\frac{d^mv}{dx_1^{\al_1}\ldots dx_n^{\al_n}}\right)^2 dx
$$
the sum being over all multi-indices $(\al_1, \ldots,
\al_n)$ such that $|\al| = \al_1 + \cdots+ \al_n = m$. The smallest
$m$ that makes this norm admissible depends on the dimension. One can
take $m=2$ in dimension 1, $m=3$ in dimension 2
and 3.

In the last case, the space $L^2([0,1], \CB)$ also is a Hilbert space,
with norm
$$
\|\bfv\|_{2, \CB}^2 = \int_0^1 \|\bfv(t, .)\|^2 dt
$$
and
$$
d_\CB(g, g') = \inf\{ \|\bfv(., .)\|_{2, \CB}: \bfg_\bfv(1,g(x)) \equiv g'(x)\}
$$

For Hilbert spaces, bounded sets are weakly relatively compact, and
the norm is lower semi-continuous. This implies that, if 
$\bfv_n$ is a mminimizing sequence for the distance  $d_\CB$, that is
if  $\|\bfv_n\|\ria
d_\CB(g, g')$ and for all $n$, $\bfg_{\bfv_n}(1,g(x)) \equiv
g'(x)$, then there exists a sub-sequence of  $\bfv_n$ that weakly converges
in $L^2([0,1], \CB)$ to some $\bfv^*\in\CB$ such that
$\|\bfv^*\| \leq d_\CB(g, g')$. One can prove that weak convergence
for the Hilbert structure is a stronger condition than the one given
in definition
\ref{weak*}; from theorem \ref{weak.closed}, we get the fact $\bfg_{\bfv^*}(1,g(x)) \equiv
g'(x)$. This implies that $d_\CB(g, g') = \|\bfv^*\|$: $\bfv^*$
provides an optimal matching trajectory between $g$ and $g'$. The
existence of such an optimal trajectory is very important in practice,
since, as we will see later, it is closely related to the issue of
aligning deformable objects.


\chapter{Estimation of Diffeomorphisms}
\label{est.diff}
\section{Introduction}
In the previous chapters, we have already noticed the importance of
performing a correct registration betwee deformable objects.
Such a registration can formally be interpreted as estimating a
diffeomorphism between the compared objects.

This chapter provides several algorithms that achieve this task. It is
organized as follows. We first provide a list of measures that
evaluate the ``size'' of a diffeomorphism. These definitions will
provide essential components for matching techniques, which will be
presented in the second part of the chapter.


\section{Quantitative Evaluation of Diffeomorphisms}
\label{size}
\subsection{Definitions}
We first introduce some notation. We let $\Om$ be a bounded open set
in $\mR^d$. We will consider a group $G$ of
diffeomorphisms (like one of those proposed in the previous chapter)

This group acts on {\em deformable structures} that will correspond to
shapes or other visiaull objects. For example, one can define the
action on configurations of points and on images as follows

\medskip
\encadre{
\begin{definition}
\label{action}
If $\bfx = (x_1, \ldots, x_N) \in
\Om^N$, and $g\in G$, we let
$$
g.\bfx = (g(x_1), \ldots, g(x_N))
$$
If $I$ is an image defined on $\Om$ and $g\in G$, we define $g.I$ by
$$
g.I(x) = I \circ g^{-1}(x)
$$
\end{definition}
}
\medskip

It is easy to check that these define actions. Let us do it for
images, since the case of landmarks is really straightforward. We want
to prove $g.(h.I) = (g\circ h).I$. But the former is $g.(I\circ
h^{-1}) = I \circ h^{-1} \circ g^{-1} = I \circ (g\circ h)^{-1} =
(g\circ h).I$. We will study these actions (and some other) in more
detail in the next chapter. For now, our goal is to quantify the size
of an element $g$ in $G$, by a quantity denoted $E(g)$, which will
measure, in some way, how $g$ differs from the identity mapping. The
idea, in order to quantify the variation of deformable
objects, will be to use this measure to evaluate the amount of
distorsion that is required to align them.

\subsection{Standard norms on functions}
One approach, to evaluate the signe of $g\in G$, is to define $u = g-
\id$ and use one of the numerous norms provided by functional analysis
to measure $u$. We cannot provide a complete outlook of these norms
here, but present some important families of examples.

We first start with norms of Sobolev type, that is, involving the
$L^p$ norms of some derivatives of $u$. The simplest example, say in
dimension 1, is to let
$$
E(g)=\int_\Om (g_x-1)^2 dx\,
$$
with some suitable boundary condition (e.g. $u=0$ at the extrimities
of $\Om$.

More generally, we can take, this time in any dimension
$$
E(g) = \|u\|_L^2 = \scp{Lu}{u}_2 = \int_\Om \scp{Lu(x)}{u(x)} dx\,.
$$
where $L$ is an operator defined on a space $\CH_L\subset \CL^2(\Om,
\mR^n)$, with the assumption that $\scp{Lu}{u} \geq c \norm{u}_2^2$,
for some $c>0$
($L$ said to be strictly monotonous). One of the advatages of this
last assumption is that it allows one to complete $\CH_L$, equipped
with $\|.\|_L$, into a
Hilbert space embedded in $L^2$ (this is the Friedrich extension,
cf. \cite{zei95}). One simple choice is to take $L = (\al - \Delta)^k$
for some $k>0$. For such norms, Sobolev inclusion theorem are
typically used to control the smoothness properties of elements of $\CH_L$.


\bigskip
One can also build a norm using an orthonormal basis of  $\CL^2(\Om,
\mR^k)$, that we shall denote $(f_1, \ldots, f_n, \ldots)$. Any $u$ in
$L^2(\Om, \mR^k)$ can be decomposed under the form
$$
u = \sum_k u_k f_k
$$
with
$$
u_k = \int_\Om u(x) f_k(x) dx.
$$
Letting $c = (c_1, \ldots, c_k, \ldots)$ be a sequence of positive numbers,
we can set
$$
\|u\|_c^2 = \sum_{k=1}^\infty c_k u_k^2\,.
$$

When the $c_k$'s are bounded, this will converge for all $u\in
\CL^2(\Om, \mR^k)$. But this is not the interesting situation; when
the $c_k$'s tend to infinity, the set $H_c$ that contains all $u$'s such
that $\|u\|_c$ is bounded is a strict subspace of $L^2(\Om, \mR^k)$,
which forms a Hilbert space when equipped with $\|.\|_c$. In this case,
for an image $u$ to belong to $H_c$, its high order coefficient must
tend to 0 faster than they would have had under the usual $L^2$
constraint which requires that the sum of squares of the $u_k$
converge. Because orthonormal bases of $L^2(\Om, \mR^k)$ are usually
ordered so that high order coefficients analyze high frequencies of
the function, a function in $H_c$ will generally be a smooth
function. For several bases (like Fourier, wavelets), the smoothness
of $u$ can be deduced from the rate of convergence of its coefficients
to 0   \cite{mey92}. 


There is another advantage in using such a decomposition, which comes
from the fact that it
provides a graded representation of the function. By truncating this
decomposition, one can obtain a good approximation of $u$. When
solving an optimization problem involving $u$, it becomes easy to
start clamping high order coefficients to zero, and progressively
release them during the procedure. This provides a coarse-to-fine
algorithm that is often computationally efficient, and also
potentially avoids being trapped in early local minima. One of the
problems with this representation, however, is that the evaluation of
$u$ at a point $x\in \Om$ can sometime be expensive, since it requires
summing the series that decomposes $u$. Fast transform exits, however,
for this purpose, on the most popular orthonormal bases (Fourier, wavelets).


\bigskip
These two points of view are equivalent when the basis $(f_k)$
diagonalizes the operator $L$. In such a case, letting
$L f_k = c_k f_k$, we have
$$
\int_\Om |Lu|^2 = \sum_{k=1}^\infty c_k u_k^2.
$$
Such a decomposition has been used to optimize deformations, for
example in
 \cite{ap91, dss96, ass98}, \cite{tro98}.


\subsection{Hyperelastic models}

\index{hyperelasticity}
The theory of elasticity uses a few ``universal'' principles,
like material indifference, or isotropy to derive general constraints
on the evaluation of the deformation that is applied on an object. To
these principles, that remain valid for many shape recognition
problems, one adds the constraint the the elastic energy only depens
on the first derivative of the deformation. Such constraints naturally
lead to the definition of a hyperelastic material; if   $g$ is a
diffeomorphism defined on  $\Om$, its associated deformation energy
must take the form 
$$
E(g) = \int_\Om W(x, C) dx
$$
where $C = {}^tDg.Dg$ is called the Cauchy stress tensor. For a
homogeneous material, $W$ does not depend on $x$. If the material is
also isotropic, $W$ only depends on the eigenvalues of $C$ (the
singular values of $Dg$). In this case, designing $W$ is simply
designing a function of $d$ variables (where $d$ is the dimension).

There are several classical definitions of such models. The simplest
nonlinear model is for  Saint-Venant Kirchhoff materials, for which (leting $E =
(C- I)/2$)
$$
W(C) = \frac{\la}{2} \left[\trace(E) \right]^2 + \mu \trace
\left(E^2\right).
$$
Here, $\la$ and $\mu$ are called the {\em Lam\'e} coefficients of the material (cf.
\cite{rwcm95}).

Most often, one uses the linearized version of this energy. If $g =
\id + u$ and $u$ is small, the approximation  $E
\simeq (du + {}^t du)/2$ can be made. Replacing $u$ by this
approximation yields an energy which is quadratic in $u$ and linear
Euler equations. An interesting matching algorithm based on this model
is presented in  \cite{ric02}.

One of the issues with Saint-Venant Kirchhoff materials is that their
energy does not penalize small eigenvalues of the tensor. This may
lead to singularities, and non-diffeomorphic solutions in large
deformation matching problems. To avoid this, one needs to penalize
small determinants of $C$. For example  \cite{hgygm99}, one can use
(in 2D) 
\begin{equation}
\label{elas.ax}
W(C) = W(\al, \be) = (\al^2+\be^2) (1+(\al\be)^{-2})
\end{equation}
$\al$ and $\be$ being the eigenvalues of $C$.

\subsection{Geodesic energies}
\label{viscous}
In chapter \ref{grp.diff}, we have considered diffeomorphisms $h$ for
which there exist solutions $\bfv$  of the boundary value problem
\begin{equation}
\label{ode}
\der{\bfg}{t}(t, .) = \bfv(t, g(t, .))
\end{equation}
with conditions $\bfg(0, .) = \id$ and $\bfg(1, .) = h$,
where $\bfv$ is a time dependent vector field such that
$$
\Ga(\bfv) := \int_0^1 \|\bfv(t,.)\|^2 dt < \infty,
$$
with the admissibility condition on $\|\bfv(t,.)\|$, as described in
section \ref{ext.diff}, chapter \ref{grp.diff}.

When they exist, the solutions $\bfv$ associated to a given $h$ are
not unique. It is natural to let the size of $h$ be the minimum of
$\Ga(\bfv)$ over all such $\bfv$; more precisely, letting $\CV_h$ be
the set of all time-dependent vector fields  $t\mapsto \bfv(t, .)$ on
$\Om$ such that the solution of the ordinary differential equation
$$
\der{y}{t} = \bfv(t, y)
$$
with initial condition $y(0) = x$ satisfies, for all $x$,  $y(1) =
h(x)$. We define
$$
E(h) = \inf_{\bfv\in \CV_h}\int_0^1 \|\bfv(t)\|^2 dt
$$

This may seem a rather awkward way to define the size of $h$. In
particular, defining it as an optimization problem may be
computationally inefficient. Also, for a given $h$, it is generally
difficult to decide whether  $\CV_h\neq \emp$, and even harder to
describe its elements.

This point of view, however, has several advantages. First, the
description of $\CV_h$ can be avoided by parameterizing the problem
dircetly in terms of  $\bfv$: instead of looking for the smallest $h$
achieving a given matching problem, one would look for the smallest
$\bfv$ such that the solution of the ODE at time  1 solves the
same matching problem. les mêmes contraintes. There is a numerical
cost, however, since this add a new dimension (time) to the
problem. But the additional complexity if balanced by the simplicity
of the cost function expressed in terms of $\bfv$. The continuous time
deformation
process (flow) that is obtained by integrating $\bfv$ also has some
interest, since it can provide smooth continuous evolution of one
initial deformable object to another
(cf. \cite{lv98}).

Anther advantage (that we will check later) is that the minimized cost
function can be interpreted as a metric distance (between the identity
and the function  $h$) on the group $G$. This diatance can in turn
induce distances between deformable objects. Symmetry and especially
triangular inequality are much harder to obtain with elastic
formulations.


\section{Landmark matching interpolation}

We start our review of specific matching problems with what is in fcat
an interpolation issue. In this setting, a certain number of point
correspondences are given, and the goal is to extrapolate them to a
global diffeomorphism on $\Om$. Unsurprisingly, the relevant methods
in this framework will borrow largely from the theory of interpolating
splines.

As before, $\Om$ is the support of the  configurations. We assume that
two sets of landmarks $(x_1, \ldots,
x_N)$ and $(y_1,
\ldots, y_N)$, bothe belonging to $\Om^N$. Our goal is to find a
diffeomorphism $g$ on $\Om$, with minimal size (as defined in the
previous section), such that, for all  $i$, $g(x_i) = y_i$ ({\em exact
  interpolation}), or,  $g(x_i) \simeq y_i$ ({\em inexact
  interpolation}). The last situation will be implemented using
penalities on the difference within an optimization problem.
Before providing a solution of these problems, we need to present some
required results for spline theory.
\index{splines}

\subsection{Splines} 

From an abstract point of view, spline approximation can be seen as
the application of the following very simple algebraic problem.
Let $\CH$ be a Hilbert space, and assume that $f_1, \ldots, f_N\in
\CH$, and $c_1, \ldots, c_N\in \mR$ are given. We introduce two
variational problems:
\begin{itemize}
\item[1.] Minimize $\|h\|$ over $h\in \CH$, under the constraints that
$\scp{f_i}{h}  = c_i$ for $i=1, \ldots, N$.
\item[2.] For a parameter $\la > 0$,  minimize $\|h\|^2 + \la \sum_{i=1}^N
(\scp{f_i}{h} - c_i)^2$
\end{itemize}
The two problems will respectively correspond to exact and inexact
interpolation.
The constraints, case 1., and the penalty in case 2., are not affected
when $h$ is replaced by $h+v$ and $v$ is othogonal to the finite
dimensional vector space generated by $f_1, \ldots, f_N$.

Introduce the $N$ by $N$ matrix $S$ with $S_{ij} =
\scp{f_i}{f_j}$. Acording to the discussion above, we can look for $h$ under the form
$$
h =\sum_{i=1}^N \al_i f_i,$$
for which $\|h\|^2 = \trp{\al} S \al$. 

Consider problem 1. We need to minimize $\trp{\al} S \al$ under the
constraints  $S\al = c$ ($\al$ and $c$ being vectors with coordinates
$\al_i$ and $c_i$). Assume that $S$ is invertible: then, the only
solution satisfying the constraints is $\al = S^{-1} c$ and there is
no minimization issue. When $S$ is not invertible, we must assume that
$c$ belongs to the renge of $S$, otherwise the problem will have no
solution. This implies that $c = S \al_0$ for some $\al_0$, and any
solution $\al$ must take the form $\al= \al_0 + \be$ with $\be \in
\text{ker}(S)$. But, for any such solution, we have $\trp{\al} S \al
= \trp{\al_0} S \al_0$ so that any $\al$ is a valid minimizer.

The fact that $S$ is not invertible is equivalent to the existence of
a non-vanishing $\be$ such that $\trp{\be} S \be = 0$, which can be
rewritten as $\|\sum_{i=1}^N \be_i f_i\|^2 = 0$. In other terms, $S$
is not invertible if and only if $f_1, \ldots, f_N$ are linearly
dependent. The solution $\al$ is this case is thus defined up
to
$\be$'s for which $\sum_{i=1}^N \be_i f_i=0$  which is  
obvious since adding such a linear combination does not change the
value of $h$.

Consider now problem 2. We need to minimize
$$\trp{\al} S \al + \la \trp{(S\al - c)}(S\al - c)$$
with respect to $\al$. This is a convex function of $\al$ and its
gradient is $S((\la S + I)\al - \la c)$. If $S$ is invertible, the
unique solution is $\al = S_\la c$ with $S_\la = S + I/\la$. In the
general case, it takes the form $S_\la^{-1}(c + \be)$ with $S\be = 0$.
Note that in this case, a solution always exists.
\bigskip

We now make the connection with spline interpolation. The goal here is
to find a smooth real-valued function $h$ à valeurs réelle, defined on
$\Om$, such that  $h(x_i) = c_i$ (or
$h(x_i)\simeq c_i$) for some $x_i\in\Om$ and
$c_i\in\mR$. The smoothness of $h$ is measured by a Hilbert space
norm, for example
$$
\|h\|^2_L = \int_\Om \scp{Lh}{h}^2 dx
$$
where is is a strictly monotonous operator. We let $\CH_L$ be the
corresponding Hilbert space.

We can educe the linear constraints  $h(x_i) = c_i$ to those in the
abstract problem provided there exists, for each  $x_i$, an element
$f_{x_i}$ in $\CH_L$ such that, for all $h\in \CH_L$
$$
h(x_i) = \scp{f_{x_i}}{h}_L.
$$
By the Riesz representation theorem, this is equivalent to the fact
that the evaluation functional $h \mapsto h(x)$ is continuous for the
Hilbert structure. Spaces that satisfy this property for every $x$ are
called {\em reproducing kernel Hilbert spaces} (RKHS). The fact that a
space $\CH_L$ as above is a RKHS can typically be proed by invoking a
Sobolev inclusion theorem. We will henceforth assume that this is the
case, and therefore obtain the existence, for each $x$, of a function
$f_x\in \CH_L$ with, for all $h\in\CH_L$, $
h(x) = \scp{f_{x}}{h}_L.$ 

It can be noted that, taking $h=f_y$ in the previous formula yields 
$f_y(x) = \scp{f_{x}}{f_y}_L = f_x(y).$ The function of two variables
$(x,y) \mapsto K(x,y) = f_x(y)$ is the kernel of the space $\CH_L$,
which therefore satisfies the eproducing identity
$$
K(x,y) = \scp{K(x,.)}{K(y,.)}_L.
$$

Returning to our interpolation problem, we see that the constraints
now are  $\scp{f_{x_i}}{h}_L = c_i$ with $f_{x_i} = K(x_i, .)$ which
places us directly in the abstract situation we have studied. We
therefore obtain solutions $h$ of the form
$$
h(.) = \sum_{i=1}^N \al_i K(., x_i).
$$
The matrix $S$ being formed with the dot products of the $f_{x_i}$'s
is there the matrix with coefficients $S_{ij} = K(x_i, x_j)$, which
yields explicit formulas to compute $\al$ when $K$ is known.

\medskip

The availability of an explicit expression for $K$ is therefore an
essential practical requirement. When $L$ is a differential operator, there are very few situations in
which this kernel (which is also called the Green kernel of the
operator $L$) is computable. They generally are limited to cases for
which $L$ is some polynomial of the Laplacian, and to specific
boundary conditions on $\Om$ (or at infinity if $\Om$ is not bounded).
An important case of affine conditions at infinity provides thin-plate
splines, and will be presented in section \ref{bookstein}. For
operators of the form $(a - \Delta)^n$, the kernel can be computed via
the evaluation of Bessel functions. Explicit expressions for $L = -
\nabla ^n$ on rectangular domains with zero
boundary conditions is also available.

I one does not restrict to differential operators, however, there is
an explicit way to proceed, which consists in directly defining the
kernel $K$, provided one can prove that a valid $L$ exists without
necessarily having to compute it. Note that for the practical use of
the spline problem,
only $K$ is needed, not $L$.

Suficient conditions for $K$ can be taken as follows.
\begin{itemize}
\item Symmetry: $f_x(y) = f_y(x)$
\item $K$ is continuous and, for all $x\in\Om $
$$
\int_\Om K(x,y)^2 dy < \infty
$$
\item $K$ induces a positie operator on  $\CL^2$: for all $u\in \CL^2$
$$\int_\Om u(x) u(y) f_x(y) dx dy \geq 0.$$
\end{itemize}
One simple way to ensure the last condition is to take $K(x,y) =
F(x-y)$ where 
$F$ is the Fourier transform of an even, positive function; $K$ is, in
this case, a convolution kernel.

One can also restrict to radial kernels, which take the form $K(x,y) =
G(|x-y|)$ (\cite{ar95}, \cite{adry94}). For such a kernel to be valid
in every dimension, one can show that  $q(t)
= G(\sqrt{t})$
must be the Laplace transform of a meaure $\mu$ on $\mR^+$:
$$
q(t) = \int_0^{+\infty} e^{-\la u} d\mu(\la)\,.
$$
When $\mu$ is a Dirac measure, we obtain the important example of a
Gaussian kernel given by
$$
G(t) = \exp\left(-\frac{t^2}{\sig^2}\right).
$$
For more details, we refer to \cite{dyn89} and references therein.
\index{Gaussian kernel}



\subsection{Diffeomorphic interpolation}

\label{par:splines}
\subsubsection{Generalities}

We now extend spline theory to our diffeomorphic interpolation: extend
to $\Om$ a correspondence $x_i \to y_i, i=1, \ldots, N$. One important
remark, in this context, is that the interpolation to e computed is a
function from $\Om$ to $\Om$ and not from $\Om$ to $\mR$ as before. We
will therefore have to deal with several components. 


Before addressing the corespondence problem, we first start
with a direct generalization of the prevous section, in which we
consider a Hilbert space $\CH$ of smooth vector fields on $\Om$ and the
issue is to find a function $h$ in $\CH$ subject to
the constraints $h(x_i)= v_i$ for $x_1, \ldots, x_N\in\Om$ and $v_1,
\ldots, v_N \in\mR^d$. We will assume as before that the evaluation
function $h\mapsto h(x)$ is continuous.

The difference with the previous problem therefore is that the
function $h$ takes vector values, so that the function $h\to h(x)$ is
not a linear form anymore. Clearly, one can consider coordinate
functions and apply the previous theory. More generally, one can
associate to any vector $a\in \mR^d$ and any $x\in\Om$ the linear form
$\de_x^a: h \mapsto a^T h(x)$. By Riesz representation theorem, there
exists a vector field $f_x^a\in \CH$ such that $\scp{f_x^a}{h} = a^T
h(x)$ for all $h\in H$. Since $\de_x^a$ is linear in
$a$, the same property is true for $f_x^a$. Fixing $x,y\in \Om$, we
therefore obtain the fact that $a \mapsto f_x^a(y)$ in linear from
$\mR^d$ to $\mR^d$. It can therefore be put under the form
$f_x^a(y) = K(y, x)a$ where $K(y, x)$ is a $d$ by $d$ matrix. The
matrix-valued function $K$, defined on $\Om^2$, if the reproducing
kernel of the space $\CH$. It is characterized by the property that,
for all $h\in \CH$, for all $x\in\Om$ and $a \in \mR^d$:
$$
a^Th(x) = \scp{K(x,.)a}{h}_V.
$$
This implies in particular that, for all $x$ and $a$, $K(., x) a \in
\CH$. Moreover, we can write, for all $x,y\in\Om$, for all
$a,b\in\mR^d$:
$$
\scp{K(., x)a}{K(., y)b}_\CH = a^T K(x,y) b
$$
which is the $d$-dimensional reproducing property of the kernel
$K$. This implies in particular the symmetry property: $K(x,y) =
K(y,x)^T$ for all $x,y\in\Om$.

Returning to our interpolation problem, each constraint $h(x_i) = v_i$
is equivalent to $e_k^T h(x_i) = v_{ik}$ for $k=1, \ldots, d$, where
$e_1, \ldots, e_d$ is the canonical basis of $\mR^d$ and $v_i =
(v_{i1}, \ldots, v_{id})$ is the decomposition of $v_i$ in this
basis. Since $e_k^T h(x_i) = \scp{K(., x_i)e_k}{h}_\CH$, we are reduced
to our previous abstract problem, this time with $d N$ constraints
instead of $N$. We obtain, in particular the fact that an optimal
solution for the exact and inexact interpolation problems can be
written under the form, for some real numbers $\al_{ik}$,
$$
h(.) = \sum_{i=1}^N \sum_{k=1}^d \al_{ik} K(., x_i) e_k
$$
which can also be expressed as (letting $al_i = (\al_{i1}, \ldots, \al_{id})^T\in\mR^d$)
$$
h(.) = \sum_{i=1}^N K(., x_i) \al_i.
$$

The solution of the exact matching problem now can be obtained by
solving the linear system
$h(x_j) = \sum_{i=1}^N K(x_j, x_i) \al_i$. Introducing the $dN$ by
$dN$ matrix $S$, organized in $d$ by $d$ blocs, with $i, j$ bloc given
by $K(x_i, x_j)$, and assuming that $S$ is invertible, the solution if
the the system is
$$
\begin{pmatrix} \al_1\\ \vdots \\ \al_N\end{pmatrix} = S^{-1}
\begin{pmatrix} h(x_1)\\ \vdots \\ h(x_N)\end{pmatrix}.
$$

The solution of the inexact matching problem, namely minimize
$$
\|h\|_{\CH} + \la \sum_{i=1}^N |h(x_i) -  v_i|^2
$$
is given by the same expression with $S$ replaced by $S_\la  = S +
\Id/\la$. 

The systems above becomes simpler uneder the assumption, which is
widely made in practice, that the kernel is diagonal, i.e.,
$K(x,y) = k(x,y) \Id$ with $k(x,y)\in\mR$. In this case, the previous
solution can be reordered as
$$
\begin{pmatrix} \al_{11} \ldots \al_{1d} \\ \vdots \\ \al_{N1} \ldots
\al_{Nd} \end{pmatrix} = \tilde S^{-1}
\begin{pmatrix} h_1(x_1)\ldots h_d(x_1) \\ \vdots \\ h_1(x_N)\ldots
h_d(x_N) \end{pmatrix}
$$
where $\tilde S_{ij}  = k(x_i,x_k)$ is a $N$ by $N$ matrix. This
reduces the issue of solving a $dN$-dimensional system to solving $d$
$N$-dimensional systems, which is much less expensive.

\subsubsection{Invariance of the inner-product}

We haven't discussed so far under which criteria the dot product (or
the operator $L$) should be selected. One important criterion, in
particular for shape recognition is equivariance or invariance with
respect to rigid transformations. We here consider the situation $\Om
= \mR^d$.

Our first requirement is as follows. Let $x_1, \ldots, x_N$ be the
landmarks, and $v_1, \ldots, v_N$ the vectors. We want the obtained
interpolation $h$ to be invariant by an orthogonal change of
coordinates. This means that, if $A$ is a rotation and $b\in\mR^d$, and if we consider the problem associated
to the landmarks $Ax_1+b, \ldots. Ax_N+b$ and the constraints $Av_1,
\ldots, Av_N$, the obtained function $h^{A,b}$ must satisfy
$h^{A,b}(Ax+b) = A h(x)$ or $h^{A,b}(x) = A h (A^{-1}x - A^{-1} b) := ((A,b)\star h)(x) $.
The transformation $h \to (A,b)\star h$ is an action of the group of
translations-rotations on functions defined on $\Om$. To ensure that
$h^{A,b}$ always satisfies this condition, it is sufficient to enforce
that the norm is invariant by this transformation: $\|(A,b)\star h\|_\CH  = \|h\|_\CH$.

So, we need the action of translation and rotations to be an isometry
in $\CH$. Assume that $\|h\|_\CH^2 = \lform{Lh}{h}$ for some operator
$L$, and define the operator $A*L$ the fact that, for all $h, \tilde h\in
\CH$ 
$$
\lform{L((A,b)\star h)}{(A,b)\star \tilde h} = \lform{((A,b)\star L) h}{\tilde h}
$$
so that, the invariance condition becomes expressed in terms of $L$:
$(A,b)\star L  = L$. 

Denoting $h_k$ the $k$th coordinate of $h$, and
$(Lh)_k$ the $k$th coordinate of $Lh$, we can write the matrix
operator $L$ under the form
$$
(Lh)_k  = \sum_{l=1}^d L_{kl} h_l
$$
where $L_{kl}$ is a scalar operator.  We first consider the case when
eack $L_{kl}$ is a pseudo-differential operator in the sense that, for
any $C^\infty$ scalar function $u$, the Fourier transform of $L_{kl} u$ takes the
form, for $\xi\in\mR^d$:
$$
\hat{L_{kl} u} (\xi) = f_{kl}(\xi) \hat u(\xi) 
$$
for some scalar function $f_{kl}$. An interesting case is when
$f_{kl}$ is a polynomial, which corresponds, from standard properties
of the Fourier transform, to $L_{kl}$ being a differential
operator. Also, by the isometric property of Fourier transforms,
\begin{eqnarray*}
\lform{Lh}{h} &=& \sum_{k=1}^d \lform{(Lh)_k}{h_k} \\
&=& \sum_{k, l=1}^d \lform{L_{kl} h_l}{h_k} \\
&=& \sum_{k, l=1}^d \lform{\hat{(L_{kl} h_l)}}{\hat h_k} \\
&=& \sum_{k, l=1}^d \lform{f_{kl} \hat h_l}{\hat h_k}.
\end{eqnarray*}
Note that since we want $L$ to be a positive operator, we need the
matrix $f(\xi) = (f_{kl}(\xi))$ to be a complex, positive, Hermitian
matrix. Moreover, since we want $\lform{Lh}{h} \geq c \lform{h}{h}$
for some $c>0$, it is natural to enforce that the smallest eigenvalue
of $f(\xi)$ is uniformly bounded from below (by $c$). 

To use this expression, we need to compute $\hat{(A,b)\star h}$ in
function of $\hat h$. We have
\begin{eqnarray*}
\hat{(A,b)\star h}(\xi) &=& \int_{\mR^d} e^{-i\xi^T x} (A,b)\star h(x)
dx\\
&=& \int_{\mR^d} e^{-i\xi^T x} Ah(A^{-1} x - A^{-1} b)
dx\\
&=& \int_{\mR^d} e^{-i\xi^T (Ay+b) } Ah(y) dy\\
&=& e^{-i\xi^T b}A h(A^T \xi)
\end{eqnarray*}
where we have used the fact that $\det A = 1$ (since $A$ is a rotation
matrix) in the change of variable. We can therefore write, denoting
$\phi_b$ the function $\xi \mapsto \exp(-i\xi^T b)$
\begin{eqnarray*}
\lform{L(A\star h)}{A\star h} &=& \sum_{k, l=1}^d \sum_{k', l'=1}^d
\lform{\phi_b f_{kl} a_{ll'} \hat h_{l'} \circ A^T}{\phi_b a_{kk'} \hat
h_{k'}\circ A^T}\\
&=& \sum_{k, l=1}^d \sum_{k', l'=1}^d
\lform{ f_{kl} \circ A  a_{ll'} \hat h_{l'}}{a_{kk'} \hat
h_{k'}}.
\end{eqnarray*}
We have used the fact that $\det A = 1$ and that $A^T = A^{-1}$. The
function $\phi_b$ cancels in the complex product:
$$
\lform{u}{v} = \int_{\mR^d} u \bar v d\xi
$$
where $\bar v$ is the complex conjugate of $v$.

Reodering the last equation, we obtain 
$$
\lform{L(A\star h)}{A\star h} = \sum_{k', l'=1}^d
\lform{ \sum_{k, l=1}^d a_{kk'} f_{kl} \circ A  a_{ll'} \hat h_{l'}}{ \hat
h_{k'}}
$$
which yields our invariance condition in terms of the $f_{kl}$: for
all $k,l$
$$
f_{kl} = \sum_{k', l'=1}^d a_{k'k} f_{k'l'} \circ A  a_{l'l}
$$
or representing $f$ as a hermitian matrix $A^T f(A\xi) A = f(\xi)$ for all $\xi$ and
all rotation matrix $A$. 

Consider first the case $\xi=0$. The identity $A^Tf(0) A = f(0)$ for
all $A$ implies, by a standard linear algebra theorem, that $f(0) =
\la \Id$ for some $\la \in \mR$.  
We now fix $\xi\neq 0$, and let $\eta_1 = \xi/|\xi|$. Extend $\eta_1$
into an orthonormal basis, $(\eta_1, \ldots, \eta_d)$ and let $(e_1,
\ldots, e_d)$ be the canonical basis of $\mR^d$. Define $A_0$ by $A_0
\eta_i = e_i$ so that $A_0\xi = |\xi| e_1$ and
$f(\xi) = A_0^T f(|\xi| e_1) A_0 = M_0$. Now, for any  rotation $A$ that
leaves $eta_1$ invariant, we also have
$f(\xi) = A^T A_0^T f(|\xi| e_1) A_0 A$ since $A_0 A\eta_1 =
e_1$. This yield the fact that, for any $A$ such that $A \eta_1  =
\eta_1$, we have $A^T M_0 A = M_0$.

This property implies, in particular that $A^T M_0\eta_1 = M_0 \eta_1$
for all $A$ such that $A\eta_1 = \eta_1$. Taking a decomposition of
$M_0\eta_1$ on $\eta_1$ and $\eta_1^\perp$, it is easy to see that
this implies that $M_0 \eta_1 = \al \eta_1$ for some $\al$. So
$\eta_1$ is an eigenvector of $M_0$, which implies that $\eta^\perp$
is closed by the action of $M_0$. But the fact that $A^T M_0 A  = M_0$
for any rotation $A$ of $\eta_1^\perp$ implies that $M_0$ restricted
to $\eta_1\perp$ is a homothetie, i.e., that there exists $\la$ such
that $M_0\eta_i = \la \eta_1$ for
$i\geq 2$. 

Using the decomposition $u= \scp{u}{\eta_1} \eta_1 + u -
\scp{u}{\eta_1} \eta_1$, we can write
$$
M_0u= \al \scp{u}{\eta_1} \eta_1 + \la (u -
\scp{u}{\eta_1} \eta_1) = ((\al-\la) \eta_1 \eta^T  + \la \Id) u
$$
which finally yields the fact that (letting $\mu = \al- \la$ and using
the fact that the eigenvalues of $M_0 = A^T f_0(\|xi\| e_1) A$ are the
same as those of $f_0(|\xi|e_1)$ and therefore only depend on $|\xi|$) 
$$
f(\xi) = \mu(|\xi|) \frac{\xi\xi^T}{|\xi|^2} + \la(|\xi|)\Id.
$$
Note that, since we know that $f(0) = \la\Id$, we must have $\mu(0) =
0$.

Let's first consider the case $\mu = 0$: in this case, we have $f_{kl}
= 0 $ if $k\neq l$ and $f_{kk} (\xi) = \la(|\xi|)$ for all $k$, which
implies that $L_{kl} = 0$ for $k\neq l$ and all $L_{kk}$ are equal to
a fixed scalar operator $L_0$, i.e.,
$$
Lh = (L_0h_1, \ldots, L_0 h_d).
$$

This is the type of operators which is mostly used in practice. If one
wants $L_0$ to be a differential operator, $\la(|\xi|)$ must be a
polynomial in the coefficients of $\xi$, which is only possible  if it
tales the form
$$
\la(|\xi|) = \sum_{i=0}^p \la_p |\xi\|^{2p}
$$
in which case the corresponding operator is $L_0 u = \sum_{i=0}^p
(-1)^p \Delta^p u$. For example, if $\la(|\xi|) = (\al + 
|\xi|^2)^2$, we get $L_0 = (\al I - \Delta)^2$. 

Let's consider an example of valid differential operator with $\mu\neq
0$, and take $\mu(|\xi|) = \al |\xi\|^2$ and $\la$ as above. This
yields the operator 
$$L_{kl} u  =  - \al   \frac{\prt^2 u}{\prt x_k\prt x_l} + \de_{kl} \sum_{i=0}^p
(-1)^p \Delta^p u$$
so that
$$
Lh = - \al \nabla \text{div} h + (\sum_{i=0}^p
(-1)^p \Delta^p )h.
$$

\bigskip

The Kernel (or Green function) associated to an operator associated to
a given $f$ can be computed simply in the Fourier domain. It is indeed
given by
$$
\hat{K_{kl} u} (\xi) = g_{kl}(\xi) \hat u(\xi) 
$$
with $g= f^{-1}$ (the matrix inverse), as can be checked by a simple
computation. Note that, for the spline application, we need $K\de_x^a$
to be well defined. The $k$th component of $\de_x^a$ being $a_k
\de_x$, we can write $\hat {(\de_x^a)_k} (\xi) = a_k \exp(-i\xi^T x)$
so that
$$
\hat{(K\de_x^a)_k} = \sum_{l=1}^d g_{kl}(\xi) a_l \exp(-i\xi^T x).
$$
A sufficient condition for this to provide a well-defined function is
that all $g_{kl}$ are integrable , in which case
$$
(K\de_x^a(y))_k = \sum_{l=1}^d \tilde g_{kl}(y-x) a_l
$$ 
where $\tilde g$ is the inverse Fourier transform of $g$.
In the case $f = \la \Id + \mu \eta \eta ^T$, we have 
$$
f^{-1} = \frac{1}{\la} (\Id - \frac{\mu}{\la + \mu} \eta \eta^T).
$$

Let $\rho(\xi) = 1/\la(|\xi|)$ and $\psi(\xi) = \mu(\xi) / (\la(\xi)
|\xi|^2 (\la(\xi) +
\mu(\xi)))$, so that
$f^{-1}(\xi) = \rho(|\xi|) \Id - \psi(|\xi|) |\xi|^2 \eta
\eta^T$. The eigenvalues of $f^{-1}$ therefore are $\rho(\xi)$ and
$\rho(\xi) - \psi(\xi) |\xi|^2$. Since the eigenvalues of $f$ must be
bounded from below by $c$, we obtain the following constraints on
$\rho$ and $\psi$:
$$ |\xi|^2 \max(\psi, 0) \leq \rho \leq c. $$ 

We can moreover obtain the expression of the Kernel in terms of the
inverse Fourier transforms of $\rho$ and $\psi$, which is:
$$
K(x,y)_{kl} = \tilde g_{kl}(x-y) = \de_{kl} \tilde \rho (x-y) + \pddr{\tilde\psi}{x_k}{x_l}(x-y).
$$

The inverse Fourier transform of a radial function is a radial
function. We have in fact
\begin{eqnarray*}
\tilde\rho(x) &=& \int_{\mR^d} \rho(|\xi|) e^{i\xi^T x} d\xi \\
&=& \int_0^\infty \rho(t) t^{d-1} \int_{S^{d-1}} e^{i\eta^T t x}
ds(\eta) \\
&=& \int_0^\infty \rho(t) t^{d-1} \int_{S^{d-1}} e^{i\eta_1 t |x|}
ds(\eta) 
\end{eqnarray*}
where $S^{d-1}$ is the unit sphere in $\mR^d$, and the last identity
comes from the fact that the integral is invariant by roration of $x$,
which allows us to replace $x$ by $|x|$. The last integral can in trun
be expressed in terms of the Bessel function $J_{d/2}$ (\cite{so97}),
which will not be used here.

There therfore exists two functions $\ga_1$ and $\ga_2$ such that
$\rho(x) = \ga_1(|x|^2)$ and $\psi(x) = \ga_2(|x|^2)$ and the
expression for $K$ becomes
$$
K(x,y) = (\ga_1(|x-y|^2) + 2 \ga'_2(|x-y|^2)) I + 2\ga''_2(|x-y|^2) (x-y)(x-y)^T.
$$

Again, the choice $\ga_2 = 0$ is commonly made in practice, yielding
diagonal radial kernels \cite{dyn89}.
\index{radial kernels}



\subsection{Thin plate interpolation}
\label{bookstein}
\index{Thin plates}

Thin plate theory corresponds to the situation in which the operator
$L$ is some power of the Laplacian. As a tool for shape analysis, it
is been originally described by  Bookstein
\cite{boo91}. Consider the following bilinear form
\begin{equation}
\label{lapl}
\scp{f}{g}= \int_{\mR^2} \Delta f \Delta g dx\,.
\end{equation}

We need to define it on a Hilbert space which is somewhat
unusual. We consider the space $\CH_1$ of all functions in $\mR^d$ with
square integrable second derivatives, which have a bounded gradient at
infinity. In this space, $\|f\| = 0$ is equivalent to the fact that $f$
is affine, i.e., $f(x) = a^Tx + b$, for some $a\in \mR^d$ and
$b\in\mR$. The Hilbert space we consider is the space of $f\in \CH$
modulo the affine functions, i.e., the set of equivalent classes
$$
[f] = \defset{g: g(x) = f(x) + a^T x + b, a\in\mR^d, b\in\mR}.
$$ 
For $f\in\CH_1$. Obviously the norm associated to \eqref{lapl} is
constant over $[f]$ and $\|f\| = 0$ if and only if $[f] = [0]$ so that

This space also has a kernel, although the analysis has to be
different from what we have done previously, since the evaluation
functional is not defined on $\CH$ (functions are only known up to the
addition of an affine term). However, the following is true 
\cite{mei79}. Let $ U(r) = (1/8\pi) r^2\log r$ if the dimension, $d$, is 2, and
$U(r) = (1/16\pi) r^3$ for $d=3$. Then, for all $u\in\CH_1$, there
exists $a_u\in\mR^d$ and $b_u\in\mR$ such that 
$$
u(x) = \int_{\mR^2} U(|x-y|) \Delta^2 u(y) dy + a_u^Tx + b_u.
$$
We wil denote $U_x$ the function $y\mapsto U(|x-y|)$.

Fix, as in the previous section, landmarks $x_1, \ldots, x_N$ and
function values  $(c_1, \ldots,
c_N)$. Again, the constraint $h(x_i) = c_i$ has no meaning in $\CH$,
but the constraint  $\scp{U_{x_i}}{h}_\CH = c_i$ does, and means
$$
h(x_i) + a_h^Tx_i + b_h = c_i,
$$
i.e., $h$  satisfies the constraints un to an affine term.

Denote, as before
$S_{ij} =  U(|x_i-x_j|).$
The function $h$ which is optiml under the constraints
$\scp{U_{x_i}}{h}_\CH = c_i, i=1, \ldots N$ will therfore take the form
$$
h(x) = \sum_{i=1}^N\al_i U(|x-x_i|) + a^Tx + b.
$$
The corresponding interpolation problem is: minimize $\|h\|$ under the
constraint that there exists $a,b$ such that $h(x_i) + a_h^Tx_i + b_h
= c_i, i=1, \ldots, N$.The inexact matching problem simply consists in
minimizing
$$
\|h\|^2_\CH + \la \sum_{i=1}^N (h(x_i) + a^Tx_i + b - c_i)^2
$$
with respect to $h$ {\em and} $a,b$. 

Replacing $h$ by its expression in terms of the $\al$'s, $a$ and $b$
yields the finite dimensional problem: minimize
$$\al^T S \al$$
under the constraint  $S\al + Q\ga = c $ with $\ga = (a_1, \ldots, a_d,
b)^T$ (with size $d+1 \ti 1$) and $Q$, with size $N\ti d+1$ given by
(letting $x_i = (x_i^1, \ldots, x^d_i)$):
$$
Q = \left(\begin{matrix}
x_1^1& \cdots & x_1^d&1\\
\vdots&\vdots&\vdots\\
x_N^1&\cdots & x_N^d&1
    \end{matrix}\right).
$$
The optimal   $(\al, \ga)$ can be computed by identifying the gradient
to 0. One obtains
$$
\hat{\gamma} = \left(Q^T S^{-1}Q\right)^{-1} Q^T S^{-1}c
$$
et
$\hat{\al} = S^{-1}(c - Q\hat{\ga})$.

For the inexact matching problem, one minimizes
$$\al^T S \al + \la{}(S\al + {}^tax_i + b - c)^T(S\al + {}^tax_i + b
- c)\,,$$
and the solution is provided by the same formulae, simply replacing
$S$ by $S_\la = S + (1/\la)I$.

When the function $h$ (and the $c_i$) take $d$-dimensional values
(e.g., correspond to displacements), the above computation has to be
applied to each coordinate, which simply corresponds to using a
diagonal operator, each component equal to $\Delta^2$, in the
definition of the dot product.

The figure \ref{book.ex} provides an example of such an 
interpolation, togother with an interpolation with radial functions (\cite{ar95}).
\begin{figure}
\begin{center}
\includegraphics[width=4cm]{TUTORIALPS/one.ps}\ \
\includegraphics[width=4cm]{TUTORIALPS/two.ps}\\
\includegraphics[width=4cm]{TUTORIALPS/onetotwo.ps}\ \
\includegraphics[width=4cm]{TUTORIALPS/twotoone.ps}\\
\includegraphics[width=4cm]{TUTORIALPS/onetotwoG.ps}\ \
\includegraphics[width=4cm]{TUTORIALPS/twotooneG.ps}\\
\end{center}
\caption{\label{book.ex} Exact landmark interpolation. First Row:
landmaks placed on original images; Second Row: thin-plate
interpolation, form the first image to the second and vice-versa;
Third Row: interpolation using radial functions, with $K(x, y) = log(|x-y|^2 + c)$
(images take from the olivetti face database).}
\end{figure}

\medskip


When thin-plate spline methods (or the spline interpolation methods)
are applied to displacement field, there is no constraing that
guarantees that the obtained function, $\id + h$ is a
diffeomorphism. It is indeed not rare to observe folds in the
obtained solution. The following section describe a solution to
diffeomorphic interpolation.


\subsection{Diffeomorphic interpolation}
\label{joshi}

The distance we have defined on groups of diffeomorphisms (chapter
\ref{grp.diff}) can be used to interpolate landmark correspondences
\cite{jos97}. In this framework we introduce a time-dependent velocity
field on $\Om$, denoted   $t\mapsto v(t, .)$, and the ODE
$$
\der{y}{t} = \bfv(t, y)
$$
Let $\bfg_\bfv(t, x)$ be the solution of this equation at time $t$
with initial condition $\bfg_\bfv(0, x) = x$. The exact matching
problem consists in finding 
$\bfv$ to minimize
$$
E(\bfv) = \int_0^1 |\bfv(t)|^2_{\CH} dt
$$
under the constraints 
 $\bfg_\bfv(1, x_i) = y_i$ for $i=1, \ldots, N$.

Introduce the time dependent displacements, at each landmark, given by
$u_i(t) = \bfg_\bfv(t, x_i) $; these trajectories are unknown,
but once they are obtained, $\bfv$ can be reconstructed in a simple
way. Indeed, let's fix  $u_i(t), i=1, \ldots N, t\in[0, 1]$. First
notice that we have
$$
\der{}{t} u_i(t) = \bfv(t, u_i(t))
$$
so that specifying the $u_i$'s also specifies the values of 
$\bfv(t,  .)$ at $u_i(t)$ (it is in fact equivalent, when
combined with the initial condition $u_i(0) = x_i$). The remaining
problem therefore boils down to: minimize $E(\bfv)$ under the
constraints that $\bfv(t, u_i(t)) = \prt u_i /\prt t$. This
problem can be solved separately for each time, 
 i.e., minimize, for all $t$, $\|\bfv(t)\|_{\CH}$ under the
constraints. This is exactly the kind of problem that have been solved
in the previous sections. Let $(x,y) \mapsto K_x(y) =
K(x,y) $ be the reproducing kernel for $\CH$. Let $S(\bfu(t))$ be the bloc
matrix composed with $s_{ij}(t) = K(u_i(t),
x_j+u_j(t))$, we have, stacking the $u_i$ in a coloumn vertor $\bfu$,
$$
\bfv(t, x) = \sum_{i=1}^N  K_{u_i(t)}(x) \al_i(t)
$$
with $\al(t) = S(\bfu(t))^{-1} \der{\bfu}{t}$.
Again, when $K$ is diagonal, the computation can be split in $d$ $N$
dimensional systems.

Using this we obtained a residual energy which only depends on the
evolution of the $Nd$-dimensional vector $\bfu$:
 L'énergie obtenue est
$$
E(\bfv) = E(\bfu) = \int_0^1 {}^t\der{\bfu}{t} S(\bfu(t))^{-1} \der{\bfu}{t} dt
$$
which needs to be minimized with constraints $u_i(0) = x_i$ and
$u_i(1) = y_i$. Several algorithms have been proposed for this purpose
\cite{jos97,
vmty04, aty05} and we refer the reader to these references for
implementation details. It is quite easy to come up with examples in
which the spline approach fails whereas the diffeomorphic
interpolation provides a smooth diffeomorphism
(Fig. \ref{fig:splines}).

\begin{figure}
\begin{center}
\includegraphics[width=0.4\textwidth]{FIGURES/init.eps}
\includegraphics[width=0.4\textwidth]{FIGURES/final0.eps} \\
\includegraphics[width=0.4\textwidth]{FIGURES/final.eps}
\includegraphics[width=0.4\textwidth]{FIGURES/trajectories.eps}
\caption{\label{fig:splines} Comparison between linear and
diffeomorphic landmark interpolation. First Row: Initial landmarks and
their displacements (Left); Deformation obtained by linear splines
(Right). Second Row: Deformation obtained by diffeomorphic inexact
matching, using the method proposed in \cite{aty05} (Left); Optimal
trajectories ($u_i(t)$) provided by diffeomorphic inexact landmark
matching.}
\end{center}
\end{figure}


\section{Matching Unlabelled Points}

\subsection{The assignment problem}

\subsection{Assignment combined with thin plates}

\subsection{Measure matching}

\section{Matching Images}

Matching images is somewhat different from matching sets of points that we
have considered so far. The matching procedure is not driven here by
the information of which point or set is matched to another, but by
the fact that some numerical quantity (a signature) is transported by
the deformation. This signature can be gray values for scalar images,
but can also, as we shall see, have other interpretation.

We will consider, here again, a bounded open subset $\Om \sub \mR^d$,
and images $I$ will be scalar or vector-valued functions $f:\Om\to
\mR^k$. If a deformation $g$ acts on $\Om$, each points $x$ is
transformed into $g(x)$. If the value of the function has moved with
$x$, we will therefore retrieve the value $I(x)$ at location $y =g(x)$
on the deformed image, $I'$. We therefore have $I'(g(x)) = I(x)$ or $I' =
I\circ g^{-1}$.

The transformation $I \mapsto I\circ g^{-1}$ represent the action of
the diffeomorphism $g$ on functions defined on $\Om$. The matching
problem in this case can be formulated as: given $I$ and $I'$, find a
diffeomorphism $g$, as ``small'' as possible, such that $I\circ g{-1}$
is similar to $I'$.
 

\subsection{Variational approaches}

Starting with \cite{bb82}, a very large number of algorithms have been
based on variational formulations. In this framework, one looks for
the minimum of
\begin{equation}
\label{eq:var.U}
U(g) = S(g) + \lambda D(I\circ g^{-1}, I')
\end{equation}
where $\lambda$ is a est un parameter, $S(g)$ measures the size of the
diffeomorphism (like in section \ref{size}) and
$D$ is some metric that evaluates the difference between $I\circ g^{-1}$ and
$I'$, for example
$$
D(I\circ g^{-1}, I') = \int_\Om \left|I\circ g^{-1} - I'\right|^2 dx
$$


\subsubsection{1D matching}

\nocite{ma97, pj87, pd95, sc78, gmk88, ggcv95}

One of the first situations in which these techniques have been
applied is for speech processing. If two acoustic signals are recorded
during a certain time, they need to be synchronized before safely
compariung them. Although current methods use a probabilistic approach
for this problem (with hidded Markov models), earlier attemps have
modeled distorsions due to variations in speech speed by a
diffeomorphism acting on the time variable. a  signal $I$ becoming
$I\circ g^{-1}$. The dynamic time warping technique has been
introduced for this purpose \cite{sc78}. It can be summarized as
follows. Assume that the signals are discretized, denoting  $I = (I_1,
\ldots, I_N)$ and $I' = (I'_1, \ldots, I'_{N'})$. The original algorithm
minimizes a function of the form 
$$
\De(I,I') = \sum_{k=1}^N d(I_k, I'_{\psi(k)})
$$
where $\psi(k)$ is the intex of the point which is homologous to
$I_k$ in $I'$. This term is the direct analogue of the second term in
\eqref{eq:var.U}. The smoothness penalty in \eqref{eq:var.U} is
replaced in DTW by a hard constraint on the differences  $\psi(k+1)
- \psi(k)$. The minimization is performed by dynamic programming
(which accounts for the D in DTW). Dynamic programming algorithms will
be described in appendix \ref{prog.dyn}.

DTW in general does not incorporate a diffeomorphic constraint. An
interesting contribution that accounts for this can be found in
\cite{pst98}. There two continuous signals $I$ and $I'$ are matched by
minimizing 
$$
U(g) = \arccos\left[\int_0^1 \sqrt{{g}_x} dx\right] + \la
\int_0^1(I(g^{-1}(x)) - I'(x))^2 dx.
$$
The unusual smoothness term is in fact, as we shall see later, a
geodesic distance on a particular group of diffeomorphisms.

One dimensional matching has direct implications for shape comparison,
when the compared shapes are paremetrized (say by arc-length). Indeed,
they are, in this case, functions from some interval to $\mR^2$, and
therefore belong in the very general class of images we are
considering here. The only issue is that curves withe different
lengths are defined ion different intervals, but this can be addressed
by rescaling all curves to have length 1, with is justifed since it provides
a scale invariant matching. Two curves $I,I': [0,1] \to \mR^2$ can then be matched by
minimizing 
$$
\De(I, I') = S(g) + \la \int_0^1 |I'(t) - I\circ g(t)|^2 dt,
$$
although most of the applications in shape comparison prefer working
with invariant signatures of the curve (like the curvature) rather
than curves as $R^2$-valued functions.

There is an extra complication to this framework when working with
shapes, because they are generally represented as closed curves. This
creates an undeterminacy in the arc-length representation, which comes
from the choice of the origin of the parameterization (the point for
which $s=0$). In most cases, this choice is arbitrary, so that a valid
matching procedure must also ensure that the origins in both curves
are chosen consistently, inducing an extra variable on which the
quality of the correspondence must be optimized. From a mathematical
point of view, this extra variable can be taken into account by
assuming that parameterizations are defined on the unit circle rather
than the unit interval. Modeling $g$ as a diffeomorphism of the unit
circle incorporates the change of origin. Unfortunately, this
variation has very little use for practical algorithms, because the
very efficient dynamic programming implementation require knowing the
origins which is therefore estimated separately (or via an exhaustive search). 


\subsubsection*{Examples}
\begin{itemize}
\item A generic method for matching plane curves would apply
\eqref{eq:var.U} to a geometric representation of the curve. For
example, assuming that all curves are defined on $[0,1]$, $I(s)$ can
be the Euclidean curvature of the curve (which is rotation and
translation invariant) or the angle of the tangent with the horizontal
(which is scale and translation invariant), or any other signature,
being given that the fewer derivatives the signature involves, the
more robust the method is likely to be. A typical energy in this
context can be
$$
U(g) = \int_0^1 |g_x|^2 dx + \la \int_0^1 (I \circ g^{-1}(x) - I'(x))
dx.
$$

\item A variant of this formulation \cite{cas92} can be given as
follows. Let $I$ and $J$ be parameterized with arc-length, $I$ having
length 1 and  $J$ length $\al$. Matching is searched as a bijection
$g: [0,\al]\to [0,1]$, that minimizes
$$
U(g) = \int_0^\al (\ka_I(g^{-1}(s)) - \ka_J(s))^2 ds + \la \int_0^\al
\left|\der{}{s}(I(g^{-1}(s)) - J)\right|^2 ds
$$
where $\ka_I$ and $\ka_J$ are the curvatures of $I$ an $J$.

Let's
rewite this energy in a form which is closer to the variatioal problem
we have been discussing. Introduce the unit tangents
 $T_I$ and $T_J$, and expand the second integral which becomes,
letting $h=g^{-1}$ and using the fact that $I$ and $J$ are
parameterinzed with arc-length,
$$
\al + \int_0^\al {h}_s^2 ds - 2\int_0^\al {h}_s
\scp{T_J}{T_I\circ h}(s) ds
$$
If $(s'\mapsto J(s'))$ is reparameterized by $s'\mapsto s'/\al$, and if
$\tilde h(s) = h(\al s)$, the previous formula becomes
$$
\al + \al^{-1}\int_0^1 \tilde h_s^2 ds - 2 \int_0^1 {\tilde h}_s
\scp{T_J}{T_I\circ \tilde h}(s) ds
$$
which is 
$$
\al + \al^{-1}\int_0^1 \tilde h_s^2 ds - 2 \int_0^1 
\scp{T_J\circ \tilde h^{-1}}{T_I}(s) ds.
$$
This can finally be rewritten as 
$$
\al  - 2 + \al^{-1}\int_0^1 \tilde h_s^2 ds + \int_0^1
|T_J \circ \tilde h^{-1} - T_I|^2 ds.
$$
Going back to the initial energy, we have to minimize
\begin{eqnarray*}
\tilde U(\tilde h) &=&  \la \al^{-1}\int_0^1 \tilde h_s^2 ds +
\int_0^\al (\ka_I(\tilde h(s/\al)) -
\ka_J)^2 ds \\
&+& \la \int_0^1
|T_J \circ \tilde h^{-1} - T_I|^2 ds.
\end{eqnarray*}
The first term is an elastic deformation energy for $\tilde h$. The
last two compare the curvature and unit tangents at homologous points.
 \nocite{ggcv95}

\item Some curve-matching energy have been proposed on an axiomatic
basis. The problem with such approaches is that different choices of
axioms lead to different forms of energy, so that they cannot be
expected to provide a universal answer, but nonetheless define
interesting families of matching problems.

One of these approaches \cite{bcgj95} let to constraints for which a
typical energy is
$$
U(g) = \int_0^1 |g_s - 1| ds + \la \int_0^1 (g_s + 1) |f(\ka_I\circ g) -
f(\ka_J)|ds
$$
with $f(\ka) = c\ka - \text{sign}(\ka) e^{-\al \ka}$. Another choice is
$$
U(g) = \int_0^1 |g_s - 1| ds + \la \int_0^1 |g_s \ka_I\circ g  - \ka_J|ds
$$

In \cite{ty00}, another set of axioms has been used, leading to
energies of the kind
$$
U(g) = \int_0^1 \sqrt{\dg} F(I, I'\circ g^{-1}) ds.
$$
Here, $U$ must be maximized in $g$; $F$ must be a symmetric, positive
function and satisfy the condition
$$
F(u, v) \leq \sqrt{F(u, u) F(v, v)}.
$$

\item One particular instance of the energy $U$ in \cite{ty00} is \cite{you98}
$$
U(g) = \frac{ \sqrt{2}}{2} \int_0^1
\sqrt{\dg\left(1 + \scp{T_I\circ g}{T_J}\right)}ds
$$
We will give later a justification of this energy in terms of
distances between plane curves.



\item Energies similar to \eqref{eq:var.U} can also be devised for 3D
curves. A simple choice  \cite{bgkm00} is to use the intrinsic
representation of section \ref{sec:3D.curve}, chapter \ref{surfaces}
and minimize, $I$ and $J$ being two curves with curvature $\ka_I$ and
$\ka_J$ and torsion $\tau_I$ and $\tau_J$, the energy
$$
U(g) = \int_0^1 g_s ds + \int_0^1 \big((\ka_I\circ g^{-1} - \ka_J)^2 +
(\tau_I\circ g^{-1} - \tau_J)^2\big)ds.
$$
\end{itemize}

Most of the energies described above can be minimized, in a very
efficient way, by dynamic programming (once a choice of the origins
has been made for closed curves). More details can be found in
appendix \ref{prog.dyn}.


\subsubsection{Matching higher dimensional images}

The main problem, when passing to high dimensional images (high
starting at 2 here) is of numerical nature. Feasible problem in 1D can
be challenging in 2D and simply impossible in 3D. Solving such
problems require either large scale computational power, or some
efforts in devising suitable simplifications and approximations.

Let us first review some specific domains of application of image matching.

\subsubsection*{Optical flow and stereo-vision}
These two old problems in image processing involve in one way or
another the use of a matching procedure.

For motion estimation, a displacement field  $u$ (the optical flow)
must be estimated between two consecutive images  $I$ and $I'$, in
order that $I(x-u) \simeq
I'(x)$. There is a very rich literature on this subject, which is one
of the most important problems in image processing. We will not try to
provide an exhaustive account of the methods, which fall outside the
scope of this book anyway \cite{fp02}.

A large variety of variational approaches used for optical flow,
however, are variants of the one initially introduced by Horn and
Schunk  \cite{hs81}, in which one minimizes the energy  (with $g = \id - u$),
\begin{equation}
\label{hs.en}
U(g) = \int_{\Om} \al^2 |u(x)|^2du +  \int_{\Om} |I(g(x)) -
I'(x)|^2 dx.
\end{equation}
Most of the time, the second term is lenearized in a neighborhood of
$u=0$ and replaced by
$$
I(x) - I'(x) - \nabla I(x).u(x)
$$

In stereo vision \cite{msks03}, matching two images that have been
simultaneously acquired by two cameras allows one to compute a depth
map within the matched parts of the two images. Compared to the
optical flow, there is an additional constraint (called epipolar)
which ensures that homologous points belong to specific lines which
only depend on the relative position of the cameras and their internal
geometry. 


\subsubsection*{Face comparison}
\nocite{bhk97} 

Deformation also plays an important role in the analysis of facial
images. One can list three main factors for the variation of face images
of a single person: illumination, position and expression. We focus on
the latter than can be represented as a diffeomorphism (for a complete
theory including the three factors, we refer to 
\cite{hgygm99}).

Although using non-rigid matching methods is not systematic in this
domain, some fundamental contributions have been made using this
technique \cite{fe73}. In the work of  Von
der Malsburg and his collaborators, for example \cite{dkl92, wv93},
face comparison incorporates a discrete form of elastic deformation,
represented as neural networks; the aligned quantities are not image
grey levels, but Gabor filters \cite{gab46}, in accordance with biological
observations.

In \cite{hgygm99}, a (quite complex) model is proposed for face variation in terms of illumination,
position and expression, to provide a single variational problem. The
deformation part incorporates the hyperelastic energy we have
described in equation
(\ref{elas.ax}).




\subsubsection*{Medical imaging}

Medical imaging may be the primary domain of application of
deformations, in 2, but mainly 3, dimensions.
Increasingly sophisticated acquisition systems provide anatomical
images in higher number with more and more accuracy, with new informations and
modalities. The need to, at least partially, automatize the processing
and analysis of these images has become more and more important. The
whole field of computerized analysis of medical images is called
computational anatomy \cite{gm98}. Several matching methods applied to
brain images are described in  \cite{tog99}.

\subsection{Using flows of diffeomophisms}
\label{fluid.grad}

Like for interpolation, the previous techniques do not 
guarantee that the optimal deformation is a diffeomorphim. Such a
property can be obtained by using the formulation given in chapter
\ref{grp.diff}. This leads to minimizing
$$
U(\bfv) = \int_0^1 \int_\Om \scp{L\bfv(t, .)}{\bfv(t, .)} dx dt + \la \int_\Om
\left(I\circ \bfg_\bfv(1,x) - I'(x)\right)^2 dx
$$
with respect to  $\bfv$, where $L$ is a strictly monotonous admissible
operator (i.e., such that $\CH_L$, according to definition \ref{adm}),
and, as before,  $\bfg_\bfv(t,x)$ is the value at time 
$t$ of the solution of $y_t = \bfv(t, y)$ with initial condition
 $y(0) = x$ ($x\in\Om$).

Because the operator $L$ is admissible, the function  $U$ achieves a
global minimum, for a time-dependent vector filed  $\bfv$ that
generates a diffeomorphim. Let's prove this in the case when  $I$ and
$I'$ are continuous on $\Om$ (the result remains true for $L^2$
functions). The mapping
$$
g\mapsto q(g) = \int_\Om |I'(x) - I\circ g(x)|^2 dx
$$
is continuous for uniform convergence: if $g_n$ converges to $g$
uniformly on $\Om$, then, from the continuity of $I$ and the dominated
convergence theorem,  $q(g_n)$ converges to $q(g)$. This fact,
combined with theorem \ref{weak.closed} and to the lower
semi-continuity of norms on Hilbert spaces implies that there exists a
$\bfv^*$ minimizing $U(\bfv)$.

\bigskip
To minimize this expression using gradient descent, we need to compute
the differential of of $U$ with respect to  $\bfv$. This require some
care, in particular for the term  $\bfg_\bfv$. We now proceed to this
computation assuming that $I$ and $I'$ are $C^1$ functions. We
evaluate the 
variation $U(\bfv+ \ep h) - U(\bfv)$ for small $\ep$.

The first term of $U(\bfv+\ep h) - U(\bfv)$ is $\|\bfv+\ep h\|^2 -
\|\bfv\|^2$, which can be written $\ep \scp{h}{\bfv} + o(\ep)$ with
$$
\scp{h}{\bfv} = \int_0^1 \int_\Om \scp{Lh}{\bfv} dx dt.
$$
The study of the second term, which is
$$
\int_\Om \left(I\circ \bfg_{\bfv+\ep h}(1,x) - I'(x)\right)^2 dx -
\int_\Om \left(I\circ \bfg_{\bfv}(1,x) - I'(x)\right)^2 dx
$$
requires more work.

We first show that the differential
$$
q_h(t) = \pdr{}{\ep}\bfg_{\bfv+\ep h}(t, x)_{|_{\ep=0}}
$$
exists. This can be handled in the same way as the existence of the
differential  of $\bfg_\bfv$ with respect to $x$ (theorem
\ref{flot.exist}), and we rapidly sketch the details. One first
formally computes a candidate by writing
$$
\pdr{}{t} \bfg_{\bfv+\ep h}(t, x) = \bfv(t, \bfg_{\bfv+\ep h}(t, x)) +
\ep h(t, \bfg_{\bfv+\ep h}(t, x))
$$
to get
\begin{equation}
\label{qh}
\der{q_h}{t} = D \bfv(t, .) (\bfg_\bfv(t, x)) q_h + h(t,\bfg_{\bfv}(t,x)).
\end{equation}
This is a linear, non-homogeneous differential equation, for which we
introduce a solution $\tilde{q}_h$ (with
$\tilde{q}_h(0) = 0$). It remains to make this formal computation
rigorous, by showing that 
$q_h$ does exist, and is equal to $\tilde{q}_h$. This can be done by
returning to the definition of the derivative and use Gronwall's lemma
like in the proof of theorem \ref{flot.exist}.

Remarking that the homogeneous equation associated to \eqref{qh} is in
fact \eqref{flot.diff},  $q_h$ can be computed analytically by the
mathod of variation of the constant, yielding
$$
q_h(t, x) = D\bfg_\bfv(t,x)\int_0^t D\bfg_\bfv(s,x)^{-1}.h(s,
\bfg_\bfv(s,x)) ds.
$$

The previous computation therefore yields
\begin{multline*}
U(\bfv+\ep h) - U(\bfv) = 2 \ep \scp{h}{\bfv} \\
+ 2\ep \la \int_\Om \scp{I\circ
\bfg_\bfv(1,x) - I'(x)}{DI\circ \bfg_\bfv(1,x)q_h(1,x)} dx
+
o(\|h\|).
\end{multline*}
Replacing  $q_h$ b its expression, we get, denoting 
$\ga_\bfv(t, .)$ the inverse of $\bfg_\bfv(t,.)$
\begin{multline*}
\int_\Om \scp{I\circ \bfg_\bfv(1,x) - I'(x)}{DI\circ
\bfg_\bfv(1,x).q_h(1,x)} dx
\\ = \int_0^1\int_\Om \left\langle I\circ
\bfg_\bfv(1,x) - I'(x), \right. \\
\left.DI\circ
\bfg_\bfv(1,x).d\bfg_\bfv(1,x)d\bfg_\bfv(t,x)^{-1}.h(t,
\bfg_\bfv(t,x)) \right \rangle dx dt
\\=
 \int_0^1\int_\Om \lan  DI\circ
\bfg_\bfv(1,\ga_\bfv(t,y))D\bfg_\bfv(1,\ga_\bfv(t,y))D\bfg_\bfv(t,\ga_\bfv(t,y))^{-1}.
h(t, y),
\\ I\circ \bfg_\bfv(1,\ga_\bfv(t,y)) -
I'(\ga_\bfv(t,y))\ran |\det D\ga_\bfv(t,y)|dy dt.
\end{multline*}
To simplify this formula, introduce the function $\chi_\bfv(t, y) = \bfg_\bfv(1,
\ga_\bfv(t,y))$, and the notation $\bfJ(t,y) = I(\chi_\bfv(t,y))$
and $\bfJ'(t,y) = I'(\ga_\bfv(t,y))$. We have
$$D\bfg_\bfv(t,\ga_\bfv(t,y))^{-1} = D\ga_\bfv(t,y)\,,
\ \ 
D\bfg_\bfv(1,\ga_\bfv(t,y)) D\ga_\bfv(t,y) = D\chi_\bfv(t,y)
$$
and
$\dps
D\bfJ(t,y) = DI\circ \bfg_\bfv(1,\ga_\bfv(t,y)) D\chi_\bfv(t,y)\,.$
We finally obtain the expression
\begin{multline*}
\int_\Om \scp{I\circ \bfg_\bfv(1,x) - I'(x)}{DI\circ
\bfg_\bfv(1,x) q_h(1,x)}
\\ =   \int_0^1\int_\Om \scp{\bfJ(t,y) - \bfJ'(t,y)}{D\bfJ(t,y) |\det
D\ga_\bfv(t,y)| h(t, y)} dy dt \\ = \int_0^1\int_\Om |\det
D\ga_\bfv(t,y)|\scp{D\bfJ(t,y)^T (\bfJ(t,y) - \bfJ'(t,y))}{h(t,
y)} dy dt
\end{multline*}
and the proposition
\encadre{
\begin{proposition} [Beg et al., 2002]
\label{grad.prop}
Let
$$
U(\bfv) = \int_0^1 \int_\Om |L\bfv|^2 dx dt + \la \int_\Om
\left(I\circ \bfg_\bfv(1,x) - I'(x)\right)^2 dx
$$
If $u \mapsto \left(\int_\Om |Lu|^2 dx\right)^{1/2}$ induces an
admissible norm on functions $u:\Om\to\mR$, we have, letting
$\|\bfv\|^2 = \int_0^1 \int_\Om |L\bfv|^2 dx dt\,:$
$$
U(\bfv+\ep h) = 2 \ep \scp{\bfv}{h} + 2\ep \la \int_0^1\int_\Om
\scp{b_\bfv(t,y)}{h(t,y)} dy + o(\ep)
$$
with
$$
b_\bfv(t, y) = |\det D\ga_\bfv(t,y)|D\bfJ(t,y)^T (\bfJ(t,y) -
\bfJ'(t,y))
$$
where $\ga_\bfv(t, y)$ is the inverse of $\bfg_\bfv(t,y)$ and
$
\bfJ(t, y) = I(\bfg_\bfv(1,\ga_\bfv(t, y)))$, $\bfJ'(t,y) =
I'(\ga_\bfv(t, y))$.
\end{proposition}
}

Figure \ref{match.beg} provides a matching experiment using this
algorithm for shape matching.

\begin{figure}
\begin{center}
\includegraphics[width=5.5cm]{TUTORIALPS/SY0.ps}\hfill
\includegraphics[width=5.5cm]{TUTORIALPS/SY299.ps}\\
\includegraphics[width=5.5cm]{TUTORIALPS/SYgrid270.ps}
\end{center}
\caption{\label{match.beg} First Row: two shapes before
alignment. Second Row: Estimated deformation applied to a regular grid.}
\end{figure}


\subsection{Numerical aspects}
In this section, we make (without geting into imlpementation details)
some important remarks on the numerical 
implementation of diffeomorphic matching. 

\subsubsection{Discretization}
The simplest and mostly used way to discretize a function is to use a
regular grid, approximate integrals by sums and derivatives by finite
differences. This leads to rather simple implementations, but involves
a huge number of variables, that can require considerable computer
power in 3D.

One can also use a decomposition on a basis of functions. One
possibility is to use finite elements 
\cite{rwcm95}, which consists  \cite{zt89} in defining a basis of
smooth function (generally piecewise polynomial, with compact support)
on which the unknow diffeomorphism is projected. Another possible
choice of basis are the eigenvectors of the operator $L$ which form an
orthonormal basis of  $\CL^2$.


\subsubsection{Definition of the gradient}

Here is a simple, but fundamental remark, on gradient descent
algorithms. At the difference of the differential of a function, the
gradient depens on a dot product (or a Riemannian structure) on the
ambient space. For example, if $U$ is a differentiable function on
$\mR^p$, the differential of $U$ at $g$ is a linear operator, $DU(g)$,
defined by 
$U(g+\ep h) \simeq U(g) + \ep DU(g).h + o(\ep)$, avec
$$
DU(g).h = \sum_{i=1}^p \pdr{U}{g_i} h_i.
$$
To define a gradient, we need a Eclidean or Riemannian
structure. Denoting it  $\scp{.}{.}_g$, the gradient of  $U$ at $g$ is {\em defined}
by
$$
\forall h,  DU(g).h = \scp{\nabla U(g)}{h}_g.
$$
The discrete gradient descent algorithm with step  $\ga$ is
$$
g(\tau+1) - g(\tau) = -\ga \nabla U(g(\tau)).
$$
This algorithm therefore also depends on the Riemannian structure. On
$\mR^p$, the standard Euclidean structure provides the usual gradient
descent, 
$$
g(\tau+1) - g(\tau) = - \ga \der{U}{g}
$$
where $\der{U}{g}$ is the vector composed with partial derivatives of $U$
at $g(\tau)$; but, letting
$$
\scp{u}{v}_g = {}^tuA_gv,
$$
where $A_g$ is a symmetric positive matrix, the algorithm becomes
$$
g(\tau+1) - g(\tau) = - \ga A_{g(\tau)}^{-1}\der{U}{g}.
$$

Such variations may have importance consequences on the quality and
stability of the algorithm, especially in infinite dimensions. From a
heuristic point of view, the Riemannian metric defines directions that
are easier to take than other in the space, and make others almost
impossible. If  $g$ is a function, a suitable choice of the metric
will favor trajectories where $g$ remains bounded or smooth, for example.
Even in finite dimensions, selecting a good metric can lead to
improved algorithms. For example, when a function is optimized over
invertible matrices, one can ensure that the matrix remains invertible
along the algorithm (like for independent component analysis, appendix
\ref{ica}). 

Let's provide some illustrations of this for the optimization over
functions. Consider the following typical situation in the calculus of
variation where a function $g$ defined n $\O$ is searched to minimize
$$
U(g) = \int_\Om F(Dg(x), g(x), x) dx.
$$
We first compute the equivalent of directional derivatives, which
coreespond to computing a function $b_g$ defined on $\Om$, such that,
for every function $h$ with compact support in $\Om$
$$
\der{}{\ep} U(g+\ep h) = \int_\Om b_g(x).h(x) dx
$$
at $\ep=0$. This can be interpreted as a gradient of $U$ for the
$\CL^2$ dot product
$$
\scp{h}{k}_2 = \int_\Om k h dx\,.
$$

Take, for example, $\Om = ]0,1[$ and
$$
U(g) = \int_0^1 (|\dg|^2 + V(g(x))) dx
$$
where $V$ is a positive function and  $g: [0,1]\to [0,1]$ satisfies
$g(0) = 0$ and $g(1) = 1$. By a standard computation using integration
by parts, we obtain, at $\ep=0$,
$$
\der{}{\ep}U(g+\ep h) = \int_0^1(-\dder{g}{x} + V'\circ g).h dx.
$$
This provides the $\CL^2$-gradient of $U$
$$
\nabla_g U = -\dder{g}{x} + V'\circ g.
$$
The gradient dscent algorithm (expressed in continuous time) is
$$
\pdr{g}{\tau} = -\dder{g}{x} + V'\circ g.
$$

\bigskip

Return now to the general case. Assume that the dot product is
selected so that 
$$
\scp{h}{k} = \int_\Om \scp{k}{Lh} dx
$$
where $L$ is a strictly monotnus operator. Still assuming that we can
write
$$
\der{}{\ep}U(g+\ep h) = \int_\Om \scp{b_g}{h} dx\,,
$$
we see that the gradient of $U$ for the new dot.product must satisfy
$Lv = b_g$, yielding the numerical scheme
$$
\left\{
\begin{array}{l}
\dps \pdr{g}{\tau} = - v\\
\ \\
\dps Lv = b_g
\end{array}
\right. .
$$
In this discussion, we have neglected the boundary conditions on $\prt
\Om$ (or implicitely assumed that valid variations $h$ must vanish at
the boundary, like in our example, so that they do not add any new
term in the integration by parts).

Let's return to out 1D example, and consider the dot product
$$
\scp{k}{h}_L = \int_0^1 \dot{k}\dh dx = \int_0^1 k Lh dx
$$
with $Lh = - \dder{h}{x}$; this yields the algorithm
$$
\left\{
\begin{array}{l}
\dps \pdr{g}{\tau} = - v\\
\ \\
\dps \dder{v}{x} = -\dder{g}{x} + V'\circ g\\
\ \\
\dps v(0) = v(1) = 0
\end{array}
\right.
$$

We have therfore built a two-step numerical scheme. First compute the
$\CL^2$ gradient then {\em smooth it}, by applying to it the inverse
of the operator $L$, to obtain the increment of the crent function
$g$. More precisely, if $K = L^{-1}$ is a kernel operator, the
algorithm is
$$
\pdr{g}{\tau} = -\int_{\Om} K(x, y) b_g(y) dy.
$$
This implies in particular that $g$ inherits the smoothness of the
kernel during evolution, which is generally a factor of stability in
the algorithm.

The situation is even more interesting in the case of groups of
diffemorphisms, in which we deal here with a ``true'' Riemannian metric and
not a change of Hilbert space dot product. The application of this
idea to groups of diffeomorphisms has been suggested in
\cite{tro98}. Consider the function
\begin{equation}
\label{eq:image.data}
U(g) = \int_\Om \left| I \circ g(x) - J(x) \right|^2 dx
\end{equation}
where $I$ and $J$ are two $C^1$ images defined on $\Om$, and $g$ is a
diffeomorphism of $\Om$. It is very easy to compute the
$\CL^2$ gradient of $U$, and is given by
\begin{equation}
\label{grad.l2}
b_g(x) = 2(I(g(x)) - J(x)) DI(g(x)).
\end{equation}
The $\CL^2$ gradient descent would therefore be given by
$$
\pdr{g}{t} = - (I(g(x)) - J(x)) DI(g(x)).
$$

This procedure is extremely unstable. It is in fact never used as such,
and always combined with some form of regularization (see the method
of deamons in the next section). Another issue is that the procedure
does not take into acount the fact that  $g$ must be a
difeomorphism. Let's consider a Riemannian dot product for
diffeomorphisms, given by
$$
\scp{h}{k}_g = \int_\Om \scp{L(h\circ g^{-1})}{k\circ g^{-1}} dx.
$$
(The operator $L$ is applied to the function $h\circ g^{-1}$.) This
choice will be justfified in chapter \ref{dist.diff}. To obtain the
associated gradient descent, we need to express
\begin{equation}
\label{eq:grad.img}
\der{}{\ep}U(g+\ep h)  \int_\Om 2(I(g(x)) - J(x)) DI({g(x)}) h(x)
dx 
\end{equation}
under the form
$$
\der{}{\ep}U(g+\ep h) = \scp{\beta_g}{h}_g. $$
Let us first make the change of variables  $y = g(x)$ in
\eqref{eq:grad.img}. This yields
$$
\der{}{\ep}U(g+\ep h) = \int_\Om 2(I(y) - J(g^{-1}(y)))
DI(y) h(g^{-1}(y)) |\det Dg^{-1}(y)| dy + o(\ep).
$$
This implies that  $\beta_g$ must be such that $\beta_g\circ g^{-1}$
satisfies the equation
$$
L.u(y) = 2|\det Dg^{-1}(y)|(I(y) - J(g^{-1}(y)))
DI(y).
$$

This means that the gradient descent for the considered dot product
must proceed as follows.Solve
\begin{equation}
\label{eq:flow.grad}
\pdr{g}{\tau}(\tau,x) = u(\tau, g(\tau,x))
\end{equation}
with 
\begin{equation}
\label{eq:smooth.grad}
L(t,.) = - 2|\det D{g}^{-1}(y)|(I(y) - J({g}^{-1}(y)))
DI(y).
\end{equation}
Equation \eqref{eq:smooth.grad} is a smoothing operation applied to
the $\CL^2$ gradient. The particular form of the evolution equation
\eqref{eq:flow.grad} is a dircet consequence of the form that has been
selected for the Riemannian metric. It shows that the evolution
generated by this particular
implementation of gradient descent s a flow (a solution of an ODE)
that generates a diffeomorphism as long as $u$ remains smooth. A
similar algorithm as been proposed by \cite{crm96}, based on different
motivations. 

It is important to note that that the function $U$ in \eqref{eq:image.data} contains no
regularization term for $g$. This implies that, unless $I$ and $J$ are
can be made in correspondence exactly by diffeomorphism, there is
probably no global minimum, and the evolution will generate wild
deformations if pushed too far. A suitable stopping rule must be
designed \cite{tro98}. 




\subsubsection{Deamons algorithm}

The method of deamons is a popular matching algorithm in medical
imaging \cite{thi98, thi99, gram99}. Although it does not exactly
correspond to a gradient descent implementation, it can almost be
interpreted as such. Consider the energy
$$
U(g) = \int_\Om |J(x) - I(g(x))|^2 dx
$$
with $\CL^2$ gradient given by
$$b_g(x) = 2(I(g(x)) - J(x)) DI ({g(x)})$$

Consider the following dot product
$$
\scp{h}{k}_g = \int_\Om (|J(x) - I(g(x))|^2 + |D J(x)|^2) h(x)
Lk(x) dx
$$
for some operator $L$.
The gradient of  $U$ for this dot product is given by
$$
L^{-1} \Big(\frac{b_g(x)}{|J(x) - I(g(x))|^2 + |D J(x)|^2}\Big)
$$
that can be approached by
$$
-2L^{-1}\left(\frac{J(x) - I(x)}{|J(x) - I(g(x))|^2 + |D J(x)|^2} D
J(x)\right).
$$

This provides a gradient descent algorithm which can be written, in
discrete time, under the form (letting $K=L^{-1}$)
\begin{equation}
\label{thi}
u(\tau+1, y) = u(\tau, y) + \ga\int K(y,x) \frac{J(x) - I(x)}{|J(x) - I(g(\tau, x))|^2 + |\nabla J(x)|^2} \nabla
J(x) dx
\end{equation}
with $g(\tau, x) = x + u(\tau, x)$. The method of deamons applies an
additional smoothing to the current $u$ before adding the increment,
yielding
\begin{multline*}
u(\tau+1, y) = \int K(y,x) u(\tau,x))dx\\
 + \int K(y,x) \ga\frac{J(x) - I(x)}{|J(x) - I(g(\tau, x))|^2 + |\nabla J(x)|^2} \nabla
J(x) dx.
\end{multline*}
This addictional smoothing is hard to interpret and to justify.
To interpret the dot product introduced in this section, one must
remember that the norm
$\scp{h}{h}_g$ can be interpreted as an infinitesimal cost function
for the variation $g\to g+h$; as we have already noticed, the operator
$L$ penalizes a lack of smoothness; the multiplicative factor
penalizes variations at location $x$ according to the value of  $|J(x)
- I(g(x))|^2 + |D J(x)|^2$. This implies that changes of $h(x)$
are limited when the matching is unsatisfactory and when $J$ has a
large gradient. 



\nocite{yos70}

\subsubsection{Multigrid approaches}

For these very high dimensional, non-convex, multigrid algorithms
often bring significant improvements, both in efficiency and
quality, in avoiding some local minima. Several strategies are available for this.
One can start solving a problem with coarser images and discretization grids, to
progressively refine the solutions. One can also use representations
of the unknown variable (the diffeomorphism) that allow for a
progressive release of the degrees of freedom. This can be done easily
by using a decomposition on orthogonal bases and playing with the
number of coefficients that are retained \cite{bk89, ghlb97, bk99}.









\chapter{Distances and group actions}
\label{dist.grp}

\section{General principles}
\subsection{Distance induced by a group action}

This chapter shows how transformation groups acting on spaces can help
defining or altering distances on these spaces. The first part will
essentially focus of the algebraic aspects of the contructions based
on the least action principle. In the second part, we will develop the
related
differential point of view, when a Lie group acts on a manifold.

\index{distance (axioms)}

\bigskip
We start with some terminology. A distance on a set  $\CC$ is a mapping
$d:\CC^2\mapsto \mR_+$ such that, for all $m, m', m''\in\CC$,\\
\indent D1) $d(m, m') = 0 \Leftrightarrow m= m'$.\\
\indent D2) $d(m. m') = d(m', m)$\\
\indent D3) $d(m, m'') \leq d(m, m') + d(m', m'')$.

If D1 is not satisfied, but only the fact that $d(m, m)=0$ pour tout
$m$, we will say (still assuming D2 and D3) that $d$ is a {\em pseudo-distance}.

If $G$ is a group acting on $\CC$, we will say that a distance $d$ on
$\CC$ is $G$-equivariant if and only if for all $g\in G$, for all
$m, m'\in \CC$, $d(g.m, g.m') = d(m, m')$.

A mapping $d:\CC^2\mapsto \mR_+$ is a $G$-invariant distance if and
only if it is a pseudo-distance such that $d(m, m') = 0
\Leftrightarrow \exists g\in G,\, g.m = m'$. This is equivalent to
stating that $d$ is a distance distance on the coset space $\CC/G$,
composed with orbits
$$
[m] = \{g.m, g\in G\},
$$
with the identification $d([m], [m']) = d(m,, m')$.

The next proposition shows how a $G$-equivariant distance induces a
$G$-invariant pseudo-distance.
%\encadre{
\begin{proposition}
\label{modulo}
Let $d$ be equivariant for the left action of $G$ on $\CC$. The function $\td$,
defined by
$$
\td([m], [m']) = \inf\{d(gm, g'm'), g, g'\in G\}
$$
is a pseudo-distance on $\CC/G$.
\end{proposition}
%}
\index{invariant distance} \index{equivariant distance}
Since $d$ is $G$-equivariant, we could have defined $\td$ in the
previous proposition by
$$
\td([m], [m']) = \inf\{d(gm, m'), g\in G\}.
$$
\begin{proof}
The symmetry of $\td$ is obvious, as well as the fact that $\td((m],
[m]) =0$ for all $m$. For the triangle inequality, D3, it suffices to
show that, for all $g_1, g'_1, g'_2, g''_1\in G$, there exists $g_2,
g''_2\in G$ such that
\begin{equation}
\label{eq:d3}
d(g_2m, g''_2 m'') \leq d(g_1m, g'_1m') + d(g'_2m', g''_1m'').
\end{equation}
Indeed, if this is true, the minimum of the right-hand term in $g_1, g'_1, g'_2, g''_1$, which is
$\td([m], [m']) + \td([m'], [m''])$ is larger than the minimum of the
left-hand term in $g_2, g''_2$, which is $\td([m], [m''])$, which is
precisely D3. To prove \eqref{eq:d3}, write $d(g'_2m', g''_1m'') = d(g'_1m', g'_1 (g'_2)^{-1}
g''_1m'')$, and take $g_2 = g_1$ and 
$g''_2 = g'_1 (g'_2)^{-1}
g''_1$; \eqref{eq:d3} is just an application of the triangle
inequality for $d$.
\end{proof}

Whether $\td$ is a distance, and not just a pseudo-distance is
statement about the minimizer of a function. Excepted in the trivial
case of finite groups, this will require some topological assumptions
on the structure of $G$ and of the action.

The same statement can clearly be made with $G$ acting on the right on $m$,
with $m \mapsto m.g$. We state it without proof
\begin{proposition}
\label{modulo.right}
Let $d$ be equivariant for the left action of $G$ on $\CC$. The function $\td$,
defined by
$$
\td([m], [m']) = \inf\{d(mg, m'g'), g, g'\in G\}
$$
is a pseudo-distance on $G\backslash \CC$.
\end{proposition}
Here $G\backslash M$ denotes the coset space for the right action of $G$.



\subsection{Distance altered by a group action}

In this section, $G$ is still a group acting on the left on  $\CC$, but we consider
the product space $\CO  = G\ti \CC$ and project on $\CC$ a distance
defined on $\CO$.

The group $G$ acts on the right on $\CO$, letting, for $k\in G$,
$o=(h, m)\in \CO$, $o.k = (hk, k^{-1}m)$. For $o=(h, m)\in \CO$, we define
the projection 
$\pi(o) = hm$. This projection is such that, for all $k\in G$,
$\pi(o.k) = \pi(o)$. 

Let $d_\CO$ be a distance on $\CO$. We let, for $m, m'\in \CC$
\begin{equation}
\label{inv.eq.gen}
d(m, m') = \inf\{d_\CO(o, o'), o, o'\in \CO, \pi(o) = m,  \pi(o') = m'\}.
\end{equation}

We have the proposition
\encadre{
\begin{proposition}
\label{inv.gch.gen}
If $d_\CO$ is equivariante by the right-action of $G$, then, the
function $d$ defined by \ref{inv.eq.gen} is a pseudo-distance on $\CC$.
\end{proposition}}

This is in fact a corollary of proposition \ref{modulo.right}. One only has
to remark that the quotient space  $G\backslash \CO$ can be identified to $\CC$
via the projection $\pi$, and that the distance in \eqref{inv.eq.gen}
then becomes the projection distance introduced in proposition
\ref{modulo.right}.

\subsection{Existence of a minimum}

We assume that the group  $G$ is a topological space, but no special
structure on $\CC$.
For $m\in \CC$, define the mapping $I_m: G\mapsto \CO$ by
$I_m(h) = (h, h^{-1}m)$. We make the following hypotheses.
\begin{itemize}
\item The canonical projection  $(h, m)\in
\CO \to h$ of sets of finite diameters for  $d_\CO$ are sequentially
precompact sets in $G$.
\item For all $o\in \CO$, for all $m\in \CC$, the function $h\mapsto
d_\CO(o, I_m(h))$ is lower semi-continuous: if $h_n\to
h$ in $G$, then
$$
d_\CO(o, I_m(h)) \leq \liminf d_\CO(o, I_m(h_n))
$$
\end{itemize}
A subset  $A$ of the topological space $G$ is sequentially precompact
if one can extract a sequence that converges in $G$ from any sequence
in  $A$.

We have
\begin{proposition}
\label{exist.gen}
Assume the previous hypotheses. If $d_\CO$ is equivariant by the
left-action of  $G$, then, for all  $m,
m'\in\CC$, there exists $o, o'\in G$ such that $\pi(o) = m$,
$\pi(o')=m'$ and $d(m, m') = d_\CO(o, o')$. In particular, $d$ is a
distance on  $\CC$.
\end{proposition}
\begin{proof}
Let $m$ and $m'$ be two elements of $\CC$. From the definition of
$d$, there exists two sequences  $(o_n, n\geq 0)$ and $(o'_n, n\geq
0)$ such that  $\pi(o_n) = m$, $\pi(o'_n) = m'$, and $d_\CO(o_n, o'_n) \ria
d(m, m')$. From the definition of  $\pi$, $o_n$ takes the form $o_n =
(h_n, h_n^{-1}.m)$, and $o'_n = (h'_n, {h'_n}^{-1}.m')$. Using the
left-equivariance, we can replace  $o_n$ and $o'_n$ by $h_n o_n$ and
$h_n o'_n$; this is equivalent to assuming that  $h_n = \id_G$ for
all $n$, that we shall do without changing the notation, letting
$o_n \equiv o=(\id_G, m)$ for al $n$. Since $o_n$ is constant, the
sequence  $(o'_n, n\geq 0)$ is bounded in $\CO$, so that we can
extract a converging subsequence from  $(h'_n, n\geq 0)$; we let
$h'\in G$ be the limit. We have $o'_n = I_{m'}(h'_n)$, and, letting
$o'=(h', h'^{-1}m') = I_{m'}(h')$, our second hypothesis yields
$$
d_\CO(o, o') \leq \liminf d_\CO(o, o'_n) = d(m, m').
$$
Since $d(m, m') \leq d_\CO(o, o')$, we obtain the required result.
\end{proof}

\subsection{Transitive action}
\subsubsection{Induced distance}
An important particular instance of the previous construction is when
$\CO$ itself is a group that acts transitively on $\CC$. This means
that for any $m, m'$ in $\CC$, there exists an element $o\in\CO$ such
that $m' = om$.

So our initial assumption is that $\CO$ is a group that acts
transitively on the set $\CC$. We fix a reference element 
 $m_0$ in $\CC$, and define the group $G$ by
$$G = \{o\in \CO, o.m_0 = m_0\}\,.$$
This group $G$ is called the stabilizer of  $m_0$ in $\CO$. The
relation to the previous section comes with the identification of
$\CO$ with $G\ti\CC$. 

One way to see that is by assuming that a function  $\rho: \CC\to \CO$
has been defined, such that for all $m\in\CC$, $m = \rho(m).m_0$. This
is possible, since the action is transitive (using anyway
the axiom of choice). Define
$$
\map{\Psi}{G\ti\CC}{\CO}{(h, m)}{\rho(h.m)h}.
$$
We show that $\Psi$ is a bijection: if $o\in \CO$, one can write, we
look for $(h,m)$ such that 
$o = \Psi(h, m)$. If this is true, we have 
$$o.m_0 = \rho(hm)h m_0 = \rho(hm)m_0 = hm$$
which imples that $\rho(hm) = \rho(om_0)$ and therefore $h =
\rho(om_0)^{-1} o$ which is uniquely specified; but this also specifies $m =
h^{-1}om_0$. This proves that $\Psi$ is one-to-one and onto
and provides the identification we are looking for.

The right action of $G$ on $G\ti\CC$, which is $(h, m)k = (hk,
k^{-1}m)$, translates to $\CO$ via $\Psi$ with
$$
\Psi(hk, k^{-1}m) = \rho(hkk^{-1}m)hk = \Psi(h,m)k
$$
which coincides with the right action of $G$ on $\CO$. Finally, the
constraint $\pi(h,m_1) = m$ which is involved in 
Proposition \ref{inv.gch.gen} becomes $om_0 = m$ via the
identification. All this provides a new version of Proposition
\ref{inv.gch.gen} in our present context given by
\begin{corollary}
\label{inv.gch}
Let $d_\CO$ be a distance on $\CO$, which is invariant under the
right-action of  $G$, the stabilizer of $m_0\in\CC$. Define, for all
$m, m'\in\CC$
\begin{equation}
\label{inv.eqg}
d(m, m') = \inf\{d_\CO(o, o'), o.m_0 = m, o'.m_0=m'\}\,.
\end{equation}
Then $d$ is a pseudo distance on  $\CC$.
\end{corollary}

The translation of the hypotheses made for 
proposition  \ref{exist.gen} is as follows. We assume that  $G$ can
be equipped with a topology such that
\begin{itemize}
\item Images of sets of finite diameters for  $d_\CO$ by $o \mapsto
\rho(om_0)^{-1} o$ are sequentially compact sets in  $G$.
\item For all  $o\in \CO$, for all $m\in \CC$, the function  $h\mapsto
d_\CO(o, \rho(m)h)$ is lower semi-continuous..
\end{itemize}
We have
\begin{corollary}
\label{exist.gch}
We assume the previous hypotheses. If $d_\CO$ is equivariant by the
right action of  $G$, then, for all $m, m'\in\CC$, there exists $o,
o'\in \CO$ such that $\pi(o) = m$, $\pi(o')=m'$ and $d(m, m') = d_\CO(o,
o')$. In particular, $d$ is a distance on $\CC$.
\end{corollary}





\subsubsection{Effort functional}
\bigskip
\index{Effort functional}
As formalized in \cite{gre93}, one can built a distance on
 $\CC$ on which a group acts transitively using the notion of effort
functionals. The definition we give here is slightly more general than
in  \cite{gre93}, to take into account a possible influence of the
deformed object on the effort. We also make a connection with the
previous, distance based, formulations.

We attribute a cost $\Ga(o, m)$ to  a transformation $m\ria o.m$. If
$m$ and 
$m'$ are two objects, we define 
$d(m, m')$ as the minimal cost (effort) required to transform  $m$ in
$m'$, i.e.,
\begin{equation}
\label{ga.gch}
d(m, m') = \inf\{\Ga(o,m), g\in G, o^{-1}.m = m'\}
\end{equation}

The proof of the following proposition is almost obvious.
\begin{proposition}
\label{cout.gch}
If $\Ga$ satisfies

C1) $\Ga(o, m) = 0 \Leftrightarrow o=e$

C2) $\Ga(o, m) = \Ga(o^{-1}, om)$

C3) $\Ga(oo', m) \leq \Ga(o, m) + \Ga(o', om)$

Then, $d$ defined by (\ref{ga.gch}) is a pseudo-distance on $\CC$.
\end{proposition}

In fact, this is equivalent to the construction of corollary
\ref{inv.gch}. To see this, let as before  $G$ be the stabilizer of
$m_0$ for the action of $\CO$ on $\CC$. We have
\begin{proposition}
\label{cdis.gch}
If $\Ga$ satisfies C1), C2) and C3), then, for all $m_0\in\CC$, the
function  $d_\CO$ defined by
$$
d_\CO(o, o') = \Ga((o')^{-1}o, o^{-1}.m_0)
$$
is a distance on $\CO$ which is equivariant for the left action of
$G$. Conversely, given such a distance $d_\CO$, one build an effort
functional  $\Ga$ satisfying C1), C2), C3) b letting
$$\Ga(h, m) = d_\CO(oh, o)$$
where $o$ is any element of $\CO$ with the property $o.m = m_0$.
\end{proposition}
Here again, we leave the proposition to the reader.


\subsection{Infinitesimal approach}
\label{var}
The previous sections have demonstrated the interest of equivariant
distances on $\CO$. It may be, however, very difficult to come up with
an analytical expression for such a distance. Very often, fortunately
(in particular when  $\CC$ is a differential manifold and $G$ is a Lie
group) a left invarant Riemannian metric  can be designed, leading to a
left-invariant distance defined as a variational problem.

We need to build a left invariant metric on $\CO$. Recall that a
Riemannian metric on $\CO$ defines, for all $o\in\CO$, a dot product
$\scp{.}{.}_o$ on the tangent space, $T_o\CO$,  to $\CO$ at $o$, which
depends smoothly on $o$. With such a metric, one can define
the energy of a differentiable path  $\bfo$ in $\CO$ by
\begin{equation}
\label{ener.1}
E(\bfo) = \int_0^1 \left\|\der{\bfo}{t}\right\|^2 dt.
\end{equation}
The associated Riemannian distance on $\CO$ is
\begin{equation}
\label{geod.1}
d_\CO(o, o') = \inf\{ \sqrt{E(\bfo)}, \bfo(0) = o, \bfo(1) = o'\}.
\end{equation}

To obtain a left invariant distance, it suffices to ensure that the
metric has this property. For $h\in G$, we left $L_h$ denote the left
action of $h$ on $\CO$: $L_h: o \mapsto h.o$. Let $d_oL_h$ be its
differential at $o\in \CO$. It is a linear map, defined on 
$T_o\CO$, with values in $T_{h.o}\CO$ such that, for all
differentiable path $\bfo$ on $\CO$ such that $\bfo(0)=o$, we have
\begin{equation}
\label{left.trans}
\der{h\bfo}{t}_{|_{t=0}} = d_oL_h.\der{\bfo}{t}_{|{t=0}}.
\end{equation}
The left invariance of the metric is expressed by the identity, true
for all  $o\in \CO$, $A\in T_o\CO$ and $h\in G$,
\begin{equation}
\label{left.inv.1} 
\|A\|_o = \left\|d_oL_h.A\right\|_{ho}.
\end{equation}

When  $\CO = G\ti \CC$, condition
(\ref{left.inv.1}) implies that it suffices to define $\scp{.}{.}_o$
at elements  $o\in \CO$ of the form $o = (\id, m)$ with $m\in
\CC$. The metric at a generic point $(h,m)$ can then be computed, by
left invariance, from the metric at $(\id, h^{-1}m)$. Since the metric
at $(\id, m)$
can be interpreted as a way to attribute a cost to a deformation
$(\id, h(t)m)$ with $h(0) = \id$ and small $t$, defining it
corresponds to an analysis of the cost of an infinitesimal
perturbation of $m$ by an element of $G$.

In the next sections, we will apply this construction to several
situations, depending on the choice of the deformable objects and on
the group $G$.


\section{Invariant distances between landmarks}

\subsection{Introduction}
The purpose of this section is to present the construction provided by
Kendall \cite{ken84} on distances between landmarks, under the
infinitesimal point of view that we have just outlined. Here,
configurations of landmarks are considered up to similitude
(translation, rotation, scaling).

We only consider the 2D case, which is also the simplest. For a fixed
integer  $N >0$ let $\CP_N$ denote the set of configurations of 
$N$ points $(z_1, \ldots, z_N) \in (\mR^2)^{N}$. We assume that the
order in which the points are listed maters, which says that we
consider labelled landmarks. The set $\CP_N$ can therfore be ientified
to 
$\mR^{2N}$.

If the order between points is important, we will consider however,
that their global location in the 2D space is irrelevant.Two
configurations $(z_1, \ldots, z_N)$ and $(z'_1, \ldots, z'_N)$ will be
identified  if one can be deduced from the other by the composition
$g$ of a translation and a plane similitude, i.e., $z'_i = g.z_i$ for
all $i$. Objets of interest therefore are equivalent classes of
landmark configurations, which will be referred to as
$N$-shapes.

It will be convenient to identify the plane  $\mR^2$ with the set of
complex numbers $\mC$, a point $z =
(x,y)$ being represented as $x+iy$. A plane similitude composed with a
translation canthen be written under the form
$z \mapsto a.z + b$ with $a, b\in \mC$, $a\neq 0$.

For $Z = (z_1, \ldots, z_N)\in \CP_N$, we let $\bz$ be the center of inertia
$$
\bz = (z_1+\cdots+z_N)/N.$$
We also let  $\dps \|Z\|^2 = \sum_{i=1}^N |z_i-\bz|^2$.


\subsection{Space of planar $N$-shapes}

\subsubsection{Construction of a distance}
Let $\Sig_N$ be the quatient space of  $\CP_N$ by the equivalent
relation  $Z\,\CR\, Z'$ if there exists $a, b\in\mC$ such that
$Z'= aZ+b$. We denote $[Z]$ th equivalence class of 
$Z$. We shall define a distance between two equivalence classes $[Z]$
and $[Z']$. 

We can apply the results of the previous sections, which ensures that,
in order to define a distance in the quotient space, it suffices to
start with a distance on  $\CP_N$ which is equivariant for the
considered operations. So we need a  distance $D$ such that for all
$a, b\in\mC$ and all $W, Z\in \CP_N$,
$$
D(aZ+b, aW+b) = D(Z, W).
$$

To obtain such a distance, it suffices to definr a Riemannian metric
on $\CP_N = 
\mR^{2N}$ which is invariant by the action. We therefore must define,
for all  $Z\in \CP_N$, a norm $\|A\|_Z$ defined for all $A = (a_1,
\ldots, a_N)\in 
\mC^N$ such that for all $a, b\in \mC$:
$$
\|A\|_Z = \|a.A\|_{a.Z + b}.
$$
This formula implies that i suffices to define such a norm for  $Z$
such that $\|Z\| = 1$ and $\bz = 0$, since we have, for all
$Z$,
$$
\|A\|_Z = \|\frac{1}{\|Z\|}.A\|_{\frac{Z-\bz}{\|Z\|}}.
$$
Once the metric has been chosen, the distance $D(W, Z)$ is defined by
$$
D(W, Z)^2 = \inf \int_0^1 \norm{\der{\bfZ}{t}}^2_{\bfZ(t)} dt
$$
the infimum being taken over all paths  $\bfZ(.)$ such that $\bfZ(0)
= W$ and $\bfZ(1)  = Z$.

Le's make the following choice. When $\bz = 0$ and $\|Z\|=1$, we let
$$
\|A\|_Z = \sum_{i=1}^N |a_i|^2
$$
so that we need to minimize, among all paths between  $W$ and $Z$,
$$
\int_0^1
\frac{\sum_{i=1}^N|\dot{\bfZ_i}(t)|^2}{\sum_{i=1}^N|\bfZ_i(t)-\bar{\bfz}(t)|^2}
dt.
$$
Denote $\bfv_i(t) = (\bfZ_i(t) - \bfz(t))/\|\bfZ(t)\|$ and $\rho(t) =
\|\bfZ(t)\|$. The path $\bfZ(.)$ is uniquely $(\bfv(.), \rho(.),
\bz(.))$. Moreover, we have
$$
\der{\bfZ_i}{t} = \der{\bfz}{t} + \rho \der{\bfv}{t} + \bfv \der{\rho}{t}
$$
so that we need to minimize
$$
\int_0^1 \sum_{i=1}^N
\left|\frac{\der{\bfz}{t}}{\rho}+\frac{\der{\rho}{t}}{\rho}.\bfv_i + 
\der{\bfv_i}{t} \right|^2 dt.
$$
This is equal (using $\sum_i \bfv_i = 0$ and $\sum_i|\bfv_i|^2 =
1$, together with the differential on these expressions) to
$$
N\int_0^1 \left(\frac{\der{\bfz}{t}}{\rho}\right)^2
+ \int_0^1 \left(\frac{\der{\rho}{t}}{\rho}\right)^2 dt + \int_0^1
\sum_{i=1}^N \left|\der{\bfv_i}{t}\right|^2 dt\,.
$$
The boundary conditions directly deduced from those on  $W$ and $Z$.

The last term of this expression, which only depends on $\bfv$, can be
minimized explicitly, under the constraints 
$\sum_i \bfv_i = 0$ and $\sum_i|\bfv_i|^2 = 1$, which imply that
$\bfv$ varies on a $(N-1)$-dimensional sphere. The geodesic distance
is therefore given by the length of great circles, which yields the
expression of the minimum of the last term:
$ \arccos(\scp{\bfv(0)}{\bfv(1)})^2$.

We therefore have
\begin{eqnarray*}
D(W, Z)^2 &=& \inf \left(N\int_0^1 \left(\frac{\der{\bfz}{t}}{\rho}\right)^2
+ \int_0^1 \left(\frac{\der{\rho}{t}}{\rho}\right)^2 dt\right)\\
&& + \arccos\left(\scp{\frac{W-\bw}{\|W\|}}{\frac{Z-\bz}{\|Z\|}}\right)^2,
\end{eqnarray*}
where the first infimum is over functions $t\mapsto
(\bfz(t), \rho(t)) \in \mC \ti [0, +\infty[$, such that $\bfz(0) =
\bw$, $\bfz(1) = \bz(1)$, $\rho(0) = |W|$, $\rho(1) = |Z|$.

The induced distance on  $\Sig_N$ is then given by
$$
d([Z], [W]) = \inf\{D(Z, aW+b), a, b\in \mC\}.
$$
Since we can always select  $|a|$ and $b$ such that $|Z| =
|aW+b|$ and $\bz = a \bw + b$, we have
$$
d([Z], [W]) = \inf_{a}
\left[\arccos\left(\scp{\frac{a}{|a|}\frac{W-\bw}{\|W\|}}{\frac{Z-\bz}{\|Z\|}}\right)\right].
$$
Finally, optimizing this over the unit vector $a/\abs{a}$, we get
\encadre{
\begin{equation}
\label{dist.pol}
d([Z], [W]) =
\arccos\left|\scp{\frac{W-\bw}{\|W\|}}{\frac{Z-\bz}{\|Z\|}}\right|.
\end{equation}
}

Remark that the class $[Z]$ is characterized by $v = (Z-
\bz)/\|Z\|$, which varies in a complex sphere of dimension
$N-2$, denoted $\tS^{N-2}$, because it is the intersection of the
$(N-2)$-dimensional sphere and the 
complex hyperplane $\bz=0$. We have the equivalence
l'équivalence
\begin{equation}
\label{carte}
[Z] = [Z'] \Leftrightarrow \exists \nu \in\mC: |\nu| = 1 \text{ and }
\Phi(Z) = \nu \Phi(Z')
\end{equation}

Denote by $S^{2N-3}$ the set of  $v = (v_1, \ldots, v_{N-1})\in
\mC^{N-1}$ such that 
$\sum_i |v_i|^2 = 1$ (this can be identified to a real sphere of
dimension  $2N-3$). The complex projective space, denoted $\mC
P^{N-2}$, is defined as the space $S^{2N-3}$ quotiented by the
equivalence relation $v\CR v'$ if and only if $\exists
\nu\in\mC$ such that $v'= \nu v$; in other words, $\mC P^{N-2}$
contains all sets
$$
S^1.v = \{\nu.v, \nu\in\mC, |\nu| = 1\|$$ when $v$ varies in
$S^{2N-3}$ (this is also called the {\em Hopf fibration} of spheres of
odd dimension). This set has a strcte of $(N-2)$ dimensional complex
manifold, which means that it can be covered by an atlas of open set
which are in bijection with open subsets of  $\mC^{N-2}$. It suffices
indeed to define  $\CO_i$ to be the set of $S^1. v
\in\mC P^{N-2}$ with $v_i\neq 0$, and then to set $\Psi(S^1 v) =
(v_1/v_i, \ldots, v_{i-1}/v_i, v_{i+1}/v_i, \ldots, v_{N-1}/v_i)
\in \mC^{N-2}$ for all $S^1 v\in \CO_i$. This provides $\mC
P^{N-2}$ with a structure of $C^\infty$ complex manifold. The
equivalence (\ref{carte}) therefore provides a representation of 
$\Sig_{N}$ as a $C^{\infty}$ complex manifold.

Let us be more precise with this identification \cite{ken84}. We
associate to $Z = (z_1, \ldots,
z_N)$ the family $(\ze_1, \ldots, \ze_{N-1})$ defined by
$$
\ze_i = (jz_{j+1} - (z_1+\cdots+z_j))/\sqrt{j^2+j}.
$$
One can verify that  $\sum_{i=1}^{N-1} |\ze_i|^2 = \|Z\|^2$. Denote
$F(Z)$ the element $S^1.(\ze/\|Z\|)$ in $\mC P^{N-2}$. One checks that
$F(Z)$ only depends on $[Z]$ and that $[Z]\mapsto F(Z)$ is a bijection
between  $\Sig_N$ and $\mC P^{N-2}$.


\subsubsection{The space of triangles}
Consider the case $N=3$, which coresponds to labelled triangles. For a
triangle $Z = (z_1, z_2, z_3)$, the previous function $F(Z)$ can be
written 
\begin{eqnarray*}
F(Z) &=& S^1.\left\{\frac{1}{\sqrt{|z_2-z_1|^2/2 + |2z_3 - z_1 -
z_2|^2/6}}\left[ \frac{z_2-z_1}{\sqrt{2}}, \frac{2z_3 - z_1 -
z_2}{\sqrt{6}} \right] \right\}\\
&=& S^1.[v_1, v_2].
\end{eqnarray*}
On the set $v_1 \neq 0$ (i.e., the set $z_1\neq z_2$) we have the
local chart
$$
Z \mapsto v_2/v_1 = \frac{1}{\sqrt{3}}\left(\frac{2z^3 - z_2 -
z_1}{z_2 -z_1}\right) \in\mC. 
$$
If we let $v_2/v_1 = \tan\frac{\th}{2} e^{i\phi}$, and $M(Z) =
(\sin\th\cos\phi, \sin\th\sin\psi, \cos\th) \in\mR^3$, we obtain a
correspondence between the  triangles and the unit sphere $S^2$. This
correspondence is isometric: the distance between two triangles  $[Z]$
and $[\tZ]$, which has been defined above by 
$$
d([Z], [Z']) = \arccos \left|\frac{\sum_{i=1}^3 z_i\tz_i^*}{\|Z\|.\|\tZ\|}\right|
$$
gives, after passing to coordinates $\th$ and $\phi$, exactly the
lenth of the great circle between the images  $M(Z)$ and $M(Z')$. We
therefore obtain a representation of labelled triangular shapes as
points on the sphere $S^2$, with the possibility of comparing them
using the standard metric on  $S^2$.


\subsection{Extension to plane curves}

It is interesting to analyze whether this distance has a limit when
the landmarks correspond to increasingly refined discretizations of
plane curves. Consider for this two plane curves $m$ and $\tm$,
parameterized on $[0,1]$. Discretize the interval  $[0,1]$ into $N+1$
points $t_k =  k/N, k=0,
\ldots, N$. Denote $Z_k = m(t_k)$ and $W_k = \tm(t_k)$. Let also 
$m^N$ and $\tm^N$ be the piecewise constant approximations of  $m$ and
$\tm$ given by $m^N(t) = Z_k$ (resp. $\tm^N(t) = W_k$)
on $]t_{k-1}, t_k]$.

We have $\dps \bz = (1/N)\sum_k m(t_k) \simeq \int_0^1 m(t) dt$. Similarly
$$
\|Z\|^2  \simeq N \left[\int_0^1 |m(t)|^2 dt - \left|\int_0^1
m(t)dt\right|^2\right]
$$
and
$$
\scp{Z}{W} \simeq N \left[\int_0^1 m(t)\tm(t)^* dt - \int_0^1
m(t)dt\int_0^1\tm(t)^*dt\right]
$$
which gives, for large  $N$,
$$
d(m, \tm) = \arccos\left\{\frac{\dps \left|\int_0^1 m(t)\tm(t)^* dt - \int_0^1
m(t)dt\int_0^1\tm(t)^*dt\right|}{\left[ V_m\right]^{1/2} \left[V_{\tilde m}\right]^{1/2}}\right\}
$$
with $V_m = 
\dps \int_0^1 |m(t)|^2 dt - \left|\int_0^1
m(t)dt\right|^2$ (and a similar definition for $V_{\tilde m}$).

We can get rid of the translation component by comparing the
differences $Z_k = m(t_k) - m(t_{k-1})$ instead of the points
$m(t_k)$. Doing so, we obtain the same formula, replacing  $m(t)$ by
$dm/dt$. Since 
$$
\int_0^1\der{m}{t}dt = m(1) - m(0),
$$
we have, if $m$ and $\tm$ are closed, which will be assumed for
simplification,
$$
d(m, \tm) = \arccos\left\{\frac{\dps \left|\int_0^1
\der{m}{t}\der{\tm}{t}^* dt\right|}{\left[\int_0^1
\left|\der{m}{t}\right|^2 dt \right]^{1/2} \left[\int_0^1
\left|\der{\tm}{t}\right|^2 dt \right]^{1/2}}\right\}.
$$
(If the cures are open, the obtanied formulae
coresponds to comparing them after application of the closing
operation  $m(t) \mapsto m(t) - t (m(1)-m(0))$.)

We now introduce a parameterization in this formula. Assume that the
curves have length one (which is no loss of generality, since the
distance is scale-invariant). We let  $s = \phi(t)$ for curve $m$ and $s
= \psi(t)$ for curve $\tm$, where $s$ is the arc-length. We then have
$\der{m}{t} = \dphi(t) 
\tau(\phi(t))$ where $\tau$ is the unit tangent (expressed in function
of the arc-length). To keep with complex notation, we let $\tau =
e^{i\th}$. We then have 
$$
\int_0^1 \left|\der{m}{t}\right|^2 dt = \int_0^1 \dphi(t)^2 dt
$$
and
$$
\int_0^1 \der{m}{t}\der{\tm}{t}^* dt = \int_0^1 \dphi(t)\dpsi(t)
e^{i(\th(\phi(t))-\tth(\psi(t)))} dt.
$$
This yields the formula
$$
d(m, \tm) = \arccos \left\{\frac{\left|\int_0^1 \dphi(t)\dpsi(t)
e^{i(\th(\phi(t))-\tth(\psi(t)))} dt\right|}
{\sqrt{\int_0^1 \dphi(t)^2 dt}\sqrt{\int_0^1 \dpsi(t)^2 dt}}\right\}.
$$
The interest in making the parameterization apparent is that this
offers the possibility for optimizing the distance with respect to it,
which relates to the optimal matching problems discussed in the
previous section.




\section{Distances and Diffeomorphisms}
\label{dist.diff}
\subsection{Invariant Distances between Diffeomorphisms}
\label{dist.inv.diff}

Our goal here is to build a right invariant distance between
diffeomorphisms. This study has its own interest, but will also be
useful when we will deal with  more general
actions involving diffeomorphisms. It will also allow us to retrieve
the construction that we have made previously for the groups of
diffeomorphisms.

We only make here a formal (non-rigorous) discussion. We consider a
group  $G$ of diffeomorphisms of $\Om$, and define (to fix the ideas)
the tangent space to $G$ at $g$ by the set of  $u:\Om\to\mR^d$ such
that $\id + tu\circ
g^{-1}\in G$ for small enough $t$. Since the ``product'' on $G$ is the
composition, $gh = g\circ h$, the right translation $R_g:
h\mapsto h\circ g$ is linear, and therefore equal to its differential:
for 
$u\in T_hG$:
$$
d_h R_g . u = u\circ g.
$$

A metric on  $G$ is right invariant if, for all  $g, h\in G$ and for
all $u\in T_hG$:
$$
\|d_h R_g u\|_{h\circ g} = \|u\|_h
$$
which yields, taking $g = h^{-1}$:
$$
\|u\|_h = \|u\circ h^{-1}\|_\id.
$$


This implies that the energy of a path $(t\mapsto \bfg(t, .))$ in 
$G$ must be defined by
$$
E(\bfg) = \int_0^1 \left\|\pdr{\bfg}{t}(t, \bfg^{-1}(t, .))\right\|^2_\id dt.
$$
Define 
$$\bfv(t, x) = \pdr{\bfg}{t}(t, \bfg^{-1}(t, x))$$
so that the energy can be written
$$
E(\bfg) = \int_0^1 \left\|\bfv(t,.)\right\|^2_\id dt
$$
with the identity
$$
\pdr{\bfg}{t}(t, x) = \bfv(t, \bfg(t, x)).
$$
This implies that $\bfg$ is the flow associated to the velocity field
$\bfv(t, .)$, which provides the construction given in chapter \ref{grp.diff}.

The construction of $G$ directly from flows of diffeomorphisms
therefore becomes natural, as well as the condition that  $\|.\|_\id$
is admissible, according to definition \ref{adm}. The right invariant
distance on  $G$ therefore is 
$$
d(g_0, g_1) = \inf\sqrt{\int_0^1 \left\|\bfv(t,.)\right\|_\id^2 dt}
$$
where the minimum is taken over all $\bfv$ such that, for all
$x\in\Om$, the solution of the ODE
$$
\der{y}{t} = \bfv(t,y)
$$
with initial conditions $y(0) = g_0(x)$ is such that $y(1) =
g_1(x)$. This provides an interpretation of the cost function defined
in section \ref{viscous}, chapter \ref{est.diff} as a squared distance
to the identity
$$
E(g)= d(\id, g)^2.
$$

An explicit computation of this distance is generally impossible, but
there exists an exception, in 1D. Take  $\Om = [0,1]$
and
$$
\|u\|^2_\id = \int_0^1 \left| u_x\right|^2 dx.
$$
This not is not admissible, because it cannot control the supremum
norm of  $u_x = \prt u/\prt x$. One can define anyway the energy of a
path of diffeomorphisms  $\bfg(t,.)$
by
$$
U(\bfg) = \int_0^1 \int_0^1 \left|\pdr{\ }{x}\left(\pdr{\bfg}{t}\circ \bfg(t,
.)\right)\right|^2dxdt.
$$
This gives, after expanding the derivative and making the change of
variables  $ x = \bfg(t, y)$:
$$
U(\bfg) = \int_0^1 \int_0^1 \left|\pddr{\bfg}{t}{x}\right|^2
\left|\pdr{\bfg}{x}\right|^{-1} dy dt.
$$
Define $q(t, y) = \sqrt{\der{\bfg}{x}(t,y)}$: we have
$$
U(\bfg) = 4 \int_0^1 \int_0^1 \left|\der{q}{t}\right|^2 dy dt
$$
which yields
$$
U(\bfg) = 4 \int_0^1\norm{\der{q}{t}(t, .)}_2^2 dt.
$$
If the problem was to minimize this energy under the constraints  $q(0, .) =
\sqrt{\der{g_0}{x}}$ and $q(1, .) =
\sqrt{\der{g_1}{x}}$, the solution $q$ would be given by the line segments
$$
q(t, x) = t q(1, x) + (1-t) q(0, x).
$$
There is however an additional constraint that comes from the fcat
that $q(t, .)$ must provide a homeomorphism of $[0,1]$ for all $t$,
which implies  $\bfg(t, 1) = 1$, or, in terms of $q$
$$
\|q(t, .)\|_2^2 = \int_0^1 q(t, x)^2 dx = 1.
$$

We therefore need to minimize the length of the path $q$ under the
constraint that it remains on a Hilbert ($\CL^2$) sphere. Like in
finite dimension, geodesics on Hilbert spheres are great circles. This
implies that the optimal  $q$ is given by
$$
q(t, .) = \frac{1}{\sin \al} (\sin(\al(1-t)) q_0 + \sin(\al t) q_1)
$$
with $\al = \arccos\scp{q_0}{q_1}_2$. The length of  the geodesic is
precisely given by  $\al$, which provides a closed-form expression of
the distance on  $G$
\encadre{
$$
d(g_0, g_1) = 2\arccos\int_0^1 \sqrt{\der{g_0}{x}\der{g_1}{x}} dx.
$$}

If one defines the cost of a diffeomorphism $g$ by its squared
distance to the identity, one gets
\encadre{
$$
E(g) = 2\arccos\int_0^1 \sqrt{\der{g_0}{x}} dx
$$}
\noindent which has been used in \cite{pst98}.


\subsection{Distance between deformable objects}
\subsubsection{Distance between Landmarks}

We here define a metric on the set $\Om^N$, composed with $N$-tuples
of labelled landmarks. Let $G$ be a group of diffeomorphisms, as built
in chapter  \ref{grp.diff}. We consider the space $\CO = G\ti
\Om^N$. The action of  $G$ on $\Om^N$ is
$$
g.(x_1, \ldots, x_N) = (g(x_1), \ldots, g(x_N))
$$
and the right action on $\CO$ is
$$
(h, x_1, \ldots, x_N)g = (h\circ g, g^{-1}(x_1), \ldots, g^{-1}(x_N)).
$$
The derivative of the right action therefore is
$$
dR_g(\xi, \al_1, \ldots, \al_N) = (\xi\circ g, Dg^{-1}(x_1)\al_1,
\ldots, Dg^{-1}(x_N)\al_N).
$$

We want to apply the construction given in section \ref{var}, and
therefore build a metric on $\CO$ which is right invariant by the
action of $G$. This metric must satisfy, for all  $(g, x_1, \ldots,
x_N)\in\CO$:
\begin{multline*}
\|(\xi, \al_1, \ldots, \al_N)\|_{g, x_1, \ldots, x_N} = \\
\|(\xi\circ
g^{-1}, Dg(x_1) \al_1, \ldots, Dg (x_N) \al_N)\|_{\id, g(x_1),
\ldots, g(x_N)}
\end{multline*}

Let a curve $\bfo(t) = (\bfg(t), \bfx_1(t), \ldots, \bfx_N(t))$ be
given in  $\CO$. Denote $y_i = \bfg(t,\bfx_i)$ and introduce 
$\bfv$ such that
$$
\pdr{\bfg}{t} = \bfv(t, \bfg).
$$

The previous formula provides the energy of the curve, which is
\begin{eqnarray*}
E(\bfo(.)) &=& \int_0^1 \norm{\der{\bfo}{t}}_{\bfo(t)}^2 dt\\
 &=& \int_0^1 \norm{\bfv,
\der{y_1}{t} - \bfv(t, y_1),\ldots, \der{y_N}{t} - \bfv(t, y_N)
}_{\id, y_1, \ldots, y_N}^2 dt\\
&=&\tE(\bfv, y)
\end{eqnarray*}
using the fact that 
$$
\der{y_i}{t} = \der{}{t} \bfg(t, x_i) = \bfv(t, y_i) +
D\bfg(x_i)\der{x_i}{t}.
$$

The geodesic distance associated to  $D$ on $\CO$ can be obtained by
minimizing this energy with fixed boundary conditions. These
conditions are, if the
compared objects are  $o_0$ et $o_1$, 
$$
o_0 = \bfo(0) = (\bfg(0)^{-1}, \bfg(0, y_1(0)), \ldots, \bfg(0,
y_N(0)))
$$
and
$$
o_1 = \bfo(1) = (\bfg(1)^{-1}, \bfg(1, y_1(1)), \ldots, \bfg(1,
y_N(1))).
$$

The projected distance between two landmark configurations is then
given by, denoting  $y^0 = (y^0_1, \ldots, y^0_N)$ and $y^1 = (y^1_1, \ldots,
y^1_N)$,
\begin{eqnarray*}
d(y^0, y^1) &=& \inf\defset{D(o_0, o_1): o_0 = (g^{-1}, g.y^0), o_1 = (h^{-1},
hy^1)}\\
&=& \inf\defset{\sqrt{E(\bfo)}: o(0) = (g^{-1}, g.y^0), o(1) = (h^{-1},
h.y^1)}\\
&=& \inf\defset{\sqrt{\tE(\bfv, y)}: y(0) = y^0, y(1) = y^1}.
\end{eqnarray*}
We can see that the last expression does not involve the
diffeomorphism in the boundary conditions: $\bfv$ becomes an
auxilliary variable for the minimization. This will allow us to define
a new form of interpolating splines.

For this, let's make the following choice for the norm at the identity
$$
\|\xi, \al_1, \ldots, \al_N\|^2_{\id, y_1, \ldots, y_N} = \|\xi\|^2 +
\la \sum_{i=1}^N |\al_i|^2,
$$
with an admissible norm for $\xi$, so that
\encadre{
$$
\tE(\bfv, y) = \int_0^1 \|\bfv\|^2 dt + \la\sum_{i=1}^N \left|
\der{y_i}{t} - \bfv(t, y_i)\right|^2
$$}

If the norm that is used for $\bfv$ comes from a dot product
associated to a kernel $K: (x, y)\mapsto K(x, y)$, with values in the
set of $d$ by $d$ matrices, such that, for all $a\in \mR^d$ and
$x\in\Om$, $a^T v(x) =  \scp{K(x,
.)a}{v}$. With the same arguments as in section \ref{joshi}, chapter
\ref{est.diff}, the optimal path $\bfv$ is such that there exist
vectors $a_1(t), \ldots, a_N(t)$ such that, for all  $t$:
$$
v(t, x) = \sum_{i=1}^N K(x, y_i(t))a_i(t).
$$
This implies that $\tE$ can be written
\begin{multline*}
\tE(a, y) = \sum_{i, j=1}^N \int_0^1 {}^ta_i(t) K(y_i(t), y_j(t))
a_j(t)dt \\
+ \la\sum_{i=1}^N \int_0^1 \left|\der{y_i}{t} - \sum_{j=1}^n
K(y_i(t), y_j(t)) a_j(t)\right|^2 dt.
\end{multline*}
The vectors $a_1, \ldots, a_N$ can be computed explicitly given the
trajectories $y_1, \ldots, y_N$, namely
$$
a = (S(y) + \la I)^{-1} \der{y}{t}.
$$
This provides an expression of the energy in terms of $y_1, \ldots,
y_N$ that can be minimized by gradient descent, for example. Figure
\ref{fig:splines0} provides some examples of deformations using this
method, called {\em geodesic splines} \cite{cy01}, with a comparison
to the linear techniques of section \ref{par:splines}, chapter \ref{est.diff}.

\begin{figure}
\begin{center}
\includegraphics[width=0.48\textwidth]{FIGURES/ini3.eps}\  
\includegraphics[width=0.48\textwidth]{FIGURES/path3.eps}\\ 
\includegraphics[width=0.48\textwidth]{FIGURES/diff3.eps}\  
\includegraphics[width=0.48\textwidth]{FIGURES/stat3.eps}
\end{center}
\caption{\label{fig:splines0} First Row: Random displacements of
16 points uniformly distributed on a grid (left). Optimal trajectories
for Geodesic Splines (right). Second Row: Grid deformation provided by
geodesic splines (left). Grid deformation provided by classic splines.} 
\end{figure}




\subsubsection{Distance between functions}
\label{cons.cons}
In this section, the object space  $\CC$ contains function  $m:
\Om\to\mR^d$. We use the same construction as before, the action of
$G$ on $\CC$ being here $g.m = m\circ g^{-1}$. We let again $\CO = G\ti \CC$.

The right action of $G$ on $\CO$ is $R_h(g,m) = (g\circ h, m\circ
h)$. If $o=(g, m)$, the tangent space to $\CO$ at $m$ contains pairs of
function  $(\xi, \eta)$ defined on $\Om$, and the diffrential of the
right translation at $o$ is given by $DR_h(o) (\xi, \eta) = (\xi \circ h,
\eta\circ h)$.
To define a right-invariant metric on, we must provide, for all $o$, a
norm
$$
(\xi. \eta)\mapsto \|\xi, \eta\|_o
$$
such that, for all $h$,
$$
\|\xi\circ h, \eta\circ h\|_{(g\circ h, m\circ h)} = \|\xi,
\eta\|_{(g, m)}.
$$
This implies that it suffices to define $\|\xi, \eta\|_{(\id, m)}$ for
all $m$ and to set
$$
\|\xi, \eta\|_{(g, m)} = \|\xi\circ g^{-1}, \eta\circ g^{-1}\|_{(\id, m\circ g^{-1})}.
$$

Given such a metric, we evaluate the energy of a path $\bfo(.)$ in
$\CO$, given as always by
$$
E(\bfo) = \int_0^1 \norm{\der{\bfo}{t}(t)}^2_{\bfo(t)}dt.
$$

Introduce, as before, $\bfv(t, .) = \pdr{\bfg}{t} \circ \bfg^{-1}(t,
.)$. Let also $\bfM(t, .) = \bfm(t, \bfg^{-1}(t, .))$. We have
$$
\pdr{\bfm}{t} (t, y) = \pdr{\bfM}{t}(t, g(t, y)) + \pdr{\bfM}{x}(t,
\bfg(t, y)).\pdr{\bfg}{t}(t, y)
$$
so that 
$$
E(\bfo) = F(\bfv, \bfM) := \int_0^1 \left\|\bfv(t, .),
\pdr{\bfM}{t}(t, .) + \pdr{\bfM}{x}(t,.).\bfv(t, .) \right\|_{\id, \bfM(t, .)}dt.
$$

Let $\bfg_\bfv$ denote the solution of
$$
\pdr{\bfg_\bfv}{t}(t, x) = \bfv(t, \bfg_\bfv(t, x))
$$
with $\bfg_\bfv(0, x) = x$ for all $x$. We obtain a distance
$d_\CO(o, o')$ by setting (with
$o=(g, m)$ and $o'= (g', \tm)$)
$$
d_\CO(o, o') = \inf \sqrt{F(\bfv, \bfM)}$$
where the infimum is taken over all paths $(\bfv, \bfM)$ such that
$\bfg_\bfv(1, g(x)) = g'(x)$, $\bfM(0, g(x)) = m(x)$ and $\bfM(1,
g(x)) = \tm(x)$ (this is simply the definition of the geodesic
distance on $\CO$ expressed in terms of the new variables  $\bfv$ and
$\bfM$).

The projected distance between two functions  $M$ and $M'$ is the
infimum of the previous expression, over all pairs  $o=(g, m)$ and
$o'= (g', \tm)$ such that
$m\circ g^{-1} = M$ and $\tm\circ {g'}^{-1} = M'$. By the right
equivariance of $d_\CO$,  it is also the infimum of 
$d_\CO[(\id, M), (g, \tm)]$ over all pairs $(g, \tm)$ such that
que $\tm\circ g^{-1} = M'$. Returning to the energy, it is therefore
the minimum of  $F(\bfv, \bfM)$ among all paths such that $\bfM(0,
x) = M(x)$ and $\bfM(1, \bfg_\bfv(1, x)) = \tm(x) = M(\bfg_\bfv(1,
x))$. It is therefore the  infimum of $F(\bfv, \bfM)$ over all paths
such that $\bfM(0, .) = M$ and $\bfM(1, .) = M'$. Here again, the
diffeomorphism does not appear in the boundary conditions.


\subsubsection{Application: comparison of plane curves}
\subsubsection*{Comparison based on orientation}

We first consider the issue of comparing plane curves on the basis of
the orientation of their tangents  \cite{you98}. If  $m$ is a plane
curve parameterized with arc-length, and $L$ is it length, we define
the normalized tangent  $T_m$ by
$$\map{T_m}{[0,1]}{S^1}{s}{\dm(Ls)}$$
where $S^1$ is the unit disc in $\mR^2$. The function $T_m$
characterizes $m$ up to translation and scaling, and the pair $(L,
T_m)$ characterizes $m$ up to translation.

We will identify, as we have done before, the sets $\mR^2$ and
complexe $\mC$. We consider a group of diffeomorphisms $G$ of $\Om
= (0,1)$, which acts on functions $T:[0,1]\to S^1$ par $gT =
T\circ g^{-1}$, and apply the construction of section
\ref{cons.cons} with
\begin{equation}
\label{n.tau}
\norm{\xi, \eta}^2_T= \norm{\xi, \eta}^2 = \int_0^1
\left[\left(\der{\xi}{x}\right)^2 + \eta^2\right] dx.
\end{equation}

The cost of the path $(\bfg(t, .), \bfT(t, .))$ is then
$$
U(\bfg, \bfT)= \int_0^1 \norm{\pdr{\bfg}{t}\circ \bfg^{-1},
\pdr{\bfT}{t}\circ \bfg^{-1}}^2 dt.
$$
Expand the derivative and make the change of  variables $x = \bfg(t,y)$
to write
$$
U(\bfg, \bfT) = \int_0^1 \int_0^1 \left[\left(\pddr{\bfg}{t}{x}\right)^2
\left(\pdr{\bfg}{x}\right)^{-1} +  \pdr{\bfg}{x}
\left|\pdr{\bfT}{t}\right|^2\right] dy dt
$$
Let $q(t, .)$ be differentiable in $t$ such that
$$q(t, x)^2 = \pdr{\bfg}{x}(t,x) \bfT(t,x)$$
($\bfT$ being considered as a unit complex number). Such a path always exists: for all  $x$, there exists (since $|\bfT(.,x)|=1$ a unique lifting  $\bfT(t, x) = \exp(i\th(t,x))$ with $\th(t,x)$
 differentiable in $t$ and $\th(0,x)\in[0, 2\pi[$. One can then define
\begin{equation}
\label{sqrt.q}
q(t, x) = \sqrt{\pdr{\bfg}{x}(t,x)} \exp(i\th(t,x)/2).
\end{equation}
This path is not uniquely defined, since one can always change the sign of $q(t,x)$, uniformly in $t$, for all $x$.

We have
$$
\pdr{q^2}{t}(t,x) = \pddr{\bfg}{t}{x}(t,x) \bfT(t,x)
+\pdr{\bfg}{x}(t,x) \pdr{\bfT(t,x)}{t}.
$$
Take the absolute value and use the fcat that $\bfT$ is orthogonal to
its derivative to obtain
$$
\abs{\pdr{q^2}{t}(t,x)}^2 = \left|\pddr{\bfg}{t}{x}(t,x)\right|^2
+\left(\pdr{\bfg}{x}(t,x)\right)^2
\left|\pdr{\bfT(t,x)}{t}\right|^2.
$$
Moreover
$$
\abs{\pdr{q^2}{t}(t,x)}^2 = 4|q(t,x)|^2\abs{\pdr{q}{t}(t,x)}^2 =
 4\pdr{\bfg}{x}(t,x)\abs{\pdr{q}{t}(t,x)}^2
$$
which implies
$$
|\pdr{q}{t}(t,x)|^2 = \frac{1}{4}\left[\left(\pddr{\bfg}{t}{x}\right)^2
\left(\pdr{\bfg}{x}\right)^{-1} +  \pdr{\bfg}{x}
\left|\pdr{\bfT}{t}\right|^2\right]
$$
so that
\begin{equation}
\label{eq:Uq}
U(\bfg, \bfT) = 4 \int_0^1 \int_0^1 \abs{\pdr{q}{t}(t,x)}^2 dx
dt.
\end{equation}


We now consider paths linking 
$(g_0, T_0)$ and $(g_1, T_1)$. We can already state that the  minimum
of $U(\bfg, \bfT)$ is larger than the minimum of the right-hand term of
\eqref{eq:Uq} over functions $q$ such that  $q(0,
.)^2 = \pdr{g_0}{x} T_0$ et $q(1, .)^2 = \pdr{g_1}{x} T_1$. We now
show that equality is true, provided that  $\pdr{g_0}{x}$ and
$\pdr{g_1}{x}$ are almost everywhere positive on  $[0,1]$.

First, note that, the computation the minimum of the right-hand
term of \eqref{eq:Uq} with fixed boundary conditions  $q_0$ and $q_1$
fixées can be handled similarly to the distance for 1D diffeomorphisms
that we have computed at the end of section \ref{dist.inv.diff}, the
only difference here being that $q$ is a complex-valued
function. Since we still have the constraint that the integral of the
squared modulus of $q$ is 1, we are still computing geodesics on an infinite
dimensional sphere. The optimal path is therefore given by
$$
\bfq(t, x) = \frac{1}{\sin \al} (\sin(\al(1-t)) q_0(x) + \sin(\al t) q_1(x))
$$
with $\al = \arccos\scp{q_0}{q_1}_2$ and
$$
\scp{q_0}{q_1}_2 = \int_0^1 \Re(q_0(x) \bar{q}_1(x)) dx
$$
where $\bar{q}_1$ is the complex conjugate of $q_1$. For any choice of
$q_0$ and $q_1$ satisfying $q_0^2 =
\pdr{g_0}{x} T_0$ and $q_1^2 = \pdr{g_1}{x} T_1$, the optimal path
$\bfq$ uniquely satisfies the path  $(\bfg(t, .), \tau(t,
.)$ as long as $\bfq$ does not vanish.

Let us choose  $q_0$ and $q_1$ to ensure that $\al$ is minimal. This
is achieved by choosing, for all  $x$, $q_0(x)$ and $q_1(x)$ such that
$\Re(q_0(x) \bar{q}_1(x)) \geq 0$ (since $\arccos$ is
decreasing); we then have
\begin{eqnarray*}
|\bfq(t, x)|^2 &=& \frac{1}{\sin^2 \al} (\sin^2(\al(1-t)) |q_0(x)|^2 +
 \sin^2(\al t) |q_1(x)|^2 \\
 &&+ 2 \sin(\al(1-t))\sin(\al t) \Re(q_0(x)
 \bar{q}_1(x)))\\
&\geq & \frac{1}{\sin^2 \al} (\sin^2(\al(1-t)) |q_0(x)|^2 +
 \sin^2(\al t) |q_1(x)|^2).
\end{eqnarray*}
The last inequality shows that the function 
$\bfq(t,x)$ can vanish (for $t\in (0,1)$) only if both $q_0(x)$ et
$q_1(x)$ vanish. We are assuming that this can happen only when $x$
belongs to a set of Lebesgue's measure 0 in  $[0,1]$. On this set, the
function $t\mapsto\bfT(t,x)$ is undefined, but we can make an
arbitrary choice without changing the value of $\al$.

We have therefore showed that the distance between  $o_0 = (g_0, \tau_0=
e^{i\th_0})$ and $o_1  = (g_1,
\tau_1=e^{i\th_1})$ was given by 
$$
D(o_0, o_1) = 2 \arccos \int_0^1 \sqrt{\der{g_0}{x}\der{g_1}{x}}|\cos((\th_0(x) -
\th_1(x))/2)| dx
$$
since $|\cos((\th_0(x) -\th_1(x))/2)|$ is equal to  the real part of
the square root of  $T_0\bar{T}_1$ for which $\al$ is minimized. This
can also be written
$$
D(o_0, o_1) = 2\arccos \frac{\sqrt{2}}{2}\int_0^1
\sqrt{\der{g_0}{x}\der{g_1}{x}}\sqrt{1 +
\scp{\tau_0(x)}{\tau_1(x)}}dx .
$$
with $\scp{z}{z'} = \Re(z\bar{z}')$ for complex numbers $z$ and $z'$.

The resulting distance between two functions $T$ and $T'$ is,
according to  (\ref{inv.eq.gen})
\begin{eqnarray*}
d(T, T') &=& \inf\{D(o_0, o_1), o_0 = (g_0, T_0), o_1 = (g_1,
T_1), T_0\circ g_0^{-1} = T, T_1\circ g_1^{-1} = T'\}\\
&=& \inf\{D(o_0, o_1), o_0 = (\id, T), o_1 = (g,
T_1), T_0\circ g_0^{-1} = T, T_1 = T'\circ g^{-1} \}
\end{eqnarray*}
which finally yields
\encadre{
$$
d(\tau, \tau') = 2\arccos \sup_g \int_0^1 \sqrt{\der{g}{x}} |\cos((\th - \th'\circ
g)/2)| dx.
$$}

The existence (under some conditions on $\th$ and $\th'$) of an
optimal $g$ in the previous formula is proved in \cite{ty00}. Figure
\ref{fig:exp.1D} provides examples of curve matching that can be
obtained using this method.

\begin{figure}
\begin{center}
\includegraphics[width=5cm]{FIGURES/curveMatching1.ps}
\includegraphics[width=5cm]{FIGURES/curveMatching2.ps}\\
\includegraphics[width=4cm]{FIGURES/curveMatching3.ps}
\includegraphics[width=6cm]{FIGURES/curveMatching4.ps}\\
\end{center}
\caption{\label{fig:exp.1D} Diffeomorphic matching between curves. In
each image, the geodesic is computed between the outer curve and the
inner curve. Scaling is for visualization only (the computation is
scale invariant).}
\end{figure}

\subsubsection*{Infinitesimal analysis}
We now provide an infinitesimal justification for the choice of the
metric  (\ref{n.tau}), which also offers alternative definitions.

We therefore consider infinitesimal variations of plane curves. Let
$m$ be a parameterized curve, defined on  $[0, 1]$, such that, for all  $x$
$$\left|\der{m}{x}\right|\equiv L(m)$$
where $L(m)$ is the length of $m$ (this corresponds to the arc-length
normalized by the length). Let's consider a small perturbation along
$m$, denoted  $x \mapsto \ep
\De(x)\in\mR^2$. We assume that $\ep$ is small
and only keep terms of order one in the following computation. The
deformed curve is $x\mapsto m(x) + \ep \De(x)$, that we parameterize by
normalized arc-length to obtain a new curve $\tm$, still defined on
$[0,1]$. We denote by $g$ the diffeomorphism providing the change of
parameter, so that, for all  $x\in [0,1]$,
$$
\tm \circ g(x) = m(x) + \ep \De(x).
$$
Let $\xi(x) = g(x) - 1$. Let $T$, $N$ and $\ka$ be the tangent, normal
and Euclidean curvature of $m$. We have (denoting derivatives as subscripts)
$$
m_x = L(m) T,
$$
$$
m_{mx} = L(m)  T_x = L(m)^2 \ka N.
$$
Similarly, let  $\tT$, $\tN$, $\tka$, be the tangent, normal and
curvature of $\tm$; let finally $L = L(m)$ and $\tL = L(\tm)$. At
firest order, we have  
\begin{eqnarray*}
\ep \De_x &=& (1+\xi_x) \tm_x \circ g - m_x\\
&=& \tL \xi_x \tT\circ g + \tL\tT\circ g - L T\\
&=& L\xi_x T + (\tL-L)T  + L(\tT\circ g - T) + o(\ep).
\end{eqnarray*}
We now define an infinitesimal deformation energy in terms of $\De$
and compute its expression in terms of $g$ and the geoetric
characteristics of the curves. Denote 
$$
E = \int_0^L\left|V_x\right|^2 = \frac{\ep^2}{L} \int_0^1
\left|\De_x\right|^2dx
$$
where $V$ and $\De$ are related by $V(x) = \ep \De(x/L)$. At first
order in $\ep$, $\tT\circ g-
T$ is perpendicular to $T$, which implies 
$$
E = \frac{(\tL-L)^2}{L} + L \int_0^1\left|\xi_x\right|^2
dx + L \int_0^1|\tT\circ g - T|^2dx + o(\ep^2).
$$
Introduce the group $G$ of diffeomorphisms of  $[0,1]$, and consider
the set $\CO$ consisting of pairs $o = (L, T)$, with 
$L>0$ and $T: [0, 1]\mapsto \mR^2$ such that $|T(x)| = 1$ for all
$x$. There exists a unique curve  $m$ (modulo translation) with length
$L$ and having $T$ as a unit tangent. Denote
$$
\norm{\xi, \de_L, \de_T}_{L, \tau}^2 = L \int_0^1 \left|\xi_x\right|^2 dx
\frac{\de_L^2}{L} +
L\int_0^1|\de_T|^2dx.
$$
Without the length component, this is exactly the metric introduced in
the previous section. An explicit computation of the associated
geodesic distance is still possible. Let   $o_0 = (g_0,
L_0, T_0)$
and $o_1 = (g_1, L_1, T_1)$. We obtain \cite{you98}
$$
D(o_0, o_1) = L_0 + L_1 - \sqrt{2}L_0L_1 \int_0^1
\sqrt{\der{g_0}{x}\der{g_1}{x}}\sqrt{1 + \scp{T_0(x)}{T_1(x)}}dx
\ .
$$

\bigskip
Let us consider higher derivatives, which will allow us to also deal
with rotation invariance. We have
\begin{eqnarray*}
\ep \De_{xx} &=& L^2 \xi_x \ka N +
L\xi_{xx} T + L(\tL-L)\ka N + L\tL (1+\xi_x)\tka\circ g
N\circ g - L^2 \ka N +_ o(\ep)\\
& = & L\xi_{xx} T + 2L^2 \xi_x\ka N
+2L(\tL-L)\ka N + L^2(\tka\circ g - \ka)N + L^2\ka(\tN\circ g -
N) + o(\ep)
\end{eqnarray*}
At order 1, 
$L(\tN\circ g - N)$ is perpendicular to $N$, and can be computed by
applying a $\pi/2$-rotation to the vector
$L(\ttau\circ g - \tau)$, the latter being the normal component of the
first derivative of $\ep \De$. We can therefore write
$L^2(\tN \circ g - N) = -L\ep \scp{\De_x}{N} T$, which yields
$$
\ep \De_{xx} + L\ep\ka\scp{\De_x}{N} T = L\xi_{xx} T + 2L^2 \xi_x\ka N
+2L(\tL-L)\ka N + L^2(\tka\circ g - \ka) N. 
$$

This computation suggests the definition of the following operator
along $m$:
$$
E = \frac{\ep^2}{L^3} \int_0^1 \left|\De_{xx} +
L\ka\scp{\De_x}{N} T \right|^2 dx,
$$
which is invariant by (infinitesimal) rotation. (The factor $L^{-3}$
comes from an analysis using  $V(x) = \De(x/L)$.) This energy is equal
to 
$$
E = \frac{1}{L}\int_0^1 \left|\dder{\xi}{x}\right|^2dx +
L\int_0^1 \left|2\der{\xi}{x}\ka
+2\frac{\tL-L}{L}\ka + \tka\circ g - \ka\right|^2dx + o(\ep^2).
$$

This leads us to considering curve representation under the form $m =
(L, \ka)$, $L$ being the length, and  $\ka$ the curvature
parameterized by the normalized arc-length. The previous analysis
provides a natural candidate for the norm  $\norm{.}_{L,
\ka}$. Applying our general theory (section \ref{cons.cons}), this
defines the energy of  a path in $G\ti\CC$. Introduce the variable 
$\bfv$ as before, and the evolving object,  $(\bfL,
\bfK)$, which depend on time $t$. The energy of a path can then be
written as
$$
\int_0^1\int_0^1 \frac{1}{\bfL}\left|\dder{\bfv}{x}\right|^2dxdt +
\int_0^1\int_0^1 \bfL \left|2\der{\bfv}{x}\bfK
+2\frac{1}{\bfL}\bfK\der{\bfL}{t} + \pdr{\bfK}{t} +
\bfv\pdr{\bfK}{x}\right|^2dxdt.
$$




\subsubsection{Application: images matching}

We now provide a simple application of the formulas of section
\ref{cons.cons} for image comparison. The set $\Om$ is here a square
(or a rectangle) in $\mR^2$, for example $[0,1]^2$, and objects are
images, considered as functions defined on  $\Om$ and taking values in
$\mR$. We let
$$
\|\xi, \eta\|_{\id, m} = \int_\Om \scp{L\xi}{\xi}^2dx + \la \int_{\Om}
|\eta|^2dx
$$
where $L$ is a strictly monotonous admissible operator.

From the general formula, the energy of a path is given by
\begin{equation}
\label{eq:img.sign}
\tE(\bfv, \bfM) = \int_0^1\int_\Om \scp{L\bfv}{\bfv}^2 dx dt + \la \int_0^1
\int_\Om \left|\pdr{\bfM}{t} + \scp{\nabla \bfM}{\bfv}\right|^2dx dt.
\end{equation}

Figures \ref{fig:quadrature} and \ref{fig:nova1} provide two examples
of images matched using this energy. The numerical scheme is described
in the next section.



\begin{figure}
\begin{center}
\includegraphics[width=2.5cm]{FIGURES/quadra-newI01.eps}
\includegraphics[width=2.5cm]{FIGURES/quadra-newI03.eps}
\includegraphics[width=2.5cm]{FIGURES/quadra-newI06.eps}
\includegraphics[width=2.5cm]{FIGURES/quadra-newI11.eps}\\
\includegraphics[width=2.5cm]{FIGURES/quadra-grid01.eps}
\includegraphics[width=2.5cm]{FIGURES/quadra-grid03.eps}
\includegraphics[width=2.5cm]{FIGURES/quadra-grid06.eps}
\includegraphics[width=2.5cm]{FIGURES/quadra-grid11.eps}
\end{center}
\caption{\label{fig:quadrature} Estimation of a geodesic between a
disc and a square. First Row: Image evolution in time. Second Row:
evolution of the diffeomorphism.}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=2.5cm]{FIGURES/nova1-newI01.eps}
\includegraphics[width=2.5cm]{FIGURES/nova1-newI03.eps}
\includegraphics[width=2.5cm]{FIGURES/nova1-newI06.eps}
\includegraphics[width=2.5cm]{FIGURES/nova1-newI11.eps}\\
\includegraphics[width=2.5cm]{FIGURES/nova1-grid01.eps}
\includegraphics[width=2.5cm]{FIGURES/nova1-grid03.eps}
\includegraphics[width=2.5cm]{FIGURES/nova1-grid06.eps}
\includegraphics[width=2.5cm]{FIGURES/nova1-grid11.eps}
\end{center}
\caption{\label{fig:nova1} Geodesic between an empty image and a disc.
First Row: Image evolution in time. Second Row:
evolution of the diffeomorphism.}
\end{figure}

\subsubsection{Discretization of \eqref{eq:img.sign}}

Some care is required for the discretization of 
\eqref{eq:img.sign}. This is mainly due to the ``hyperbolic'' term
$\pdr{\bfM}{t} + \scp{\nabla \bfM}{\bfv}$, which represent the total
derivative of $\bfM$ along the flow. The stablest results have been
obtained using the following scheme.

Introduce the auxilliary variable $w = L^{1/2}v$, so that $v =
K^{1/2}w$ where $K= L^{-1}$ (the numerical implementation would in
fact define $\tK = K^{1/2}$ and let $K = \tK^2$). The following
discretized energy has been used in the experiments of Figures
\ref{fig:quadrature} and \ref{fig:nova1}. 
$$
E = \sum_{t=1}^T \sum_{x\in \tilde\Om} \abs{w(x)}^2 + \la\de_t^{-2} 
\sum_{t=1}^T \sum_{x\in \tilde\Om} \abs{M(t+1, x + \de_t (K^{1/2}w)(t, x))
- M(t, x)}^2
$$
Where $x$ and $t$ now are discrete variables, $\tilde\Om$ a
discrete grid on $\Om$ and $\de_t$ the time discretization step.





==> theorem.tex <==


\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{result}{Result}
\newtheorem{proposition}{Proposition}
\newtheorem{conditions}{Conditions}
\newtheorem{hypothesis}{Hypothesis}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{properties}{Properties}
\newtheorem{property}{Property}
\newtheorem{notation}{Notation}


